Tails, Trails, and Transients: Comets, NEOs, and Supernovae in Rubin Early Data Preview 2

We identify effective single-visit imaging hidden within the deep coadded images of the NSF-DOE Vera C. Rubin Observatory Early Data Preview 2 (EDP2). We develop a workflow to locate known small Solar System bodies in these data, using our Ponder orchestrator with the Sorcha survey simulator to predict their positions and the Rubin Science Platform to identify shallow coadds and extract image cutouts. Because cometary activity and near-Earth object (NEO) trails produce extended morphologies, both remain identifiable in shallow coadds. From approximately 700 comet cutouts, we identify 59 activity detections spanning 32 objects. We discover activity in 2025 NC6, previously unknown to be active, and independently rediscover two comets through their activity. We recover 336 NEO cutouts, including 29 with predicted trails over 25 pixels. We demonstrate how the same provenance-driven methods can recover stationary transients in Rubin coadds, including ones predating the alert stream. Of 47 publicly-reported transients coinciding with EDP2, 36 occupy shallow coadds. We show Rubin photometry agrees with published lightcurves to within 0.2 mag. The imaging provides additional bands, host-galaxy context, and deeper supernova pre-discovery limits than discovery surveys could reach. We showcase seven transients, including SN 2025nbh, which we identify as lying in the outskirts of AGC 114905, an ultra-diffuse galaxy central to the dark-matter-free debate; the supernova offers an independent galaxy distance measurement. Shallow coadds are a relatively unexplored facet of Rubin data with applications beyond the examples presented here; regions with varying numbers of contributing visits will persist throughout the Legacy Survey of Space and Time (LSST).

==> comets.tex <==
% Generated by scripts/update_catalog.py; do not edit this file for lasting changes.
% Source: https://www.minorplanetcenter.net/iau/MPCORB/AllCometEls.txt
% Source SHA-256: 441f08178662a4225143046b997faf103d0fa7b661526d808f3f5ad9cf9796ed
% Source records: 4651; declarations: 4653
% Explicit LaTeX overrides: data/overrides.json
%\DeclareComet{100P}{100P}{100P/Hartley 1}
%\DeclareComet{101P}{101P}{101P/Chernykh}
%\DeclareComet{101P-B}{101P-B}{101P/Chernykh-B}
%\DeclareComet{102P}{102P}{102P/Shoemaker 1}
%\DeclareComet{103P}{103P}{103P/Hartley 2}
%\DeclareComet{104P}{104P}{104P/Kowal 2}
%\DeclareComet{105P}{105P}{105P/SingerBrewster}
%\DeclareComet{106P}{106P}{106P/Schuster}
%\DeclareComet{108P}{108P}{108P/Ciffreo}
%\DeclareComet{109P}{109P}{109P/Swift-Tuttle}
%\DeclareComet{10P}{10P}{10P/Tempel 2}
%\DeclareComet{110P}{110P}{110P/Hartley 3}
%\DeclareComet{111P}{111P}{111P/Helin-Roman-Crockett}
%\DeclareComet{112P}{112P}{112P/Urata-Niijima}
%\DeclareComet{113P}{113P}{113P/Spitaler}
%\DeclareComet{114P}{114P}{114P/Wiseman-Skiff}
%\DeclareComet{115P}{115P}{115P/Maury}
%\DeclareComet{116P}{116P}{116P/Wild 4}
%\DeclareComet{117P}{117P}{117P/Helin-Roman-Alu 1}
%\DeclareComet{118P}{118P}{118P/Shoemaker-Levy 4}
%\DeclareComet{119P}{119P}{119P/Parker-Hartley}
%\DeclareComet{11P}{11P}{11P/Tempel-Swift-LINEAR}
%\DeclareComet{120P}{120P}{120P/Mueller 1}
%\DeclareComet{121P}{121P}{121P/Shoemaker-Holt 2}
%\DeclareComet{122P}{122P}{122P/deVico}
%\DeclareComet{123P}{123P}{123P/West-Hartley}
%\DeclareComet{124P}{124P}{124P/Mrkos}
%\DeclareComet{125P}{125P}{125P/Spacewatch}
%\DeclareComet{126P}{126P}{126P/IRAS}
%\DeclareComet{127P}{127P}{127P/Holt-Olmstead}
\DeclareComet{128P}{128P}{128P/Shoemaker-Holt 1}
%\DeclareComet{129P}{129P}{129P/Shoemaker-Levy 3}
\DeclareComet{12P}{12P}{12P/Pons-Brooks}
%\DeclareComet{130P}{130P}{130P/McNaught-Hughes}
\DeclareComet{131P}{131P}{131P/Mueller 2}
%\DeclareComet{132P}{132P}{132P/Helin-Roman-Alu 2}
\DeclareComet{133P}{133P}{133P/Elst--Pizarro}
%\DeclareComet{134P}{134P}{134P/Kowal-Vavrova}
%\DeclareComet{135P}{135P}{135P/Shoemaker-Levy 8}
%\DeclareComet{136P}{136P}{136P/Mueller 3}
%\DeclareComet{137P}{137P}{137P/Shoemaker-Levy 2}
%\DeclareComet{138P}{138P}{138P/Shoemaker-Levy 7}
%\DeclareComet{139P}{139P}{139P/Vaisala-Oterma}
\DeclareComet{13P}{13P}{13P/Olbers}
%\DeclareComet{140P}{140P}{140P/Bowell-Skiff}
%\DeclareComet{141P}{141P}{141P/Machholz 2}
%\DeclareComet{141P-A}{141P-A}{141P/Machholz 2-A}
%\DeclareComet{141P-B}{141P-B}{141P/Machholz 2-B}
%\DeclareComet{141P-D}{141P-D}{141P/Machholz 2-D}
%\DeclareComet{141P-E}{141P-E}{141P/Machholz 2-E}
%\DeclareComet{141P-F}{141P-F}{141P/Machholz 2-F}
%\DeclareComet{141P-G}{141P-G}{141P/Machholz 2-G}
%\DeclareComet{141P-H}{141P-H}{141P/Machholz 2-H}
%\DeclareComet{141P-I}{141P-I}{141P/Machholz 2-I}
%\DeclareComet{142P}{142P}{142P/Ge-Wang}
%\DeclareComet{143P}{143P}{143P/Kowal-Mrkos}
%\DeclareComet{144P}{144P}{144P/Kushida}
%\DeclareComet{145P}{145P}{145P/Shoemaker-Levy 5}
%\DeclareComet{146P}{146P}{146P/Shoemaker-LINEAR}
%\DeclareComet{147P}{147P}{147P/Kushida-Muramatsu}
%\DeclareComet{148P}{148P}{148P/Anderson-LINEAR}
%\DeclareComet{149P}{149P}{149P/Mueller 4}
%\DeclareComet{14P}{14P}{14P/Wolf}
%\DeclareComet{150P}{150P}{150P/LONEOS}
%\DeclareComet{151P}{151P}{151P/Helin}
%\DeclareComet{152P}{152P}{152P/Helin-Lawrence}
%\DeclareComet{153P}{153P}{153P/Ikeya-Zhang}
%\DeclareComet{154P}{154P}{154P/Brewington}
%\DeclareComet{155P}{155P}{155P/Shoemaker 3}
%\DeclareComet{156P}{156P}{156P/Russell-LINEAR}
%\DeclareComet{157P}{157P}{157P/Tritton}
%\DeclareComet{157P-B}{157P-B}{157P/Tritton-B}
%\DeclareComet{158P}{158P}{158P/Kowal-LINEAR}
%\DeclareComet{159P}{159P}{159P/LONEOS}
%\DeclareComet{15P}{15P}{15P/Finlay}
%\DeclareComet{160P}{160P}{160P/LINEAR}
%\DeclareComet{161P}{161P}{161P/Hartley-IRAS}
%\DeclareComet{162P}{162P}{162P/Siding Spring}
%\DeclareComet{163P}{163P}{163P/NEAT}
%\DeclareComet{164P}{164P}{164P/Christensen}
%\DeclareComet{165P}{165P}{165P/LINEAR}
%\DeclareComet{166P}{166P}{166P/NEAT}
%\DeclareComet{167P}{167P}{167P/CINEOS}
%\DeclareComet{168P}{168P}{168P/Hergenrother}
%\DeclareComet{169P}{169P}{169P/NEAT}
%\DeclareComet{16P}{16P}{16P/Brooks 2}
%\DeclareComet{170P}{170P}{170P/Christensen}
%\DeclareComet{171P}{171P}{171P/Spahr}
%\DeclareComet{172P}{172P}{172P/Yeung}
%\DeclareComet{173P}{173P}{173P/Mueller 5}
%\DeclareComet{174P}{174P}{174P/Echeclus}
%\DeclareComet{175P}{175P}{175P/Hergenrother}
%\DeclareComet{176P}{176P}{176P/LINEAR}
%\DeclareComet{177P}{177P}{177P/Barnard}
%\DeclareComet{178P}{178P}{178P/Hug-Bell}
%\DeclareComet{179P}{179P}{179P/Jedicke}
%\DeclareComet{17P}{17P}{17P/Holmes}
%\DeclareComet{180P}{180P}{180P/NEAT}
%\DeclareComet{181P}{181P}{181P/Shoemaker-Levy 6}
%\DeclareComet{182P}{182P}{182P/LONEOS}
%\DeclareComet{183P}{183P}{183P/Korlevic-Juric}
%\DeclareComet{184P}{184P}{184P/Lovas 2}
%\DeclareComet{185P}{185P}{185P/Petriew}
%\DeclareComet{186P}{186P}{186P/Garradd}
%\DeclareComet{187P}{187P}{187P/LINEAR}
\DeclareComet{188P}{188P}{188P/LINEAR-Mueller}
%\DeclareComet{189P}{189P}{189P/NEAT}
%\DeclareComet{18D}{18D}{18D/Perrine-Mrkos}
%\DeclareComet{190P}{190P}{190P/Mueller}
%\DeclareComet{191P}{191P}{191P/McNaught}
%\DeclareComet{192P}{192P}{192P/Shoemaker-Levy 1}
%\DeclareComet{193P}{193P}{193P/LINEAR-NEAT}
%\DeclareComet{194P}{194P}{194P/LINEAR}
%\DeclareComet{195P}{195P}{195P/Hill}
%\DeclareComet{196P}{196P}{196P/Tichy}
%\DeclareComet{197P}{197P}{197P/LINEAR}
%\DeclareComet{198P}{198P}{198P/ODAS}
%\DeclareComet{199P}{199P}{199P/Shoemaker 4}
%\DeclareComet{19P}{19P}{19P/Borrelly}
%\DeclareComet{1I}{1I}{1I/`Oumuamua}
%\DeclareComet{1P}{1P}{1P/Halley}
%\DeclareComet{200P}{200P}{200P/Larsen}
%\DeclareComet{201P}{201P}{201P/LONEOS}
%\DeclareComet{202P}{202P}{202P/Scotti}
%\DeclareComet{203P}{203P}{203P/Korlevic}
%\DeclareComet{204P}{204P}{204P/LINEAR-NEAT}
%\DeclareComet{205P}{205P}{205P/Giacobini}
%\DeclareComet{206P}{206P}{206P/Barnard-Boattini}
%\DeclareComet{207P}{207P}{207P/NEAT}
%\DeclareComet{208P}{208P}{208P/McMillan}
%\DeclareComet{209P}{209P}{209P/LINEAR}
%\DeclareComet{20D}{20D}{20D/Westphal}
%\DeclareComet{210P}{210P}{210P/Christensen}
%\DeclareComet{211P}{211P}{211P/Hill}
%\DeclareComet{212P}{212P}{212P/NEAT}
%\DeclareComet{213P}{213P}{213P/VanNess}
%\DeclareComet{213P-B}{213P-B}{213P/Van Ness-B}
%\DeclareComet{213P-C}{213P-C}{213P/Van Ness-C}
%\DeclareComet{213P-D}{213P-D}{213P/Van Ness-D}
%\DeclareComet{214P}{214P}{214P/LINEAR}
%\DeclareComet{215P}{215P}{215P/NEAT}
%\DeclareComet{216P}{216P}{216P/LINEAR}
%\DeclareComet{217P}{217P}{217P/LINEAR}
%\DeclareComet{218P}{218P}{218P/LINEAR}
%\DeclareComet{219P}{219P}{219P/LINEAR}
%\DeclareComet{21P}{21P}{21P/Giacobini-Zinner}
%\DeclareComet{220P}{220P}{220P/McNaught}
%\DeclareComet{221P}{221P}{221P/LINEAR}
%\DeclareComet{222P}{222P}{222P/LINEAR}
%\DeclareComet{223P}{223P}{223P/Skiff}
%\DeclareComet{224P}{224P}{224P/LINEAR-NEAT}
%\DeclareComet{225P}{225P}{225P/LINEAR}
%\DeclareComet{226P}{226P}{226P/Pigott-LINEAR-Kowalski}
%\DeclareComet{227P}{227P}{227P/Catalina-LINEAR}
%\DeclareComet{228P}{228P}{228P/LINEAR}
%\DeclareComet{229P}{229P}{229P/Gibbs}
%\DeclareComet{22P}{22P}{22P/Kopff}
%\DeclareComet{230P}{230P}{230P/LINEAR}
%\DeclareComet{231P}{231P}{231P/LINEAR-NEAT}
%\DeclareComet{232P}{232P}{232P/Hill}
%\DeclareComet{233P}{233P}{233P/LaSagra}
%\DeclareComet{234P}{234P}{234P/LINEAR}
%\DeclareComet{235P}{235P}{235P/LINEAR}
%\DeclareComet{236P}{236P}{236P/LINEAR}
%\DeclareComet{237P}{237P}{237P/LINEAR}
%\DeclareComet{238P}{238P}{238P/Read}
%\DeclareComet{239P}{239P}{239P/LINEAR}
%\DeclareComet{23P}{23P}{23P/Brorsen-Metcalf}
%\DeclareComet{240P}{240P}{240P/NEAT}
%\DeclareComet{240P-B}{240P-B}{240P/NEAT-B}
%\DeclareComet{241P}{241P}{241P/LINEAR}
%\DeclareComet{242P}{242P}{242P/Spahr}
\DeclareComet{243P}{243P}{243P/NEAT}
%\DeclareComet{244P}{244P}{244P/Scotti}
%\DeclareComet{245P}{245P}{245P/WISE}
%\DeclareComet{246P}{246P}{246P/NEAT}
%\DeclareComet{247P}{247P}{247P/LINEAR}
%\DeclareComet{248P}{248P}{248P/Gibbs}
%\DeclareComet{249P}{249P}{249P/LINEAR}
%\DeclareComet{24P}{24P}{24P/Schaumasse}
%\DeclareComet{250P}{250P}{250P/Larson}
%\DeclareComet{251P}{251P}{251P/LINEAR}
%\DeclareComet{252P}{252P}{252P/LINEAR}
%\DeclareComet{253P}{253P}{253P/PANSTARRS}
%\DeclareComet{254P}{254P}{254P/McNaught}
%\DeclareComet{255P}{255P}{255P/Levy}
%\DeclareComet{256P}{256P}{256P/LINEAR}
%\DeclareComet{257P}{257P}{257P/Catalina}
%\DeclareComet{258P}{258P}{258P/PANSTARRS}
%\DeclareComet{259P}{259P}{259P/Garradd}
%\DeclareComet{25D}{25D}{25D/Neujmin 2}
%\DeclareComet{260P}{260P}{260P/McNaught}
\DeclareComet{261P}{261P}{261P/Larson}
%\DeclareComet{262P}{262P}{262P/McNaught-Russell}
%\DeclareComet{263P}{263P}{263P/Gibbs}
%\DeclareComet{264P}{264P}{264P/Larsen}
%\DeclareComet{265P}{265P}{265P/LINEAR}
%\DeclareComet{266P}{266P}{266P/Christensen}
%\DeclareComet{267P}{267P}{267P/LONEOS}
%\DeclareComet{268P}{268P}{268P/Bernardi}
%\DeclareComet{269P}{269P}{269P/Jedicke}
%\DeclareComet{26P}{26P}{26P/Grigg-Skjellerup}
%\DeclareComet{270P}{270P}{270P/Gehrels}
%\DeclareComet{271P}{271P}{271P/vanHouten-Lemmon}
%\DeclareComet{272P}{272P}{272P/NEAT}
%\DeclareComet{273P}{273P}{273P/Pons-Gambart}
%\DeclareComet{274P}{274P}{274P/Tombaugh-Tenagra}
%\DeclareComet{275P}{275P}{275P/Hermann}
%\DeclareComet{276P}{276P}{276P/Vorobjov}
%\DeclareComet{277P}{277P}{277P/LINEAR}
%\DeclareComet{278P}{278P}{278P/McNaught}
%\DeclareComet{279P}{279P}{279P/LaSagra}
%\DeclareComet{27P}{27P}{27P/Crommelin}
%\DeclareComet{280P}{280P}{280P/Larsen}
%\DeclareComet{281P}{281P}{281P/MOSS}
%\DeclareComet{283P}{283P}{283P/Spacewatch}
%\DeclareComet{284P}{284P}{284P/McNaught}
%\DeclareComet{285P}{285P}{285P/LINEAR}
%\DeclareComet{286P}{286P}{286P/Christensen}
%\DeclareComet{287P}{287P}{287P/Christensen}
%\DeclareComet{288P}{288P}{288P}
%\DeclareComet{289P}{289P}{289P/Blanpain}
%\DeclareComet{28P}{28P}{28P/Neujmin 1}
%\DeclareComet{290P}{290P}{290P/Jager}
%\DeclareComet{291P}{291P}{291P/NEAT}
%\DeclareComet{292P}{292P}{292P/Li}
%\DeclareComet{293P}{293P}{293P/Spacewatch}
%\DeclareComet{294P}{294P}{294P/LINEAR}
%\DeclareComet{295P}{295P}{295P/LINEAR}
%\DeclareComet{296P}{296P}{296P/Garradd}
%\DeclareComet{297P}{297P}{297P/Beshore}
%\DeclareComet{298P}{298P}{298P/Christensen}
\DeclareComet{299P}{299P}{299P/Catalina-PANSTARRS}
%\DeclareComet{29P}{29P}{29P/Schwassmann-Wachmann 1}
%\DeclareComet{2I}{2I}{2I/Borisov}
%\DeclareComet{2P}{2P}{2P/Encke}
%\DeclareComet{300P}{300P}{300P/Catalina}
%\DeclareComet{301P}{301P}{301P/LINEAR-NEAT}
\DeclareComet{302P}{302P}{302P/Lemmon-PANSTARRS}
\DeclareComet{303P}{303P}{303P/NEAT}
%\DeclareComet{304P}{304P}{304P/Ory}
%\DeclareComet{305P}{305P}{305P/Skiff}
\DeclareComet{306P}{306P}{306P/LINEAR}
%\DeclareComet{307P}{307P}{307P/LINEAR}
%\DeclareComet{308P}{308P}{308P/Lagerkvist-Carsenty}
%\DeclareComet{309P}{309P}{309P/LINEAR}
%\DeclareComet{30P}{30P}{30P/Reinmuth 1}
%\DeclareComet{310P}{310P}{310P/Hill}
%\DeclareComet{311P}{311P}{311P/PANSTARRS}
%\DeclareComet{312P}{312P}{312P/NEAT}
%\DeclareComet{313P}{313P}{313P/Gibbs}
%\DeclareComet{314P}{314P}{314P/Montani}
%\DeclareComet{315P}{315P}{315P/LONEOS}
%\DeclareComet{316P}{316P}{316P/LONEOS-Christensen}
%\DeclareComet{317P}{317P}{317P/WISE}
%\DeclareComet{318P}{318P}{318P/McNaught-Hartley}
%\DeclareComet{319P}{319P}{319P/Catalina-McNaught}
%\DeclareComet{31P}{31P}{31P/Schwassmann-Wachmann 2}
%\DeclareComet{320P}{320P}{320P/McNaught}
%\DeclareComet{321P}{321P}{321P/SOHO}
%\DeclareComet{322P}{322P}{322P/SOHO}
%\DeclareComet{323P}{323P}{323P/SOHO}
%\DeclareComet{323P-B}{323P-B}{323P/SOHO-B}
%\DeclareComet{323P-C}{323P-C}{323P/SOHO-C}
%\DeclareComet{324P}{324P}{324P/La Sagra}
%\DeclareComet{325P}{325P}{325P/Yang-Gao}
%\DeclareComet{326P}{326P}{326P/Hill}
%\DeclareComet{327P}{327P}{327P/VanNess}
%\DeclareComet{328P}{328P}{328P/LONEOS-Tucker}
%\DeclareComet{329P}{329P}{329P/LINEAR-Catalina}
%\DeclareComet{32P}{32P}{32P/Comas Sola}
%\DeclareComet{330P}{330P}{330P/Catalina}
%\DeclareComet{331P}{331P}{331P/Gibbs}
%\DeclareComet{332P}{332P}{332P/Ikeya-Murakami}
%\DeclareComet{332P-A}{332P-A}{332P/Ikeya-Murakami-A}
%\DeclareComet{332P-B}{332P-B}{332P/Ikeya-Murakami-B}
%\DeclareComet{332P-C}{332P-C}{332P/Ikeya-Murakami-C}
%\DeclareComet{332P-D}{332P-D}{332P/Ikeya-Murakami-D}
%\DeclareComet{332P-E}{332P-E}{332P/Ikeya-Murakami-E}
%\DeclareComet{332P-F}{332P-F}{332P/Ikeya-Murakami-F}
%\DeclareComet{332P-G}{332P-G}{332P/Ikeya-Murakami-G}
%\DeclareComet{332P-H}{332P-H}{332P/Ikeya-Murakami-H}
%\DeclareComet{332P-I}{332P-I}{332P/Ikeya-Murakami-I}
%\DeclareComet{332P-J}{332P-J}{332P/Ikeya-Murakami-J}
%\DeclareComet{333P}{333P}{333P/LINEAR}
%\DeclareComet{334P}{334P}{334P/NEAT}
%\DeclareComet{335P}{335P}{335P/Gibbs}
%\DeclareComet{336P}{336P}{336P/McNaught}
%\DeclareComet{337P}{337P}{337P/WISE}
%\DeclareComet{338P}{338P}{338P/McNaught}
%\DeclareComet{339P}{339P}{339P/Gibbs}
%\DeclareComet{33P}{33P}{33P/Daniel}
%\DeclareComet{340P}{340P}{340P/Boattini}
%\DeclareComet{341P}{341P}{341P/Gibbs}
%\DeclareComet{342P}{342P}{342P/SOHO}
%\DeclareComet{343P}{343P}{343P/NEAT-LONEOS}
%\DeclareComet{344P}{344P}{344P/Read}
%\DeclareComet{345P}{345P}{345P/LINEAR}
%\DeclareComet{346P}{346P}{346P/Catalina}
%\DeclareComet{347P}{347P}{347P/PANSTARRS}
%\DeclareComet{348P}{348P}{348P/PANSTARRS}
%\DeclareComet{349P}{349P}{349P/Lemmon}
%\DeclareComet{34D}{34D}{34D/Gale}
%\DeclareComet{350P}{350P}{350P/McNaught}
\DeclareComet{351P}{351P}{351P/Wiegert-PANSTARRS}
%\DeclareComet{352P}{352P}{352P/Skiff}
%\DeclareComet{353P}{353P}{353P/McNaught}
%\DeclareComet{354P}{354P}{354P/LINEAR}
%\DeclareComet{355P}{355P}{355P/LINEAR-NEAT}
%\DeclareComet{356P}{356P}{356P/WISE}
%\DeclareComet{357P}{357P}{357P/Hill}
%\DeclareComet{358P}{358P}{358P/PANSTARRS}
%\DeclareComet{359P}{359P}{359P/LONEOS}
%\DeclareComet{35P}{35P}{35P/Herschel-Rigollet}
%\DeclareComet{360P}{360P}{360P/WISE}
%\DeclareComet{361P}{361P}{361P/Spacewatch}
%\DeclareComet{363P}{363P}{363P/Lemmon}
%\DeclareComet{364P}{364P}{364P/PANSTARRS}
%\DeclareComet{365P}{365P}{365P/PANSTARRS}
%\DeclareComet{366P}{366P}{366P/Spacewatch}
%\DeclareComet{367P}{367P}{367P/Catalina}
%\DeclareComet{368P}{368P}{368P/NEAT}
%\DeclareComet{369P}{369P}{369P/Hill}
%\DeclareComet{36P}{36P}{36P/Whipple}
%\DeclareComet{370P}{370P}{370P/NEAT}
%\DeclareComet{371P}{371P}{371P/LINEAR-Skiff}
%\DeclareComet{372P}{372P}{372P/McNaught}
%\DeclareComet{373P}{373P}{373P/Rinner}
%\DeclareComet{374P}{374P}{374P/Larson}
%\DeclareComet{375P}{375P}{375P/Hill}
%\DeclareComet{376P}{376P}{376P/LONEOS}
%\DeclareComet{377P}{377P}{377P/Scotti}
%\DeclareComet{378P}{378P}{378P/McNaught}
%\DeclareComet{379P}{379P}{379P/Spacewatch}
%\DeclareComet{37P}{37P}{37P/Forbes}
%\DeclareComet{380P}{380P}{380P/PANSTARRS}
%\DeclareComet{381P}{381P}{381P/LINEAR-Spacewatch}
%\DeclareComet{382P}{382P}{382P/Larson}
%\DeclareComet{383P}{383P}{383P/Christensen}
%\DeclareComet{384P}{384P}{384P/Kowalski}
%\DeclareComet{385P}{385P}{385P/Hill}
%\DeclareComet{386P}{386P}{386P/PANSTARRS}
%\DeclareComet{387P}{387P}{387P/Boattini}
%\DeclareComet{388P}{388P}{388P/Gibbs}
%\DeclareComet{389P}{389P}{389P/SidingSpring}
%\DeclareComet{38P}{38P}{38P/Stephan-Oterma}
%\DeclareComet{390P}{390P}{390P/Gibbs}
%\DeclareComet{391P}{391P}{391P/Kowalski}
%\DeclareComet{392P}{392P}{392P/LINEAR}
%\DeclareComet{393P}{393P}{393P/Spacewatch-Hill}
%\DeclareComet{394P}{394P}{394P/PANSTARRS}
%\DeclareComet{395P}{395P}{395P/Catalina-NEAT}
%\DeclareComet{396P}{396P}{396P/Leonard}
%\DeclareComet{397P}{397P}{397P/Lemmon}
%\DeclareComet{398P}{398P}{398P/Boattini}
%\DeclareComet{399P}{399P}{399P/PANSTARRS}
%\DeclareComet{39P}{39P}{39P/Oterma}
%\DeclareComet{3D-A}{3D-A}{3D/Biela-A}
%\DeclareComet{3D-B}{3D-B}{3D/Biela-B}
\DeclareComet{3I}{3I}{3I/ATLAS}
%\DeclareComet{400P}{400P}{400P/PANSTARRS}
%\DeclareComet{401P}{401P}{401P/McNaught}
%\DeclareComet{402P}{402P}{402P/LINEAR}
%\DeclareComet{403P}{403P}{403P/Catalina}
%\DeclareComet{404P}{404P}{404P/Bressi}
%\DeclareComet{405P}{405P}{405P/Lemmon}
%\DeclareComet{406P}{406P}{406P/Gibbs}
%\DeclareComet{407P}{407P}{407P/PANSTARRS-Fuls}
%\DeclareComet{408P}{408P}{408P/Novichonok-Gerke}
%\DeclareComet{409P}{409P}{409P/LONEOS-Hill}
%\DeclareComet{40P}{40P}{40P/Vaisala 1}
%\DeclareComet{410P}{410P}{410P/NEAT-LINEAR}
%\DeclareComet{411P}{411P}{411P/Christensen}
%\DeclareComet{412P}{412P}{412P/WISE}
%\DeclareComet{413P}{413P}{413P/Larson}
%\DeclareComet{414P}{414P}{414P/STEREO}
%\DeclareComet{415P}{415P}{415P/Tenagra}
%\DeclareComet{416P}{416P}{416P/Scotti}
%\DeclareComet{417P}{417P}{417P/NEOWISE}
%\DeclareComet{418P}{418P}{418P/LINEAR}
%\DeclareComet{419P}{419P}{419P/PANSTARRS}
%\DeclareComet{41P}{41P}{41P/Tuttle-Giacobini-Kresak}
%\DeclareComet{420P}{420P}{420P/Hill}
%\DeclareComet{421P}{421P}{421P/McNaught}
%\DeclareComet{422P}{422P}{422P/Christensen}
%\DeclareComet{423P}{423P}{423P/Lemmon}
%\DeclareComet{424P}{424P}{424P/LaSagra}
%\DeclareComet{425P}{425P}{425P/Kowalski}
%\DeclareComet{426P}{426P}{426P/PANSTARRS}
%\DeclareComet{427P}{427P}{427P/ATLAS}
%\DeclareComet{428P}{428P}{428P/Gibbs}
%\DeclareComet{429P}{429P}{429P/LINEAR-Hill}
%\DeclareComet{42P}{42P}{42P/Neujmin 3}
%\DeclareComet{430P}{430P}{430P/Scotti}
%\DeclareComet{431P}{431P}{431P/Scotti}
%\DeclareComet{432P}{432P}{432P/PANSTARRS}
\DeclareComet{433P}{433P}{433P/(248370) 2005 QN$_{173}$}
%\DeclareComet{434P}{434P}{434P/Tenagra}
%\DeclareComet{435P}{435P}{435P/PANSTARRS}
%\DeclareComet{436P}{436P}{436P/Garradd}
%\DeclareComet{437P}{437P}{437P/Lemmon-PANSTARRS}
%\DeclareComet{438P}{438P}{438P/Christensen}
%\DeclareComet{439P}{439P}{439P/LINEAR}
%\DeclareComet{43P}{43P}{43P/Wolf-Harrington}
%\DeclareComet{440P}{440P}{440P/Kobayashi}
\DeclareComet{441P}{441P}{441P/PANSTARRS}
%\DeclareComet{442P}{442P}{442P/McNaught}
%\DeclareComet{443P}{443P}{443P/PANSTARRS-Christensen}
%\DeclareComet{444P}{444P}{444P/WISE-PANSTARRS}
%\DeclareComet{445P}{445P}{445P/Lemmon-PANSTARRS}
%\DeclareComet{446P}{446P}{446P/McNaught}
%\DeclareComet{447P}{447P}{447P/Sheppard-Tholen}
%\DeclareComet{448P}{448P}{448P/PANSTARRS}
%\DeclareComet{449P}{449P}{449P/Leonard}
%\DeclareComet{44P}{44P}{44P/Reinmuth 2}
%\DeclareComet{450P}{450P}{450P/LONEOS}
%\DeclareComet{451P}{451P}{451P/Christensen}
%\DeclareComet{452P}{452P}{452P/Sheppard-Jewitt}
%\DeclareComet{453P}{453P}{453P/WISE-Lemmon}
%\DeclareComet{454P}{454P}{454P/PANSTARRS}
%\DeclareComet{455P}{455P}{455P/PANSTARRS}
%\DeclareComet{456P}{456P}{456P/PANSTARRS}
%\DeclareComet{457P}{457P}{457P/Lemmon-PANSTARRS}
%\DeclareComet{458P}{458P}{458P/Jahn}
%\DeclareComet{459P}{459P}{459P/Catalina}
%\DeclareComet{45P}{45P}{45P/Honda-Mrkos-Pajdusakova}
%\DeclareComet{460P}{460P}{460P/PANSTARRS}
%\DeclareComet{461P}{461P}{461P/WISE}
%\DeclareComet{462P}{462P}{462P/LONEOS-PANSTARRS}
%\DeclareComet{463P}{463P}{463P/NEOWISE}
%\DeclareComet{464P}{464P}{464P/PANSTARRS}
%\DeclareComet{465P}{465P}{465P/Hill}
%\DeclareComet{466P}{466P}{466P/PANSTARRS}
%\DeclareComet{467P}{467P}{467P/LINEAR-Grauer}
%\DeclareComet{468P}{468P}{468P/SidingSpring}
%\DeclareComet{469P}{469P}{469P/PANSTARRS}
%\DeclareComet{46P}{46P}{46P/Wirtanen}
%\DeclareComet{470P}{470P}{470P/PANSTARRS}
%\DeclareComet{471P}{471P}{471P/LINEAR-Lemmon}
%\DeclareComet{472P}{472P}{472P/NEAT-LINEAR}
%\DeclareComet{473P}{473P}{473P/NEAT}
%\DeclareComet{474P}{474P}{474P/Hogan}
%\DeclareComet{475P}{475P}{475P/Spacewatch-LINEAR}
%\DeclareComet{476P}{476P}{476P/PANSTARRS}
%\DeclareComet{477P}{477P}{477P/PANSTARRS}
%\DeclareComet{478P}{478P}{478P/ATLAS}
%\DeclareComet{479P}{479P}{479P/Elenin}
%\DeclareComet{47P}{47P}{47P/Ashbrook-Jackson}
%\DeclareComet{480P}{480P}{480P/PANSTARRS}
%\DeclareComet{481P}{481P}{481P/Lemmon-PANSTARRS}
%\DeclareComet{482P}{482P}{482P/PANSTARRS}
%\DeclareComet{483P}{483P}{483P/PANSTARRS}
%\DeclareComet{483P-A}{483P-A}{483P/PANSTARRS-A}
%\DeclareComet{483P-B}{483P-B}{483P/PANSTARRS-B}
%\DeclareComet{484P}{484P}{484P/Spacewatch}
%\DeclareComet{485P}{485P}{485P/Sheppard-Tholen}
\DeclareComet{486P}{486P}{486P/Leonard}
%\DeclareComet{487P}{487P}{487P/SidingSpring}
%\DeclareComet{488P}{488P}{488P/NEAT-PANSTARRS}
%\DeclareComet{489P}{489P}{489P/Denning}
%\DeclareComet{48P}{48P}{48P/Johnson}
%\DeclareComet{490P}{490P}{490P/ATLAS}
\DeclareComet{491P}{491P}{491P/Spacewatch-PANSTARRS}
%\DeclareComet{492P}{492P}{492P/LINEAR}
%\DeclareComet{493P}{493P}{493P/LONEOS}
%\DeclareComet{494P}{494P}{494P/PANSTARRS}
%\DeclareComet{495P}{495P}{495P/Christensen}
%\DeclareComet{496P}{496P}{496P/Hill}
%\DeclareComet{497P}{497P}{497P/Spacewatch-PANSTARRS}
%\DeclareComet{498P}{498P}{498P/LINEAR}
%\DeclareComet{499P}{499P}{499P/Catalina}
%\DeclareComet{49P}{49P}{49P/Arend-Rigaux}
%\DeclareComet{4P}{4P}{4P/Faye}
%\DeclareComet{500P}{500P}{500P/PANSTARRS}
%\DeclareComet{501P}{501P}{501P/Rankin}
%\DeclareComet{502P}{502P}{502P/NEAT}
%\DeclareComet{503P}{503P}{503P/PANSTARRS}
%\DeclareComet{504P}{504P}{504P/WISE-PANSTARRS}
%\DeclareComet{505P}{505P}{505P/Palomar}
%\DeclareComet{506P}{506P}{506P/WISE-LINEAR}
%\DeclareComet{507P}{507P}{507P/Lemmon}
%\DeclareComet{508P}{508P}{508P/McNaught}
%\DeclareComet{509P}{509P}{509P/Catalina}
%\DeclareComet{50P}{50P}{50P/Arend}
\DeclareComet{510P}{510P}{510P/Boattini}
%\DeclareComet{511P}{511P}{511P/PANSTARRS}
%\DeclareComet{512P}{512P}{512P/PANSTARRS}
\DeclareComet{513P}{513P}{513P/Broughton}
%\DeclareComet{514P}{514P}{514P/Lemmon-PANSTARRS}
%\DeclareComet{515P}{515P}{515P/PANSTARRS}
%\DeclareComet{516P}{516P}{516P/PANSTARRS}
%\DeclareComet{51P}{51P}{51P/Harrington}
%\DeclareComet{51P-A}{51P-A}{51P/Harrington-A}
%\DeclareComet{51P-D}{51P-D}{51P/Harrington-D}
%\DeclareComet{52P}{52P}{52P/Harrington-Abell}
%\DeclareComet{53P}{53P}{53P/VanBiesbroeck}
%\DeclareComet{54P}{54P}{54P/deVico-Swift-NEAT}
%\DeclareComet{55P}{55P}{55P/Tempel-Tuttle}
%\DeclareComet{56P}{56P}{56P/Slaughter-Burnham}
%\DeclareComet{57P}{57P}{57P/duToit-Neujmin-Delporte}
%\DeclareComet{58P}{58P}{58P/Jackson-Neujmin}
%\DeclareComet{59P}{59P}{59P/Kearns-Kwee}
%\DeclareComet{5D}{5D}{5D/Brorsen}
%\DeclareComet{60P}{60P}{60P/Tsuchinshan 2}
%\DeclareComet{61P}{61P}{61P/Shajn-Schaldach}
%\DeclareComet{62P}{62P}{62P/Tsuchinshan 1}
%\DeclareComet{63P}{63P}{63P/Wild 1}
%\DeclareComet{64P}{64P}{64P/Swift-Gehrels}
\DeclareComet{65P}{65P}{65P/Gunn}
%\DeclareComet{66P}{66P}{66P/duToit}
%\DeclareComet{67P}{67P}{67P/Churyumov-Gerasimenko}
%\DeclareComet{68P}{68P}{68P/Klemola}
%\DeclareComet{69P}{69P}{69P/Taylor}
%\DeclareComet{6P}{6P}{6P/d'Arrest}
%\DeclareComet{70P}{70P}{70P/Kojima}
%\DeclareComet{71P}{71P}{71P/Clark}
%\DeclareComet{72P}{72P}{72P/Denning-Fujikawa}
%\DeclareComet{73P}{73P}{73P/Schwassmann-Wachmann 3}
%\DeclareComet{73P-AA}{73P-AA}{73P/Schwassmann-Wachmann 3-AA}
%\DeclareComet{73P-AB}{73P-AB}{73P/Schwassmann-Wachmann 3-AB}
%\DeclareComet{73P-AC}{73P-AC}{73P/Schwassmann-Wachmann 3-AC}
%\DeclareComet{73P-AD}{73P-AD}{73P/Schwassmann-Wachmann 3-AD}
%\DeclareComet{73P-AE}{73P-AE}{73P/Schwassmann-Wachmann 3-AE}
%\DeclareComet{73P-AF}{73P-AF}{73P/Schwassmann-Wachmann 3-AF}
%\DeclareComet{73P-AG}{73P-AG}{73P/Schwassmann-Wachmann 3-AG}
%\DeclareComet{73P-AH}{73P-AH}{73P/Schwassmann-Wachmann 3-AH}
%\DeclareComet{73P-AI}{73P-AI}{73P/Schwassmann-Wachmann 3-AI}
%\DeclareComet{73P-AJ}{73P-AJ}{73P/Schwassmann-Wachmann 3-AJ}
%\DeclareComet{73P-AK}{73P-AK}{73P/Schwassmann-Wachmann 3-AK}
%\DeclareComet{73P-AL}{73P-AL}{73P/Schwassmann-Wachmann 3-AL}
%\DeclareComet{73P-AM}{73P-AM}{73P/Schwassmann-Wachmann 3-AM}
%\DeclareComet{73P-AN}{73P-AN}{73P/Schwassmann-Wachmann 3-AN}
%\DeclareComet{73P-AO}{73P-AO}{73P/Schwassmann-Wachmann 3-AO}
%\DeclareComet{73P-AP}{73P-AP}{73P/Schwassmann-Wachmann 3-AP}
%\DeclareComet{73P-AQ}{73P-AQ}{73P/Schwassmann-Wachmann 3-AQ}
%\DeclareComet{73P-AR}{73P-AR}{73P/Schwassmann-Wachmann 3-AR}
%\DeclareComet{73P-AS}{73P-AS}{73P/Schwassmann-Wachmann 3-AS}
%\DeclareComet{73P-AT}{73P-AT}{73P/Schwassmann-Wachmann 3-AT}
%\DeclareComet{73P-AU}{73P-AU}{73P/Schwassmann-Wachmann 3-AU}
%\DeclareComet{73P-AV}{73P-AV}{73P/Schwassmann-Wachmann 3-AV}
%\DeclareComet{73P-AW}{73P-AW}{73P/Schwassmann-Wachmann 3-AW}
%\DeclareComet{73P-AX}{73P-AX}{73P/Schwassmann-Wachmann 3-AX}
%\DeclareComet{73P-AY}{73P-AY}{73P/Schwassmann-Wachmann 3-AY}
%\DeclareComet{73P-AZ}{73P-AZ}{73P/Schwassmann-Wachmann 3-AZ}
%\DeclareComet{73P-B}{73P-B}{73P/Schwassmann-Wachmann 3-B}
%\DeclareComet{73P-BA}{73P-BA}{73P/Schwassmann-Wachmann 3-BA}
%\DeclareComet{73P-BB}{73P-BB}{73P/Schwassmann-Wachmann 3-BB}
%\DeclareComet{73P-BC}{73P-BC}{73P/Schwassmann-Wachmann 3-BC}
%\DeclareComet{73P-BD}{73P-BD}{73P/Schwassmann-Wachmann 3-BD}
%\DeclareComet{73P-BE}{73P-BE}{73P/Schwassmann-Wachmann 3-BE}
%\DeclareComet{73P-BF}{73P-BF}{73P/Schwassmann-Wachmann 3-BF}
%\DeclareComet{73P-BG}{73P-BG}{73P/Schwassmann-Wachmann 3-BG}
%\DeclareComet{73P-BH}{73P-BH}{73P/Schwassmann-Wachmann 3-BH}
%\DeclareComet{73P-BI}{73P-BI}{73P/Schwassmann-Wachmann 3-BI}
%\DeclareComet{73P-BJ}{73P-BJ}{73P/Schwassmann-Wachmann 3-BJ}
%\DeclareComet{73P-BK}{73P-BK}{73P/Schwassmann-Wachmann 3-BK}
%\DeclareComet{73P-BL}{73P-BL}{73P/Schwassmann-Wachmann 3-BL}
%\DeclareComet{73P-BM}{73P-BM}{73P/Schwassmann-Wachmann 3-BM}
%\DeclareComet{73P-BN}{73P-BN}{73P/Schwassmann-Wachmann 3-BN}
%\DeclareComet{73P-BO}{73P-BO}{73P/Schwassmann-Wachmann 3-BO}
%\DeclareComet{73P-BP}{73P-BP}{73P/Schwassmann-Wachmann 3-BP}
%\DeclareComet{73P-BQ}{73P-BQ}{73P/Schwassmann-Wachmann 3-BQ}
%\DeclareComet{73P-BR}{73P-BR}{73P/Schwassmann-Wachmann 3-BR}
%\DeclareComet{73P-BS}{73P-BS}{73P/Schwassmann-Wachmann 3-BS}
%\DeclareComet{73P-BT}{73P-BT}{73P/Schwassmann-Wachmann 3-BT}
%\DeclareComet{73P-BU}{73P-BU}{73P/Schwassmann-Wachmann 3-BU}
%\DeclareComet{73P-BV}{73P-BV}{73P/Schwassmann-Wachmann 3-BV}
%\DeclareComet{73P-BW}{73P-BW}{73P/Schwassmann-Wachmann 3-BW}
%\DeclareComet{73P-BX}{73P-BX}{73P/Schwassmann-Wachmann 3-BX}
%\DeclareComet{73P-BY}{73P-BY}{73P/Schwassmann-Wachmann 3-BY}
%\DeclareComet{73P-C}{73P-C}{73P/Schwassmann-Wachmann 3-C}
%\DeclareComet{73P-E}{73P-E}{73P/Schwassmann-Wachmann 3-E}
%\DeclareComet{73P-G}{73P-G}{73P/Schwassmann-Wachmann 3-G}
%\DeclareComet{73P-H}{73P-H}{73P/Schwassmann-Wachmann 3-H}
%\DeclareComet{73P-J}{73P-J}{73P/Schwassmann-Wachmann 3-J}
%\DeclareComet{73P-K}{73P-K}{73P/Schwassmann-Wachmann 3-K}
%\DeclareComet{73P-L}{73P-L}{73P/Schwassmann-Wachmann 3-L}
%\DeclareComet{73P-M}{73P-M}{73P/Schwassmann-Wachmann 3-M}
%\DeclareComet{73P-N}{73P-N}{73P/Schwassmann-Wachmann 3-N}
%\DeclareComet{73P-P}{73P-P}{73P/Schwassmann-Wachmann 3-P}
%\DeclareComet{73P-Q}{73P-Q}{73P/Schwassmann-Wachmann 3-Q}
%\DeclareComet{73P-R}{73P-R}{73P/Schwassmann-Wachmann 3-R}
%\DeclareComet{73P-S}{73P-S}{73P/Schwassmann-Wachmann 3-S}
%\DeclareComet{73P-T}{73P-T}{73P/Schwassmann-Wachmann 3-T}
%\DeclareComet{73P-U}{73P-U}{73P/Schwassmann-Wachmann 3-U}
%\DeclareComet{73P-V}{73P-V}{73P/Schwassmann-Wachmann 3-V}
%\DeclareComet{73P-W}{73P-W}{73P/Schwassmann-Wachmann 3-W}
%\DeclareComet{73P-X}{73P-X}{73P/Schwassmann-Wachmann 3-X}
%\DeclareComet{73P-Y}{73P-Y}{73P/Schwassmann-Wachmann 3-Y}
%\DeclareComet{73P-Z}{73P-Z}{73P/Schwassmann-Wachmann 3-Z}
%\DeclareComet{74P}{74P}{74P/Smirnova-Chernykh}
%\DeclareComet{75D}{75D}{75D/Kohoutek}
%\DeclareComet{76P}{76P}{76P/West-Kohoutek-Ikemura}
\DeclareComet{77P}{77P}{77P/Longmore}
\DeclareComet{78P}{78P}{78P/Gehrels 2}
%\DeclareComet{79P}{79P}{79P/duToit-Hartley}
%\DeclareComet{7P}{7P}{7P/Pons-Winnecke}
%\DeclareComet{80P}{80P}{80P/Peters-Hartley}
%\DeclareComet{81P}{81P}{81P/Wild 2}
%\DeclareComet{82P}{82P}{82P/Gehrels 3}
%\DeclareComet{83D}{83D}{83D/Russell 1}
%\DeclareComet{84P}{84P}{84P/Giclas}
%\DeclareComet{85D}{85D}{85D/Boethin}
%\DeclareComet{86P}{86P}{86P/Wild 3}
%\DeclareComet{87P}{87P}{87P/Bus}
%\DeclareComet{88P}{88P}{88P/Howell}
%\DeclareComet{89P}{89P}{89P/Russell 2}
%\DeclareComet{8P}{8P}{8P/Tuttle}
%\DeclareComet{90P}{90P}{90P/Gehrels 1}
%\DeclareComet{91P}{91P}{91P/Russell 3}
%\DeclareComet{92P}{92P}{92P/Sanguin}
%\DeclareComet{93P}{93P}{93P/Lovas 1}
%\DeclareComet{94P}{94P}{94P/Russell 4}
%\DeclareComet{96P}{96P}{96P/Machholz 1}
%\DeclareComet{96P-B}{96P-B}{96P/Machholz 1-B}
%\DeclareComet{96P-C}{96P-C}{96P/Machholz 1-C}
%\DeclareComet{97P}{97P}{97P/Metcalf-Brewington}
%\DeclareComet{98P}{98P}{98P/Takamizawa}
\DeclareComet{99P}{99P}{99P/Kowal 1}
%\DeclareComet{9P}{9P}{9P/Tempel 1}
%\DeclareComet{A2010LN135}{A/2010 LN135}{A/2010 LN135}
%\DeclareComet{A2018V3}{A/2018 V3}{A/2018 V3}
%\DeclareComet{A2018W3}{A/2018 W3}{A/2018 W3}
%\DeclareComet{A2019G3}{A/2019 G3}{A/2019 G3}
%\DeclareComet{A2019N2}{A/2019 N2}{A/2019 N2}
%\DeclareComet{A2019O4}{A/2019 O4}{A/2019 O4}
%\DeclareComet{A2019Q2}{A/2019 Q2}{A/2019 Q2}
%\DeclareComet{A2019T1}{A/2019 T1}{A/2019 T1}
%\DeclareComet{A2020A1}{A/2020 A1}{A/2020 A1}
%\DeclareComet{A2020B1}{A/2020 B1}{A/2020 B1}
%\DeclareComet{A2020H9}{A/2020 H9}{A/2020 H9}
%\DeclareComet{A2020M4}{A/2020 M4}{A/2020 M4}
%\DeclareComet{A2021E2}{A/2021 E2}{A/2021 E2}
%\DeclareComet{A2021E4}{A/2021 E4}{A/2021 E4}
%\DeclareComet{A2022B3}{A/2022 B3}{A/2022 B3}
%\DeclareComet{A2023H4}{A/2023 H4}{A/2023 H4}
%\DeclareComet{A2023R3}{A/2023 R3}{A/2023 R3}
%\DeclareComet{A2024G8}{A/2024 G8}{A/2024 G8}
%\DeclareComet{A2024U2}{A/2024 U2}{A/2024 U2}
%\DeclareComet{A2024W2}{A/2024 W2}{A/2024 W2}
%\DeclareComet{A2025A7}{A/2025 A7}{A/2025 A7}
%\DeclareComet{A2025O4}{A/2025 O4}{A/2025 O4}
%\DeclareComet{A2025P1}{A/2025 P1}{A/2025 P1}
%\DeclareComet{A2025S2}{A/2025 S2}{A/2025 S2}
%\DeclareComet{A2025S3}{A/2025 S3}{A/2025 S3}
%\DeclareComet{A2026E1}{A/2026 E1}{A/2026 E1}
%\DeclareComet{C-146P1}{C/-146 P1}{C/-146 P1}
%\DeclareComet{C-43K1}{C/- 43 K1}{C/- 43 K1}
%\DeclareComet{C1014C1}{C/1014 C1}{C/1014 C1}
%\DeclareComet{C1018P1}{C/1018 P1}{C/1018 P1}
%\DeclareComet{C1080P1}{C/1080 P1}{C/1080 P1}
%\DeclareComet{C1092A1}{C/1092 A1}{C/1092 A1}
%\DeclareComet{C1097T1}{C/1097 T1}{C/1097 T1}
%\DeclareComet{C1110K1}{C/1110 K1}{C/1110 K1}
%\DeclareComet{C1132T1}{C/1132 T1}{C/1132 T1}
%\DeclareComet{C1147A1}{C/1147 A1}{C/1147 A1}
%\DeclareComet{C1230X1}{C/1230 X1}{C/1230 X1}
%\DeclareComet{C1240B1}{C/1240 B1}{C/1240 B1}
%\DeclareComet{C1245D1}{C/1245 D1}{C/1245 D1}
%\DeclareComet{C1264N1}{C/1264 N1}{C/1264 N1}
%\DeclareComet{C1293V1}{C/1293 V1}{C/1293 V1}
%\DeclareComet{C1299B1}{C/1299 B1}{C/1299 B1}
%\DeclareComet{C1304C1}{C/1304 C1}{C/1304 C1}
%\DeclareComet{C1304Y1}{C/1304 Y1}{C/1304 Y1}
%\DeclareComet{C1315U1}{C/1315 U1}{C/1315 U1}
%\DeclareComet{C1337M1}{C/1337 M1}{C/1337 M1}
%\DeclareComet{C1340F1}{C/1340 F1}{C/1340 F1}
%\DeclareComet{C1345O1}{C/1345 O1}{C/1345 O1}
%\DeclareComet{C1351W1}{C/1351 W1}{C/1351 W1}
%\DeclareComet{C1362E1}{C/1362 E1}{C/1362 E1}
%\DeclareComet{C1368E1}{C/1368 E1}{C/1368 E1}
%\DeclareComet{C1376M1}{C/1376 M1}{C/1376 M1}
%\DeclareComet{C1402D1}{C/1402 D1}{C/1402 D1}
%\DeclareComet{C1433R1}{C/1433 R1}{C/1433 R1}
%\DeclareComet{C1439F1}{C/1439 F1}{C/1439 F1}
%\DeclareComet{C1449Y1}{C/1449 Y1}{C/1449 Y1}
%\DeclareComet{C1457L1}{C/1457 L1}{C/1457 L1}
%\DeclareComet{C1458Y1}{C/1458 Y1}{C/1458 Y1}
%\DeclareComet{C1462M1}{C/1462 M1}{C/1462 M1}
%\DeclareComet{C1468S1}{C/1468 S1}{C/1468 S1}
%\DeclareComet{C1471Y1}{C/1471 Y1}{C/1471 Y1}
%\DeclareComet{C1490Y1}{C/1490 Y1}{C/1490 Y1}
%\DeclareComet{C1499Q1}{C/1499 Q1}{C/1499 Q1}
%\DeclareComet{C1500H1}{C/1500 H1}{C/1500 H1}
%\DeclareComet{C1506O1}{C/1506 O1}{C/1506 O1}
%\DeclareComet{C1532R1}{C/1532 R1}{C/1532 R1}
%\DeclareComet{C1533M1}{C/1533 M1}{C/1533 M1}
%\DeclareComet{C1538A1}{C/1538 A1}{C/1538 A1}
%\DeclareComet{C1539H1}{C/1539 H1}{C/1539 H1}
%\DeclareComet{C1556D1}{C/1556 D1}{C/1556 D1}
%\DeclareComet{C1557T1}{C/1557 T1}{C/1557 T1}
%\DeclareComet{C1558P1}{C/1558 P1}{C/1558 P1}
%\DeclareComet{C1577V1}{C/1577 V1}{C/1577 V1}
%\DeclareComet{C1580T1}{C/1580 T1}{C/1580 T1}
%\DeclareComet{C1582J1}{C/1582 J1}{C/1582 J1}
%\DeclareComet{C1585T1}{C/1585 T1}{C/1585 T1}
%\DeclareComet{C1590E1}{C/1590 E1}{C/1590 E1}
%\DeclareComet{C1593O1}{C/1593 O1}{C/1593 O1}
%\DeclareComet{C1596N1}{C/1596 N1}{C/1596 N1}
%\DeclareComet{C1618Q1}{C/1618 Q1}{C/1618 Q1}
%\DeclareComet{C1618V1}{C/1618 V1}{C/1618 V1}
%\DeclareComet{C1618W1}{C/1618 W1}{C/1618 W1}
%\DeclareComet{C1639U1}{C/1639 U1}{C/1639 U1}
%\DeclareComet{C1652Y1}{C/1652 Y1}{C/1652 Y1}
%\DeclareComet{C1664W1}{C/1664 W1}{C/1664 W1}
%\DeclareComet{C1665F1}{C/1665 F1}{C/1665 F1}
%\DeclareComet{C1668E1}{C/1668 E1}{C/1668 E1}
%\DeclareComet{C1672E1}{C/1672 E1}{C/1672 E1}
%\DeclareComet{C1677H1}{C/1677 H1}{C/1677 H1}
%\DeclareComet{C1680V1}{C/1680 V1}{C/1680 V1}
%\DeclareComet{C1683O1}{C/1683 O1}{C/1683 O1}
%\DeclareComet{C1684N1}{C/1684 N1}{C/1684 N1}
%\DeclareComet{C1686R1}{C/1686 R1}{C/1686 R1}
%\DeclareComet{C1689X1}{C/1689 X1}{C/1689 X1}
%\DeclareComet{C1695U1}{C/1695 U1}{C/1695 U1}
%\DeclareComet{C1698R1}{C/1698 R1}{C/1698 R1}
%\DeclareComet{C1699D1}{C/1699 D1}{C/1699 D1}
%\DeclareComet{C1701U1}{C/1701 U1}{C/1701 U1}
%\DeclareComet{C1702H1}{C/1702 H1}{C/1702 H1}
%\DeclareComet{C1706F1}{C/1706 F1}{C/1706 F1}
%\DeclareComet{C1707W1}{C/1707 W1}{C/1707 W1}
%\DeclareComet{C1718B1}{C/1718 B1}{C/1718 B1}
%\DeclareComet{C1723T1}{C/1723 T1}{C/1723 T1}
%\DeclareComet{C1729P1}{C/1729 P1}{C/1729 P1}
%\DeclareComet{C1733K1}{C/1733 K1}{C/1733 K1}
%\DeclareComet{C1737C1}{C/1737 C1}{C/1737 C1}
%\DeclareComet{C1739K1}{C/1739 K1}{C/1739 K1}
%\DeclareComet{C1742C1}{C/1742 C1}{C/1742 C1}
%\DeclareComet{C1743C1}{C/1743 C1}{C/1743 C1}
%\DeclareComet{C1743Q1}{C/1743 Q1}{C/1743 Q1}
%\DeclareComet{C1743X1}{C/1743 X1}{C/1743 X1}
%\DeclareComet{C1746P1}{C/1746 P1}{C/1746 P1}
%\DeclareComet{C1748H1}{C/1748 H1}{C/1748 H1}
%\DeclareComet{C1748K1}{C/1748 K1}{C/1748 K1}
%\DeclareComet{C1750C1}{C/1750 C1}{C/1750 C1}
%\DeclareComet{C1757R1}{C/1757 R1}{C/1757 R1}
%\DeclareComet{C1758K1}{C/1758 K1}{C/1758 K1}
%\DeclareComet{C1760A1}{C/1760 A1}{C/1760 A1 (Great comet)}
%\DeclareComet{C1760B1}{C/1760 B1}{C/1760 B1 (Messier)}
%\DeclareComet{C1762K1}{C/1762 K1}{C/1762 K1 (Klinkenberg)}
%\DeclareComet{C1763S1}{C/1763 S1}{C/1763 S1 (Messier)}
%\DeclareComet{C1764A1}{C/1764 A1}{C/1764 A1 (Messier)}
%\DeclareComet{C1766E1}{C/1766 E1}{C/1766 E1 (Messier)}
%\DeclareComet{C1769P1}{C/1769 P1}{C/1769 P1 (Messier)}
%\DeclareComet{C1771A1}{C/1771 A1}{C/1771 A1 (Great comet)}
%\DeclareComet{C1771G1}{C/1771 G1}{C/1771 G1 (Messier)}
%\DeclareComet{C1773T1}{C/1773 T1}{C/1773 T1 (Messier)}
%\DeclareComet{C1774P1}{C/1774 P1}{C/1774 P1 (Montaigne)}
%\DeclareComet{C1779A1}{C/1779 A1}{C/1779 A1 (Bode)}
%\DeclareComet{C1780U1}{C/1780 U1}{C/1780 U1 (Montaigne-Olbers)}
%\DeclareComet{C1780U2}{C/1780 U2}{C/1780 U2 (Messier)}
%\DeclareComet{C1781M1}{C/1781 M1}{C/1781 M1 (Mechain)}
%\DeclareComet{C1781T1}{C/1781 T1}{C/1781 T1 (Mechain)}
%\DeclareComet{C1783X1}{C/1783 X1}{C/1783 X1 (Great comet)}
%\DeclareComet{C1785A1}{C/1785 A1}{C/1785 A1 (Messier-Mechain)}
%\DeclareComet{C1785E1}{C/1785 E1}{C/1785 E1 (Mechain)}
%\DeclareComet{C1786P1}{C/1786 P1}{C/1786 P1 (Herschel)}
%\DeclareComet{C1787G1}{C/1787 G1}{C/1787 G1 (Mechain)}
%\DeclareComet{C1788W1}{C/1788 W1}{C/1788 W1 (Messier)}
%\DeclareComet{C1790A1}{C/1790 A1}{C/1790 A1 (Herschel)}
%\DeclareComet{C1790H1}{C/1790 H1}{C/1790 H1 (Herschel)}
%\DeclareComet{C1791X1}{C/1791 X1}{C/1791 X1 (Herschel)}
%\DeclareComet{C1793A1}{C/1793 A1}{C/1793 A1 (Gregory)}
%\DeclareComet{C1793S1}{C/1793 S1}{C/1793 S1 (Perny)}
%\DeclareComet{C1793S2}{C/1793 S2}{C/1793 S2 (Messier)}
%\DeclareComet{C1796F1}{C/1796 F1}{C/1796 F1 (Olbers)}
%\DeclareComet{C1797P1}{C/1797 P1}{C/1797 P1 (Bouvard-Herschel)}
%\DeclareComet{C1798G1}{C/1798 G1}{C/1798 G1 (Messier)}
%\DeclareComet{C1798X1}{C/1798 X1}{C/1798 X1 (Bouvard)}
%\DeclareComet{C1799P1}{C/1799 P1}{C/1799 P1 (Mechain)}
%\DeclareComet{C1799Y1}{C/1799 Y1}{C/1799 Y1 (Mechain)}
%\DeclareComet{C1801N1}{C/1801 N1}{C/1801 N1 (Pons)}
%\DeclareComet{C1802Q1}{C/1802 Q1}{C/1802 Q1 (Pons)}
%\DeclareComet{C1804E1}{C/1804 E1}{C/1804 E1 (Pons)}
%\DeclareComet{C1806V1}{C/1806 V1}{C/1806 V1 (Pons)}
%\DeclareComet{C1807R1}{C/1807 R1}{C/1807 R1 (Great comet)}
%\DeclareComet{C1808F1}{C/1808 F1}{C/1808 F1 (Pons)}
%\DeclareComet{C1808M1}{C/1808 M1}{C/1808 M1 (Pons)}
%\DeclareComet{C1810Q1}{C/1810 Q1}{C/1810 Q1 (Pons)}
%\DeclareComet{C1811F1}{C/1811 F1}{C/1811 F1 (Great comet)}
%\DeclareComet{C1811W1}{C/1811 W1}{C/1811 W1 (Pons)}
%\DeclareComet{C1813C1}{C/1813 C1}{C/1813 C1 (Pons)}
%\DeclareComet{C1813G1}{C/1813 G1}{C/1813 G1 (Pons)}
%\DeclareComet{C1816B1}{C/1816 B1}{C/1816 B1 (Pons)}
%\DeclareComet{C1817Y1}{C/1817 Y1}{C/1817 Y1 (Pons)}
%\DeclareComet{C1818W2}{C/1818 W2}{C/1818 W2 (Pons)}
%\DeclareComet{C1819N1}{C/1819 N1}{C/1819 N1 (Great comet)}
%\DeclareComet{C1821B1}{C/1821 B1}{C/1821 B1 (Nicollet-Pons)}
%\DeclareComet{C1822J1}{C/1822 J1}{C/1822 J1 (Gambart)}
%\DeclareComet{C1822K1}{C/1822 K1}{C/1822 K1 (Pons)}
%\DeclareComet{C1822N1}{C/1822 N1}{C/1822 N1 (Pons)}
%\DeclareComet{C1823Y1}{C/1823 Y1}{C/1823 Y1 (Great comet)}
%\DeclareComet{C1824N1}{C/1824 N1}{C/1824 N1 (Rumker)}
%\DeclareComet{C1824O1}{C/1824 O1}{C/1824 O1 (Scheithauer)}
%\DeclareComet{C1825K1}{C/1825 K1}{C/1825 K1 (Gambart)}
%\DeclareComet{C1825N1}{C/1825 N1}{C/1825 N1 (Pons)}
%\DeclareComet{C1825P1}{C/1825 P1}{C/1825 P1 (Pons)}
%\DeclareComet{C1825V1}{C/1825 V1}{C/1825 V1 (Pons)}
%\DeclareComet{C1826P1}{C/1826 P1}{C/1826 P1 (Pons)}
%\DeclareComet{C1826U1}{C/1826 U1}{C/1826 U1 (Pons)}
%\DeclareComet{C1826Y1}{C/1826 Y1}{C/1826 Y1 (Pons)}
%\DeclareComet{C1827P1}{C/1827 P1}{C/1827 P1 (Pons)}
%\DeclareComet{C1830F1}{C/1830 F1}{C/1830 F1 (Great comet)}
%\DeclareComet{C1831A1}{C/1831 A1}{C/1831 A1 (Great comet)}
%\DeclareComet{C1832O1}{C/1832 O1}{C/1832 O1 (Gambart)}
%\DeclareComet{C1833S1}{C/1833 S1}{C/1833 S1 (Dunlop)}
%\DeclareComet{C1834E1}{C/1834 E1}{C/1834 E1 (Gambart)}
%\DeclareComet{C1835H1}{C/1835 H1}{C/1835 H1 (Boguslawski)}
%\DeclareComet{C1839X1}{C/1839 X1}{C/1839 X1 (Galle)}
%\DeclareComet{C1840B1}{C/1840 B1}{C/1840 B1 (Galle)}
%\DeclareComet{C1840E1}{C/1840 E1}{C/1840 E1 (Galle)}
%\DeclareComet{C1840U1}{C/1840 U1}{C/1840 U1 (Bremiker)}
%\DeclareComet{C1842U1}{C/1842 U1}{C/1842 U1 (Laugier)}
%\DeclareComet{C1843D1}{C/1843 D1}{C/1843 D1 (Great March comet)}
%\DeclareComet{C1843J1}{C/1843 J1}{C/1843 J1 (Mauvais)}
%\DeclareComet{C1844N1}{C/1844 N1}{C/1844 N1 (Mauvais)}
%\DeclareComet{C1844Y1}{C/1844 Y1}{C/1844 Y1 (Great comet)}
%\DeclareComet{C1844Y2}{C/1844 Y2}{C/1844 Y2 (d'Arrest)}
%\DeclareComet{C1845D1}{C/1845 D1}{C/1845 D1 (de Vico)}
%\DeclareComet{C1845L1}{C/1845 L1}{C/1845 L1 (Great June comet)}
%\DeclareComet{C1846B1}{C/1846 B1}{C/1846 B1 (de Vico)}
%\DeclareComet{C1846J1}{C/1846 J1}{C/1846 J1 (Brorsen)}
%\DeclareComet{C1846O1}{C/1846 O1}{C/1846 O1 (de Vico-Hind)}
%\DeclareComet{C1846S1}{C/1846 S1}{C/1846 S1 (de Vico)}
%\DeclareComet{C1847C1}{C/1847 C1}{C/1847 C1 (Hind)}
%\DeclareComet{C1847J1}{C/1847 J1}{C/1847 J1 (Colla)}
%\DeclareComet{C1847N1}{C/1847 N1}{C/1847 N1 (Mauvais)}
%\DeclareComet{C1847Q1}{C/1847 Q1}{C/1847 Q1 (Schweizer)}
%\DeclareComet{C1847T1}{C/1847 T1}{C/1847 T1 (Mitchell)}
%\DeclareComet{C1848P1}{C/1848 P1}{C/1848 P1 (Petersen)}
%\DeclareComet{C1848U1}{C/1848 U1}{C/1848 U1 (Petersen)}
%\DeclareComet{C1849G1}{C/1849 G1}{C/1849 G1 (Schweizer)}
%\DeclareComet{C1849G2}{C/1849 G2}{C/1849 G2 (Goujon)}
%\DeclareComet{C1850J1}{C/1850 J1}{C/1850 J1 (Petersen)}
%\DeclareComet{C1850Q1}{C/1850 Q1}{C/1850 Q1 (Bond)}
%\DeclareComet{C1851P1}{C/1851 P1}{C/1851 P1 (Brorsen)}
%\DeclareComet{C1851U1}{C/1851 U1}{C/1851 U1 (Brorsen)}
%\DeclareComet{C1852K1}{C/1852 K1}{C/1852 K1 (Chacornac)}
%\DeclareComet{C1853E1}{C/1853 E1}{C/1853 E1 (Secchi)}
%\DeclareComet{C1853G1}{C/1853 G1}{C/1853 G1 (Schweizer)}
%\DeclareComet{C1853L1}{C/1853 L1}{C/1853 L1 (Klinkerfues)}
%\DeclareComet{C1853R1}{C/1853 R1}{C/1853 R1 (Bruhns)}
%\DeclareComet{C1853W1}{C/1853 W1}{C/1853 W1 (van Arsdale)}
%\DeclareComet{C1854F1}{C/1854 F1}{C/1854 F1 (Great comet)}
%\DeclareComet{C1854L1}{C/1854 L1}{C/1854 L1 (Klinkerfues)}
%\DeclareComet{C1854R1}{C/1854 R1}{C/1854 R1 (Klinkerfues)}
%\DeclareComet{C1854Y1}{C/1854 Y1}{C/1854 Y1 (Winnecke-Dien)}
%\DeclareComet{C1855G1}{C/1855 G1}{C/1855 G1 (Schweizer)}
%\DeclareComet{C1855L1}{C/1855 L1}{C/1855 L1 (Donati)}
%\DeclareComet{C1855V1}{C/1855 V1}{C/1855 V1 (Bruhns)}
%\DeclareComet{C1857D1}{C/1857 D1}{C/1857 D1 (d'Arrest)}
%\DeclareComet{C1857M1}{C/1857 M1}{C/1857 M1 (Klinkerfues)}
%\DeclareComet{C1857O1}{C/1857 O1}{C/1857 O1 (Peters)}
%\DeclareComet{C1857Q1}{C/1857 Q1}{C/1857 Q1 (Klinkerfues)}
%\DeclareComet{C1857V1}{C/1857 V1}{C/1857 V1 (Donati-van Arsdale)}
%\DeclareComet{C1858K1}{C/1858 K1}{C/1858 K1 (Bruhns)}
%\DeclareComet{C1858L1}{C/1858 L1}{C/1858 L1 (Donati)}
%\DeclareComet{C1858R1}{C/1858 R1}{C/1858 R1 (Tuttle)}
%\DeclareComet{C1859G1}{C/1859 G1}{C/1859 G1 (Tempel)}
%\DeclareComet{C1860D1-A}{C/1860 D1-A}{C/1860 D1-A (Liais)}
%\DeclareComet{C1860D1-B}{C/1860 D1-B}{C/1860 D1-B (Liais)}
%\DeclareComet{C1860H1}{C/1860 H1}{C/1860 H1 (Rumker)}
%\DeclareComet{C1860M1}{C/1860 M1}{C/1860 M1 (Great comet)}
%\DeclareComet{C1860U1}{C/1860 U1}{C/1860 U1 (Tempel)}
%\DeclareComet{C1861G1}{C/1861 G1}{C/1861 G1 (Thatcher)}
%\DeclareComet{C1861J1}{C/1861 J1}{C/1861 J1 (Great comet)}
%\DeclareComet{C1861Y1}{C/1861 Y1}{C/1861 Y1 (Tuttle)}
%\DeclareComet{C1862N1}{C/1862 N1}{C/1862 N1 (Schmidt)}
%\DeclareComet{C1862W1}{C/1862 W1}{C/1862 W1 (Respighi)}
%\DeclareComet{C1862X1}{C/1862 X1}{C/1862 X1 (Bruhns)}
%\DeclareComet{C1863G1}{C/1863 G1}{C/1863 G1 (Klinkerfues)}
%\DeclareComet{C1863G2}{C/1863 G2}{C/1863 G2 (Respighi)}
%\DeclareComet{C1863T1}{C/1863 T1}{C/1863 T1 (Baeker)}
%\DeclareComet{C1863V1}{C/1863 V1}{C/1863 V1 (Tempel)}
%\DeclareComet{C1863Y1}{C/1863 Y1}{C/1863 Y1 (Respighi)}
%\DeclareComet{C1864N1}{C/1864 N1}{C/1864 N1 (Tempel)}
%\DeclareComet{C1864O1}{C/1864 O1}{C/1864 O1 (Donati-Toussaint)}
%\DeclareComet{C1864R1}{C/1864 R1}{C/1864 R1 (Donati)}
%\DeclareComet{C1864X1}{C/1864 X1}{C/1864 X1 (Baeker)}
%\DeclareComet{C1864Y1}{C/1864 Y1}{C/1864 Y1 (Bruhns)}
%\DeclareComet{C1865B1}{C/1865 B1}{C/1865 B1 (Great southern comet)}
%\DeclareComet{C1867S1}{C/1867 S1}{C/1867 S1 (Baeker-Winnecke)}
%\DeclareComet{C1868L1}{C/1868 L1}{C/1868 L1 (Winnecke)}
%\DeclareComet{C1869T1}{C/1869 T1}{C/1869 T1 (Tempel)}
%\DeclareComet{C1870K1}{C/1870 K1}{C/1870 K1 (Winnecke)}
%\DeclareComet{C1870Q1}{C/1870 Q1}{C/1870 Q1 (Coggia)}
%\DeclareComet{C1870W1}{C/1870 W1}{C/1870 W1 (Winnecke)}
%\DeclareComet{C1871G1}{C/1871 G1}{C/1871 G1 (Winnecke)}
%\DeclareComet{C1871L1}{C/1871 L1}{C/1871 L1 (Tempel)}
%\DeclareComet{C1871V1}{C/1871 V1}{C/1871 V1 (Tempel)}
%\DeclareComet{C1873Q1}{C/1873 Q1}{C/1873 Q1 (Borrelly)}
%\DeclareComet{C1873Q2}{C/1873 Q2}{C/1873 Q2 (Henry)}
%\DeclareComet{C1874D1}{C/1874 D1}{C/1874 D1 (Winnecke)}
%\DeclareComet{C1874G1}{C/1874 G1}{C/1874 G1 (Winnecke)}
%\DeclareComet{C1874H1}{C/1874 H1}{C/1874 H1 (Coggia)}
%\DeclareComet{C1874O1}{C/1874 O1}{C/1874 O1 (Borrelly)}
%\DeclareComet{C1874Q1}{C/1874 Q1}{C/1874 Q1 (Coggia)}
%\DeclareComet{C1874X1}{C/1874 X1}{C/1874 X1 (Borrelly)}
%\DeclareComet{C1877C1}{C/1877 C1}{C/1877 C1 (Borrelly)}
%\DeclareComet{C1877G1}{C/1877 G1}{C/1877 G1 (Winnecke)}
%\DeclareComet{C1877G2}{C/1877 G2}{C/1877 G2 (Swift)}
%\DeclareComet{C1877R1}{C/1877 R1}{C/1877 R1 (Coggia)}
%\DeclareComet{C1877T1}{C/1877 T1}{C/1877 T1 (Tempel)}
%\DeclareComet{C1878N1}{C/1878 N1}{C/1878 N1 (Swift)}
%\DeclareComet{C1879M1}{C/1879 M1}{C/1879 M1 (Swift)}
%\DeclareComet{C1879Q1}{C/1879 Q1}{C/1879 Q1 (Palisa)}
%\DeclareComet{C1879Q2}{C/1879 Q2}{C/1879 Q2 (Hartwig)}
%\DeclareComet{C1880C1}{C/1880 C1}{C/1880 C1 (Great southern comet)}
%\DeclareComet{C1880G1}{C/1880 G1}{C/1880 G1 (Schaeberle)}
%\DeclareComet{C1880S1}{C/1880 S1}{C/1880 S1 (Hartwig)}
%\DeclareComet{C1880Y1}{C/1880 Y1}{C/1880 Y1 (Pechule)}
%\DeclareComet{C1881J1}{C/1881 J1}{C/1881 J1 (Swift)}
%\DeclareComet{C1881K1}{C/1881 K1}{C/1881 K1 (Great comet)}
%\DeclareComet{C1881N1}{C/1881 N1}{C/1881 N1 (Schaeberle)}
%\DeclareComet{C1881S1}{C/1881 S1}{C/1881 S1 (Barnard)}
%\DeclareComet{C1881W1}{C/1881 W1}{C/1881 W1 (Swift)}
%\DeclareComet{C1882F1}{C/1882 F1}{C/1882 F1 (Wells)}
%\DeclareComet{C1882R1-A}{C/1882 R1-A}{C/1882 R1-A (Great September comet)}
%\DeclareComet{C1882R1-B}{C/1882 R1-B}{C/1882 R1-B (Great September comet)}
%\DeclareComet{C1882R1-C}{C/1882 R1-C}{C/1882 R1-C (Great September comet)}
%\DeclareComet{C1882R1-D}{C/1882 R1-D}{C/1882 R1-D (Great September comet)}
%\DeclareComet{C1882R2}{C/1882 R2}{C/1882 R2 (Barnard)}
%\DeclareComet{C1883D1}{C/1883 D1}{C/1883 D1 (Brooks-Swift)}
%\DeclareComet{C1884A1}{C/1884 A1}{C/1884 A1 (Ross)}
%\DeclareComet{C1885N1}{C/1885 N1}{C/1885 N1 (Barnard)}
%\DeclareComet{C1885R1}{C/1885 R1}{C/1885 R1 (Brooks)}
%\DeclareComet{C1885X1}{C/1885 X1}{C/1885 X1 (Fabry)}
%\DeclareComet{C1885X2}{C/1885 X2}{C/1885 X2 (Barnard)}
%\DeclareComet{C1885Y1}{C/1885 Y1}{C/1885 Y1 (Brooks)}
%\DeclareComet{C1886H1}{C/1886 H1}{C/1886 H1 (Brooks)}
%\DeclareComet{C1886J1}{C/1886 J1}{C/1886 J1 (Brooks)}
%\DeclareComet{C1886T1}{C/1886 T1}{C/1886 T1 (Barnard-Hartwig)}
%\DeclareComet{C1887B1}{C/1887 B1}{C/1887 B1 (Great southern comet)}
%\DeclareComet{C1887B2}{C/1887 B2}{C/1887 B2 (Brooks)}
%\DeclareComet{C1887B3}{C/1887 B3}{C/1887 B3 (Barnard)}
%\DeclareComet{C1887D1}{C/1887 D1}{C/1887 D1 (Barnard)}
%\DeclareComet{C1887J1}{C/1887 J1}{C/1887 J1 (Barnard)}
%\DeclareComet{C1888D1}{C/1888 D1}{C/1888 D1 (Sawerthal)}
%\DeclareComet{C1888P1}{C/1888 P1}{C/1888 P1 (Brooks)}
%\DeclareComet{C1888R1}{C/1888 R1}{C/1888 R1 (Barnard)}
%\DeclareComet{C1888U1}{C/1888 U1}{C/1888 U1 (Barnard)}
%\DeclareComet{C1889G1}{C/1889 G1}{C/1889 G1 (Barnard)}
%\DeclareComet{C1889O1}{C/1889 O1}{C/1889 O1 (Davidson)}
%\DeclareComet{C1889X1}{C/1889 X1}{C/1889 X1 (Borrelly)}
%\DeclareComet{C1890F1}{C/1890 F1}{C/1890 F1 (Brooks)}
%\DeclareComet{C1890O1}{C/1890 O1}{C/1890 O1 (Coggia)}
%\DeclareComet{C1890O2}{C/1890 O2}{C/1890 O2 (Denning)}
%\DeclareComet{C1890V1}{C/1890 V1}{C/1890 V1 (Zona)}
%\DeclareComet{C1891F1}{C/1891 F1}{C/1891 F1 (Barnard-Denning)}
%\DeclareComet{C1891T1}{C/1891 T1}{C/1891 T1 (Barnard)}
%\DeclareComet{C1892E1}{C/1892 E1}{C/1892 E1 (Swift)}
%\DeclareComet{C1892F1}{C/1892 F1}{C/1892 F1 (Denning)}
%\DeclareComet{C1892Q1}{C/1892 Q1}{C/1892 Q1 (Brooks)}
%\DeclareComet{C1892W1}{C/1892 W1}{C/1892 W1 (Brooks)}
%\DeclareComet{C1893N1}{C/1893 N1}{C/1893 N1 (Rordame-Quenisset)}
%\DeclareComet{C1893U1}{C/1893 U1}{C/1893 U1 (Brooks)}
%\DeclareComet{C1894G1}{C/1894 G1}{C/1894 G1 (Gale)}
%\DeclareComet{C1895W1}{C/1895 W1}{C/1895 W1 (Perrine)}
%\DeclareComet{C1895W2}{C/1895 W2}{C/1895 W2 (Brooks)}
%\DeclareComet{C1896C1}{C/1896 C1}{C/1896 C1 (Perrine-Lamp)}
%\DeclareComet{C1896G1}{C/1896 G1}{C/1896 G1 (Swift)}
%\DeclareComet{C1896R1}{C/1896 R1}{C/1896 R1 (Sperra)}
%\DeclareComet{C1896V1}{C/1896 V1}{C/1896 V1 (Perrine)}
%\DeclareComet{C1897U1}{C/1897 U1}{C/1897 U1 (Perrine)}
%\DeclareComet{C1898F1}{C/1898 F1}{C/1898 F1 (Perrine)}
%\DeclareComet{C1898L1}{C/1898 L1}{C/1898 L1 (Coddington-Pauly)}
%\DeclareComet{C1898L2}{C/1898 L2}{C/1898 L2 (Perrine)}
%\DeclareComet{C1898M1}{C/1898 M1}{C/1898 M1 (Giacobini)}
%\DeclareComet{C1898R1}{C/1898 R1}{C/1898 R1 (Perrine-Chofardet)}
%\DeclareComet{C1898U1}{C/1898 U1}{C/1898 U1 (Brooks)}
%\DeclareComet{C1898V1}{C/1898 V1}{C/1898 V1 (Chase)}
%\DeclareComet{C1899E1}{C/1899 E1}{C/1899 E1 (Swift)}
%\DeclareComet{C1899S1}{C/1899 S1}{C/1899 S1 (Giacobini)}
%\DeclareComet{C1900B1}{C/1900 B1}{C/1900 B1 (Giacobini)}
%\DeclareComet{C1900O1}{C/1900 O1}{C/1900 O1 (Borrelly-Brooks)}
%\DeclareComet{C1901G1}{C/1901 G1}{C/1901 G1 (Greatcomet)}
%\DeclareComet{C1902G1}{C/1902 G1}{C/1902 G1 (Brooks)}
%\DeclareComet{C1902R1}{C/1902 R1}{C/1902 R1 (Perrine)}
%\DeclareComet{C1902X1}{C/1902 X1}{C/1902 X1 (Giacobini)}
%\DeclareComet{C1903A1}{C/1903 A1}{C/1903 A1 (Giacobini)}
%\DeclareComet{C1903H1}{C/1903 H1}{C/1903 H1 (Grigg)}
%\DeclareComet{C1903M1}{C/1903 M1}{C/1903 M1 (Borrelly)}
%\DeclareComet{C1904H1}{C/1904 H1}{C/1904 H1 (Brooks)}
%\DeclareComet{C1904Y1}{C/1904 Y1}{C/1904 Y1 (Giacobini)}
%\DeclareComet{C1905F1}{C/1905 F1}{C/1905 F1 (Giacobini)}
%\DeclareComet{C1905W1}{C/1905 W1}{C/1905 W1 (Schaer)}
%\DeclareComet{C1905X1}{C/1905 X1}{C/1905 X1 (Giacobini)}
%\DeclareComet{C1906B1}{C/1906 B1}{C/1906 B1 (Brooks)}
%\DeclareComet{C1906E1}{C/1906 E1}{C/1906 E1 (Kopff)}
%\DeclareComet{C1906F1}{C/1906 F1}{C/1906 F1 (Ross)}
%\DeclareComet{C1906V1}{C/1906 V1}{C/1906 V1 (Thiele)}
%\DeclareComet{C1907E1}{C/1907 E1}{C/1907 E1 (Giacobini)}
%\DeclareComet{C1907G1}{C/1907 G1}{C/1907 G1 (Grigg-Mellish)}
%\DeclareComet{C1907L2}{C/1907 L2}{C/1907 L2 (Daniel)}
%\DeclareComet{C1907T1}{C/1907 T1}{C/1907 T1 (Mellish)}
%\DeclareComet{C1908R1}{C/1908 R1}{C/1908 R1 (Morehouse)}
%\DeclareComet{C1909L1}{C/1909 L1}{C/1909 L1 (Borrelly-Daniel)}
%\DeclareComet{C1910A1}{C/1910 A1}{C/1910 A1 (Great January comet)}
%\DeclareComet{C1910P1}{C/1910 P1}{C/1910 P1 (Metcalf)}
%\DeclareComet{C1911N1}{C/1911 N1}{C/1911 N1 (Kiess)}
%\DeclareComet{C1911O1}{C/1911 O1}{C/1911 O1 (Brooks)}
%\DeclareComet{C1911S2}{C/1911 S2}{C/1911 S2 (Quenisset)}
%\DeclareComet{C1911S3}{C/1911 S3}{C/1911 S3 (Beljawsky)}
%\DeclareComet{C1912R1}{C/1912 R1}{C/1912 R1 (Gale)}
%\DeclareComet{C1912V1}{C/1912 V1}{C/1912 V1 (Borrelly)}
%\DeclareComet{C1913J1}{C/1913 J1}{C/1913 J1 (Schaumasse)}
%\DeclareComet{C1913R1}{C/1913 R1}{C/1913 R1 (Metcalf)}
%\DeclareComet{C1913Y1}{C/1913 Y1}{C/1913 Y1 (Delavan)}
%\DeclareComet{C1914F1}{C/1914 F1}{C/1914 F1 (Kritzinger)}
%\DeclareComet{C1914J1}{C/1914 J1}{C/1914 J1 (Zlatinsky)}
%\DeclareComet{C1914M1}{C/1914 M1}{C/1914 M1 (Neujmin)}
%\DeclareComet{C1914S1}{C/1914 S1}{C/1914 S1 (Campbell)}
%\DeclareComet{C1915C1}{C/1915 C1}{C/1915 C1 (Mellish)}
%\DeclareComet{C1915R1}{C/1915 R1}{C/1915 R1 (Mellish)}
%\DeclareComet{C1916G1}{C/1916 G1}{C/1916 G1 (Wolf)}
%\DeclareComet{C1917F1}{C/1917 F1}{C/1917 F1 (Mellish)}
%\DeclareComet{C1917H1}{C/1917 H1}{C/1917 H1 (Schaumasse)}
%\DeclareComet{C1918L1}{C/1918 L1}{C/1918 L1 (Reid)}
%\DeclareComet{C1919Q2}{C/1919 Q2}{C/1919 Q2 (Metcalf)}
%\DeclareComet{C1919Y1}{C/1919 Y1}{C/1919 Y1 (Skjellerup)}
%\DeclareComet{C1920X1}{C/1920 X1}{C/1920 X1 (Skjellerup)}
%\DeclareComet{C1921E1}{C/1921 E1}{C/1921 E1 (Reid)}
%\DeclareComet{C1921H1}{C/1921 H1}{C/1921 H1 (Dubiago)}
%\DeclareComet{C1922B1}{C/1922 B1}{C/1922 B1 (Reid)}
%\DeclareComet{C1922U1}{C/1922 U1}{C/1922 U1 (Baade)}
%\DeclareComet{C1922W1}{C/1922 W1}{C/1922 W1 (Skjellerup)}
%\DeclareComet{C1923T1}{C/1923 T1}{C/1923 T1 (Dubiago-Bernard)}
%\DeclareComet{C1924F1}{C/1924 F1}{C/1924 F1 (Reid)}
%\DeclareComet{C1924R1}{C/1924 R1}{C/1924 R1 (Finsler)}
%\DeclareComet{C1925F1}{C/1925 F1}{C/1925 F1 (Shajn-Comas Sola)}
%\DeclareComet{C1925F2}{C/1925 F2}{C/1925 F2 (Reid)}
%\DeclareComet{C1925G1}{C/1925 G1}{C/1925 G1 (Orkisz)}
%\DeclareComet{C1925V1}{C/1925 V1}{C/1925 V1 (Wilk-Peltier)}
%\DeclareComet{C1925W1}{C/1925 W1}{C/1925 W1 (Van Biesbroeck)}
%\DeclareComet{C1925X1}{C/1925 X1}{C/1925 X1 (Ensor)}
%\DeclareComet{C1926B1}{C/1926 B1}{C/1926 B1 (Blathwayt)}
%\DeclareComet{C1927A1}{C/1927 A1}{C/1927 A1 (Blathwayt)}
%\DeclareComet{C1927B1}{C/1927 B1}{C/1927 B1 (Reid)}
%\DeclareComet{C1927E1}{C/1927 E1}{C/1927 E1 (Stearns)}
%\DeclareComet{C1927X1}{C/1927 X1}{C/1927 X1 (Skjellerup-Maristany)}
%\DeclareComet{C1929Y1}{C/1929 Y1}{C/1929 Y1 (Wilk)}
%\DeclareComet{C1930D1}{C/1930 D1}{C/1930 D1 (Peltier-Schwassmann-Wachmann)}
%\DeclareComet{C1930E1}{C/1930 E1}{C/1930 E1 (Beyer)}
%\DeclareComet{C1930F1}{C/1930 F1}{C/1930 F1 (Wilk)}
%\DeclareComet{C1930L1}{C/1930 L1}{C/1930 L1 (Forbes)}
%\DeclareComet{C1931O1}{C/1931 O1}{C/1931 O1 (Nagata)}
%\DeclareComet{C1931P1}{C/1931 P1}{C/1931 P1 (Ryves)}
%\DeclareComet{C1932G1}{C/1932 G1}{C/1932 G1 (Houghton-Ensor)}
%\DeclareComet{C1932H1}{C/1932 H1}{C/1932 H1 (Carrasco)}
%\DeclareComet{C1932M1}{C/1932 M1}{C/1932 M1 (Newman)}
%\DeclareComet{C1932M2}{C/1932 M2}{C/1932 M2 (Geddes)}
%\DeclareComet{C1932P1}{C/1932 P1}{C/1932 P1 (Peltier-Whipple)}
%\DeclareComet{C1932Y1}{C/1932 Y1}{C/1932 Y1 (Dodwell-Forbes)}
%\DeclareComet{C1933D1}{C/1933 D1}{C/1933 D1 (Peltier)}
%\DeclareComet{C1935A1}{C/1935 A1}{C/1935 A1 (Johnson)}
%\DeclareComet{C1935M1}{C/1935 M1}{C/1935 M1 (Jackson)}
%\DeclareComet{C1935Q1}{C/1935 Q1}{C/1935 Q1 (Van Biesbroeck)}
%\DeclareComet{C1936K1}{C/1936 K1}{C/1936 K1 (Peltier)}
%\DeclareComet{C1936O1}{C/1936 O1}{C/1936 O1 (Kaho-Kozik-Lis)}
%\DeclareComet{C1937C1}{C/1937 C1}{C/1937 C1 (Whipple)}
%\DeclareComet{C1937D1}{C/1937 D1}{C/1937 D1 (Wilk)}
%\DeclareComet{C1937N1}{C/1937 N1}{C/1937 N1 (Finsler)}
%\DeclareComet{C1937P1}{C/1937 P1}{C/1937 P1 (Hubble)}
%\DeclareComet{C1939B1}{C/1939 B1}{C/1939 B1 (Kozik-Peltier)}
%\DeclareComet{C1939H1}{C/1939 H1}{C/1939 H1 (Jurlof-Achmarof-Hassel)}
%\DeclareComet{C1939V1}{C/1939 V1}{C/1939 V1 (Friend)}
%\DeclareComet{C1940O1}{C/1940 O1}{C/1940 O1 (Whipple-Paraskevopoulos)}
%\DeclareComet{C1940R2}{C/1940 R2}{C/1940 R2 (Cunningham)}
%\DeclareComet{C1940S1}{C/1940 S1}{C/1940 S1 (Okabayasi-Honda)}
%\DeclareComet{C1941B1}{C/1941 B1}{C/1941 B1 (Friend-Reese-Honda)}
%\DeclareComet{C1941B2}{C/1941 B2}{C/1941 B2 (de Kock-Paraskevopoulos)}
%\DeclareComet{C1941K1}{C/1941 K1}{C/1941 K1 (van Gent)}
%\DeclareComet{C1942C1}{C/1942 C1}{C/1942 C1 (Whipple-Bernasconi-Kulin)}
%\DeclareComet{C1942C2}{C/1942 C2}{C/1942 C2 (Oterma)}
%\DeclareComet{C1942EA}{C/1942 EA}{C/1942 EA (Vaisala)}
%\DeclareComet{C1942X1}{C/1942 X1}{C/1942 X1 (Whipple-Fedtke-Tevzadze)}
%\DeclareComet{C1943R1}{C/1943 R1}{C/1943 R1 (Daimaca)}
%\DeclareComet{C1943W1}{C/1943 W1}{C/1943 W1 (van Gent-Peltier-Daimaca)}
%\DeclareComet{C1944H1}{C/1944 H1}{C/1944 H1 (Vaisala)}
%\DeclareComet{C1944K2}{C/1944 K2}{C/1944 K2 (van Gent)}
%\DeclareComet{C1945L1}{C/1945 L1}{C/1945 L1 (du Toit)}
%\DeclareComet{C1945W1}{C/1945 W1}{C/1945 W1 (Friend-Peltier)}
%\DeclareComet{C1945X1}{C/1945 X1}{C/1945 X1 (du Toit)}
%\DeclareComet{C1946C1}{C/1946 C1}{C/1946 C1 (Timmers)}
%\DeclareComet{C1946K1}{C/1946 K1}{C/1946 K1 (Pajdusakova-Rotbart-Weber)}
%\DeclareComet{C1946P1}{C/1946 P1}{C/1946 P1 (Jones)}
%\DeclareComet{C1946U1}{C/1946 U1}{C/1946 U1 (Bester)}
%\DeclareComet{C1947F1}{C/1947 F1}{C/1947 F1 (Rondanina-Bester)}
%\DeclareComet{C1947F2}{C/1947 F2}{C/1947 F2 (Becvar)}
%\DeclareComet{C1947K1}{C/1947 K1}{C/1947 K1 (Bester)}
%\DeclareComet{C1947O1}{C/1947 O1}{C/1947 O1 (Wirtanen)}
%\DeclareComet{C1947S1}{C/1947 S1}{C/1947 S1 (Bester)}
%\DeclareComet{C1947V1}{C/1947 V1}{C/1947 V1 (Honda)}
%\DeclareComet{C1947X1-A}{C/1947 X1-A}{C/1947 X1-A (Southern comet)}
%\DeclareComet{C1947X1-B}{C/1947 X1-B}{C/1947 X1-B (Southern comet)}
%\DeclareComet{C1947Y1}{C/1947 Y1}{C/1947 Y1 (Mrkos)}
%\DeclareComet{C1948E1}{C/1948 E1}{C/1948 E1 (Pajdusakova-Mrkos)}
%\DeclareComet{C1948L1}{C/1948 L1}{C/1948 L1 (Honda-Bernasconi)}
%\DeclareComet{C1948N1}{C/1948 N1}{C/1948 N1 (Wirtanen)}
%\DeclareComet{C1948R1}{C/1948 R1}{C/1948 R1 (Johnson)}
%\DeclareComet{C1948T1}{C/1948 T1}{C/1948 T1 (Wirtanen)}
%\DeclareComet{C1948V1}{C/1948 V1}{C/1948 V1 (Eclipsecomet)}
%\DeclareComet{C1948W1}{C/1948 W1}{C/1948 W1 (Bester)}
%\DeclareComet{C1949K1}{C/1949 K1}{C/1949 K1 (Johnson)}
%\DeclareComet{C1949N1}{C/1949 N1}{C/1949 N1 (Bappu-Bok-Newkirk)}
%\DeclareComet{C1950K1}{C/1950 K1}{C/1950 K1 (Minkowski)}
%\DeclareComet{C1951C1}{C/1951 C1}{C/1951 C1 (Pajdusakova)}
%\DeclareComet{C1951G1}{C/1951 G1}{C/1951 G1 (Groeneveld)}
%\DeclareComet{C1951G2}{C/1951 G2}{C/1951 G2 (Groeneveld-Palomar)}
%\DeclareComet{C1951P1}{C/1951 P1}{C/1951 P1 (Wilson-Harrington)}
%\DeclareComet{C1952H1}{C/1952 H1}{C/1952 H1 (Mrkos)}
%\DeclareComet{C1952M1}{C/1952 M1}{C/1952 M1 (Peltier)}
%\DeclareComet{C1952Q1}{C/1952 Q1}{C/1952 Q1 (Harrington)}
%\DeclareComet{C1952W1}{C/1952 W1}{C/1952 W1 (Mrkos)}
%\DeclareComet{C1953G1}{C/1953 G1}{C/1953 G1 (Mrkos-Honda)}
%\DeclareComet{C1953T1}{C/1953 T1}{C/1953 T1 (Abell)}
%\DeclareComet{C1953X1}{C/1953 X1}{C/1953 X1 (Pajdusakova)}
%\DeclareComet{C1954M1}{C/1954 M1}{C/1954 M1 (Harrington)}
%\DeclareComet{C1954M2}{C/1954 M2}{C/1954 M2 (Kresak-Peltier)}
%\DeclareComet{C1954O1}{C/1954 O1}{C/1954 O1 (Vozarova)}
%\DeclareComet{C1954O2}{C/1954 O2}{C/1954 O2 (Baade)}
%\DeclareComet{C1954Y1}{C/1954 Y1}{C/1954 Y1 (Haro-Chavira)}
%\DeclareComet{C1955G1}{C/1955 G1}{C/1955 G1 (Abell)}
%\DeclareComet{C1955L1}{C/1955 L1}{C/1955 L1 (Mrkos)}
%\DeclareComet{C1955N1}{C/1955 N1}{C/1955 N1 (Bakharev-Macfarlane-Krienke)}
%\DeclareComet{C1955O1}{C/1955 O1}{C/1955 O1 (Honda)}
%\DeclareComet{C1956E1}{C/1956 E1}{C/1956 E1 (Mrkos)}
%\DeclareComet{C1956F1-A}{C/1956 F1-A}{C/1956 F1-A (Wirtanen)}
%\DeclareComet{C1956R1}{C/1956 R1}{C/1956 R1 (Arend-Roland)}
%\DeclareComet{C1957P1}{C/1957 P1}{C/1957 P1 (Mrkos)}
%\DeclareComet{C1957U1}{C/1957 U1}{C/1957 U1 (Latyshev-Wild-Burnham)}
%\DeclareComet{C1958D1}{C/1958 D1}{C/1958 D1 (Burnham)}
%\DeclareComet{C1958R1}{C/1958 R1}{C/1958 R1 (Burnham-Slaughter)}
%\DeclareComet{C1959O1}{C/1959 O1}{C/1959 O1 (Bester-Hoffmeister)}
%\DeclareComet{C1959Q1}{C/1959 Q1}{C/1959 Q1 (Alcock)}
%\DeclareComet{C1959Q2}{C/1959 Q2}{C/1959 Q2 (Alcock)}
%\DeclareComet{C1959X1}{C/1959 X1}{C/1959 X1 (Mrkos)}
%\DeclareComet{C1959Y1}{C/1959 Y1}{C/1959 Y1 (Burnham)}
%\DeclareComet{C1960B1}{C/1960 B1}{C/1960 B1 (Burnham)}
%\DeclareComet{C1960M1}{C/1960 M1}{C/1960 M1 (Humason)}
%\DeclareComet{C1960Y1}{C/1960 Y1}{C/1960 Y1 (Candy)}
%\DeclareComet{C1961O1}{C/1961 O1}{C/1961 O1 (Wilson-Hubbard)}
%\DeclareComet{C1961R1}{C/1961 R1}{C/1961 R1 (Humason)}
%\DeclareComet{C1961T1}{C/1961 T1}{C/1961 T1 (Seki)}
%\DeclareComet{C1962C1}{C/1962 C1}{C/1962 C1 (Seki-Lines)}
%\DeclareComet{C1962H1}{C/1962 H1}{C/1962 H1 (Honda)}
%\DeclareComet{C1963A1}{C/1963 A1}{C/1963 A1 (Ikeya)}
%\DeclareComet{C1963F1}{C/1963 F1}{C/1963 F1 (Alcock)}
%\DeclareComet{C1963R1}{C/1963 R1}{C/1963 R1 (Pereyra)}
%\DeclareComet{C1964L1}{C/1964 L1}{C/1964 L1 (Tomita-Gerber-Honda)}
%\DeclareComet{C1964N1}{C/1964 N1}{C/1964 N1 (Ikeya)}
%\DeclareComet{C1964P1}{C/1964 P1}{C/1964 P1 (Everhart)}
%\DeclareComet{C1965S1-A}{C/1965 S1-A}{C/1965 S1-A (Ikeya-Seki)}
%\DeclareComet{C1965S1-B}{C/1965 S1-B}{C/1965 S1-B (Ikeya-Seki)}
%\DeclareComet{C1965S2}{C/1965 S2}{C/1965 S2 (Alcock)}
%\DeclareComet{C1966P1}{C/1966 P1}{C/1966 P1 (Kilston)}
%\DeclareComet{C1966P2}{C/1966 P2}{C/1966 P2 (Barbon)}
%\DeclareComet{C1966R1}{C/1966 R1}{C/1966 R1 (Ikeya-Everhart)}
%\DeclareComet{C1966T1}{C/1966 T1}{C/1966 T1 (Rudnicki)}
%\DeclareComet{C1967C1}{C/1967 C1}{C/1967 C1 (Seki)}
%\DeclareComet{C1967C2}{C/1967 C2}{C/1967 C2 (Wild)}
%\DeclareComet{C1967M1}{C/1967 M1}{C/1967 M1 (Mitchell-Jones-Gerber)}
%\DeclareComet{C1967Y1}{C/1967 Y1}{C/1967 Y1 (Ikeya-Seki)}
%\DeclareComet{C1968H1}{C/1968 H1}{C/1968 H1 (Tago-Honda-Yamamoto)}
%\DeclareComet{C1968L1}{C/1968 L1}{C/1968 L1 (Whitaker-Thomas)}
%\DeclareComet{C1968N1}{C/1968 N1}{C/1968 N1 (Honda)}
%\DeclareComet{C1968Q1}{C/1968 Q1}{C/1968 Q1 (Bally-Clayton)}
%\DeclareComet{C1968Q2}{C/1968 Q2}{C/1968 Q2 (Honda)}
%\DeclareComet{C1968U1}{C/1968 U1}{C/1968 U1 (Wild)}
%\DeclareComet{C1968Y1}{C/1968 Y1}{C/1968 Y1 (Thomas)}
%\DeclareComet{C1969O1-A}{C/1969 O1-A}{C/1969 O1-A (Kohoutek)}
%\DeclareComet{C1969P1}{C/1969 P1}{C/1969 P1 (Fujikawa)}
%\DeclareComet{C1969T1}{C/1969 T1}{C/1969 T1 (Tago-Sato-Kosaka)}
%\DeclareComet{C1969Y1}{C/1969 Y1}{C/1969 Y1 (Bennett)}
%\DeclareComet{C1970B1}{C/1970 B1}{C/1970 B1 (Daido-Fujikawa)}
%\DeclareComet{C1970K1}{C/1970 K1}{C/1970 K1 (White-Ortiz-Bolelli)}
%\DeclareComet{C1970N1}{C/1970 N1}{C/1970 N1 (Abe)}
%\DeclareComet{C1970U1}{C/1970 U1}{C/1970 U1 (Suzuki-Sato-Seki)}
%\DeclareComet{C1971E1}{C/1971 E1}{C/1971 E1 (Toba)}
%\DeclareComet{C1971M1}{C/1971 M1}{C/1971 M1 (Edwards)}
%\DeclareComet{C1972E1}{C/1972 E1}{C/1972 E1 (Bradfield)}
%\DeclareComet{C1972F1}{C/1972 F1}{C/1972 F1 (Gehrels)}
%\DeclareComet{C1972L1}{C/1972 L1}{C/1972 L1 (Sandage)}
%\DeclareComet{C1972U1}{C/1972 U1}{C/1972 U1 (Kojima)}
%\DeclareComet{C1972X1}{C/1972 X1}{C/1972 X1 (Araya)}
%\DeclareComet{C1973A1}{C/1973 A1}{C/1973 A1 (Heck-Sause)}
%\DeclareComet{C1973D1}{C/1973 D1}{C/1973 D1 (Kohoutek)}
%\DeclareComet{C1973E1}{C/1973 E1}{C/1973 E1 (Kohoutek)}
%\DeclareComet{C1973H1}{C/1973 H1}{C/1973 H1 (Huchra)}
%\DeclareComet{C1973N1}{C/1973 N1}{C/1973 N1 (Sandage)}
%\DeclareComet{C1973W1}{C/1973 W1}{C/1973 W1 (Gibson)}
%\DeclareComet{C1974C1}{C/1974 C1}{C/1974 C1 (Bradfield)}
%\DeclareComet{C1974F1}{C/1974 F1}{C/1974 F1 (Lovas)}
%\DeclareComet{C1974O1}{C/1974 O1}{C/1974 O1 (Cesco)}
%\DeclareComet{C1974V1}{C/1974 V1}{C/1974 V1 (vandenBergh)}
%\DeclareComet{C1974V2}{C/1974 V2}{C/1974 V2 (Bennett)}
%\DeclareComet{C1975E1}{C/1975 E1}{C/1975 E1 (Bradfield)}
%\DeclareComet{C1975N1}{C/1975 N1}{C/1975 N1 (Kobayashi-Berger-Milon)}
%\DeclareComet{C1975T1}{C/1975 T1}{C/1975 T1 (Mori-Sato-Fujikawa)}
%\DeclareComet{C1975T2}{C/1975 T2}{C/1975 T2 (Suzuki-Saigusa-Mori)}
%\DeclareComet{C1975V1-A}{C/1975 V1-A}{C/1975 V1-A (West)}
%\DeclareComet{C1975V2}{C/1975 V2}{C/1975 V2 (Bradfield)}
%\DeclareComet{C1975X1}{C/1975 X1}{C/1975 X1 (Sato)}
%\DeclareComet{C1976D1}{C/1976 D1}{C/1976 D1 (Bradfield)}
%\DeclareComet{C1976D2}{C/1976 D2}{C/1976 D2 (Schuster)}
%\DeclareComet{C1976E1}{C/1976 E1}{C/1976 E1 (Bradfield)}
%\DeclareComet{C1976J1}{C/1976 J1}{C/1976 J1 (Harlan)}
%\DeclareComet{C1976U1}{C/1976 U1}{C/1976 U1 (Lovas)}
%\DeclareComet{C1977D1}{C/1977 D1}{C/1977 D1 (Lovas)}
%\DeclareComet{C1977H1}{C/1977 H1}{C/1977 H1 (Helin)}
%\DeclareComet{C1977R1}{C/1977 R1}{C/1977 R1 (Kohler)}
%\DeclareComet{C1977V1}{C/1977 V1}{C/1977 V1 (Tsuchinshan)}
%\DeclareComet{C1978A1}{C/1978 A1}{C/1978 A1 (West)}
%\DeclareComet{C1978C1}{C/1978 C1}{C/1978 C1 (Bradfield)}
%\DeclareComet{C1978G2}{C/1978 G2}{C/1978 G2 (McNaught-Tritton)}
%\DeclareComet{C1978H1}{C/1978 H1}{C/1978 H1 (Meier)}
%\DeclareComet{C1978R3}{C/1978 R3}{C/1978 R3 (Machholz)}
%\DeclareComet{C1978T1}{C/1978 T1}{C/1978 T1 (Seargent)}
%\DeclareComet{C1978T3}{C/1978 T3}{C/1978 T3 (Bradfield)}
%\DeclareComet{C1979M1}{C/1979 M1}{C/1979 M1 (Bradfield)}
%\DeclareComet{C1979M3}{C/1979 M3}{C/1979 M3 (Torres)}
%\DeclareComet{C1979Q1}{C/1979 Q1}{C/1979 Q1 (SOLWIND)}
%\DeclareComet{C1979S1}{C/1979 S1}{C/1979 S1 (Meier)}
%\DeclareComet{C1979Y1}{C/1979 Y1}{C/1979 Y1 (Bradfield)}
%\DeclareComet{C1980E1}{C/1980 E1}{C/1980 E1 (Bowell)}
%\DeclareComet{C1980L1}{C/1980 L1}{C/1980 L1 (Torres)}
%\DeclareComet{C1980O1}{C/1980 O1}{C/1980 O1 (Cernis-Petrauskas)}
%\DeclareComet{C1980R1}{C/1980 R1}{C/1980 R1 (Russell)}
%\DeclareComet{C1980V1}{C/1980 V1}{C/1980 V1 (Meier)}
%\DeclareComet{C1980Y1}{C/1980 Y1}{C/1980 Y1 (Bradfield)}
%\DeclareComet{C1980Y2}{C/1980 Y2}{C/1980 Y2 (Panther)}
%\DeclareComet{C1981B1}{C/1981 B1}{C/1981 B1 (SOLWIND)}
%\DeclareComet{C1981G1}{C/1981 G1}{C/1981 G1 (Elias)}
%\DeclareComet{C1981H1}{C/1981 H1}{C/1981 H1 (Bus)}
%\DeclareComet{C1981M1}{C/1981 M1}{C/1981 M1 (Gonzalez)}
%\DeclareComet{C1981O1}{C/1981 O1}{C/1981 O1 (SOLWIND)}
%\DeclareComet{C1981V1}{C/1981 V1}{C/1981 V1 (SOLWIND)}
%\DeclareComet{C1981W1}{C/1981 W1}{C/1981 W1 (SOLWIND)}
%\DeclareComet{C1982M1}{C/1982 M1}{C/1982 M1 (Austin)}
%\DeclareComet{C1983H1}{C/1983 H1}{C/1983 H1 (IRAS-Araki-Alcock)}
%\DeclareComet{C1983J1}{C/1983 J1}{C/1983 J1 (Sugano-Saigusa-Fujikawa)}
%\DeclareComet{C1983J2}{C/1983 J2}{C/1983 J2 (IRAS)}
%\DeclareComet{C1983N1}{C/1983 N1}{C/1983 N1 (IRAS)}
%\DeclareComet{C1983N2}{C/1983 N2}{C/1983 N2 (SOLWIND)}
%\DeclareComet{C1983O1}{C/1983 O1}{C/1983 O1 (Cernis)}
%\DeclareComet{C1983O2}{C/1983 O2}{C/1983 O2 (IRAS)}
%\DeclareComet{C1983R1}{C/1983 R1}{C/1983 R1 (Shoemaker)}
%\DeclareComet{C1983S2}{C/1983 S2}{C/1983 S2 (SOLWIND)}
%\DeclareComet{C1984A1}{C/1984 A1}{C/1984 A1 (Bradfield)}
%\DeclareComet{C1984K1}{C/1984 K1}{C/1984 K1 (Shoemaker)}
%\DeclareComet{C1984N1}{C/1984 N1}{C/1984 N1 (Austin)}
%\DeclareComet{C1984O2}{C/1984 O2}{C/1984 O2 (SOLWIND)}
%\DeclareComet{C1984Q1}{C/1984 Q1}{C/1984 Q1 (SOLWIND)}
%\DeclareComet{C1984R1}{C/1984 R1}{C/1984 R1 (SOLWIND)}
%\DeclareComet{C1984S1}{C/1984 S1}{C/1984 S1 (Meier)}
%\DeclareComet{C1984U1}{C/1984 U1}{C/1984 U1 (Shoemaker)}
%\DeclareComet{C1984U2}{C/1984 U2}{C/1984 U2 (Shoemaker)}
%\DeclareComet{C1984V1}{C/1984 V1}{C/1984 V1 (Levy-Rudenko)}
%\DeclareComet{C1984W2}{C/1984 W2}{C/1984 W2 (Hartley)}
%\DeclareComet{C1985K1}{C/1985 K1}{C/1985 K1 (Machholz)}
%\DeclareComet{C1985R1}{C/1985 R1}{C/1985 R1 (Hartley-Good)}
%\DeclareComet{C1985T1}{C/1985 T1}{C/1985 T1 (Thiele)}
%\DeclareComet{C1986E1}{C/1986 E1}{C/1986 E1 (Shoemaker)}
%\DeclareComet{C1986N1}{C/1986 N1}{C/1986 N1 (Churyumov-Solodovnikov)}
%\DeclareComet{C1986P1-A}{C/1986 P1-A}{C/1986 P1-A (Wilson)}
%\DeclareComet{C1986P1-B}{C/1986 P1-B}{C/1986 P1-B (Wilson)}
%\DeclareComet{C1986V1}{C/1986 V1}{C/1986 V1 (Sorrells)}
%\DeclareComet{C1987A1}{C/1987 A1}{C/1987 A1 (Levy)}
%\DeclareComet{C1987B1}{C/1987 B1}{C/1987 B1 (Nishikawa-Takamizawa-Tago)}
%\DeclareComet{C1987B2}{C/1987 B2}{C/1987 B2 (Terasako)}
%\DeclareComet{C1987F1}{C/1987 F1}{C/1987 F1 (Torres)}
%\DeclareComet{C1987H1}{C/1987 H1}{C/1987 H1 (Shoemaker)}
%\DeclareComet{C1987P1}{C/1987 P1}{C/1987 P1 (Bradfield)}
%\DeclareComet{C1987Q1}{C/1987 Q1}{C/1987 Q1 (Rudenko)}
%\DeclareComet{C1987T1}{C/1987 T1}{C/1987 T1 (Levy)}
%\DeclareComet{C1987T2}{C/1987 T2}{C/1987 T2 (SMM)}
%\DeclareComet{C1987U3}{C/1987 U3}{C/1987 U3 (McNaught)}
%\DeclareComet{C1987U4}{C/1987 U4}{C/1987 U4 (SMM)}
%\DeclareComet{C1987W1}{C/1987 W1}{C/1987 W1 (Ichimura)}
%\DeclareComet{C1987W2}{C/1987 W2}{C/1987 W2 (Furuyama)}
%\DeclareComet{C1987W3}{C/1987 W3}{C/1987 W3 (Jensen-Shoemaker)}
%\DeclareComet{C1988A1}{C/1988 A1}{C/1988 A1 (Liller)}
%\DeclareComet{C1988B1}{C/1988 B1}{C/1988 B1 (Shoemaker)}
%\DeclareComet{C1988C1}{C/1988 C1}{C/1988 C1 (Maury-Phinney)}
%\DeclareComet{C1988F1}{C/1988 F1}{C/1988 F1 (Levy)}
%\DeclareComet{C1988J1}{C/1988 J1}{C/1988 J1 (Shoemaker-Holt)}
%\DeclareComet{C1988L1}{C/1988 L1}{C/1988 L1 (Shoemaker-Holt-Rodriquez)}
%\DeclareComet{C1988M1}{C/1988 M1}{C/1988 M1 (SMM)}
%\DeclareComet{C1988P1}{C/1988 P1}{C/1988 P1 (Machholz)}
%\DeclareComet{C1988Q1}{C/1988 Q1}{C/1988 Q1 (SMM)}
%\DeclareComet{C1988T1}{C/1988 T1}{C/1988 T1 (SMM)}
%\DeclareComet{C1988U1}{C/1988 U1}{C/1988 U1 (SMM)}
%\DeclareComet{C1988W1}{C/1988 W1}{C/1988 W1 (SMM)}
%\DeclareComet{C1988Y1}{C/1988 Y1}{C/1988 Y1 (Yanaka)}
%\DeclareComet{C1989A1}{C/1989 A1}{C/1989 A1 (Yanaka)}
%\DeclareComet{C1989A3}{C/1989 A3}{C/1989 A3 (Bradfield)}
%\DeclareComet{C1989A5}{C/1989 A5}{C/1989 A5 (Shoemaker)}
%\DeclareComet{C1989A6}{C/1989 A6}{C/1989 A6 (Shoemaker)}
%\DeclareComet{C1989L1}{C/1989 L1}{C/1989 L1 (SMM)}
%\DeclareComet{C1989N3}{C/1989 N3}{C/1989 N3 (SMM)}
%\DeclareComet{C1989Q1}{C/1989 Q1}{C/1989 Q1 (Okazaki-Levy-Rudenko)}
%\DeclareComet{C1989R1}{C/1989 R1}{C/1989 R1 (Helin-Roman)}
%\DeclareComet{C1989S1}{C/1989 S1}{C/1989 S1 (SMM)}
%\DeclareComet{C1989T1}{C/1989 T1}{C/1989 T1 (Helin-Roman-Alu)}
%\DeclareComet{C1989W1}{C/1989 W1}{C/1989 W1 (Aarseth-Brewington)}
%\DeclareComet{C1989X1}{C/1989 X1}{C/1989 X1 (Austin)}
%\DeclareComet{C1989Y1}{C/1989 Y1}{C/1989 Y1 (Skorichenko-George)}
%\DeclareComet{C1989Y2}{C/1989 Y2}{C/1989 Y2 (McKenzie-Russell)}
%\DeclareComet{C1990E1}{C/1990 E1}{C/1990 E1 (Cernis-Kiuchi-Nakamura)}
%\DeclareComet{C1990K1}{C/1990 K1}{C/1990 K1 (Levy)}
%\DeclareComet{C1990M1}{C/1990 M1}{C/1990 M1 (McNaught-Hughes)}
%\DeclareComet{C1990N1}{C/1990 N1}{C/1990 N1 (Tsuchiya-Kiuchi)}
%\DeclareComet{C1991A2}{C/1991 A2}{C/1991 A2 (Arai)}
%\DeclareComet{C1991B1}{C/1991 B1}{C/1991 B1 (Shoemaker-Levy)}
%\DeclareComet{C1991C3}{C/1991 C3}{C/1991 C3 (McNaught-Russell)}
%\DeclareComet{C1991F2}{C/1991 F2}{C/1991 F2 (Helin-Lawrence)}
%\DeclareComet{C1991L3}{C/1991 L3}{C/1991 L3 (Levy)}
%\DeclareComet{C1991L4}{C/1991 L4}{C/1991 L4 (Helin-Alu)}
%\DeclareComet{C1991Q1}{C/1991 Q1}{C/1991 Q1 (McNaught-Russell)}
%\DeclareComet{C1991R1}{C/1991 R1}{C/1991 R1 (McNaught-Russell)}
%\DeclareComet{C1991T2}{C/1991 T2}{C/1991 T2 (Shoemaker-Levy)}
%\DeclareComet{C1991X2}{C/1991 X2}{C/1991 X2 (Mueller)}
%\DeclareComet{C1991Y1}{C/1991 Y1}{C/1991 Y1 (Zanotta-Brewington)}
%\DeclareComet{C1992A1}{C/1992 A1}{C/1992 A1 (Helin-Alu)}
%\DeclareComet{C1992B1}{C/1992 B1}{C/1992 B1 (Bradfield)}
%\DeclareComet{C1992F1}{C/1992 F1}{C/1992 F1 (Tanaka-Machholz)}
%\DeclareComet{C1992J1}{C/1992 J1}{C/1992 J1 (Spacewatch)}
%\DeclareComet{C1992J2}{C/1992 J2}{C/1992 J2 (Bradfield)}
%\DeclareComet{C1992N1}{C/1992 N1}{C/1992 N1 (Machholz)}
%\DeclareComet{C1992Q2}{C/1992 Q2}{C/1992 Q2 (Helin-Lawrence)}
%\DeclareComet{C1992U1}{C/1992 U1}{C/1992 U1 (Shoemaker)}
%\DeclareComet{C1992W1}{C/1992 W1}{C/1992 W1 (Ohshita)}
%\DeclareComet{C1993A1}{C/1993 A1}{C/1993 A1 (Mueller)}
%\DeclareComet{C1993F1}{C/1993 F1}{C/1993 F1 (Mueller)}
%\DeclareComet{C1993K1}{C/1993 K1}{C/1993 K1 (Shoemaker-Levy)}
%\DeclareComet{C1993Q1}{C/1993 Q1}{C/1993 Q1 (Mueller)}
%\DeclareComet{C1993Y1}{C/1993 Y1}{C/1993 Y1 (McNaught-Russell)}
%\DeclareComet{C1994E1}{C/1994 E1}{C/1994 E1 (Mueller)}
%\DeclareComet{C1994E2}{C/1994 E2}{C/1994 E2 (Shoemaker-Levy)}
%\DeclareComet{C1994G1-A}{C/1994 G1-A}{C/1994 G1-A (Takamizawa-Levy)}
%\DeclareComet{C1994G1-B}{C/1994 G1-B}{C/1994 G1-B (Takamizawa-Levy)}
%\DeclareComet{C1994J2}{C/1994 J2}{C/1994 J2 (Takamizawa)}
%\DeclareComet{C1994N1}{C/1994 N1}{C/1994 N1 (Nakamura-Nishimura-Machholz)}
%\DeclareComet{C1994T1}{C/1994 T1}{C/1994 T1 (Machholz)}
%\DeclareComet{C1995O1}{C/1995 O1}{C/1995 O1 (Hale-Bopp)}
%\DeclareComet{C1995Q1}{C/1995 Q1}{C/1995 Q1 (Bradfield)}
%\DeclareComet{C1995Q2}{C/1995 Q2}{C/1995 Q2 (Hartley-Drinkwater)}
%\DeclareComet{C1995Y1}{C/1995 Y1}{C/1995 Y1 (Hyakutake)}
%\DeclareComet{C1996A2}{C/1996 A2}{C/1996 A2 (SOHO)}
%\DeclareComet{C1996B1}{C/1996 B1}{C/1996 B1 (Szczepanski)}
%\DeclareComet{C1996B2}{C/1996 B2}{C/1996 B2 (Hyakutake)}
%\DeclareComet{C1996B3}{C/1996 B3}{C/1996 B3 (SOHO)}
%\DeclareComet{C1996B4}{C/1996 B4}{C/1996 B4 (SOHO)}
%\DeclareComet{C1996B5}{C/1996 B5}{C/1996 B5 (SOHO)}
%\DeclareComet{C1996D1}{C/1996 D1}{C/1996 D1 (SOHO)}
%\DeclareComet{C1996E1}{C/1996 E1}{C/1996 E1 (NEAT)}
%\DeclareComet{C1996E2}{C/1996 E2}{C/1996 E2 (SOHO)}
%\DeclareComet{C1996F2}{C/1996 F2}{C/1996 F2 (SOHO)}
%\DeclareComet{C1996H1}{C/1996 H1}{C/1996 H1 (SOHO)}
%\DeclareComet{C1996J1-A}{C/1996 J1-A}{C/1996 J1-A (Evans-Drinkwater)}
%\DeclareComet{C1996J1-B}{C/1996 J1-B}{C/1996 J1-B (Evans-Drinkwater)}
%\DeclareComet{C1996L1}{C/1996 L1}{C/1996 L1 (SOHO)}
%\DeclareComet{C1996L2}{C/1996 L2}{C/1996 L2 (SOHO)}
%\DeclareComet{C1996M1}{C/1996 M1}{C/1996 M1 (SOHO)}
%\DeclareComet{C1996M2}{C/1996 M2}{C/1996 M2 (SOHO)}
%\DeclareComet{C1996M3}{C/1996 M3}{C/1996 M3 (SOHO)}
%\DeclareComet{C1996N1}{C/1996 N1}{C/1996 N1 (Brewington)}
%\DeclareComet{C1996N3}{C/1996 N3}{C/1996 N3 (SOHO)}
%\DeclareComet{C1996O1}{C/1996 O1}{C/1996 O1 (SOHO)}
%\DeclareComet{C1996O2}{C/1996 O2}{C/1996 O2 (SOHO)}
%\DeclareComet{C1996O3}{C/1996 O3}{C/1996 O3 (SOHO)}
%\DeclareComet{C1996O4}{C/1996 O4}{C/1996 O4 (SOHO)}
%\DeclareComet{C1996P2}{C/1996 P2}{C/1996 P2 (Russell-Watson)}
%\DeclareComet{C1996Q1}{C/1996 Q1}{C/1996 Q1 (Tabur)}
%\DeclareComet{C1996Q2}{C/1996 Q2}{C/1996 Q2 (SOHO)}
%\DeclareComet{C1996Q3}{C/1996 Q3}{C/1996 Q3 (SOHO)}
%\DeclareComet{C1996R1}{C/1996 R1}{C/1996 R1 (Hergenrother-Spahr)}
%\DeclareComet{C1996R3}{C/1996 R3}{C/1996 R3 (Lagerkvist)}
%\DeclareComet{C1996R4}{C/1996 R4}{C/1996 R4 (SOHO)}
%\DeclareComet{C1996R5}{C/1996 R5}{C/1996 R5 (SOHO)}
%\DeclareComet{C1996S3}{C/1996 S3}{C/1996 S3 (SOHO)}
%\DeclareComet{C1996V1}{C/1996 V1}{C/1996 V1 (SOHO)}
%\DeclareComet{C1996V2}{C/1996 V2}{C/1996 V2 (SOHO)}
%\DeclareComet{C1996X1}{C/1996 X1}{C/1996 X1 (SOHO)}
%\DeclareComet{C1996X2}{C/1996 X2}{C/1996 X2 (SOHO)}
%\DeclareComet{C1996X3}{C/1996 X3}{C/1996 X3 (SOHO)}
%\DeclareComet{C1996X4}{C/1996 X4}{C/1996 X4 (SOHO)}
%\DeclareComet{C1996X5}{C/1996 X5}{C/1996 X5 (SOHO)}
%\DeclareComet{C1996Y1}{C/1996 Y1}{C/1996 Y1 (SOHO)}
%\DeclareComet{C1996Y2}{C/1996 Y2}{C/1996 Y2 (SOHO)}
%\DeclareComet{C1997A1}{C/1997 A1}{C/1997 A1 (NEAT)}
%\DeclareComet{C1997B2}{C/1997 B2}{C/1997 B2 (SOHO)}
%\DeclareComet{C1997B3}{C/1997 B3}{C/1997 B3 (SOHO)}
%\DeclareComet{C1997B4}{C/1997 B4}{C/1997 B4 (SOHO)}
%\DeclareComet{C1997B5}{C/1997 B5}{C/1997 B5 (SOHO)}
%\DeclareComet{C1997B6}{C/1997 B6}{C/1997 B6 (SOHO)}
%\DeclareComet{C1997B7}{C/1997 B7}{C/1997 B7 (SOHO)}
%\DeclareComet{C1997BA6}{C/1997 BA6}{C/1997 BA6 (Spacewatch)}
%\DeclareComet{C1997C2}{C/1997 C2}{C/1997 C2 (SOHO)}
%\DeclareComet{C1997D1}{C/1997 D1}{C/1997 D1 (Mueller)}
%\DeclareComet{C1997E2}{C/1997 E2}{C/1997 E2 (SOHO)}
%\DeclareComet{C1997G2}{C/1997 G2}{C/1997 G2 (Montani)}
%\DeclareComet{C1997G3}{C/1997 G3}{C/1997 G3 (SOHO)}
%\DeclareComet{C1997G4}{C/1997 G4}{C/1997 G4 (SOHO)}
%\DeclareComet{C1997G5}{C/1997 G5}{C/1997 G5 (SOHO)}
%\DeclareComet{C1997G6}{C/1997 G6}{C/1997 G6 (SOHO)}
%\DeclareComet{C1997G7}{C/1997 G7}{C/1997 G7 (SOHO)}
%\DeclareComet{C1997H2}{C/1997 H2}{C/1997 H2 (SOHO)}
%\DeclareComet{C1997H3}{C/1997 H3}{C/1997 H3 (SOHO)}
%\DeclareComet{C1997H4}{C/1997 H4}{C/1997 H4 (SOHO)}
%\DeclareComet{C1997H5}{C/1997 H5}{C/1997 H5 (SOHO)}
%\DeclareComet{C1997J1}{C/1997 J1}{C/1997 J1 (Mueller)}
%\DeclareComet{C1997J2}{C/1997 J2}{C/1997 J2 (Meunier-Dupouy)}
%\DeclareComet{C1997J3}{C/1997 J3}{C/1997 J3 (SOHO)}
%\DeclareComet{C1997J4}{C/1997 J4}{C/1997 J4 (SOHO)}
%\DeclareComet{C1997J5}{C/1997 J5}{C/1997 J5 (SOHO)}
%\DeclareComet{C1997K1}{C/1997 K1}{C/1997 K1 (SOHO)}
%\DeclareComet{C1997K2}{C/1997 K2}{C/1997 K2}
%\DeclareComet{C1997K3}{C/1997 K3}{C/1997 K3 (SOHO)}
%\DeclareComet{C1997K4}{C/1997 K4}{C/1997 K4 (SOHO)}
%\DeclareComet{C1997K5}{C/1997 K5}{C/1997 K5 (SOHO)}
%\DeclareComet{C1997K6}{C/1997 K6}{C/1997 K6 (SOHO)}
%\DeclareComet{C1997K7}{C/1997 K7}{C/1997 K7 (SOHO)}
%\DeclareComet{C1997L1}{C/1997 L1}{C/1997 L1 (Zhu-Balam)}
%\DeclareComet{C1997L2}{C/1997 L2}{C/1997 L2 (SOHO)}
%\DeclareComet{C1997L3}{C/1997 L3}{C/1997 L3 (SOHO)}
%\DeclareComet{C1997L4}{C/1997 L4}{C/1997 L4 (SOHO)}
%\DeclareComet{C1997L5}{C/1997 L5}{C/1997 L5 (SOHO)}
%\DeclareComet{C1997M1}{C/1997 M1}{C/1997 M1 (SOHO)}
%\DeclareComet{C1997M3}{C/1997 M3}{C/1997 M3 (SOHO)}
%\DeclareComet{C1997M4}{C/1997 M4}{C/1997 M4 (SOHO)}
%\DeclareComet{C1997M5}{C/1997 M5}{C/1997 M5 (SOHO)}
%\DeclareComet{C1997N1}{C/1997 N1}{C/1997 N1 (Tabur)}
%\DeclareComet{C1997N3}{C/1997 N3}{C/1997 N3 (SOHO)}
%\DeclareComet{C1997O1}{C/1997 O1}{C/1997 O1 (Tilbrook)}
%\DeclareComet{C1997O2}{C/1997 O2}{C/1997 O2 (SOHO)}
%\DeclareComet{C1997O3}{C/1997 O3}{C/1997 O3 (SOHO)}
%\DeclareComet{C1997P1}{C/1997 P1}{C/1997 P1 (SOHO)}
%\DeclareComet{C1997P2}{C/1997 P2}{C/1997 P2 (Spacewatch)}
%\DeclareComet{C1997P3}{C/1997 P3}{C/1997 P3 (SOHO)}
%\DeclareComet{C1997P4}{C/1997 P4}{C/1997 P4 (SOHO)}
%\DeclareComet{C1997P5}{C/1997 P5}{C/1997 P5 (SOHO)}
%\DeclareComet{C1997Q1}{C/1997 Q1}{C/1997 Q1 (SOHO)}
%\DeclareComet{C1997Q2}{C/1997 Q2}{C/1997 Q2 (SOHO)}
%\DeclareComet{C1997R1}{C/1997 R1}{C/1997 R1 (SOHO)}
%\DeclareComet{C1997R2}{C/1997 R2}{C/1997 R2 (SOHO)}
%\DeclareComet{C1997R3}{C/1997 R3}{C/1997 R3 (SOHO)}
%\DeclareComet{C1997S1}{C/1997 S1}{C/1997 S1 (SOHO)}
%\DeclareComet{C1997S2}{C/1997 S2}{C/1997 S2 (SOHO)}
%\DeclareComet{C1997S3}{C/1997 S3}{C/1997 S3 (SOHO)}
%\DeclareComet{C1997S4}{C/1997 S4}{C/1997 S4 (SOHO)}
%\DeclareComet{C1997S5}{C/1997 S5}{C/1997 S5 (SOHO)}
%\DeclareComet{C1997S6}{C/1997 S6}{C/1997 S6 (SOHO)}
%\DeclareComet{C1997T1}{C/1997 T1}{C/1997 T1 (Utsunomiya)}
%\DeclareComet{C1997T2}{C/1997 T2}{C/1997 T2 (SOHO)}
%\DeclareComet{C1997T4}{C/1997 T4}{C/1997 T4 (SOHO)}
%\DeclareComet{C1997T5}{C/1997 T5}{C/1997 T5 (SOHO)}
%\DeclareComet{C1997T6}{C/1997 T6}{C/1997 T6 (SOHO)}
%\DeclareComet{C1997T7}{C/1997 T7}{C/1997 T7 (SOHO)}
%\DeclareComet{C1997T8}{C/1997 T8}{C/1997 T8 (SOHO)}
%\DeclareComet{C1997T9}{C/1997 T9}{C/1997 T9 (SOHO)}
%\DeclareComet{C1997U1}{C/1997 U1}{C/1997 U1 (SOHO)}
%\DeclareComet{C1997U2}{C/1997 U2}{C/1997 U2 (SOHO)}
%\DeclareComet{C1997U3}{C/1997 U3}{C/1997 U3 (SOHO)}
%\DeclareComet{C1997U4}{C/1997 U4}{C/1997 U4 (SOHO)}
%\DeclareComet{C1997U5}{C/1997 U5}{C/1997 U5 (SOHO)}
%\DeclareComet{C1997U6}{C/1997 U6}{C/1997 U6 (SOHO)}
%\DeclareComet{C1997U7}{C/1997 U7}{C/1997 U7 (SOHO)}
%\DeclareComet{C1997U8}{C/1997 U8}{C/1997 U8 (SOHO)}
%\DeclareComet{C1997U9}{C/1997 U9}{C/1997 U9 (SOHO)}
%\DeclareComet{C1997V2}{C/1997 V2}{C/1997 V2 (SOHO)}
%\DeclareComet{C1997V3}{C/1997 V3}{C/1997 V3 (SOHO)}
%\DeclareComet{C1997V4}{C/1997 V4}{C/1997 V4 (SOHO)}
%\DeclareComet{C1997V5}{C/1997 V5}{C/1997 V5 (SOHO)}
%\DeclareComet{C1997V6}{C/1997 V6}{C/1997 V6 (SOHO)}
%\DeclareComet{C1997V7}{C/1997 V7}{C/1997 V7 (SOHO)}
%\DeclareComet{C1997V8}{C/1997 V8}{C/1997 V8 (SOHO)}
%\DeclareComet{C1997V9}{C/1997 V9}{C/1997 V9 (SOHO)}
%\DeclareComet{C1997W1}{C/1997 W1}{C/1997 W1 (SOHO)}
%\DeclareComet{C1997W2}{C/1997 W2}{C/1997 W2 (SOHO)}
%\DeclareComet{C1997W3}{C/1997 W3}{C/1997 W3 (SOHO)}
%\DeclareComet{C1997X1}{C/1997 X1}{C/1997 X1 (SOHO)}
%\DeclareComet{C1997X3}{C/1997 X3}{C/1997 X3 (SOHO)}
%\DeclareComet{C1997X4}{C/1997 X4}{C/1997 X4 (SOHO)}
%\DeclareComet{C1997X5}{C/1997 X5}{C/1997 X5 (SOHO)}
%\DeclareComet{C1997X6}{C/1997 X6}{C/1997 X6 (SOHO)}
%\DeclareComet{C1997X7}{C/1997 X7}{C/1997 X7 (SOHO)}
%\DeclareComet{C1997Y1}{C/1997 Y1}{C/1997 Y1 (SOHO)}
%\DeclareComet{C1997Y2}{C/1997 Y2}{C/1997 Y2 (SOHO)}
%\DeclareComet{C1997Y3}{C/1997 Y3}{C/1997 Y3 (SOHO)}
%\DeclareComet{C1998A1}{C/1998 A1}{C/1998 A1 (SOHO)}
%\DeclareComet{C1998A2}{C/1998 A2}{C/1998 A2 (SOHO)}
%\DeclareComet{C1998A3}{C/1998 A3}{C/1998 A3 (SOHO)}
%\DeclareComet{C1998A4}{C/1998 A4}{C/1998 A4 (SOHO)}
%\DeclareComet{C1998B2}{C/1998 B2}{C/1998 B2 (SOHO)}
%\DeclareComet{C1998D1}{C/1998 D1}{C/1998 D1 (SOHO)}
%\DeclareComet{C1998E1}{C/1998 E1}{C/1998 E1 (SOHO)}
%\DeclareComet{C1998F1}{C/1998 F1}{C/1998 F1 (SOHO)}
%\DeclareComet{C1998F2}{C/1998 F2}{C/1998 F2 (SOHO)}
%\DeclareComet{C1998G2}{C/1998 G2}{C/1998 G2 (SOHO)}
%\DeclareComet{C1998G3}{C/1998 G3}{C/1998 G3 (SOHO)}
%\DeclareComet{C1998G4}{C/1998 G4}{C/1998 G4 (SOHO)}
%\DeclareComet{C1998G5}{C/1998 G5}{C/1998 G5 (SOHO)}
%\DeclareComet{C1998G6}{C/1998 G6}{C/1998 G6 (SOHO)}
%\DeclareComet{C1998G7}{C/1998 G7}{C/1998 G7 (SOHO)}
%\DeclareComet{C1998G8}{C/1998 G8}{C/1998 G8 (SOHO)}
%\DeclareComet{C1998G9}{C/1998 G9}{C/1998 G9 (SOHO)}
%\DeclareComet{C1998H1}{C/1998 H1}{C/1998 H1 (Stonehouse)}
%\DeclareComet{C1998H2}{C/1998 H2}{C/1998 H2 (SOHO)}
%\DeclareComet{C1998H3}{C/1998 H3}{C/1998 H3 (SOHO)}
%\DeclareComet{C1998H4}{C/1998 H4}{C/1998 H4 (SOHO)}
%\DeclareComet{C1998H5}{C/1998 H5}{C/1998 H5 (SOHO)}
%\DeclareComet{C1998H6}{C/1998 H6}{C/1998 H6 (SOHO)}
%\DeclareComet{C1998J1}{C/1998 J1}{C/1998 J1 (SOHO)}
%\DeclareComet{C1998J2}{C/1998 J2}{C/1998 J2 (SOHO)}
%\DeclareComet{C1998J3}{C/1998 J3}{C/1998 J3 (SOHO)}
%\DeclareComet{C1998J4}{C/1998 J4}{C/1998 J4 (SOHO)}
%\DeclareComet{C1998J5}{C/1998 J5}{C/1998 J5 (SOHO)}
%\DeclareComet{C1998K1}{C/1998 K1}{C/1998 K1 (Mueller)}
%\DeclareComet{C1998K10}{C/1998 K10}{C/1998 K10 (SOHO)}
%\DeclareComet{C1998K11}{C/1998 K11}{C/1998 K11 (SOHO)}
%\DeclareComet{C1998K12}{C/1998 K12}{C/1998 K12 (SOHO)}
%\DeclareComet{C1998K13}{C/1998 K13}{C/1998 K13 (SOHO)}
%\DeclareComet{C1998K14}{C/1998 K14}{C/1998 K14 (SOHO)}
%\DeclareComet{C1998K15}{C/1998 K15}{C/1998 K15 (SOHO)}
%\DeclareComet{C1998K16}{C/1998 K16}{C/1998 K16 (SOHO)}
%\DeclareComet{C1998K17}{C/1998 K17}{C/1998 K17 (SOHO)}
%\DeclareComet{C1998K2}{C/1998 K2}{C/1998 K2 (LINEAR)}
%\DeclareComet{C1998K3}{C/1998 K3}{C/1998 K3 (LINEAR)}
%\DeclareComet{C1998K5}{C/1998 K5}{C/1998 K5 (LINEAR)}
%\DeclareComet{C1998K7}{C/1998 K7}{C/1998 K7 (SOHO)}
%\DeclareComet{C1998K8}{C/1998 K8}{C/1998 K8 (SOHO)}
%\DeclareComet{C1998K9}{C/1998 K9}{C/1998 K9 (SOHO)}
%\DeclareComet{C1998L1}{C/1998 L1}{C/1998 L1 (SOHO)}
%\DeclareComet{C1998L10}{C/1998 L10}{C/1998 L10 (SOHO)}
%\DeclareComet{C1998L2}{C/1998 L2}{C/1998 L2 (SOHO)}
%\DeclareComet{C1998L3}{C/1998 L3}{C/1998 L3 (SOHO)}
%\DeclareComet{C1998L4}{C/1998 L4}{C/1998 L4 (SOHO)}
%\DeclareComet{C1998L5}{C/1998 L5}{C/1998 L5 (SOHO)}
%\DeclareComet{C1998L6}{C/1998 L6}{C/1998 L6 (SOHO)}
%\DeclareComet{C1998L7}{C/1998 L7}{C/1998 L7 (SOHO)}
%\DeclareComet{C1998L8}{C/1998 L8}{C/1998 L8 (SOHO)}
%\DeclareComet{C1998L9}{C/1998 L9}{C/1998 L9 (SOHO)}
%\DeclareComet{C1998M1}{C/1998 M1}{C/1998 M1 (LINEAR)}
%\DeclareComet{C1998M10}{C/1998 M10}{C/1998 M10 (SOHO)}
%\DeclareComet{C1998M2}{C/1998 M2}{C/1998 M2 (LINEAR)}
%\DeclareComet{C1998M3}{C/1998 M3}{C/1998 M3 (Larsen)}
%\DeclareComet{C1998M4}{C/1998 M4}{C/1998 M4 (LINEAR)}
%\DeclareComet{C1998M5}{C/1998 M5}{C/1998 M5 (LINEAR)}
%\DeclareComet{C1998M6}{C/1998 M6}{C/1998 M6 (Montani)}
%\DeclareComet{C1998M7}{C/1998 M7}{C/1998 M7 (SOHO)}
%\DeclareComet{C1998M8}{C/1998 M8}{C/1998 M8 (SOHO)}
%\DeclareComet{C1998M9}{C/1998 M9}{C/1998 M9 (SOHO)}
%\DeclareComet{C1998P1}{C/1998 P1}{C/1998 P1 (Williams)}
%\DeclareComet{C1998Q1}{C/1998 Q1}{C/1998 Q1 (LINEAR)}
%\DeclareComet{C1998T1}{C/1998 T1}{C/1998 T1 (LINEAR)}
%\DeclareComet{C1998T2}{C/1998 T2}{C/1998 T2 (SOHO)}
%\DeclareComet{C1998U1}{C/1998 U1}{C/1998 U1 (LINEAR)}
%\DeclareComet{C1998U5}{C/1998 U5}{C/1998 U5 (LINEAR)}
%\DeclareComet{C1998U6}{C/1998 U6}{C/1998 U6 (SOHO)}
%\DeclareComet{C1998U7}{C/1998 U7}{C/1998 U7 (SOHO)}
%\DeclareComet{C1998V1}{C/1998 V1}{C/1998 V1 (SOHO)}
%\DeclareComet{C1998V2}{C/1998 V2}{C/1998 V2 (SOHO)}
%\DeclareComet{C1998V3}{C/1998 V3}{C/1998 V3 (SOHO)}
%\DeclareComet{C1998V4}{C/1998 V4}{C/1998 V4 (SOHO)}
%\DeclareComet{C1998V5}{C/1998 V5}{C/1998 V5 (SOHO)}
%\DeclareComet{C1998V6}{C/1998 V6}{C/1998 V6 (SOHO)}
%\DeclareComet{C1998V7}{C/1998 V7}{C/1998 V7 (SOHO)}
%\DeclareComet{C1998V8}{C/1998 V8}{C/1998 V8 (SOHO)}
%\DeclareComet{C1998V9}{C/1998 V9}{C/1998 V9 (SOHO)}
%\DeclareComet{C1998W3}{C/1998 W3}{C/1998 W3 (LINEAR)}
%\DeclareComet{C1998W4}{C/1998 W4}{C/1998 W4 (SOHO)}
%\DeclareComet{C1998W5}{C/1998 W5}{C/1998 W5 (SOHO)}
%\DeclareComet{C1998W6}{C/1998 W6}{C/1998 W6 (SOHO)}
%\DeclareComet{C1998W7}{C/1998 W7}{C/1998 W7 (SOHO)}
%\DeclareComet{C1998W8}{C/1998 W8}{C/1998 W8 (SOHO)}
%\DeclareComet{C1998X10}{C/1998 X10}{C/1998 X10 (SOHO)}
%\DeclareComet{C1998X11}{C/1998 X11}{C/1998 X11 (SOHO)}
%\DeclareComet{C1998X12}{C/1998 X12}{C/1998 X12 (SOHO)}
%\DeclareComet{C1998X3}{C/1998 X3}{C/1998 X3 (SOHO)}
%\DeclareComet{C1998X4}{C/1998 X4}{C/1998 X4 (SOHO)}
%\DeclareComet{C1998X5}{C/1998 X5}{C/1998 X5 (SOHO)}
%\DeclareComet{C1998X6}{C/1998 X6}{C/1998 X6 (SOHO)}
%\DeclareComet{C1998X7}{C/1998 X7}{C/1998 X7 (SOHO)}
%\DeclareComet{C1998X8}{C/1998 X8}{C/1998 X8 (SOHO)}
%\DeclareComet{C1998X9}{C/1998 X9}{C/1998 X9 (SOHO)}
%\DeclareComet{C1998Y1}{C/1998 Y1}{C/1998 Y1 (LINEAR)}
%\DeclareComet{C1999A1}{C/1999 A1}{C/1999 A1 (Tilbrook)}
%\DeclareComet{C1999C1}{C/1999 C1}{C/1999 C1 (SOHO)}
%\DeclareComet{C1999C2}{C/1999 C2}{C/1999 C2 (SOHO)}
%\DeclareComet{C1999D2}{C/1999 D2}{C/1999 D2 (SOHO)}
%\DeclareComet{C1999D3}{C/1999 D3}{C/1999 D3 (SOHO)}
%\DeclareComet{C1999E1}{C/1999 E1}{C/1999 E1 (Li)}
%\DeclareComet{C1999E2}{C/1999 E2}{C/1999 E2 (SOHO)}
%\DeclareComet{C1999F1}{C/1999 F1}{C/1999 F1 (Catalina)}
%\DeclareComet{C1999F2}{C/1999 F2}{C/1999 F2 (Dalcanton)}
%\DeclareComet{C1999F3}{C/1999 F3}{C/1999 F3 (SOHO)}
%\DeclareComet{C1999F4}{C/1999 F4}{C/1999 F4 (SOHO)}
%\DeclareComet{C1999G2}{C/1999 G2}{C/1999 G2 (SOHO)}
%\DeclareComet{C1999G3}{C/1999 G3}{C/1999 G3 (SOHO)}
%\DeclareComet{C1999G4}{C/1999 G4}{C/1999 G4 (SOHO)}
%\DeclareComet{C1999G5}{C/1999 G5}{C/1999 G5 (SOHO)}
%\DeclareComet{C1999H1}{C/1999 H1}{C/1999 H1 (Lee)}
%\DeclareComet{C1999H2}{C/1999 H2}{C/1999 H2 (SOHO)}
%\DeclareComet{C1999H3}{C/1999 H3}{C/1999 H3 (LINEAR)}
%\DeclareComet{C1999H4}{C/1999 H4}{C/1999 H4 (SOHO)}
%\DeclareComet{C1999H5}{C/1999 H5}{C/1999 H5 (SOHO)}
%\DeclareComet{C1999H6}{C/1999 H6}{C/1999 H6 (SOHO)}
%\DeclareComet{C1999H7}{C/1999 H7}{C/1999 H7 (SOHO)}
%\DeclareComet{C1999H8}{C/1999 H8}{C/1999 H8 (SOHO)}
%\DeclareComet{C1999H9}{C/1999 H9}{C/1999 H9 (SOHO)}
%\DeclareComet{C1999J1}{C/1999 J1}{C/1999 J1 (SOHO)}
%\DeclareComet{C1999J10}{C/1999 J10}{C/1999 J10 (SOHO)}
%\DeclareComet{C1999J11}{C/1999 J11}{C/1999 J11 (SOHO)}
%\DeclareComet{C1999J12}{C/1999 J12}{C/1999 J12 (SOHO)}
%\DeclareComet{C1999J13}{C/1999 J13}{C/1999 J13 (SOHO)}
%\DeclareComet{C1999J2}{C/1999 J2}{C/1999 J2 (Skiff)}
%\DeclareComet{C1999J3}{C/1999 J3}{C/1999 J3 (LINEAR)}
%\DeclareComet{C1999J4}{C/1999 J4}{C/1999 J4 (LINEAR)}
%\DeclareComet{C1999J7}{C/1999 J7}{C/1999 J7 (SOHO)}
%\DeclareComet{C1999J8}{C/1999 J8}{C/1999 J8 (SOHO)}
%\DeclareComet{C1999J9}{C/1999 J9}{C/1999 J9 (SOHO)}
%\DeclareComet{C1999K1}{C/1999 K1}{C/1999 K1 (SOHO)}
%\DeclareComet{C1999K10}{C/1999 K10}{C/1999 K10 (SOHO)}
%\DeclareComet{C1999K11}{C/1999 K11}{C/1999 K11 (SOHO)}
%\DeclareComet{C1999K12}{C/1999 K12}{C/1999 K12 (SOHO)}
%\DeclareComet{C1999K13}{C/1999 K13}{C/1999 K13 (SOHO)}
%\DeclareComet{C1999K14}{C/1999 K14}{C/1999 K14 (SOHO)}
%\DeclareComet{C1999K15}{C/1999 K15}{C/1999 K15 (SOHO)}
%\DeclareComet{C1999K16}{C/1999 K16}{C/1999 K16 (SOHO)}
%\DeclareComet{C1999K17}{C/1999 K17}{C/1999 K17 (SOHO)}
%\DeclareComet{C1999K2}{C/1999 K2}{C/1999 K2 (Ferris)}
%\DeclareComet{C1999K3}{C/1999 K3}{C/1999 K3 (LINEAR)}
%\DeclareComet{C1999K4}{C/1999 K4}{C/1999 K4 (LINEAR)}
%\DeclareComet{C1999K5}{C/1999 K5}{C/1999 K5 (LINEAR)}
%\DeclareComet{C1999K6}{C/1999 K6}{C/1999 K6 (LINEAR)}
%\DeclareComet{C1999K7}{C/1999 K7}{C/1999 K7 (LINEAR)}
%\DeclareComet{C1999K8}{C/1999 K8}{C/1999 K8 (LINEAR)}
%\DeclareComet{C1999K9}{C/1999 K9}{C/1999 K9 (SOHO)}
%\DeclareComet{C1999L1}{C/1999 L1}{C/1999 L1 (SOHO)}
%\DeclareComet{C1999L2}{C/1999 L2}{C/1999 L2 (LINEAR)}
%\DeclareComet{C1999L3}{C/1999 L3}{C/1999 L3 (LINEAR)}
%\DeclareComet{C1999L4}{C/1999 L4}{C/1999 L4 (SOHO)}
%\DeclareComet{C1999L5}{C/1999 L5}{C/1999 L5 (SOHO)}
%\DeclareComet{C1999L6}{C/1999 L6}{C/1999 L6 (SOHO)}
%\DeclareComet{C1999L7}{C/1999 L7}{C/1999 L7 (SOHO)}
%\DeclareComet{C1999L8}{C/1999 L8}{C/1999 L8 (SOHO)}
%\DeclareComet{C1999L9}{C/1999 L9}{C/1999 L9 (SOHO)}
%\DeclareComet{C1999M1}{C/1999 M1}{C/1999 M1 (SOHO)}
%\DeclareComet{C1999M2}{C/1999 M2}{C/1999 M2 (SOHO)}
%\DeclareComet{C1999M3}{C/1999 M3}{C/1999 M3 (SOHO)}
%\DeclareComet{C1999M4}{C/1999 M4}{C/1999 M4 (SOHO)}
%\DeclareComet{C1999N1}{C/1999 N1}{C/1999 N1 (SOHO)}
%\DeclareComet{C1999N2}{C/1999 N2}{C/1999 N2 (Lynn)}
%\DeclareComet{C1999N3}{C/1999 N3}{C/1999 N3 (SOHO)}
%\DeclareComet{C1999N4}{C/1999 N4}{C/1999 N4 (LINEAR)}
%\DeclareComet{C1999N5}{C/1999 N5}{C/1999 N5 (SOHO)}
%\DeclareComet{C1999N6}{C/1999 N6}{C/1999 N6 (SOHO)}
%\DeclareComet{C1999O1}{C/1999 O1}{C/1999 O1 (SOHO)}
%\DeclareComet{C1999O2}{C/1999 O2}{C/1999 O2 (SOHO)}
%\DeclareComet{C1999O3}{C/1999 O3}{C/1999 O3 (SOHO)}
%\DeclareComet{C1999O4}{C/1999 O4}{C/1999 O4 (SOHO)}
%\DeclareComet{C1999O5}{C/1999 O5}{C/1999 O5 (SOHO)}
%\DeclareComet{C1999P2}{C/1999 P2}{C/1999 P2 (SOHO)}
%\DeclareComet{C1999P3}{C/1999 P3}{C/1999 P3 (SOHO)}
%\DeclareComet{C1999P4}{C/1999 P4}{C/1999 P4 (SOHO)}
%\DeclareComet{C1999P5}{C/1999 P5}{C/1999 P5 (SOHO)}
%\DeclareComet{C1999P6}{C/1999 P6}{C/1999 P6 (SOHO)}
%\DeclareComet{C1999P7}{C/1999 P7}{C/1999 P7 (SOHO)}
%\DeclareComet{C1999P8}{C/1999 P8}{C/1999 P8 (SOHO)}
%\DeclareComet{C1999P9}{C/1999 P9}{C/1999 P9 (SOHO)}
%\DeclareComet{C1999Q1}{C/1999 Q1}{C/1999 Q1 (SOHO)}
%\DeclareComet{C1999Q2}{C/1999 Q2}{C/1999 Q2 (SOHO)}
%\DeclareComet{C1999Q3}{C/1999 Q3}{C/1999 Q3 (SOHO)}
%\DeclareComet{C1999Q4}{C/1999 Q4}{C/1999 Q4 (SOHO)}
%\DeclareComet{C1999R3}{C/1999 R3}{C/1999 R3 (SOHO)}
%\DeclareComet{C1999R4}{C/1999 R4}{C/1999 R4 (SOHO)}
%\DeclareComet{C1999R5}{C/1999 R5}{C/1999 R5 (SOHO)}
%\DeclareComet{C1999S1}{C/1999 S1}{C/1999 S1 (SOHO)}
%\DeclareComet{C1999S2}{C/1999 S2}{C/1999 S2 (McNaught-Watson)}
%\DeclareComet{C1999S3}{C/1999 S3}{C/1999 S3 (LINEAR)}
%\DeclareComet{C1999S4}{C/1999 S4}{C/1999 S4 (LINEAR)}
%\DeclareComet{C1999S5}{C/1999 S5}{C/1999 S5 (SOHO)}
%\DeclareComet{C1999S6}{C/1999 S6}{C/1999 S6 (SOHO)}
%\DeclareComet{C1999S7}{C/1999 S7}{C/1999 S7 (SOHO)}
%\DeclareComet{C1999S8}{C/1999 S8}{C/1999 S8 (SOHO)}
%\DeclareComet{C1999T1}{C/1999 T1}{C/1999 T1 (McNaught-Hartley)}
%\DeclareComet{C1999T2}{C/1999 T2}{C/1999 T2 (LINEAR)}
%\DeclareComet{C1999T3}{C/1999 T3}{C/1999 T3 (LINEAR)}
%\DeclareComet{C1999U1}{C/1999 U1}{C/1999 U1 (Ferris)}
%\DeclareComet{C1999U2}{C/1999 U2}{C/1999 U2 (SOHO)}
%\DeclareComet{C1999U4}{C/1999 U4}{C/1999 U4 (Catalina-Skiff)}
%\DeclareComet{C1999U5}{C/1999 U5}{C/1999 U5 (SOHO)}
%\DeclareComet{C1999U6}{C/1999 U6}{C/1999 U6 (SOHO)}
%\DeclareComet{C1999U7}{C/1999 U7}{C/1999 U7 (SOHO)}
%\DeclareComet{C1999U8}{C/1999 U8}{C/1999 U8 (SOHO)}
%\DeclareComet{C1999U9}{C/1999 U9}{C/1999 U9 (SOHO)}
%\DeclareComet{C1999V2}{C/1999 V2}{C/1999 V2 (SOHO)}
%\DeclareComet{C1999V3}{C/1999 V3}{C/1999 V3 (SOHO)}
%\DeclareComet{C1999V4}{C/1999 V4}{C/1999 V4 (SOHO)}
%\DeclareComet{C1999V5}{C/1999 V5}{C/1999 V5 (SOHO)}
%\DeclareComet{C1999W1}{C/1999 W1}{C/1999 W1 (SOHO)}
%\DeclareComet{C1999W2}{C/1999 W2}{C/1999 W2 (SOHO)}
%\DeclareComet{C1999X2}{C/1999 X2}{C/1999 X2 (SOHO)}
%\DeclareComet{C1999XS87}{C/1999 XS87}{C/1999 XS87 (LINEAR)}
%\DeclareComet{C1999Y1}{C/1999 Y1}{C/1999 Y1 (LINEAR)}
%\DeclareComet{C1999Y2}{C/1999 Y2}{C/1999 Y2 (SOHO)}
%\DeclareComet{C1999Y3}{C/1999 Y3}{C/1999 Y3 (SOHO)}
%\DeclareComet{C2000A1}{C/2000 A1}{C/2000 A1 (Montani)}
%\DeclareComet{C2000A2}{C/2000 A2}{C/2000 A2 (SOHO)}
%\DeclareComet{C2000B1}{C/2000 B1}{C/2000 B1 (SOHO)}
%\DeclareComet{C2000B2}{C/2000 B2}{C/2000 B2 (LINEAR)}
%\DeclareComet{C2000B5}{C/2000 B5}{C/2000 B5 (SOHO)}
%\DeclareComet{C2000B6}{C/2000 B6}{C/2000 B6 (SOHO)}
%\DeclareComet{C2000B7}{C/2000 B7}{C/2000 B7 (SOHO)}
%\DeclareComet{C2000B8}{C/2000 B8}{C/2000 B8 (SOHO)}
%\DeclareComet{C2000C2}{C/2000 C2}{C/2000 C2 (SOHO)}
%\DeclareComet{C2000C3}{C/2000 C3}{C/2000 C3 (SOHO)}
%\DeclareComet{C2000C4}{C/2000 C4}{C/2000 C4 (SOHO)}
%\DeclareComet{C2000C5}{C/2000 C5}{C/2000 C5 (SOHO)}
%\DeclareComet{C2000C6}{C/2000 C6}{C/2000 C6 (SOHO)}
%\DeclareComet{C2000C7}{C/2000 C7}{C/2000 C7 (SOHO)}
%\DeclareComet{C2000CT54}{C/2000 CT54}{C/2000 CT54 (LINEAR)}
%\DeclareComet{C2000D1}{C/2000 D1}{C/2000 D1 (SOHO)}
%\DeclareComet{C2000D2}{C/2000 D2}{C/2000 D2 (LINEAR)}
%\DeclareComet{C2000D3}{C/2000 D3}{C/2000 D3 (SOHO)}
%\DeclareComet{C2000D4}{C/2000 D4}{C/2000 D4 (SOHO)}
%\DeclareComet{C2000E1}{C/2000 E1}{C/2000 E1 (SOHO)}
%\DeclareComet{C2000F1}{C/2000 F1}{C/2000 F1 (SOHO)}
%\DeclareComet{C2000F2}{C/2000 F2}{C/2000 F2 (SOHO)}
%\DeclareComet{C2000F3}{C/2000 F3}{C/2000 F3 (SOHO)}
%\DeclareComet{C2000G2}{C/2000 G2}{C/2000 G2 (LINEAR)}
%\DeclareComet{C2000G3}{C/2000 G3}{C/2000 G3 (SOHO)}
%\DeclareComet{C2000H1}{C/2000 H1}{C/2000 H1 (LINEAR)}
%\DeclareComet{C2000H2}{C/2000 H2}{C/2000 H2 (SOHO)}
%\DeclareComet{C2000H3}{C/2000 H3}{C/2000 H3 (SOHO)}
%\DeclareComet{C2000H4}{C/2000 H4}{C/2000 H4 (SOHO)}
%\DeclareComet{C2000H5}{C/2000 H5}{C/2000 H5 (SOHO)}
%\DeclareComet{C2000H6}{C/2000 H6}{C/2000 H6 (SOHO)}
%\DeclareComet{C2000H7}{C/2000 H7}{C/2000 H7 (SOHO)}
%\DeclareComet{C2000J1}{C/2000 J1}{C/2000 J1 (Ferris)}
%\DeclareComet{C2000J2}{C/2000 J2}{C/2000 J2 (SOHO)}
%\DeclareComet{C2000J3}{C/2000 J3}{C/2000 J3 (SOHO)}
%\DeclareComet{C2000J4}{C/2000 J4}{C/2000 J4 (SOHO)}
%\DeclareComet{C2000J5}{C/2000 J5}{C/2000 J5 (SOHO)}
%\DeclareComet{C2000J6}{C/2000 J6}{C/2000 J6 (SOHO)}
%\DeclareComet{C2000J7}{C/2000 J7}{C/2000 J7 (SOHO)}
%\DeclareComet{C2000J8}{C/2000 J8}{C/2000 J8 (SOHO)}
%\DeclareComet{C2000K1}{C/2000 K1}{C/2000 K1 (LINEAR)}
%\DeclareComet{C2000K2}{C/2000 K2}{C/2000 K2 (LINEAR)}
%\DeclareComet{C2000K3}{C/2000 K3}{C/2000 K3 (SOHO)}
%\DeclareComet{C2000K4}{C/2000 K4}{C/2000 K4 (SOHO)}
%\DeclareComet{C2000K5}{C/2000 K5}{C/2000 K5 (SOHO)}
%\DeclareComet{C2000K6}{C/2000 K6}{C/2000 K6 (SOHO)}
%\DeclareComet{C2000K7}{C/2000 K7}{C/2000 K7 (SOHO)}
%\DeclareComet{C2000K8}{C/2000 K8}{C/2000 K8 (SOHO)}
%\DeclareComet{C2000L1}{C/2000 L1}{C/2000 L1 (SOHO)}
%\DeclareComet{C2000L2}{C/2000 L2}{C/2000 L2 (SOHO)}
%\DeclareComet{C2000L3}{C/2000 L3}{C/2000 L3 (SOHO)}
%\DeclareComet{C2000L4}{C/2000 L4}{C/2000 L4 (SOHO)}
%\DeclareComet{C2000L5}{C/2000 L5}{C/2000 L5 (SOHO)}
%\DeclareComet{C2000L6}{C/2000 L6}{C/2000 L6 (SOHO)}
%\DeclareComet{C2000M1}{C/2000 M1}{C/2000 M1 (SOHO)}
%\DeclareComet{C2000M2}{C/2000 M2}{C/2000 M2 (SOHO)}
%\DeclareComet{C2000M3}{C/2000 M3}{C/2000 M3 (SOHO)}
%\DeclareComet{C2000M4}{C/2000 M4}{C/2000 M4 (SOHO)}
%\DeclareComet{C2000M5}{C/2000 M5}{C/2000 M5 (SOHO)}
%\DeclareComet{C2000M6}{C/2000 M6}{C/2000 M6 (SOHO)}
%\DeclareComet{C2000M7}{C/2000 M7}{C/2000 M7 (SOHO)}
%\DeclareComet{C2000M8}{C/2000 M8}{C/2000 M8 (SOHO)}
%\DeclareComet{C2000M9}{C/2000 M9}{C/2000 M9 (SOHO)}
%\DeclareComet{C2000N1}{C/2000 N1}{C/2000 N1 (SOHO)}
%\DeclareComet{C2000N2}{C/2000 N2}{C/2000 N2 (SOHO)}
%\DeclareComet{C2000N3}{C/2000 N3}{C/2000 N3 (SOHO)}
%\DeclareComet{C2000N4}{C/2000 N4}{C/2000 N4 (SOHO)}
%\DeclareComet{C2000O1}{C/2000 O1}{C/2000 O1 (Koehn)}
%\DeclareComet{C2000OF8}{C/2000 OF8}{C/2000 OF8 (Spacewatch)}
%\DeclareComet{C2000P1}{C/2000 P1}{C/2000 P1 (SOHO)}
%\DeclareComet{C2000P2}{C/2000 P2}{C/2000 P2 (SOHO)}
%\DeclareComet{C2000P4}{C/2000 P4}{C/2000 P4 (SOHO)}
%\DeclareComet{C2000P5}{C/2000 P5}{C/2000 P5 (SOHO)}
%\DeclareComet{C2000Q1}{C/2000 Q1}{C/2000 Q1 (SOHO)}
%\DeclareComet{C2000S3}{C/2000 S3}{C/2000 S3 (LONEOS)}
%\DeclareComet{C2000S5}{C/2000 S5}{C/2000 S5}
%\DeclareComet{C2000S6}{C/2000 S6}{C/2000 S6 (SOHO)}
%\DeclareComet{C2000S8}{C/2000 S8}{C/2000 S8 (SOHO)}
%\DeclareComet{C2000S9}{C/2000 S9}{C/2000 S9 (SOHO)}
%\DeclareComet{C2000SV74}{C/2000 SV74}{C/2000 SV74 (LINEAR)}
%\DeclareComet{C2000T1}{C/2000 T1}{C/2000 T1 (SOHO)}
%\DeclareComet{C2000T3}{C/2000 T3}{C/2000 T3 (SOHO)}
%\DeclareComet{C2000T4}{C/2000 T4}{C/2000 T4 (SOHO)}
%\DeclareComet{C2000T5}{C/2000 T5}{C/2000 T5 (SOHO)}
%\DeclareComet{C2000T6}{C/2000 T6}{C/2000 T6 (SOHO)}
%\DeclareComet{C2000U1}{C/2000 U1}{C/2000 U1 (SOHO)}
%\DeclareComet{C2000U2}{C/2000 U2}{C/2000 U2 (SOHO)}
%\DeclareComet{C2000U3}{C/2000 U3}{C/2000 U3 (SOHO)}
%\DeclareComet{C2000U4}{C/2000 U4}{C/2000 U4 (SOHO)}
%\DeclareComet{C2000U5}{C/2000 U5}{C/2000 U5 (LINEAR)}
%\DeclareComet{C2000V1}{C/2000 V1}{C/2000 V1 (SOHO)}
%\DeclareComet{C2000V2}{C/2000 V2}{C/2000 V2 (SOHO)}
%\DeclareComet{C2000V3}{C/2000 V3}{C/2000 V3 (SOHO)}
%\DeclareComet{C2000V4}{C/2000 V4}{C/2000 V4 (SOHO)}
%\DeclareComet{C2000W1}{C/2000 W1}{C/2000 W1 (Utsunomiya-Jones)}
%\DeclareComet{C2000W2}{C/2000 W2}{C/2000 W2 (SOHO)}
%\DeclareComet{C2000W3}{C/2000 W3}{C/2000 W3 (SOHO)}
%\DeclareComet{C2000W4}{C/2000 W4}{C/2000 W4 (SOHO)}
%\DeclareComet{C2000W5}{C/2000 W5}{C/2000 W5 (SOHO)}
%\DeclareComet{C2000WM1}{C/2000 WM1}{C/2000 WM1 (LINEAR)}
%\DeclareComet{C2000X1}{C/2000 X1}{C/2000 X1 (SOHO)}
%\DeclareComet{C2000X2}{C/2000 X2}{C/2000 X2 (SOHO)}
%\DeclareComet{C2000X3}{C/2000 X3}{C/2000 X3 (SOHO)}
%\DeclareComet{C2000X4}{C/2000 X4}{C/2000 X4 (SOHO)}
%\DeclareComet{C2000X5}{C/2000 X5}{C/2000 X5 (SOHO)}
%\DeclareComet{C2000X6}{C/2000 X6}{C/2000 X6 (SOHO)}
%\DeclareComet{C2000X7}{C/2000 X7}{C/2000 X7 (SOHO)}
%\DeclareComet{C2000X8}{C/2000 X8}{C/2000 X8 (SOHO)}
%\DeclareComet{C2000X9}{C/2000 X9}{C/2000 X9 (SOHO)}
%\DeclareComet{C2000Y1}{C/2000 Y1}{C/2000 Y1 (Tubbiolo)}
%\DeclareComet{C2000Y2}{C/2000 Y2}{C/2000 Y2 (Skiff)}
%\DeclareComet{C2000Y4}{C/2000 Y4}{C/2000 Y4 (SOHO)}
%\DeclareComet{C2000Y5}{C/2000 Y5}{C/2000 Y5 (SOHO)}
%\DeclareComet{C2000Y6}{C/2000 Y6}{C/2000 Y6 (SOHO)}
%\DeclareComet{C2000Y7}{C/2000 Y7}{C/2000 Y7 (SOHO)}
%\DeclareComet{C2000Y8}{C/2000 Y8}{C/2000 Y8 (SOHO)}
%\DeclareComet{C2000Y9}{C/2000 Y9}{C/2000 Y9 (SOHO)}
%\DeclareComet{C2001A1}{C/2001 A1}{C/2001 A1 (LINEAR)}
%\DeclareComet{C2001A2-A}{C/2001 A2-A}{C/2001 A2-A (LINEAR)}
%\DeclareComet{C2001A2-B}{C/2001 A2-B}{C/2001 A2-B (LINEAR)}
%\DeclareComet{C2001A3}{C/2001 A3}{C/2001 A3 (SOHO)}
%\DeclareComet{C2001A4}{C/2001 A4}{C/2001 A4 (SOHO)}
%\DeclareComet{C2001A5}{C/2001 A5}{C/2001 A5 (SOHO)}
%\DeclareComet{C2001B1}{C/2001 B1}{C/2001 B1 (LINEAR)}
%\DeclareComet{C2001B2}{C/2001 B2}{C/2001 B2 (NEAT)}
%\DeclareComet{C2001B3}{C/2001 B3}{C/2001 B3 (SOHO)}
%\DeclareComet{C2001C1}{C/2001 C1}{C/2001 C1 (LINEAR)}
%\DeclareComet{C2001C2}{C/2001 C2}{C/2001 C2 (SOHO)}
%\DeclareComet{C2001C3}{C/2001 C3}{C/2001 C3 (SOHO)}
%\DeclareComet{C2001C4}{C/2001 C4}{C/2001 C4 (SOHO)}
%\DeclareComet{C2001C5}{C/2001 C5}{C/2001 C5 (SOHO)}
%\DeclareComet{C2001C6}{C/2001 C6}{C/2001 C6 (SOHO)}
%\DeclareComet{C2001C7}{C/2001 C7}{C/2001 C7 (SOHO)}
%\DeclareComet{C2001D2}{C/2001 D2}{C/2001 D2 (SOHO)}
%\DeclareComet{C2001E1}{C/2001 E1}{C/2001 E1 (SOHO)}
%\DeclareComet{C2001F2}{C/2001 F2}{C/2001 F2 (SOHO)}
%\DeclareComet{C2001G1}{C/2001 G1}{C/2001 G1 (LONEOS)}
%\DeclareComet{C2001G2}{C/2001 G2}{C/2001 G2 (SOHO)}
%\DeclareComet{C2001G3}{C/2001 G3}{C/2001 G3 (SOHO)}
%\DeclareComet{C2001H1}{C/2001 H1}{C/2001 H1 (SOHO)}
%\DeclareComet{C2001H2}{C/2001 H2}{C/2001 H2 (SOHO)}
%\DeclareComet{C2001H3}{C/2001 H3}{C/2001 H3 (SOHO)}
%\DeclareComet{C2001H4}{C/2001 H4}{C/2001 H4 (SOHO)}
%\DeclareComet{C2001H6}{C/2001 H6}{C/2001 H6 (SOHO)}
%\DeclareComet{C2001H7}{C/2001 H7}{C/2001 H7 (SOHO)}
%\DeclareComet{C2001H8}{C/2001 H8}{C/2001 H8 (SOHO)}
%\DeclareComet{C2001HT50}{C/2001 HT50}{C/2001 HT50 (LINEAR-NEAT)}
%\DeclareComet{C2001J2}{C/2001 J2}{C/2001 J2 (SOHO)}
%\DeclareComet{C2001J3}{C/2001 J3}{C/2001 J3 (SOHO)}
%\DeclareComet{C2001J4}{C/2001 J4}{C/2001 J4 (SOHO)}
%\DeclareComet{C2001J5}{C/2001 J5}{C/2001 J5 (SOHO)}
%\DeclareComet{C2001K10}{C/2001 K10}{C/2001 K10 (SOHO)}
%\DeclareComet{C2001K11}{C/2001 K11}{C/2001 K11 (SOHO)}
%\DeclareComet{C2001K2}{C/2001 K2}{C/2001 K2 (SOHO)}
%\DeclareComet{C2001K3}{C/2001 K3}{C/2001 K3 (Skiff)}
%\DeclareComet{C2001K4}{C/2001 K4}{C/2001 K4 (SOHO)}
%\DeclareComet{C2001K5}{C/2001 K5}{C/2001 K5 (LINEAR)}
%\DeclareComet{C2001K6}{C/2001 K6}{C/2001 K6 (SOHO)}
%\DeclareComet{C2001K7}{C/2001 K7}{C/2001 K7 (SOHO)}
%\DeclareComet{C2001K8}{C/2001 K8}{C/2001 K8 (SOHO)}
%\DeclareComet{C2001K9}{C/2001 K9}{C/2001 K9 (SOHO)}
%\DeclareComet{C2001L1}{C/2001 L1}{C/2001 L1 (SOHO)}
%\DeclareComet{C2001L10}{C/2001 L10}{C/2001 L10 (SOHO)}
%\DeclareComet{C2001L11}{C/2001 L11}{C/2001 L11 (SOHO)}
%\DeclareComet{C2001L2}{C/2001 L2}{C/2001 L2 (SOHO)}
%\DeclareComet{C2001L3}{C/2001 L3}{C/2001 L3 (SOHO)}
%\DeclareComet{C2001L4}{C/2001 L4}{C/2001 L4 (SOHO)}
%\DeclareComet{C2001L5}{C/2001 L5}{C/2001 L5 (SOHO)}
%\DeclareComet{C2001L6}{C/2001 L6}{C/2001 L6 (SOHO)}
%\DeclareComet{C2001L7}{C/2001 L7}{C/2001 L7 (SOHO)}
%\DeclareComet{C2001L8}{C/2001 L8}{C/2001 L8 (SOHO)}
%\DeclareComet{C2001L9}{C/2001 L9}{C/2001 L9 (SOHO)}
%\DeclareComet{C2001M10}{C/2001 M10}{C/2001 M10 (NEAT)}
%\DeclareComet{C2001M11}{C/2001 M11}{C/2001 M11 (SOHO)}
%\DeclareComet{C2001M2}{C/2001 M2}{C/2001 M2 (SOHO)}
%\DeclareComet{C2001M3}{C/2001 M3}{C/2001 M3 (SOHO)}
%\DeclareComet{C2001M4}{C/2001 M4}{C/2001 M4 (SOHO)}
%\DeclareComet{C2001M5}{C/2001 M5}{C/2001 M5 (SOHO)}
%\DeclareComet{C2001M6}{C/2001 M6}{C/2001 M6 (SOHO)}
%\DeclareComet{C2001M7}{C/2001 M7}{C/2001 M7 (SOHO)}
%\DeclareComet{C2001M8}{C/2001 M8}{C/2001 M8 (SOHO)}
%\DeclareComet{C2001M9}{C/2001 M9}{C/2001 M9 (SOHO)}
%\DeclareComet{C2001N1}{C/2001 N1}{C/2001 N1 (SOHO)}
%\DeclareComet{C2001N2}{C/2001 N2}{C/2001 N2 (LINEAR)}
%\DeclareComet{C2001O1}{C/2001 O1}{C/2001 O1 (SOHO)}
%\DeclareComet{C2001O2}{C/2001 O2}{C/2001 O2 (NEAT)}
%\DeclareComet{C2001O3}{C/2001 O3}{C/2001 O3 (SOHO)}
%\DeclareComet{C2001OG108}{C/2001 OG108}{C/2001 OG108 (LONEOS)}
%\DeclareComet{C2001P1}{C/2001 P1}{C/2001 P1 (SOHO)}
%\DeclareComet{C2001P2}{C/2001 P2}{C/2001 P2 (SOHO)}
%\DeclareComet{C2001Q1}{C/2001 Q1}{C/2001 Q1 (NEAT)}
%\DeclareComet{C2001Q3}{C/2001 Q3}{C/2001 Q3 (SOHO)}
%\DeclareComet{C2001Q4}{C/2001 Q4}{C/2001 Q4 (NEAT)}
%\DeclareComet{C2001Q7}{C/2001 Q7}{C/2001 Q7 (SOHO)}
%\DeclareComet{C2001Q8}{C/2001 Q8}{C/2001 Q8 (SOHO)}
%\DeclareComet{C2001Q9}{C/2001 Q9}{C/2001 Q9 (SOHO)}
%\DeclareComet{C2001R10}{C/2001 R10}{C/2001 R10 (SOHO)}
%\DeclareComet{C2001R2}{C/2001 R2}{C/2001 R2 (SOHO)}
%\DeclareComet{C2001R3}{C/2001 R3}{C/2001 R3 (SOHO)}
%\DeclareComet{C2001R4}{C/2001 R4}{C/2001 R4 (SOHO)}
%\DeclareComet{C2001R5}{C/2001 R5}{C/2001 R5 (SOHO)}
%\DeclareComet{C2001R7}{C/2001 R7}{C/2001 R7 (SOHO)}
%\DeclareComet{C2001R8}{C/2001 R8}{C/2001 R8 (SOHO)}
%\DeclareComet{C2001R9}{C/2001 R9}{C/2001 R9 (SOHO)}
%\DeclareComet{C2001RX14}{C/2001 RX14}{C/2001 RX14 (LINEAR)}
%\DeclareComet{C2001S1}{C/2001 S1}{C/2001 S1 (Skiff)}
%\DeclareComet{C2001S2}{C/2001 S2}{C/2001 S2 (SOHO)}
%\DeclareComet{C2001S3}{C/2001 S3}{C/2001 S3 (SOHO)}
%\DeclareComet{C2001T1}{C/2001 T1}{C/2001 T1 (SOHO)}
%\DeclareComet{C2001T2}{C/2001 T2}{C/2001 T2 (SOHO)}
%\DeclareComet{C2001T5}{C/2001 T5}{C/2001 T5 (SOHO)}
%\DeclareComet{C2001T6}{C/2001 T6}{C/2001 T6 (SOHO)}
%\DeclareComet{C2001T7}{C/2001 T7}{C/2001 T7 (SOHO)}
%\DeclareComet{C2001U1}{C/2001 U1}{C/2001 U1 (SOHO)}
%\DeclareComet{C2001U10}{C/2001 U10}{C/2001 U10 (SOHO)}
%\DeclareComet{C2001U2}{C/2001 U2}{C/2001 U2 (SOHO)}
%\DeclareComet{C2001U3}{C/2001 U3}{C/2001 U3 (SOHO)}
%\DeclareComet{C2001U4}{C/2001 U4}{C/2001 U4 (SOHO)}
%\DeclareComet{C2001U5}{C/2001 U5}{C/2001 U5 (SOHO)}
%\DeclareComet{C2001U6}{C/2001 U6}{C/2001 U6 (LINEAR)}
%\DeclareComet{C2001U7}{C/2001 U7}{C/2001 U7 (SOHO)}
%\DeclareComet{C2001U8}{C/2001 U8}{C/2001 U8 (SOHO)}
%\DeclareComet{C2001U9}{C/2001 U9}{C/2001 U9 (SOHO)}
%\DeclareComet{C2001V1}{C/2001 V1}{C/2001 V1 (SOHO)}
%\DeclareComet{C2001V2}{C/2001 V2}{C/2001 V2 (SOHO)}
%\DeclareComet{C2001V3}{C/2001 V3}{C/2001 V3 (SOHO)}
%\DeclareComet{C2001V4}{C/2001 V4}{C/2001 V4 (SOHO)}
%\DeclareComet{C2001V5}{C/2001 V5}{C/2001 V5 (SOHO)}
%\DeclareComet{C2001V6}{C/2001 V6}{C/2001 V6 (SOHO)}
%\DeclareComet{C2001W1}{C/2001 W1}{C/2001 W1 (LINEAR)}
%\DeclareComet{C2001W2}{C/2001 W2}{C/2001 W2 (BATTERS)}
%\DeclareComet{C2001W3}{C/2001 W3}{C/2001 W3 (SOHO)}
%\DeclareComet{C2001W4}{C/2001 W4}{C/2001 W4 (SOHO)}
%\DeclareComet{C2001W5}{C/2001 W5}{C/2001 W5 (SOHO)}
%\DeclareComet{C2001X1}{C/2001 X1}{C/2001 X1 (LINEAR)}
%\DeclareComet{C2001X10}{C/2001 X10}{C/2001 X10 (SOHO)}
%\DeclareComet{C2001X4}{C/2001 X4}{C/2001 X4 (SOHO)}
%\DeclareComet{C2001X5}{C/2001 X5}{C/2001 X5 (SOHO)}
%\DeclareComet{C2001X6}{C/2001 X6}{C/2001 X6 (SOHO)}
%\DeclareComet{C2001X7}{C/2001 X7}{C/2001 X7 (SOHO)}
%\DeclareComet{C2001X8}{C/2001 X8}{C/2001 X8 (SOHO)}
%\DeclareComet{C2001X9}{C/2001 X9}{C/2001 X9 (SOHO)}
%\DeclareComet{C2001Y2}{C/2001 Y2}{C/2001 Y2 (SOHO)}
%\DeclareComet{C2001Y3}{C/2001 Y3}{C/2001 Y3 (SOHO)}
%\DeclareComet{C2001Y4}{C/2001 Y4}{C/2001 Y4 (SOHO)}
%\DeclareComet{C2001Y5}{C/2001 Y5}{C/2001 Y5 (SOHO)}
%\DeclareComet{C2002A1}{C/2002 A1}{C/2002 A1 (LINEAR)}
%\DeclareComet{C2002A2}{C/2002 A2}{C/2002 A2 (LINEAR)}
%\DeclareComet{C2002A3}{C/2002 A3}{C/2002 A3 (LINEAR)}
%\DeclareComet{C2002A4}{C/2002 A4}{C/2002 A4 (SOHO)}
%\DeclareComet{C2002B1}{C/2002 B1}{C/2002 B1 (LINEAR)}
%\DeclareComet{C2002B2}{C/2002 B2}{C/2002 B2 (LINEAR)}
%\DeclareComet{C2002B3}{C/2002 B3}{C/2002 B3 (LINEAR)}
%\DeclareComet{C2002B4}{C/2002 B4}{C/2002 B4 (SOHO)}
%\DeclareComet{C2002C2}{C/2002 C2}{C/2002 C2 (LINEAR)}
%\DeclareComet{C2002C3}{C/2002 C3}{C/2002 C3 (SOHO)}
%\DeclareComet{C2002C4}{C/2002 C4}{C/2002 C4 (SOHO)}
%\DeclareComet{C2002CE10}{C/2002 CE10}{C/2002 CE10 (LINEAR)}
%\DeclareComet{C2002D1}{C/2002 D1}{C/2002 D1 (SOHO)}
%\DeclareComet{C2002E1}{C/2002 E1}{C/2002 E1 (SOHO)}
%\DeclareComet{C2002E2}{C/2002 E2}{C/2002 E2 (Snyder-Murakami)}
%\DeclareComet{C2002E3}{C/2002 E3}{C/2002 E3 (SOHO)}
%\DeclareComet{C2002F1}{C/2002 F1}{C/2002 F1 (Utsunomiya)}
%\DeclareComet{C2002F2}{C/2002 F2}{C/2002 F2 (SOHO)}
%\DeclareComet{C2002F3}{C/2002 F3}{C/2002 F3 (SOHO)}
%\DeclareComet{C2002G1}{C/2002 G1}{C/2002 G1 (SOHO)}
%\DeclareComet{C2002G2}{C/2002 G2}{C/2002 G2 (SOHO)}
%\DeclareComet{C2002G3}{C/2002 G3}{C/2002 G3 (SOHO)}
%\DeclareComet{C2002G4}{C/2002 G4}{C/2002 G4 (SOHO)}
%\DeclareComet{C2002G5}{C/2002 G5}{C/2002 G5 (SOHO)}
%\DeclareComet{C2002H1}{C/2002 H1}{C/2002 H1 (SOHO)}
%\DeclareComet{C2002H2}{C/2002 H2}{C/2002 H2 (LINEAR)}
%\DeclareComet{C2002H3}{C/2002 H3}{C/2002 H3 (SOHO)}
%\DeclareComet{C2002H4}{C/2002 H4}{C/2002 H4 (SOHO)}
%\DeclareComet{C2002H5}{C/2002 H5}{C/2002 H5 (SOHO)}
%\DeclareComet{C2002H6}{C/2002 H6}{C/2002 H6 (SOHO)}
%\DeclareComet{C2002H7}{C/2002 H7}{C/2002 H7 (SOHO)}
%\DeclareComet{C2002H8}{C/2002 H8}{C/2002 H8 (SOHO)}
%\DeclareComet{C2002J1}{C/2002 J1}{C/2002 J1 (SOHO)}
%\DeclareComet{C2002J2}{C/2002 J2}{C/2002 J2 (SOHO)}
%\DeclareComet{C2002J3}{C/2002 J3}{C/2002 J3 (SOHO)}
%\DeclareComet{C2002J4}{C/2002 J4}{C/2002 J4 (NEAT)}
%\DeclareComet{C2002J5}{C/2002 J5}{C/2002 J5 (LINEAR)}
%\DeclareComet{C2002J6}{C/2002 J6}{C/2002 J6 (SOHO)}
%\DeclareComet{C2002J7}{C/2002 J7}{C/2002 J7 (SOHO)}
%\DeclareComet{C2002J8}{C/2002 J8}{C/2002 J8 (SOHO)}
%\DeclareComet{C2002K1}{C/2002 K1}{C/2002 K1 (NEAT)}
%\DeclareComet{C2002K10}{C/2002 K10}{C/2002 K10 (SOHO)}
%\DeclareComet{C2002K11}{C/2002 K11}{C/2002 K11 (SOHO)}
%\DeclareComet{C2002K2}{C/2002 K2}{C/2002 K2 (LINEAR)}
%\DeclareComet{C2002K3}{C/2002 K3}{C/2002 K3 (SOHO)}
%\DeclareComet{C2002K4}{C/2002 K4}{C/2002 K4 (NEAT)}
%\DeclareComet{C2002K5}{C/2002 K5}{C/2002 K5 (SOHO)}
%\DeclareComet{C2002K6}{C/2002 K6}{C/2002 K6 (SOHO)}
%\DeclareComet{C2002K7}{C/2002 K7}{C/2002 K7 (SOHO)}
%\DeclareComet{C2002K8}{C/2002 K8}{C/2002 K8 (SOHO)}
%\DeclareComet{C2002K9}{C/2002 K9}{C/2002 K9 (SOHO)}
%\DeclareComet{C2002L1}{C/2002 L1}{C/2002 L1 (SOHO)}
%\DeclareComet{C2002L2}{C/2002 L2}{C/2002 L2 (SOHO)}
%\DeclareComet{C2002L3}{C/2002 L3}{C/2002 L3 (SOHO)}
%\DeclareComet{C2002L4}{C/2002 L4}{C/2002 L4 (SOHO)}
%\DeclareComet{C2002L5}{C/2002 L5}{C/2002 L5 (SOHO)}
%\DeclareComet{C2002L6}{C/2002 L6}{C/2002 L6 (SOHO)}
%\DeclareComet{C2002L7}{C/2002 L7}{C/2002 L7 (SOHO)}
%\DeclareComet{C2002L8}{C/2002 L8}{C/2002 L8 (SOHO)}
%\DeclareComet{C2002L9}{C/2002 L9}{C/2002 L9 (NEAT)}
%\DeclareComet{C2002M1}{C/2002 M1}{C/2002 M1 (SOHO)}
%\DeclareComet{C2002M2}{C/2002 M2}{C/2002 M2 (SOHO)}
%\DeclareComet{C2002M3}{C/2002 M3}{C/2002 M3 (SOHO)}
%\DeclareComet{C2002M4}{C/2002 M4}{C/2002 M4 (SOHO)}
%\DeclareComet{C2002M5}{C/2002 M5}{C/2002 M5 (SOHO)}
%\DeclareComet{C2002M6}{C/2002 M6}{C/2002 M6 (SOHO)}
%\DeclareComet{C2002M7}{C/2002 M7}{C/2002 M7 (SOHO)}
%\DeclareComet{C2002M8}{C/2002 M8}{C/2002 M8 (SOHO)}
%\DeclareComet{C2002N1}{C/2002 N1}{C/2002 N1 (SOHO)}
%\DeclareComet{C2002N2}{C/2002 N2}{C/2002 N2 (SOHO)}
%\DeclareComet{C2002O1}{C/2002 O1}{C/2002 O1 (SOHO)}
%\DeclareComet{C2002O2}{C/2002 O2}{C/2002 O2 (SOHO)}
%\DeclareComet{C2002O3}{C/2002 O3}{C/2002 O3 (SOHO)}
%\DeclareComet{C2002O4}{C/2002 O4}{C/2002 O4 (Hoenig)}
%\DeclareComet{C2002O6}{C/2002 O6}{C/2002 O6 (SWAN)}
%\DeclareComet{C2002O7}{C/2002 O7}{C/2002 O7 (LINEAR)}
%\DeclareComet{C2002P1}{C/2002 P1}{C/2002 P1 (NEAT)}
%\DeclareComet{C2002P2}{C/2002 P2}{C/2002 P2 (SOHO)}
%\DeclareComet{C2002P3}{C/2002 P3}{C/2002 P3 (SOHO)}
%\DeclareComet{C2002Q10}{C/2002 Q10}{C/2002 Q10 (SOHO)}
%\DeclareComet{C2002Q11}{C/2002 Q11}{C/2002 Q11 (SOHO)}
%\DeclareComet{C2002Q12}{C/2002 Q12}{C/2002 Q12 (SOHO)}
%\DeclareComet{C2002Q13}{C/2002 Q13}{C/2002 Q13 (SOHO)}
%\DeclareComet{C2002Q14}{C/2002 Q14}{C/2002 Q14 (SOHO)}
%\DeclareComet{C2002Q2}{C/2002 Q2}{C/2002 Q2 (LINEAR)}
%\DeclareComet{C2002Q3}{C/2002 Q3}{C/2002 Q3 (LINEAR)}
%\DeclareComet{C2002Q5}{C/2002 Q5}{C/2002 Q5 (LINEAR)}
%\DeclareComet{C2002Q6}{C/2002 Q6}{C/2002 Q6 (SOHO)}
%\DeclareComet{C2002Q7}{C/2002 Q7}{C/2002 Q7 (SOHO)}
%\DeclareComet{C2002Q8}{C/2002 Q8}{C/2002 Q8 (SOHO)}
%\DeclareComet{C2002Q9}{C/2002 Q9}{C/2002 Q9 (SOHO)}
%\DeclareComet{C2002R1}{C/2002 R1}{C/2002 R1 (SOHO)}
%\DeclareComet{C2002R3}{C/2002 R3}{C/2002 R3 (LONEOS)}
%\DeclareComet{C2002R4}{C/2002 R4}{C/2002 R4 (SOHO)}
%\DeclareComet{C2002R5}{C/2002 R5}{C/2002 R5 (SOHO)}
%\DeclareComet{C2002R6}{C/2002 R6}{C/2002 R6 (SOHO)}
%\DeclareComet{C2002R7}{C/2002 R7}{C/2002 R7 (SOHO)}
%\DeclareComet{C2002R8}{C/2002 R8}{C/2002 R8 (SOHO)}
%\DeclareComet{C2002S10}{C/2002 S10}{C/2002 S10 (SOHO)}
%\DeclareComet{C2002S11}{C/2002 S11}{C/2002 S11 (SOHO)}
%\DeclareComet{C2002S2}{C/2002 S2}{C/2002 S2 (SOHO)}
%\DeclareComet{C2002S3}{C/2002 S3}{C/2002 S3 (SOHO)}
%\DeclareComet{C2002S4}{C/2002 S4}{C/2002 S4 (SOHO)}
%\DeclareComet{C2002S5}{C/2002 S5}{C/2002 S5 (SOHO)}
%\DeclareComet{C2002S6}{C/2002 S6}{C/2002 S6 (SOHO)}
%\DeclareComet{C2002S7}{C/2002 S7}{C/2002 S7 (SOHO)}
%\DeclareComet{C2002S8}{C/2002 S8}{C/2002 S8 (SOHO)}
%\DeclareComet{C2002S9}{C/2002 S9}{C/2002 S9 (SOHO)}
%\DeclareComet{C2002T2}{C/2002 T2}{C/2002 T2 (SOHO)}
%\DeclareComet{C2002T3}{C/2002 T3}{C/2002 T3 (SOHO)}
%\DeclareComet{C2002T7}{C/2002 T7}{C/2002 T7 (LINEAR)}
%\DeclareComet{C2002U1}{C/2002 U1}{C/2002 U1 (SOHO)}
%\DeclareComet{C2002U2}{C/2002 U2}{C/2002 U2 (LINEAR)}
%\DeclareComet{C2002U3}{C/2002 U3}{C/2002 U3 (SOHO)}
%\DeclareComet{C2002U4}{C/2002 U4}{C/2002 U4 (SOHO)}
%\DeclareComet{C2002U5}{C/2002 U5}{C/2002 U5 (SOHO)}
%\DeclareComet{C2002U6}{C/2002 U6}{C/2002 U6 (SOHO)}
%\DeclareComet{C2002U7}{C/2002 U7}{C/2002 U7 (SOHO)}
%\DeclareComet{C2002U8}{C/2002 U8}{C/2002 U8 (SOHO)}
%\DeclareComet{C2002U9}{C/2002 U9}{C/2002 U9 (SOHO)}
%\DeclareComet{C2002V1}{C/2002 V1}{C/2002 V1 (NEAT)}
%\DeclareComet{C2002V2}{C/2002 V2}{C/2002 V2 (LINEAR)}
%\DeclareComet{C2002V3}{C/2002 V3}{C/2002 V3 (SOHO)}
%\DeclareComet{C2002V4}{C/2002 V4}{C/2002 V4 (SOHO)}
%\DeclareComet{C2002V5}{C/2002 V5}{C/2002 V5 (SOHO)}
%\DeclareComet{C2002V6}{C/2002 V6}{C/2002 V6 (SOHO)}
%\DeclareComet{C2002V7}{C/2002 V7}{C/2002 V7 (SOHO)}
%\DeclareComet{C2002VQ94}{C/2002 VQ94}{C/2002 VQ94 (LINEAR)}
%\DeclareComet{C2002W1}{C/2002 W1}{C/2002 W1 (SOHO)}
%\DeclareComet{C2002W10}{C/2002 W10}{C/2002 W10 (SOHO)}
%\DeclareComet{C2002W11}{C/2002 W11}{C/2002 W11 (SOHO)}
%\DeclareComet{C2002W12}{C/2002 W12}{C/2002 W12 (SOHO)}
%\DeclareComet{C2002W13}{C/2002 W13}{C/2002 W13 (SOHO)}
%\DeclareComet{C2002W14}{C/2002 W14}{C/2002 W14 (SOHO)}
%\DeclareComet{C2002W15}{C/2002 W15}{C/2002 W15 (SOHO)}
%\DeclareComet{C2002W16}{C/2002 W16}{C/2002 W16 (SOHO)}
%\DeclareComet{C2002W17}{C/2002 W17}{C/2002 W17 (SOHO)}
%\DeclareComet{C2002W2}{C/2002 W2}{C/2002 W2 (SOHO)}
%\DeclareComet{C2002W3}{C/2002 W3}{C/2002 W3 (SOHO)}
%\DeclareComet{C2002W4}{C/2002 W4}{C/2002 W4 (SOHO)}
%\DeclareComet{C2002W5}{C/2002 W5}{C/2002 W5 (SOHO)}
%\DeclareComet{C2002W6}{C/2002 W6}{C/2002 W6 (SOHO)}
%\DeclareComet{C2002W7}{C/2002 W7}{C/2002 W7 (SOHO)}
%\DeclareComet{C2002W8}{C/2002 W8}{C/2002 W8 (SOHO)}
%\DeclareComet{C2002W9}{C/2002 W9}{C/2002 W9 (SOHO)}
%\DeclareComet{C2002X1}{C/2002 X1}{C/2002 X1 (LINEAR)}
%\DeclareComet{C2002X10}{C/2002 X10}{C/2002 X10 (SOHO)}
%\DeclareComet{C2002X11}{C/2002 X11}{C/2002 X11 (SOHO)}
%\DeclareComet{C2002X12}{C/2002 X12}{C/2002 X12 (SOHO)}
%\DeclareComet{C2002X13}{C/2002 X13}{C/2002 X13 (SOHO)}
%\DeclareComet{C2002X14}{C/2002 X14}{C/2002 X14 (SOHO)}
%\DeclareComet{C2002X15}{C/2002 X15}{C/2002 X15 (SOHO)}
%\DeclareComet{C2002X16}{C/2002 X16}{C/2002 X16 (SOHO)}
%\DeclareComet{C2002X3}{C/2002 X3}{C/2002 X3 (SOHO)}
%\DeclareComet{C2002X4}{C/2002 X4}{C/2002 X4 (SOHO)}
%\DeclareComet{C2002X5}{C/2002 X5}{C/2002 X5 (Kudo-Fujikawa)}
%\DeclareComet{C2002X6}{C/2002 X6}{C/2002 X6 (SOHO)}
%\DeclareComet{C2002X7}{C/2002 X7}{C/2002 X7 (SOHO)}
%\DeclareComet{C2002X8}{C/2002 X8}{C/2002 X8 (SOHO)}
%\DeclareComet{C2002X9}{C/2002 X9}{C/2002 X9 (SOHO)}
%\DeclareComet{C2002Y1}{C/2002 Y1}{C/2002 Y1 (Juels-Holvorcem)}
%\DeclareComet{C2002Y2}{C/2002 Y2}{C/2002 Y2 (SOHO)}
%\DeclareComet{C2002Y3}{C/2002 Y3}{C/2002 Y3 (SOHO)}
%\DeclareComet{C2002Y4}{C/2002 Y4}{C/2002 Y4 (SOHO)}
%\DeclareComet{C2003A2}{C/2003 A2}{C/2003 A2 (Gleason)}
%\DeclareComet{C2003A3}{C/2003 A3}{C/2003 A3 (SOHO)}
%\DeclareComet{C2003A4}{C/2003 A4}{C/2003 A4 (SOHO)}
%\DeclareComet{C2003A5}{C/2003 A5}{C/2003 A5 (SOHO)}
%\DeclareComet{C2003B1}{C/2003 B1}{C/2003 B1 (SOHO)}
%\DeclareComet{C2003B2}{C/2003 B2}{C/2003 B2 (SOHO)}
%\DeclareComet{C2003B3}{C/2003 B3}{C/2003 B3 (SOHO)}
%\DeclareComet{C2003C1}{C/2003 C1}{C/2003 C1 (SOHO)}
%\DeclareComet{C2003C2}{C/2003 C2}{C/2003 C2 (SOHO)}
%\DeclareComet{C2003C3}{C/2003 C3}{C/2003 C3 (SOHO)}
%\DeclareComet{C2003C4}{C/2003 C4}{C/2003 C4 (SOHO)}
%\DeclareComet{C2003C5}{C/2003 C5}{C/2003 C5 (SOHO)}
%\DeclareComet{C2003C6}{C/2003 C6}{C/2003 C6 (SOHO)}
%\DeclareComet{C2003D1}{C/2003 D1}{C/2003 D1 (SOHO)}
%\DeclareComet{C2003E1}{C/2003 E1}{C/2003 E1 (NEAT)}
%\DeclareComet{C2003E2}{C/2003 E2}{C/2003 E2 (SOHO)}
%\DeclareComet{C2003E3}{C/2003 E3}{C/2003 E3 (SOHO)}
%\DeclareComet{C2003E4}{C/2003 E4}{C/2003 E4 (SOHO)}
%\DeclareComet{C2003F1}{C/2003 F1}{C/2003 F1 (LINEAR)}
%\DeclareComet{C2003F3}{C/2003 F3}{C/2003 F3 (SOHO)}
%\DeclareComet{C2003F4}{C/2003 F4}{C/2003 F4 (SOHO)}
%\DeclareComet{C2003F5}{C/2003 F5}{C/2003 F5 (SOHO)}
%\DeclareComet{C2003G1}{C/2003 G1}{C/2003 G1 (LINEAR)}
%\DeclareComet{C2003G2}{C/2003 G2}{C/2003 G2 (LINEAR)}
%\DeclareComet{C2003G3}{C/2003 G3}{C/2003 G3 (SOHO)}
%\DeclareComet{C2003G4}{C/2003 G4}{C/2003 G4 (SOHO)}
%\DeclareComet{C2003G5}{C/2003 G5}{C/2003 G5 (SOHO)}
%\DeclareComet{C2003H1}{C/2003 H1}{C/2003 H1 (LINEAR)}
%\DeclareComet{C2003H10}{C/2003 H10}{C/2003 H10 (SOHO)}
%\DeclareComet{C2003H11}{C/2003 H11}{C/2003 H11 (SOHO)}
%\DeclareComet{C2003H12}{C/2003 H12}{C/2003 H12 (SOHO)}
%\DeclareComet{C2003H2}{C/2003 H2}{C/2003 H2 (LINEAR)}
%\DeclareComet{C2003H3}{C/2003 H3}{C/2003 H3 (NEAT)}
%\DeclareComet{C2003H5}{C/2003 H5}{C/2003 H5 (SOHO)}
%\DeclareComet{C2003H6}{C/2003 H6}{C/2003 H6 (SOHO)}
%\DeclareComet{C2003H7}{C/2003 H7}{C/2003 H7 (SOHO)}
%\DeclareComet{C2003H8}{C/2003 H8}{C/2003 H8 (SOHO)}
%\DeclareComet{C2003H9}{C/2003 H9}{C/2003 H9 (SOHO)}
%\DeclareComet{C2003J1}{C/2003 J1}{C/2003 J1 (NEAT)}
%\DeclareComet{C2003J2}{C/2003 J2}{C/2003 J2 (SOHO)}
%\DeclareComet{C2003J3}{C/2003 J3}{C/2003 J3 (SOHO)}
%\DeclareComet{C2003J4}{C/2003 J4}{C/2003 J4 (SOHO)}
%\DeclareComet{C2003J5}{C/2003 J5}{C/2003 J5 (SOHO)}
%\DeclareComet{C2003J6}{C/2003 J6}{C/2003 J6 (SOHO)}
%\DeclareComet{C2003J7}{C/2003 J7}{C/2003 J7 (SOHO)}
%\DeclareComet{C2003J8}{C/2003 J8}{C/2003 J8 (SOHO)}
%\DeclareComet{C2003J9}{C/2003 J9}{C/2003 J9 (SOHO)}
%\DeclareComet{C2003K1}{C/2003 K1}{C/2003 K1 (Spacewatch)}
%\DeclareComet{C2003K10}{C/2003 K10}{C/2003 K10 (SOHO)}
%\DeclareComet{C2003K11}{C/2003 K11}{C/2003 K11 (SOHO)}
%\DeclareComet{C2003K12}{C/2003 K12}{C/2003 K12 (SOHO)}
%\DeclareComet{C2003K13}{C/2003 K13}{C/2003 K13 (SOHO)}
%\DeclareComet{C2003K3}{C/2003 K3}{C/2003 K3 (SOHO)}
%\DeclareComet{C2003K4}{C/2003 K4}{C/2003 K4 (LINEAR)}
%\DeclareComet{C2003K5}{C/2003 K5}{C/2003 K5 (SOHO)}
%\DeclareComet{C2003K6}{C/2003 K6}{C/2003 K6 (SOHO)}
%\DeclareComet{C2003K7}{C/2003 K7}{C/2003 K7 (SOHO)}
%\DeclareComet{C2003K8}{C/2003 K8}{C/2003 K8 (SOHO)}
%\DeclareComet{C2003K9}{C/2003 K9}{C/2003 K9 (SOHO)}
%\DeclareComet{C2003L2}{C/2003 L2}{C/2003 L2 (LINEAR)}
%\DeclareComet{C2003L3}{C/2003 L3}{C/2003 L3 (SOHO)}
%\DeclareComet{C2003L4}{C/2003 L4}{C/2003 L4 (SOHO)}
%\DeclareComet{C2003L5}{C/2003 L5}{C/2003 L5 (SOHO)}
%\DeclareComet{C2003L6}{C/2003 L6}{C/2003 L6 (SOHO)}
%\DeclareComet{C2003L7}{C/2003 L7}{C/2003 L7 (SOHO)}
%\DeclareComet{C2003L8}{C/2003 L8}{C/2003 L8 (SOHO)}
%\DeclareComet{C2003M1}{C/2003 M1}{C/2003 M1 (SOHO)}
%\DeclareComet{C2003M10}{C/2003 M10}{C/2003 M10 (SOHO)}
%\DeclareComet{C2003M11}{C/2003 M11}{C/2003 M11 (SOHO)}
%\DeclareComet{C2003M12}{C/2003 M12}{C/2003 M12 (SOHO)}
%\DeclareComet{C2003M2}{C/2003 M2}{C/2003 M2 (SOHO)}
%\DeclareComet{C2003M3}{C/2003 M3}{C/2003 M3 (SOHO)}
%\DeclareComet{C2003M4}{C/2003 M4}{C/2003 M4 (SOHO)}
%\DeclareComet{C2003M5}{C/2003 M5}{C/2003 M5 (SOHO)}
%\DeclareComet{C2003M6}{C/2003 M6}{C/2003 M6 (SOHO)}
%\DeclareComet{C2003M7}{C/2003 M7}{C/2003 M7 (SOHO)}
%\DeclareComet{C2003M8}{C/2003 M8}{C/2003 M8 (SOHO)}
%\DeclareComet{C2003M9}{C/2003 M9}{C/2003 M9 (SOHO)}
%\DeclareComet{C2003N1}{C/2003 N1}{C/2003 N1 (SOHO)}
%\DeclareComet{C2003N2}{C/2003 N2}{C/2003 N2 (SOHO)}
%\DeclareComet{C2003O1}{C/2003 O1}{C/2003 O1 (LINEAR)}
%\DeclareComet{C2003O4}{C/2003 O4}{C/2003 O4 (SOHO)}
%\DeclareComet{C2003O5}{C/2003 O5}{C/2003 O5 (SOHO)}
%\DeclareComet{C2003O6}{C/2003 O6}{C/2003 O6 (SOHO)}
%\DeclareComet{C2003O7}{C/2003 O7}{C/2003 O7 (SOHO)}
%\DeclareComet{C2003O8}{C/2003 O8}{C/2003 O8 (SOHO)}
%\DeclareComet{C2003P1}{C/2003 P1}{C/2003 P1 (SOHO)}
%\DeclareComet{C2003P2}{C/2003 P2}{C/2003 P2 (SOHO)}
%\DeclareComet{C2003P3}{C/2003 P3}{C/2003 P3 (SOHO)}
%\DeclareComet{C2003Q1}{C/2003 Q1}{C/2003 Q1 (SOHO)}
%\DeclareComet{C2003Q10}{C/2003 Q10}{C/2003 Q10 (SOHO)}
%\DeclareComet{C2003Q2}{C/2003 Q2}{C/2003 Q2 (SOHO)}
%\DeclareComet{C2003Q3}{C/2003 Q3}{C/2003 Q3 (SOHO)}
%\DeclareComet{C2003Q4}{C/2003 Q4}{C/2003 Q4 (SOHO)}
%\DeclareComet{C2003Q5}{C/2003 Q5}{C/2003 Q5 (SOHO)}
%\DeclareComet{C2003Q6}{C/2003 Q6}{C/2003 Q6 (SOHO)}
%\DeclareComet{C2003Q7}{C/2003 Q7}{C/2003 Q7 (SOHO)}
%\DeclareComet{C2003Q8}{C/2003 Q8}{C/2003 Q8 (SOHO)}
%\DeclareComet{C2003Q9}{C/2003 Q9}{C/2003 Q9 (SOHO)}
%\DeclareComet{C2003R1}{C/2003 R1}{C/2003 R1 (LINEAR)}
%\DeclareComet{C2003R2}{C/2003 R2}{C/2003 R2 (SOHO)}
%\DeclareComet{C2003R3}{C/2003 R3}{C/2003 R3 (SOHO)}
%\DeclareComet{C2003R4}{C/2003 R4}{C/2003 R4 (SOHO)}
%\DeclareComet{C2003S3}{C/2003 S3}{C/2003 S3 (LINEAR)}
%\DeclareComet{C2003S4-A}{C/2003 S4-A}{C/2003 S4-A (LINEAR)}
%\DeclareComet{C2003S4-B}{C/2003 S4-B}{C/2003 S4-B (LINEAR)}
%\DeclareComet{C2003S5}{C/2003 S5}{C/2003 S5 (SOHO)}
%\DeclareComet{C2003S6}{C/2003 S6}{C/2003 S6 (SOHO)}
%\DeclareComet{C2003S7}{C/2003 S7}{C/2003 S7 (SOHO)}
%\DeclareComet{C2003S8}{C/2003 S8}{C/2003 S8 (SOHO)}
%\DeclareComet{C2003S9}{C/2003 S9}{C/2003 S9 (SOHO)}
%\DeclareComet{C2003T10}{C/2003 T10}{C/2003 T10 (SOHO)}
%\DeclareComet{C2003T11}{C/2003 T11}{C/2003 T11 (SOHO)}
%\DeclareComet{C2003T2}{C/2003 T2}{C/2003 T2 (LINEAR)}
%\DeclareComet{C2003T3}{C/2003 T3}{C/2003 T3 (Tabur)}
%\DeclareComet{C2003T4}{C/2003 T4}{C/2003 T4 (LINEAR)}
%\DeclareComet{C2003T5}{C/2003 T5}{C/2003 T5 (SOHO)}
%\DeclareComet{C2003T6}{C/2003 T6}{C/2003 T6 (SOHO)}
%\DeclareComet{C2003T7}{C/2003 T7}{C/2003 T7 (SOHO)}
%\DeclareComet{C2003T8}{C/2003 T8}{C/2003 T8 (SOHO)}
%\DeclareComet{C2003T9}{C/2003 T9}{C/2003 T9 (SOHO)}
%\DeclareComet{C2003U1}{C/2003 U1}{C/2003 U1 (LINEAR)}
%\DeclareComet{C2003U4}{C/2003 U4}{C/2003 U4 (SOHO)}
%\DeclareComet{C2003U5}{C/2003 U5}{C/2003 U5 (SOHO)}
%\DeclareComet{C2003U6}{C/2003 U6}{C/2003 U6 (SOHO)}
%\DeclareComet{C2003U7}{C/2003 U7}{C/2003 U7 (SOHO)}
%\DeclareComet{C2003U8}{C/2003 U8}{C/2003 U8 (SOHO)}
%\DeclareComet{C2003U9}{C/2003 U9}{C/2003 U9 (SOHO)}
%\DeclareComet{C2003V1}{C/2003 V1}{C/2003 V1 (LINEAR)}
%\DeclareComet{C2003V2}{C/2003 V2}{C/2003 V2 (SOHO)}
%\DeclareComet{C2003V3}{C/2003 V3}{C/2003 V3 (SOHO)}
%\DeclareComet{C2003V4}{C/2003 V4}{C/2003 V4 (SOHO)}
%\DeclareComet{C2003V5}{C/2003 V5}{C/2003 V5 (SOHO)}
%\DeclareComet{C2003V6}{C/2003 V6}{C/2003 V6 (SOHO)}
%\DeclareComet{C2003V7}{C/2003 V7}{C/2003 V7 (SOHO)}
%\DeclareComet{C2003V8}{C/2003 V8}{C/2003 V8 (SOHO)}
%\DeclareComet{C2003W1}{C/2003 W1}{C/2003 W1 (LINEAR)}
%\DeclareComet{C2003W2}{C/2003 W2}{C/2003 W2 (SOHO)}
%\DeclareComet{C2003W3}{C/2003 W3}{C/2003 W3 (SOHO)}
%\DeclareComet{C2003W4}{C/2003 W4}{C/2003 W4 (SOHO)}
%\DeclareComet{C2003W5}{C/2003 W5}{C/2003 W5 (SOHO)}
%\DeclareComet{C2003W6}{C/2003 W6}{C/2003 W6 (SOHO)}
%\DeclareComet{C2003W7}{C/2003 W7}{C/2003 W7 (SOHO)}
%\DeclareComet{C2003W8}{C/2003 W8}{C/2003 W8 (SOHO)}
%\DeclareComet{C2003WT42}{C/2003 WT42}{C/2003 WT42 (LINEAR)}
%\DeclareComet{C2003X1}{C/2003 X1}{C/2003 X1 (SOHO)}
%\DeclareComet{C2003X10}{C/2003 X10}{C/2003 X10 (SOHO)}
%\DeclareComet{C2003X11}{C/2003 X11}{C/2003 X11 (SOHO)}
%\DeclareComet{C2003X2}{C/2003 X2}{C/2003 X2 (SOHO)}
%\DeclareComet{C2003X3}{C/2003 X3}{C/2003 X3 (SOHO)}
%\DeclareComet{C2003X4}{C/2003 X4}{C/2003 X4 (SOHO)}
%\DeclareComet{C2003X5}{C/2003 X5}{C/2003 X5 (SOHO)}
%\DeclareComet{C2003X6}{C/2003 X6}{C/2003 X6 (SOHO)}
%\DeclareComet{C2003X7}{C/2003 X7}{C/2003 X7 (SOHO)}
%\DeclareComet{C2003X8}{C/2003 X8}{C/2003 X8 (SOHO)}
%\DeclareComet{C2003X9}{C/2003 X9}{C/2003 X9 (SOHO)}
%\DeclareComet{C2003Y1}{C/2003 Y1}{C/2003 Y1 (SOHO)}
%\DeclareComet{C2003Y10}{C/2003 Y10}{C/2003 Y10 (SOHO)}
%\DeclareComet{C2003Y11}{C/2003 Y11}{C/2003 Y11 (SOHO)}
%\DeclareComet{C2003Y12}{C/2003 Y12}{C/2003 Y12 (SOHO)}
%\DeclareComet{C2003Y13}{C/2003 Y13}{C/2003 Y13 (SOHO)}
%\DeclareComet{C2003Y14}{C/2003 Y14}{C/2003 Y14 (SOHO)}
%\DeclareComet{C2003Y15}{C/2003 Y15}{C/2003 Y15 (SOHO)}
%\DeclareComet{C2003Y2}{C/2003 Y2}{C/2003 Y2 (SOHO)}
%\DeclareComet{C2003Y3}{C/2003 Y3}{C/2003 Y3 (SOHO)}
%\DeclareComet{C2003Y4}{C/2003 Y4}{C/2003 Y4 (SOHO)}
%\DeclareComet{C2003Y5}{C/2003 Y5}{C/2003 Y5 (SOHO)}
%\DeclareComet{C2003Y6}{C/2003 Y6}{C/2003 Y6 (SOHO)}
%\DeclareComet{C2003Y7}{C/2003 Y7}{C/2003 Y7 (SOHO)}
%\DeclareComet{C2003Y8}{C/2003 Y8}{C/2003 Y8 (SOHO)}
%\DeclareComet{C2003Y9}{C/2003 Y9}{C/2003 Y9 (SOHO)}
%\DeclareComet{C2004A2}{C/2004 A2}{C/2004 A2 (SOHO)}
%\DeclareComet{C2004A3}{C/2004 A3}{C/2004 A3 (SOHO)}
%\DeclareComet{C2004A4}{C/2004 A4}{C/2004 A4 (SOHO)}
%\DeclareComet{C2004B1}{C/2004 B1}{C/2004 B1 (LINEAR)}
%\DeclareComet{C2004B10}{C/2004 B10}{C/2004 B10 (SOHO)}
%\DeclareComet{C2004B11}{C/2004 B11}{C/2004 B11 (SOHO)}
%\DeclareComet{C2004B2}{C/2004 B2}{C/2004 B2 (SOHO)}
%\DeclareComet{C2004B3}{C/2004 B3}{C/2004 B3 (SOHO)}
%\DeclareComet{C2004B4}{C/2004 B4}{C/2004 B4 (SOHO)}
%\DeclareComet{C2004B5}{C/2004 B5}{C/2004 B5 (SOHO)}
%\DeclareComet{C2004B6}{C/2004 B6}{C/2004 B6 (SOHO)}
%\DeclareComet{C2004B7}{C/2004 B7}{C/2004 B7 (SOHO)}
%\DeclareComet{C2004B8}{C/2004 B8}{C/2004 B8 (SOHO)}
%\DeclareComet{C2004B9}{C/2004 B9}{C/2004 B9 (SOHO)}
%\DeclareComet{C2004C1}{C/2004 C1}{C/2004 C1 (Larsen)}
%\DeclareComet{C2004C2}{C/2004 C2}{C/2004 C2 (SOHO)}
%\DeclareComet{C2004C3}{C/2004 C3}{C/2004 C3 (SOHO)}
%\DeclareComet{C2004C4}{C/2004 C4}{C/2004 C4 (SOHO)}
%\DeclareComet{C2004C5}{C/2004 C5}{C/2004 C5 (SOHO)}
%\DeclareComet{C2004C6}{C/2004 C6}{C/2004 C6 (SOHO)}
%\DeclareComet{C2004C7}{C/2004 C7}{C/2004 C7 (SOHO)}
%\DeclareComet{C2004C8}{C/2004 C8}{C/2004 C8 (SOHO)}
%\DeclareComet{C2004D1}{C/2004 D1}{C/2004 D1 (NEAT)}
%\DeclareComet{C2004D2}{C/2004 D2}{C/2004 D2 (SOHO)}
%\DeclareComet{C2004D3}{C/2004 D3}{C/2004 D3 (SOHO)}
%\DeclareComet{C2004D4}{C/2004 D4}{C/2004 D4 (SOHO)}
%\DeclareComet{C2004DZ61}{C/2004 DZ61}{C/2004 DZ61 (Catalina-LINEAR)}
%\DeclareComet{C2004E1}{C/2004 E1}{C/2004 E1 (SOHO)}
%\DeclareComet{C2004E3}{C/2004 E3}{C/2004 E3 (SOHO)}
%\DeclareComet{C2004E4}{C/2004 E4}{C/2004 E4 (SOHO)}
%\DeclareComet{C2004E5}{C/2004 E5}{C/2004 E5 (SOHO)}
%\DeclareComet{C2004F2}{C/2004 F2}{C/2004 F2 (LINEAR)}
%\DeclareComet{C2004F4}{C/2004 F4}{C/2004 F4 (Bradfield)}
%\DeclareComet{C2004F5}{C/2004 F5}{C/2004 F5 (SOHO)}
%\DeclareComet{C2004F6}{C/2004 F6}{C/2004 F6 (SOHO)}
%\DeclareComet{C2004F7}{C/2004 F7}{C/2004 F7 (SOHO)}
%\DeclareComet{C2004G1}{C/2004 G1}{C/2004 G1 (LINEAR)}
%\DeclareComet{C2004G2}{C/2004 G2}{C/2004 G2 (SOHO)}
%\DeclareComet{C2004G3}{C/2004 G3}{C/2004 G3 (SOHO)}
%\DeclareComet{C2004G4}{C/2004 G4}{C/2004 G4 (SOHO)}
%\DeclareComet{C2004G5}{C/2004 G5}{C/2004 G5 (SOHO)}
%\DeclareComet{C2004G6}{C/2004 G6}{C/2004 G6 (SOHO)}
%\DeclareComet{C2004G7}{C/2004 G7}{C/2004 G7 (SOHO)}
%\DeclareComet{C2004G8}{C/2004 G8}{C/2004 G8 (SOHO)}
%\DeclareComet{C2004G9}{C/2004 G9}{C/2004 G9 (SOHO)}
%\DeclareComet{C2004H1}{C/2004 H1}{C/2004 H1 (LINEAR)}
%\DeclareComet{C2004H10}{C/2004 H10}{C/2004 H10 (SOHO)}
%\DeclareComet{C2004H4}{C/2004 H4}{C/2004 H4 (SOHO)}
%\DeclareComet{C2004H5}{C/2004 H5}{C/2004 H5 (SOHO)}
%\DeclareComet{C2004H6}{C/2004 H6}{C/2004 H6 (SWAN)}
%\DeclareComet{C2004H7}{C/2004 H7}{C/2004 H7 (SOHO)}
%\DeclareComet{C2004H8}{C/2004 H8}{C/2004 H8 (SOHO)}
%\DeclareComet{C2004H9}{C/2004 H9}{C/2004 H9 (SOHO)}
%\DeclareComet{C2004HV60}{C/2004 HV60}{C/2004 HV60 (Spacewatch)}
%\DeclareComet{C2004J1}{C/2004 J1}{C/2004 J1 (SOHO)}
%\DeclareComet{C2004J10}{C/2004 J10}{C/2004 J10 (SOHO)}
%\DeclareComet{C2004J11}{C/2004 J11}{C/2004 J11 (SOHO)}
%\DeclareComet{C2004J12}{C/2004 J12}{C/2004 J12 (SOHO)}
%\DeclareComet{C2004J13}{C/2004 J13}{C/2004 J13 (SOHO)}
%\DeclareComet{C2004J14}{C/2004 J14}{C/2004 J14 (SOHO)}
%\DeclareComet{C2004J15}{C/2004 J15}{C/2004 J15 (SOHO)}
%\DeclareComet{C2004J16}{C/2004 J16}{C/2004 J16 (SOHO)}
%\DeclareComet{C2004J17}{C/2004 J17}{C/2004 J17 (SOHO)}
%\DeclareComet{C2004J18}{C/2004 J18}{C/2004 J18 (SOHO)}
%\DeclareComet{C2004J19}{C/2004 J19}{C/2004 J19 (SOHO)}
%\DeclareComet{C2004J2}{C/2004 J2}{C/2004 J2 (SOHO)}
%\DeclareComet{C2004J20}{C/2004 J20}{C/2004 J20 (SOHO)}
%\DeclareComet{C2004J3}{C/2004 J3}{C/2004 J3 (SOHO)}
%\DeclareComet{C2004J4}{C/2004 J4}{C/2004 J4 (SOHO)}
%\DeclareComet{C2004J5}{C/2004 J5}{C/2004 J5 (SOHO)}
%\DeclareComet{C2004J6}{C/2004 J6}{C/2004 J6 (SOHO)}
%\DeclareComet{C2004J7}{C/2004 J7}{C/2004 J7 (SOHO)}
%\DeclareComet{C2004J8}{C/2004 J8}{C/2004 J8 (SOHO)}
%\DeclareComet{C2004J9}{C/2004 J9}{C/2004 J9 (SOHO)}
%\DeclareComet{C2004K1}{C/2004 K1}{C/2004 K1 (Catalina)}
%\DeclareComet{C2004K10}{C/2004 K10}{C/2004 K10 (SOHO)}
%\DeclareComet{C2004K11}{C/2004 K11}{C/2004 K11 (SOHO)}
%\DeclareComet{C2004K12}{C/2004 K12}{C/2004 K12 (SOHO)}
%\DeclareComet{C2004K3}{C/2004 K3}{C/2004 K3 (LINEAR)}
%\DeclareComet{C2004K4}{C/2004 K4}{C/2004 K4 (SOHO)}
%\DeclareComet{C2004K5}{C/2004 K5}{C/2004 K5 (SOHO)}
%\DeclareComet{C2004K6}{C/2004 K6}{C/2004 K6 (SOHO)}
%\DeclareComet{C2004K7}{C/2004 K7}{C/2004 K7 (SOHO)}
%\DeclareComet{C2004K8}{C/2004 K8}{C/2004 K8 (SOHO)}
%\DeclareComet{C2004K9}{C/2004 K9}{C/2004 K9 (SOHO)}
%\DeclareComet{C2004L1}{C/2004 L1}{C/2004 L1 (LINEAR)}
%\DeclareComet{C2004L10}{C/2004 L10}{C/2004 L10 (SOHO)}
%\DeclareComet{C2004L11}{C/2004 L11}{C/2004 L11 (SOHO)}
%\DeclareComet{C2004L2}{C/2004 L2}{C/2004 L2 (LINEAR)}
%\DeclareComet{C2004L3}{C/2004 L3}{C/2004 L3 (SOHO)}
%\DeclareComet{C2004L4}{C/2004 L4}{C/2004 L4 (SOHO)}
%\DeclareComet{C2004L5}{C/2004 L5}{C/2004 L5 (SOHO)}
%\DeclareComet{C2004L6}{C/2004 L6}{C/2004 L6 (SOHO)}
%\DeclareComet{C2004L7}{C/2004 L7}{C/2004 L7 (SOHO)}
%\DeclareComet{C2004L8}{C/2004 L8}{C/2004 L8 (SOHO)}
%\DeclareComet{C2004L9}{C/2004 L9}{C/2004 L9 (SOHO)}
%\DeclareComet{C2004M1}{C/2004 M1}{C/2004 M1 (SOHO)}
%\DeclareComet{C2004M2}{C/2004 M2}{C/2004 M2 (SOHO)}
%\DeclareComet{C2004M3}{C/2004 M3}{C/2004 M3 (SOHO)}
%\DeclareComet{C2004M4}{C/2004 M4}{C/2004 M4 (SOHO)}
%\DeclareComet{C2004M5}{C/2004 M5}{C/2004 M5 (SOHO)}
%\DeclareComet{C2004M6}{C/2004 M6}{C/2004 M6 (SOHO)}
%\DeclareComet{C2004M7}{C/2004 M7}{C/2004 M7 (SOHO)}
%\DeclareComet{C2004N1}{C/2004 N1}{C/2004 N1 (SOHO)}
%\DeclareComet{C2004N2}{C/2004 N2}{C/2004 N2 (SOHO)}
%\DeclareComet{C2004N3}{C/2004 N3}{C/2004 N3 (SOHO)}
%\DeclareComet{C2004N4}{C/2004 N4}{C/2004 N4 (SOHO)}
%\DeclareComet{C2004N5}{C/2004 N5}{C/2004 N5 (SOHO)}
%\DeclareComet{C2004N6}{C/2004 N6}{C/2004 N6 (SOHO)}
%\DeclareComet{C2004O1}{C/2004 O1}{C/2004 O1 (SOHO)}
%\DeclareComet{C2004O2}{C/2004 O2}{C/2004 O2 (SOHO)}
%\DeclareComet{C2004O3}{C/2004 O3}{C/2004 O3 (SOHO)}
%\DeclareComet{C2004P1}{C/2004 P1}{C/2004 P1 (NEAT)}
%\DeclareComet{C2004P2}{C/2004 P2}{C/2004 P2 (SOHO)}
%\DeclareComet{C2004P3}{C/2004 P3}{C/2004 P3 (SOHO)}
%\DeclareComet{C2004P4}{C/2004 P4}{C/2004 P4 (SOHO)}
%\DeclareComet{C2004P5}{C/2004 P5}{C/2004 P5 (SOHO)}
%\DeclareComet{C2004P6}{C/2004 P6}{C/2004 P6 (SOHO)}
%\DeclareComet{C2004P7}{C/2004 P7}{C/2004 P7 (SOHO)}
%\DeclareComet{C2004Q1}{C/2004 Q1}{C/2004 Q1 (Tucker)}
%\DeclareComet{C2004Q2}{C/2004 Q2}{C/2004 Q2 (Machholz)}
%\DeclareComet{C2004Q3}{C/2004 Q3}{C/2004 Q3 (SOHO)}
%\DeclareComet{C2004Q4}{C/2004 Q4}{C/2004 Q4 (SOHO)}
%\DeclareComet{C2004Q5}{C/2004 Q5}{C/2004 Q5 (SOHO)}
%\DeclareComet{C2004Q6}{C/2004 Q6}{C/2004 Q6 (SOHO)}
%\DeclareComet{C2004R2}{C/2004 R2}{C/2004 R2 (ASAS)}
%\DeclareComet{C2004R4}{C/2004 R4}{C/2004 R4 (SOHO)}
%\DeclareComet{C2004R5}{C/2004 R5}{C/2004 R5 (SOHO)}
%\DeclareComet{C2004R6}{C/2004 R6}{C/2004 R6 (SOHO)}
%\DeclareComet{C2004R7}{C/2004 R7}{C/2004 R7 (SOHO)}
%\DeclareComet{C2004RG113}{C/2004 RG113}{C/2004 RG113 (LINEAR)}
%\DeclareComet{C2004S1}{C/2004 S1}{C/2004 S1 (Van Ness)}
%\DeclareComet{C2004S2}{C/2004 S2}{C/2004 S2 (SOHO)}
%\DeclareComet{C2004S3}{C/2004 S3}{C/2004 S3 (SOHO)}
%\DeclareComet{C2004S4}{C/2004 S4}{C/2004 S4 (SOHO)}
%\DeclareComet{C2004T2}{C/2004 T2}{C/2004 T2 (SOHO)}
%\DeclareComet{C2004T3}{C/2004 T3}{C/2004 T3 (SidingSpring)}
%\DeclareComet{C2004T4}{C/2004 T4}{C/2004 T4 (SOHO)}
%\DeclareComet{C2004T5}{C/2004 T5}{C/2004 T5 (SOHO)}
%\DeclareComet{C2004T6}{C/2004 T6}{C/2004 T6 (SOHO)}
%\DeclareComet{C2004T7}{C/2004 T7}{C/2004 T7 (SOHO)}
%\DeclareComet{C2004T8}{C/2004 T8}{C/2004 T8 (SOHO)}
%\DeclareComet{C2004U1}{C/2004 U1}{C/2004 U1 (LINEAR)}
%\DeclareComet{C2004U10}{C/2004 U10}{C/2004 U10 (SOHO)}
%\DeclareComet{C2004U11}{C/2004 U11}{C/2004 U11 (SOHO)}
%\DeclareComet{C2004U12}{C/2004 U12}{C/2004 U12 (SOHO)}
%\DeclareComet{C2004U2}{C/2004 U2}{C/2004 U2 (SOHO)}
%\DeclareComet{C2004U3}{C/2004 U3}{C/2004 U3 (SOHO)}
%\DeclareComet{C2004U4}{C/2004 U4}{C/2004 U4 (SOHO)}
%\DeclareComet{C2004U5}{C/2004 U5}{C/2004 U5 (SOHO)}
%\DeclareComet{C2004U6}{C/2004 U6}{C/2004 U6 (SOHO)}
%\DeclareComet{C2004U7}{C/2004 U7}{C/2004 U7 (SOHO)}
%\DeclareComet{C2004U8}{C/2004 U8}{C/2004 U8 (SOHO)}
%\DeclareComet{C2004U9}{C/2004 U9}{C/2004 U9 (SOHO)}
%\DeclareComet{C2004V10}{C/2004 V10}{C/2004 V10 (SOHO)}
%\DeclareComet{C2004V11}{C/2004 V11}{C/2004 V11 (SOHO)}
%\DeclareComet{C2004V12}{C/2004 V12}{C/2004 V12 (SOHO)}
%\DeclareComet{C2004V13}{C/2004 V13}{C/2004 V13 (SWAN)}
%\DeclareComet{C2004V14}{C/2004 V14}{C/2004 V14 (SOHO)}
%\DeclareComet{C2004V15}{C/2004 V15}{C/2004 V15 (SOHO)}
%\DeclareComet{C2004V6}{C/2004 V6}{C/2004 V6 (SOHO)}
%\DeclareComet{C2004V7}{C/2004 V7}{C/2004 V7 (SOHO)}
%\DeclareComet{C2004V8}{C/2004 V8}{C/2004 V8 (SOHO)}
%\DeclareComet{C2004W1}{C/2004 W1}{C/2004 W1 (SOHO)}
%\DeclareComet{C2004W10}{C/2004 W10}{C/2004 W10 (SOHO)}
%\DeclareComet{C2004W11}{C/2004 W11}{C/2004 W11 (SOHO)}
%\DeclareComet{C2004W2}{C/2004 W2}{C/2004 W2 (SOHO)}
%\DeclareComet{C2004W3}{C/2004 W3}{C/2004 W3 (SOHO)}
%\DeclareComet{C2004W4}{C/2004 W4}{C/2004 W4 (SOHO)}
%\DeclareComet{C2004W5}{C/2004 W5}{C/2004 W5 (SOHO)}
%\DeclareComet{C2004W6}{C/2004 W6}{C/2004 W6 (SOHO)}
%\DeclareComet{C2004W7}{C/2004 W7}{C/2004 W7 (SOHO)}
%\DeclareComet{C2004W8}{C/2004 W8}{C/2004 W8 (SOHO)}
%\DeclareComet{C2004W9}{C/2004 W9}{C/2004 W9 (SOHO)}
%\DeclareComet{C2004X10}{C/2004 X10}{C/2004 X10 (SOHO)}
%\DeclareComet{C2004X11}{C/2004 X11}{C/2004 X11 (SOHO)}
%\DeclareComet{C2004X2}{C/2004 X2}{C/2004 X2 (LINEAR)}
%\DeclareComet{C2004X3}{C/2004 X3}{C/2004 X3 (LINEAR)}
%\DeclareComet{C2004X4}{C/2004 X4}{C/2004 X4 (SOHO)}
%\DeclareComet{C2004X5}{C/2004 X5}{C/2004 X5 (SOHO)}
%\DeclareComet{C2004X6}{C/2004 X6}{C/2004 X6 (SOHO)}
%\DeclareComet{C2004X8}{C/2004 X8}{C/2004 X8 (SOHO)}
%\DeclareComet{C2004X9}{C/2004 X9}{C/2004 X9 (SOHO)}
%\DeclareComet{C2004Y10}{C/2004 Y10}{C/2004 Y10 (SOHO)}
%\DeclareComet{C2004Y11}{C/2004 Y11}{C/2004 Y11 (SOHO)}
%\DeclareComet{C2004Y12}{C/2004 Y12}{C/2004 Y12 (SOHO)}
%\DeclareComet{C2004Y2}{C/2004 Y2}{C/2004 Y2 (SOHO)}
%\DeclareComet{C2004Y3}{C/2004 Y3}{C/2004 Y3 (SOHO)}
%\DeclareComet{C2004Y4}{C/2004 Y4}{C/2004 Y4 (SOHO)}
%\DeclareComet{C2004Y5}{C/2004 Y5}{C/2004 Y5 (SOHO)}
%\DeclareComet{C2004Y6}{C/2004 Y6}{C/2004 Y6 (SOHO)}
%\DeclareComet{C2004Y7}{C/2004 Y7}{C/2004 Y7 (SOHO)}
%\DeclareComet{C2004Y8}{C/2004 Y8}{C/2004 Y8 (SOHO)}
%\DeclareComet{C2004Y9}{C/2004 Y9}{C/2004 Y9 (SOHO)}
%\DeclareComet{C2004YJ35}{C/2004 YJ35}{C/2004 YJ35 (LINEAR)}
%\DeclareComet{C2005A1-A}{C/2005 A1-A}{C/2005 A1-A (LINEAR)}
%\DeclareComet{C2005A2}{C/2005 A2}{C/2005 A2 (SOHO)}
%\DeclareComet{C2005A3}{C/2005 A3}{C/2005 A3 (SOHO)}
%\DeclareComet{C2005A4}{C/2005 A4}{C/2005 A4 (SOHO)}
%\DeclareComet{C2005A5}{C/2005 A5}{C/2005 A5 (SOHO)}
%\DeclareComet{C2005B1}{C/2005 B1}{C/2005 B1 (Christensen)}
%\DeclareComet{C2005B2}{C/2005 B2}{C/2005 B2 (SOHO)}
%\DeclareComet{C2005B3}{C/2005 B3}{C/2005 B3 (SOHO)}
%\DeclareComet{C2005B4}{C/2005 B4}{C/2005 B4 (SOHO)}
%\DeclareComet{C2005B5}{C/2005 B5}{C/2005 B5 (SOHO)}
%\DeclareComet{C2005B6}{C/2005 B6}{C/2005 B6 (SOHO)}
%\DeclareComet{C2005C1}{C/2005 C1}{C/2005 C1 (SOHO)}
%\DeclareComet{C2005C2}{C/2005 C2}{C/2005 C2 (SOHO)}
%\DeclareComet{C2005C3}{C/2005 C3}{C/2005 C3 (SOHO)}
%\DeclareComet{C2005C4}{C/2005 C4}{C/2005 C4 (SOHO)}
%\DeclareComet{C2005D1}{C/2005 D1}{C/2005 D1 (SOHO)}
%\DeclareComet{C2005D2}{C/2005 D2}{C/2005 D2 (SOHO)}
%\DeclareComet{C2005D3}{C/2005 D3}{C/2005 D3 (SOHO)}
%\DeclareComet{C2005D4}{C/2005 D4}{C/2005 D4 (SOHO)}
%\DeclareComet{C2005D5}{C/2005 D5}{C/2005 D5 (SOHO)}
%\DeclareComet{C2005E2}{C/2005 E2}{C/2005 E2 (McNaught)}
%\DeclareComet{C2005E3}{C/2005 E3}{C/2005 E3 (SOHO)}
%\DeclareComet{C2005E4}{C/2005 E4}{C/2005 E4 (SOHO)}
%\DeclareComet{C2005E5}{C/2005 E5}{C/2005 E5 (SOHO)}
%\DeclareComet{C2005E6}{C/2005 E6}{C/2005 E6 (SOHO)}
%\DeclareComet{C2005E7}{C/2005 E7}{C/2005 E7 (SOHO)}
%\DeclareComet{C2005E8}{C/2005 E8}{C/2005 E8 (SOHO)}
%\DeclareComet{C2005E9}{C/2005 E9}{C/2005 E9 (SOHO)}
%\DeclareComet{C2005EL173}{C/2005 EL173}{C/2005 EL173 (LONEOS)}
%\DeclareComet{C2005F1}{C/2005 F1}{C/2005 F1 (SOHO)}
%\DeclareComet{C2005F2}{C/2005 F2}{C/2005 F2 (SOHO)}
%\DeclareComet{C2005F3}{C/2005 F3}{C/2005 F3 (SOHO)}
%\DeclareComet{C2005F4}{C/2005 F4}{C/2005 F4 (SOHO)}
%\DeclareComet{C2005F5}{C/2005 F5}{C/2005 F5 (SOHO)}
%\DeclareComet{C2005G1}{C/2005 G1}{C/2005 G1 (LINEAR)}
%\DeclareComet{C2005G2}{C/2005 G2}{C/2005 G2 (SOHO)}
%\DeclareComet{C2005G3}{C/2005 G3}{C/2005 G3 (SOHO)}
%\DeclareComet{C2005G4}{C/2005 G4}{C/2005 G4 (SOHO)}
%\DeclareComet{C2005G5}{C/2005 G5}{C/2005 G5 (SOHO)}
%\DeclareComet{C2005G6}{C/2005 G6}{C/2005 G6 (SOHO)}
%\DeclareComet{C2005G7}{C/2005 G7}{C/2005 G7 (SOHO)}
%\DeclareComet{C2005H1}{C/2005 H1}{C/2005 H1 (LINEAR)}
%\DeclareComet{C2005H2}{C/2005 H2}{C/2005 H2 (SOHO)}
%\DeclareComet{C2005H3}{C/2005 H3}{C/2005 H3 (SOHO)}
%\DeclareComet{C2005H4}{C/2005 H4}{C/2005 H4 (SOHO)}
%\DeclareComet{C2005H5}{C/2005 H5}{C/2005 H5 (SOHO)}
%\DeclareComet{C2005H6}{C/2005 H6}{C/2005 H6 (SOHO)}
%\DeclareComet{C2005H7}{C/2005 H7}{C/2005 H7 (SOHO)}
%\DeclareComet{C2005H8}{C/2005 H8}{C/2005 H8 (SOHO)}
%\DeclareComet{C2005H9}{C/2005 H9}{C/2005 H9 (SOHO)}
%\DeclareComet{C2005J10}{C/2005 J10}{C/2005 J10 (SOHO)}
%\DeclareComet{C2005J11}{C/2005 J11}{C/2005 J11 (SOHO)}
%\DeclareComet{C2005J12}{C/2005 J12}{C/2005 J12 (SOHO)}
%\DeclareComet{C2005J2}{C/2005 J2}{C/2005 J2 (Catalina)}
%\DeclareComet{C2005J3}{C/2005 J3}{C/2005 J3 (SOHO)}
%\DeclareComet{C2005J4}{C/2005 J4}{C/2005 J4 (SOHO)}
%\DeclareComet{C2005J5}{C/2005 J5}{C/2005 J5 (SOHO)}
%\DeclareComet{C2005J6}{C/2005 J6}{C/2005 J6 (SOHO)}
%\DeclareComet{C2005J7}{C/2005 J7}{C/2005 J7 (SOHO)}
%\DeclareComet{C2005J8}{C/2005 J8}{C/2005 J8 (SOHO)}
%\DeclareComet{C2005J9}{C/2005 J9}{C/2005 J9 (SOHO)}
%\DeclareComet{C2005K1}{C/2005 K1}{C/2005 K1 (Skiff)}
%\DeclareComet{C2005K10}{C/2005 K10}{C/2005 K10 (SOHO)}
%\DeclareComet{C2005K2-A}{C/2005 K2-A}{C/2005 K2-A (LINEAR)}
%\DeclareComet{C2005K4}{C/2005 K4}{C/2005 K4 (SOHO)}
%\DeclareComet{C2005K5}{C/2005 K5}{C/2005 K5 (SOHO)}
%\DeclareComet{C2005K6}{C/2005 K6}{C/2005 K6 (SOHO)}
%\DeclareComet{C2005K7}{C/2005 K7}{C/2005 K7 (SOHO)}
%\DeclareComet{C2005K8}{C/2005 K8}{C/2005 K8 (SOHO)}
%\DeclareComet{C2005K9}{C/2005 K9}{C/2005 K9 (SOHO)}
%\DeclareComet{C2005L10}{C/2005 L10}{C/2005 L10 (SOHO)}
%\DeclareComet{C2005L11}{C/2005 L11}{C/2005 L11 (SOHO)}
%\DeclareComet{C2005L12}{C/2005 L12}{C/2005 L12 (SOHO)}
%\DeclareComet{C2005L13}{C/2005 L13}{C/2005 L13 (SOHO)}
%\DeclareComet{C2005L14}{C/2005 L14}{C/2005 L14 (SOHO)}
%\DeclareComet{C2005L15}{C/2005 L15}{C/2005 L15 (SOHO)}
%\DeclareComet{C2005L2}{C/2005 L2}{C/2005 L2 (McNaught)}
%\DeclareComet{C2005L3}{C/2005 L3}{C/2005 L3 (McNaught)}
%\DeclareComet{C2005L5}{C/2005 L5}{C/2005 L5 (SOHO)}
%\DeclareComet{C2005L6}{C/2005 L6}{C/2005 L6 (SOHO)}
%\DeclareComet{C2005L7}{C/2005 L7}{C/2005 L7 (SOHO)}
%\DeclareComet{C2005L8}{C/2005 L8}{C/2005 L8 (SOHO)}
%\DeclareComet{C2005L9}{C/2005 L9}{C/2005 L9 (SOHO)}
%\DeclareComet{C2005M10}{C/2005 M10}{C/2005 M10 (SOHO)}
%\DeclareComet{C2005M2}{C/2005 M2}{C/2005 M2 (SOHO)}
%\DeclareComet{C2005M3}{C/2005 M3}{C/2005 M3 (SOHO)}
%\DeclareComet{C2005M4}{C/2005 M4}{C/2005 M4 (SOHO)}
%\DeclareComet{C2005M5}{C/2005 M5}{C/2005 M5 (SOHO)}
%\DeclareComet{C2005M6}{C/2005 M6}{C/2005 M6 (SOHO)}
%\DeclareComet{C2005M7}{C/2005 M7}{C/2005 M7 (SOHO)}
%\DeclareComet{C2005M8}{C/2005 M8}{C/2005 M8 (SOHO)}
%\DeclareComet{C2005M9}{C/2005 M9}{C/2005 M9 (SOHO)}
%\DeclareComet{C2005N1}{C/2005 N1}{C/2005 N1 (Juels-Holvorcem)}
%\DeclareComet{C2005N10}{C/2005 N10}{C/2005 N10 (SOHO)}
%\DeclareComet{C2005N4}{C/2005 N4}{C/2005 N4 (Catalina)}
%\DeclareComet{C2005N5}{C/2005 N5}{C/2005 N5 (Catalina)}
%\DeclareComet{C2005N6}{C/2005 N6}{C/2005 N6 (SOHO)}
%\DeclareComet{C2005N7}{C/2005 N7}{C/2005 N7 (SOHO)}
%\DeclareComet{C2005N8}{C/2005 N8}{C/2005 N8 (SOHO)}
%\DeclareComet{C2005N9}{C/2005 N9}{C/2005 N9 (SOHO)}
%\DeclareComet{C2005O1}{C/2005 O1}{C/2005 O1 (NEAT)}
%\DeclareComet{C2005O2}{C/2005 O2}{C/2005 O2 (Christensen)}
%\DeclareComet{C2005O3}{C/2005 O3}{C/2005 O3 (SOHO)}
%\DeclareComet{C2005O4}{C/2005 O4}{C/2005 O4 (SOHO)}
%\DeclareComet{C2005O5}{C/2005 O5}{C/2005 O5 (SOHO)}
%\DeclareComet{C2005O6}{C/2005 O6}{C/2005 O6 (SOHO)}
%\DeclareComet{C2005P1}{C/2005 P1}{C/2005 P1 (SOHO)}
%\DeclareComet{C2005P2}{C/2005 P2}{C/2005 P2 (SOHO)}
%\DeclareComet{C2005P3}{C/2005 P3}{C/2005 P3 (SWAN)}
%\DeclareComet{C2005P4}{C/2005 P4}{C/2005 P4 (SOHO)}
%\DeclareComet{C2005P5}{C/2005 P5}{C/2005 P5 (SOHO)}
%\DeclareComet{C2005P6}{C/2005 P6}{C/2005 P6 (SOHO)}
%\DeclareComet{C2005Q1}{C/2005 Q1}{C/2005 Q1 (LINEAR)}
%\DeclareComet{C2005Q10}{C/2005 Q10}{C/2005 Q10 (SOHO)}
%\DeclareComet{C2005Q2}{C/2005 Q2}{C/2005 Q2 (SOHO)}
%\DeclareComet{C2005Q3}{C/2005 Q3}{C/2005 Q3 (SOHO)}
%\DeclareComet{C2005Q5}{C/2005 Q5}{C/2005 Q5 (SOHO)}
%\DeclareComet{C2005Q6}{C/2005 Q6}{C/2005 Q6 (SOHO)}
%\DeclareComet{C2005Q7}{C/2005 Q7}{C/2005 Q7 (SOHO)}
%\DeclareComet{C2005Q8}{C/2005 Q8}{C/2005 Q8 (SOHO)}
%\DeclareComet{C2005Q9}{C/2005 Q9}{C/2005 Q9 (SOHO)}
%\DeclareComet{C2005R4}{C/2005 R4}{C/2005 R4 (LINEAR)}
%\DeclareComet{C2005R5}{C/2005 R5}{C/2005 R5 (SOHO)}
%\DeclareComet{C2005R6}{C/2005 R6}{C/2005 R6 (SOHO)}
%\DeclareComet{C2005R7}{C/2005 R7}{C/2005 R7 (SOHO)}
%\DeclareComet{C2005S1}{C/2005 S1}{C/2005 S1 (SOHO)}
%\DeclareComet{C2005S10}{C/2005 S10}{C/2005 S10 (SOHO)}
%\DeclareComet{C2005S11}{C/2005 S11}{C/2005 S11 (SOHO)}
%\DeclareComet{C2005S12}{C/2005 S12}{C/2005 S12 (SOHO)}
%\DeclareComet{C2005S13}{C/2005 S13}{C/2005 S13 (SOHO)}
%\DeclareComet{C2005S4}{C/2005 S4}{C/2005 S4 (McNaught)}
%\DeclareComet{C2005S5}{C/2005 S5}{C/2005 S5 (SOHO)}
%\DeclareComet{C2005S6}{C/2005 S6}{C/2005 S6 (SOHO)}
%\DeclareComet{C2005S7}{C/2005 S7}{C/2005 S7 (SOHO)}
%\DeclareComet{C2005S8}{C/2005 S8}{C/2005 S8 (SOHO)}
%\DeclareComet{C2005S9}{C/2005 S9}{C/2005 S9 (SOHO)}
%\DeclareComet{C2005T10}{C/2005 T10}{C/2005 T10 (SOHO)}
%\DeclareComet{C2005T11}{C/2005 T11}{C/2005 T11 (SOHO)}
%\DeclareComet{C2005T6}{C/2005 T6}{C/2005 T6 (SOHO)}
%\DeclareComet{C2005T7}{C/2005 T7}{C/2005 T7 (SOHO)}
%\DeclareComet{C2005T8}{C/2005 T8}{C/2005 T8 (SOHO)}
%\DeclareComet{C2005T9}{C/2005 T9}{C/2005 T9 (SOHO)}
%\DeclareComet{C2005U2}{C/2005 U2}{C/2005 U2 (SOHO)}
%\DeclareComet{C2005U3}{C/2005 U3}{C/2005 U3 (SOHO)}
%\DeclareComet{C2005U4}{C/2005 U4}{C/2005 U4 (SOHO)}
%\DeclareComet{C2005U5}{C/2005 U5}{C/2005 U5 (SOHO)}
%\DeclareComet{C2005U6}{C/2005 U6}{C/2005 U6 (SOHO)}
%\DeclareComet{C2005U7}{C/2005 U7}{C/2005 U7 (SOHO)}
%\DeclareComet{C2005U8}{C/2005 U8}{C/2005 U8 (SOHO)}
%\DeclareComet{C2005V2}{C/2005 V2}{C/2005 V2 (SOHO)}
%\DeclareComet{C2005V3}{C/2005 V3}{C/2005 V3 (SOHO)}
%\DeclareComet{C2005V4}{C/2005 V4}{C/2005 V4 (SOHO)}
%\DeclareComet{C2005V5}{C/2005 V5}{C/2005 V5 (SOHO)}
%\DeclareComet{C2005V6}{C/2005 V6}{C/2005 V6 (SOHO)}
%\DeclareComet{C2005V7}{C/2005 V7}{C/2005 V7 (SOHO)}
%\DeclareComet{C2005V8}{C/2005 V8}{C/2005 V8 (SOHO)}
%\DeclareComet{C2005V9}{C/2005 V9}{C/2005 V9 (SOHO)}
%\DeclareComet{C2005W1}{C/2005 W1}{C/2005 W1 (SOHO)}
%\DeclareComet{C2005W10}{C/2005 W10}{C/2005 W10 (SOHO)}
%\DeclareComet{C2005W11}{C/2005 W11}{C/2005 W11 (SOHO)}
%\DeclareComet{C2005W12}{C/2005 W12}{C/2005 W12 (SOHO)}
%\DeclareComet{C2005W13}{C/2005 W13}{C/2005 W13 (SOHO)}
%\DeclareComet{C2005W14}{C/2005 W14}{C/2005 W14 (SOHO)}
%\DeclareComet{C2005W15}{C/2005 W15}{C/2005 W15 (SOHO)}
%\DeclareComet{C2005W16}{C/2005 W16}{C/2005 W16 (SOHO)}
%\DeclareComet{C2005W17}{C/2005 W17}{C/2005 W17 (SOHO)}
%\DeclareComet{C2005W2}{C/2005 W2}{C/2005 W2 (Christensen)}
%\DeclareComet{C2005W5}{C/2005 W5}{C/2005 W5 (SOHO)}
%\DeclareComet{C2005W6}{C/2005 W6}{C/2005 W6 (SOHO)}
%\DeclareComet{C2005W7}{C/2005 W7}{C/2005 W7 (SOHO)}
%\DeclareComet{C2005W8}{C/2005 W8}{C/2005 W8 (SOHO)}
%\DeclareComet{C2005W9}{C/2005 W9}{C/2005 W9 (SOHO)}
%\DeclareComet{C2005X1}{C/2005 X1}{C/2005 X1 (Beshore)}
%\DeclareComet{C2005X2}{C/2005 X2}{C/2005 X2 (SOHO)}
%\DeclareComet{C2005X3}{C/2005 X3}{C/2005 X3 (SOHO)}
%\DeclareComet{C2005X4}{C/2005 X4}{C/2005 X4 (SOHO)}
%\DeclareComet{C2005X5}{C/2005 X5}{C/2005 X5 (SOHO)}
%\DeclareComet{C2005X6}{C/2005 X6}{C/2005 X6 (SOHO)}
%\DeclareComet{C2005X7}{C/2005 X7}{C/2005 X7 (SOHO)}
%\DeclareComet{C2005X8}{C/2005 X8}{C/2005 X8 (SOHO)}
%\DeclareComet{C2005X9}{C/2005 X9}{C/2005 X9 (SOHO)}
%\DeclareComet{C2005Y1}{C/2005 Y1}{C/2005 Y1 (SOHO)}
%\DeclareComet{C2005Y10}{C/2005 Y10}{C/2005 Y10 (SOHO)}
%\DeclareComet{C2005Y3}{C/2005 Y3}{C/2005 Y3 (SOHO)}
%\DeclareComet{C2005Y4}{C/2005 Y4}{C/2005 Y4 (SOHO)}
%\DeclareComet{C2005Y5}{C/2005 Y5}{C/2005 Y5 (SOHO)}
%\DeclareComet{C2005Y6}{C/2005 Y6}{C/2005 Y6 (SOHO)}
%\DeclareComet{C2005Y7}{C/2005 Y7}{C/2005 Y7 (SOHO)}
%\DeclareComet{C2005Y8}{C/2005 Y8}{C/2005 Y8 (SOHO)}
%\DeclareComet{C2005Y9}{C/2005 Y9}{C/2005 Y9 (SOHO)}
%\DeclareComet{C2005YW}{C/2005 YW}{C/2005 YW (LINEAR)}
%\DeclareComet{C2006A1}{C/2006 A1}{C/2006 A1 (Pojmanski)}
%\DeclareComet{C2006A2}{C/2006 A2}{C/2006 A2 (Catalina)}
%\DeclareComet{C2006A4}{C/2006 A4}{C/2006 A4 (SOHO)}
%\DeclareComet{C2006A5}{C/2006 A5}{C/2006 A5 (SOHO)}
%\DeclareComet{C2006A6}{C/2006 A6}{C/2006 A6 (SOHO)}
%\DeclareComet{C2006A7}{C/2006 A7}{C/2006 A7 (SOHO)}
%\DeclareComet{C2006A8}{C/2006 A8}{C/2006 A8 (SOHO)}
%\DeclareComet{C2006B1}{C/2006 B1}{C/2006 B1 (McNaught)}
%\DeclareComet{C2006B2}{C/2006 B2}{C/2006 B2 (SOHO)}
%\DeclareComet{C2006B3}{C/2006 B3}{C/2006 B3 (SOHO)}
%\DeclareComet{C2006B4}{C/2006 B4}{C/2006 B4 (SOHO)}
%\DeclareComet{C2006B5}{C/2006 B5}{C/2006 B5 (SOHO)}
%\DeclareComet{C2006B6}{C/2006 B6}{C/2006 B6 (SOHO)}
%\DeclareComet{C2006C1}{C/2006 C1}{C/2006 C1 (SOHO)}
%\DeclareComet{C2006C2}{C/2006 C2}{C/2006 C2 (SOHO)}
%\DeclareComet{C2006C3}{C/2006 C3}{C/2006 C3 (SOHO)}
%\DeclareComet{C2006CK10}{C/2006 CK10}{C/2006 CK10 (Catalina)}
%\DeclareComet{C2006D2}{C/2006 D2}{C/2006 D2 (SOHO)}
%\DeclareComet{C2006D3}{C/2006 D3}{C/2006 D3 (SOHO)}
%\DeclareComet{C2006D4}{C/2006 D4}{C/2006 D4 (SOHO)}
%\DeclareComet{C2006D5}{C/2006 D5}{C/2006 D5 (SOHO)}
%\DeclareComet{C2006D6}{C/2006 D6}{C/2006 D6 (SOHO)}
%\DeclareComet{C2006E1}{C/2006 E1}{C/2006 E1 (McNaught)}
%\DeclareComet{C2006E2}{C/2006 E2}{C/2006 E2 (SOHO)}
%\DeclareComet{C2006E3}{C/2006 E3}{C/2006 E3 (SOHO)}
%\DeclareComet{C2006E4}{C/2006 E4}{C/2006 E4 (SOHO)}
%\DeclareComet{C2006F2}{C/2006 F2}{C/2006 F2 (Christensen)}
%\DeclareComet{C2006F3}{C/2006 F3}{C/2006 F3 (SOHO)}
%\DeclareComet{C2006F5}{C/2006 F5}{C/2006 F5 (SOHO)}
%\DeclareComet{C2006F6}{C/2006 F6}{C/2006 F6 (SOHO)}
%\DeclareComet{C2006F7}{C/2006 F7}{C/2006 F7 (SOHO)}
%\DeclareComet{C2006F8}{C/2006 F8}{C/2006 F8 (SOHO)}
%\DeclareComet{C2006G2}{C/2006 G2}{C/2006 G2 (SOHO)}
%\DeclareComet{C2006G3}{C/2006 G3}{C/2006 G3 (SOHO)}
%\DeclareComet{C2006GZ2}{C/2006 GZ2}{C/2006 GZ2 (Spacewatch)}
%\DeclareComet{C2006H2}{C/2006 H2}{C/2006 H2 (SOHO)}
%\DeclareComet{C2006H3}{C/2006 H3}{C/2006 H3 (SOHO)}
%\DeclareComet{C2006H4}{C/2006 H4}{C/2006 H4 (SOHO)}
%\DeclareComet{C2006H5}{C/2006 H5}{C/2006 H5 (SOHO)}
%\DeclareComet{C2006H6}{C/2006 H6}{C/2006 H6 (SOHO)}
%\DeclareComet{C2006HW51}{C/2006 HW51}{C/2006 HW51 (SidingSpring)}
%\DeclareComet{C2006J1}{C/2006 J1}{C/2006 J1 (SOHO)}
%\DeclareComet{C2006J10}{C/2006 J10}{C/2006 J10 (SOHO)}
%\DeclareComet{C2006J11}{C/2006 J11}{C/2006 J11 (SOHO)}
%\DeclareComet{C2006J12}{C/2006 J12}{C/2006 J12 (SOHO)}
%\DeclareComet{C2006J2}{C/2006 J2}{C/2006 J2 (SOHO)}
%\DeclareComet{C2006J3}{C/2006 J3}{C/2006 J3 (SOHO)}
%\DeclareComet{C2006J4}{C/2006 J4}{C/2006 J4 (SOHO)}
%\DeclareComet{C2006J5}{C/2006 J5}{C/2006 J5 (SOHO)}
%\DeclareComet{C2006J6}{C/2006 J6}{C/2006 J6 (SOHO)}
%\DeclareComet{C2006J7}{C/2006 J7}{C/2006 J7 (SOHO)}
%\DeclareComet{C2006J8}{C/2006 J8}{C/2006 J8 (SOHO)}
%\DeclareComet{C2006J9}{C/2006 J9}{C/2006 J9 (SOHO)}
%\DeclareComet{C2006K1}{C/2006 K1}{C/2006 K1 (McNaught)}
%\DeclareComet{C2006K10}{C/2006 K10}{C/2006 K10 (SOHO)}
%\DeclareComet{C2006K11}{C/2006 K11}{C/2006 K11 (SOHO)}
%\DeclareComet{C2006K12}{C/2006 K12}{C/2006 K12 (SOHO)}
%\DeclareComet{C2006K13}{C/2006 K13}{C/2006 K13 (SOHO)}
%\DeclareComet{C2006K14}{C/2006 K14}{C/2006 K14 (SOHO)}
%\DeclareComet{C2006K15}{C/2006 K15}{C/2006 K15 (SOHO)}
%\DeclareComet{C2006K16}{C/2006 K16}{C/2006 K16 (SOHO)}
%\DeclareComet{C2006K17}{C/2006 K17}{C/2006 K17 (SOHO)}
%\DeclareComet{C2006K18}{C/2006 K18}{C/2006 K18 (SOHO)}
%\DeclareComet{C2006K19}{C/2006 K19}{C/2006 K19 (SOHO)}
%\DeclareComet{C2006K20}{C/2006 K20}{C/2006 K20 (SOHO)}
%\DeclareComet{C2006K21}{C/2006 K21}{C/2006 K21 (SOHO)}
%\DeclareComet{C2006K3}{C/2006 K3}{C/2006 K3 (McNaught)}
%\DeclareComet{C2006K4}{C/2006 K4}{C/2006 K4 (NEAT)}
%\DeclareComet{C2006K5}{C/2006 K5}{C/2006 K5 (SOHO)}
%\DeclareComet{C2006K6}{C/2006 K6}{C/2006 K6 (SOHO)}
%\DeclareComet{C2006K7}{C/2006 K7}{C/2006 K7 (SOHO)}
%\DeclareComet{C2006K8}{C/2006 K8}{C/2006 K8 (SOHO)}
%\DeclareComet{C2006K9}{C/2006 K9}{C/2006 K9 (SOHO)}
%\DeclareComet{C2006L1}{C/2006 L1}{C/2006 L1 (Garradd)}
%\DeclareComet{C2006L2}{C/2006 L2}{C/2006 L2 (McNaught)}
%\DeclareComet{C2006L3}{C/2006 L3}{C/2006 L3 (SOHO)}
%\DeclareComet{C2006L4}{C/2006 L4}{C/2006 L4 (SOHO)}
%\DeclareComet{C2006L5}{C/2006 L5}{C/2006 L5 (SOHO)}
%\DeclareComet{C2006L6}{C/2006 L6}{C/2006 L6 (SOHO)}
%\DeclareComet{C2006L7}{C/2006 L7}{C/2006 L7 (SOHO)}
%\DeclareComet{C2006L8}{C/2006 L8}{C/2006 L8 (SOHO)}
%\DeclareComet{C2006M1}{C/2006 M1}{C/2006 M1 (LINEAR)}
%\DeclareComet{C2006M2}{C/2006 M2}{C/2006 M2 (Spacewatch)}
%\DeclareComet{C2006M4}{C/2006 M4}{C/2006 M4 (SWAN)}
%\DeclareComet{C2006M5}{C/2006 M5}{C/2006 M5 (SOHO)}
%\DeclareComet{C2006M6}{C/2006 M6}{C/2006 M6 (SOHO)}
%\DeclareComet{C2006M7}{C/2006 M7}{C/2006 M7 (SOHO)}
%\DeclareComet{C2006M8}{C/2006 M8}{C/2006 M8 (SOHO)}
%\DeclareComet{C2006M9}{C/2006 M9}{C/2006 M9 (SOHO)}
%\DeclareComet{C2006N1}{C/2006 N1}{C/2006 N1 (SOHO)}
%\DeclareComet{C2006N2}{C/2006 N2}{C/2006 N2 (SOHO)}
%\DeclareComet{C2006N3}{C/2006 N3}{C/2006 N3 (SOHO)}
%\DeclareComet{C2006O2}{C/2006 O2}{C/2006 O2 (Garradd)}
%\DeclareComet{C2006O3}{C/2006 O3}{C/2006 O3 (SOHO)}
%\DeclareComet{C2006O4}{C/2006 O4}{C/2006 O4 (SOHO)}
%\DeclareComet{C2006O5}{C/2006 O5}{C/2006 O5 (SOHO)}
%\DeclareComet{C2006O6}{C/2006 O6}{C/2006 O6 (SOHO)}
%\DeclareComet{C2006O7}{C/2006 O7}{C/2006 O7 (SOHO)}
%\DeclareComet{C2006O8}{C/2006 O8}{C/2006 O8 (SOHO)}
%\DeclareComet{C2006OF2}{C/2006 OF2}{C/2006 OF2 (Broughton)}
%\DeclareComet{C2006P1}{C/2006 P1}{C/2006 P1 (McNaught)}
%\DeclareComet{C2006P2}{C/2006 P2}{C/2006 P2 (SOHO)}
%\DeclareComet{C2006P3}{C/2006 P3}{C/2006 P3 (SOHO)}
%\DeclareComet{C2006P4}{C/2006 P4}{C/2006 P4 (SOHO)}
%\DeclareComet{C2006P5}{C/2006 P5}{C/2006 P5 (SOHO)}
%\DeclareComet{C2006P6}{C/2006 P6}{C/2006 P6 (SOHO)}
%\DeclareComet{C2006P7}{C/2006 P7}{C/2006 P7 (SOHO)}
%\DeclareComet{C2006Q1}{C/2006 Q1}{C/2006 Q1 (McNaught)}
%\DeclareComet{C2006R3}{C/2006 R3}{C/2006 R3 (SOHO)}
%\DeclareComet{C2006R4}{C/2006 R4}{C/2006 R4 (SOHO)}
%\DeclareComet{C2006S10}{C/2006 S10}{C/2006 S10 (SOHO)}
%\DeclareComet{C2006S11}{C/2006 S11}{C/2006 S11 (SOHO)}
%\DeclareComet{C2006S12}{C/2006 S12}{C/2006 S12 (SOHO)}
%\DeclareComet{C2006S13}{C/2006 S13}{C/2006 S13 (SOHO)}
%\DeclareComet{C2006S2}{C/2006 S2}{C/2006 S2 (LINEAR)}
%\DeclareComet{C2006S3}{C/2006 S3}{C/2006 S3 (LONEOS)}
%\DeclareComet{C2006S5}{C/2006 S5}{C/2006 S5 (Hill)}
%\DeclareComet{C2006S7}{C/2006 S7}{C/2006 S7 (SOHO)}
%\DeclareComet{C2006S8}{C/2006 S8}{C/2006 S8 (SOHO)}
%\DeclareComet{C2006S9}{C/2006 S9}{C/2006 S9 (SOHO)}
%\DeclareComet{C2006T10}{C/2006 T10}{C/2006 T10 (SOHO)}
%\DeclareComet{C2006T2}{C/2006 T2}{C/2006 T2 (SOHO)}
%\DeclareComet{C2006T3}{C/2006 T3}{C/2006 T3 (SOHO)}
%\DeclareComet{C2006T4}{C/2006 T4}{C/2006 T4 (SOHO)}
%\DeclareComet{C2006T5}{C/2006 T5}{C/2006 T5 (SOHO)}
%\DeclareComet{C2006T6}{C/2006 T6}{C/2006 T6 (SOHO)}
%\DeclareComet{C2006T7}{C/2006 T7}{C/2006 T7 (SOHO)}
%\DeclareComet{C2006T8}{C/2006 T8}{C/2006 T8 (SOHO)}
%\DeclareComet{C2006T9}{C/2006 T9}{C/2006 T9 (SOHO)}
%\DeclareComet{C2006U10}{C/2006 U10}{C/2006 U10 (SOHO)}
%\DeclareComet{C2006U11}{C/2006 U11}{C/2006 U11 (SOHO)}
%\DeclareComet{C2006U12}{C/2006 U12}{C/2006 U12 (SOHO)}
%\DeclareComet{C2006U13}{C/2006 U13}{C/2006 U13 (SOHO)}
%\DeclareComet{C2006U14}{C/2006 U14}{C/2006 U14 (SOHO)}
%\DeclareComet{C2006U15}{C/2006 U15}{C/2006 U15 (SOHO)}
%\DeclareComet{C2006U16}{C/2006 U16}{C/2006 U16 (SOHO)}
%\DeclareComet{C2006U6}{C/2006 U6}{C/2006 U6 (Spacewatch)}
%\DeclareComet{C2006U7}{C/2006 U7}{C/2006 U7 (Gibbs)}
%\DeclareComet{C2006U8}{C/2006 U8}{C/2006 U8 (SOHO)}
%\DeclareComet{C2006U9}{C/2006 U9}{C/2006 U9 (SOHO)}
%\DeclareComet{C2006V1}{C/2006 V1}{C/2006 V1 (Catalina)}
%\DeclareComet{C2006V10}{C/2006 V10}{C/2006 V10 (SOHO)}
%\DeclareComet{C2006V2}{C/2006 V2}{C/2006 V2 (SOHO)}
%\DeclareComet{C2006V3}{C/2006 V3}{C/2006 V3 (SOHO)}
%\DeclareComet{C2006V4}{C/2006 V4}{C/2006 V4 (SOHO)}
%\DeclareComet{C2006V5}{C/2006 V5}{C/2006 V5 (SOHO)}
%\DeclareComet{C2006V6}{C/2006 V6}{C/2006 V6 (SOHO)}
%\DeclareComet{C2006V7}{C/2006 V7}{C/2006 V7 (SOHO)}
%\DeclareComet{C2006V8}{C/2006 V8}{C/2006 V8 (SOHO)}
%\DeclareComet{C2006V9}{C/2006 V9}{C/2006 V9 (SOHO)}
%\DeclareComet{C2006VZ13}{C/2006 VZ13}{C/2006 VZ13 (LINEAR)}
%\DeclareComet{C2006W3}{C/2006 W3}{C/2006 W3 (Christensen)}
%\DeclareComet{C2006W5}{C/2006 W5}{C/2006 W5 (SOHO)}
%\DeclareComet{C2006W6}{C/2006 W6}{C/2006 W6 (SOHO)}
%\DeclareComet{C2006W7}{C/2006 W7}{C/2006 W7 (SOHO)}
%\DeclareComet{C2006WD4}{C/2006 WD4}{C/2006 WD4 (Lemmon)}
%\DeclareComet{C2006X1}{C/2006 X1}{C/2006 X1 (LINEAR)}
%\DeclareComet{C2006X10}{C/2006 X10}{C/2006 X10 (SOHO)}
%\DeclareComet{C2006X11}{C/2006 X11}{C/2006 X11 (SOHO)}
%\DeclareComet{C2006X2}{C/2006 X2}{C/2006 X2 (SOHO)}
%\DeclareComet{C2006X3}{C/2006 X3}{C/2006 X3 (SOHO)}
%\DeclareComet{C2006X4}{C/2006 X4}{C/2006 X4 (SOHO)}
%\DeclareComet{C2006X5}{C/2006 X5}{C/2006 X5 (SOHO)}
%\DeclareComet{C2006X6}{C/2006 X6}{C/2006 X6 (SOHO)}
%\DeclareComet{C2006X7}{C/2006 X7}{C/2006 X7 (SOHO)}
%\DeclareComet{C2006X8}{C/2006 X8}{C/2006 X8 (SOHO)}
%\DeclareComet{C2006X9}{C/2006 X9}{C/2006 X9 (SOHO)}
%\DeclareComet{C2006XA1}{C/2006 XA1}{C/2006 XA1 (LINEAR)}
%\DeclareComet{C2006Y10}{C/2006 Y10}{C/2006 Y10 (SOHO)}
%\DeclareComet{C2006Y11}{C/2006 Y11}{C/2006 Y11 (SOHO)}
%\DeclareComet{C2006Y12}{C/2006 Y12}{C/2006 Y12 (SOHO)}
%\DeclareComet{C2006Y13}{C/2006 Y13}{C/2006 Y13 (SOHO)}
%\DeclareComet{C2006Y14}{C/2006 Y14}{C/2006 Y14 (SOHO)}
%\DeclareComet{C2006Y15}{C/2006 Y15}{C/2006 Y15 (SOHO)}
%\DeclareComet{C2006Y16}{C/2006 Y16}{C/2006 Y16 (SOHO)}
%\DeclareComet{C2006Y17}{C/2006 Y17}{C/2006 Y17 (SOHO)}
%\DeclareComet{C2006Y3}{C/2006 Y3}{C/2006 Y3 (SOHO)}
%\DeclareComet{C2006Y4}{C/2006 Y4}{C/2006 Y4 (SOHO)}
%\DeclareComet{C2006Y5}{C/2006 Y5}{C/2006 Y5 (SOHO)}
%\DeclareComet{C2006Y6}{C/2006 Y6}{C/2006 Y6 (SOHO)}
%\DeclareComet{C2006Y7}{C/2006 Y7}{C/2006 Y7 (SOHO)}
%\DeclareComet{C2006Y8}{C/2006 Y8}{C/2006 Y8 (SOHO)}
%\DeclareComet{C2006Y9}{C/2006 Y9}{C/2006 Y9 (SOHO)}
%\DeclareComet{C2006YC}{C/2006 YC}{C/2006 YC (Catalina-Christensen)}
%\DeclareComet{C2007A4}{C/2007 A4}{C/2007 A4 (SOHO)}
%\DeclareComet{C2007A5}{C/2007 A5}{C/2007 A5 (SOHO)}
%\DeclareComet{C2007A6}{C/2007 A6}{C/2007 A6 (SOHO)}
%\DeclareComet{C2007A7}{C/2007 A7}{C/2007 A7 (SOHO)}
%\DeclareComet{C2007B2}{C/2007 B2}{C/2007 B2 (Skiff)}
%\DeclareComet{C2007B4}{C/2007 B4}{C/2007 B4 (SOHO)}
%\DeclareComet{C2007B5}{C/2007 B5}{C/2007 B5 (SOHO)}
%\DeclareComet{C2007B6}{C/2007 B6}{C/2007 B6 (SOHO)}
%\DeclareComet{C2007C10}{C/2007 C10}{C/2007 C10 (SOHO)}
%\DeclareComet{C2007C11}{C/2007 C11}{C/2007 C11 (SOHO)}
%\DeclareComet{C2007C12}{C/2007 C12}{C/2007 C12 (SOHO)}
%\DeclareComet{C2007C13}{C/2007 C13}{C/2007 C13 (SOHO)}
%\DeclareComet{C2007C3}{C/2007 C3}{C/2007 C3 (SOHO)}
%\DeclareComet{C2007C4}{C/2007 C4}{C/2007 C4 (SOHO)}
%\DeclareComet{C2007C5}{C/2007 C5}{C/2007 C5 (SOHO)}
%\DeclareComet{C2007C6}{C/2007 C6}{C/2007 C6 (SOHO)}
%\DeclareComet{C2007C7}{C/2007 C7}{C/2007 C7 (SOHO)}
%\DeclareComet{C2007C8}{C/2007 C8}{C/2007 C8 (SOHO)}
%\DeclareComet{C2007C9}{C/2007 C9}{C/2007 C9 (SOHO)}
%\DeclareComet{C2007D1}{C/2007 D1}{C/2007 D1 (LINEAR)}
%\DeclareComet{C2007D2}{C/2007 D2}{C/2007 D2 (Spacewatch)}
%\DeclareComet{C2007D3}{C/2007 D3}{C/2007 D3 (LINEAR)}
%\DeclareComet{C2007D4}{C/2007 D4}{C/2007 D4 (SOHO)}
%\DeclareComet{C2007D5}{C/2007 D5}{C/2007 D5 (SOHO)}
%\DeclareComet{C2007E1}{C/2007 E1}{C/2007 E1 (Garradd)}
%\DeclareComet{C2007E2}{C/2007 E2}{C/2007 E2 (Lovejoy)}
%\DeclareComet{C2007E4}{C/2007 E4}{C/2007 E4 (SOHO)}
%\DeclareComet{C2007E5}{C/2007 E5}{C/2007 E5 (SOHO)}
%\DeclareComet{C2007F1}{C/2007 F1}{C/2007 F1 (LONEOS)}
%\DeclareComet{C2007F2}{C/2007 F2}{C/2007 F2 (SOHO)}
%\DeclareComet{C2007F3}{C/2007 F3}{C/2007 F3 (SOHO)}
%\DeclareComet{C2007F4}{C/2007 F4}{C/2007 F4 (SOHO)}
%\DeclareComet{C2007F5}{C/2007 F5}{C/2007 F5 (SOHO)}
%\DeclareComet{C2007G1}{C/2007 G1}{C/2007 G1 (LINEAR)}
%\DeclareComet{C2007G2}{C/2007 G2}{C/2007 G2 (SOHO)}
%\DeclareComet{C2007H2}{C/2007 H2}{C/2007 H2 (Skiff)}
%\DeclareComet{C2007H4}{C/2007 H4}{C/2007 H4 (SOHO)}
%\DeclareComet{C2007H5}{C/2007 H5}{C/2007 H5 (SOHO)}
%\DeclareComet{C2007H6}{C/2007 H6}{C/2007 H6 (SOHO)}
%\DeclareComet{C2007H7}{C/2007 H7}{C/2007 H7 (SOHO)}
%\DeclareComet{C2007H8}{C/2007 H8}{C/2007 H8 (SOHO)}
%\DeclareComet{C2007H9}{C/2007 H9}{C/2007 H9 (SOHO)}
%\DeclareComet{C2007J1}{C/2007 J1}{C/2007 J1 (SOHO)}
%\DeclareComet{C2007J10}{C/2007 J10}{C/2007 J10 (SOHO)}
%\DeclareComet{C2007J11}{C/2007 J11}{C/2007 J11 (SOHO)}
%\DeclareComet{C2007J12}{C/2007 J12}{C/2007 J12 (SOHO)}
%\DeclareComet{C2007J2}{C/2007 J2}{C/2007 J2 (SOHO)}
%\DeclareComet{C2007J3}{C/2007 J3}{C/2007 J3 (SOHO)}
%\DeclareComet{C2007J4}{C/2007 J4}{C/2007 J4 (SOHO)}
%\DeclareComet{C2007J5}{C/2007 J5}{C/2007 J5 (SOHO)}
%\DeclareComet{C2007J6}{C/2007 J6}{C/2007 J6 (SOHO)}
%\DeclareComet{C2007J8}{C/2007 J8}{C/2007 J8 (SOHO)}
%\DeclareComet{C2007J9}{C/2007 J9}{C/2007 J9 (SOHO)}
%\DeclareComet{C2007JA21}{C/2007 JA21}{C/2007 JA21 (LINEAR)}
%\DeclareComet{C2007K1}{C/2007 K1}{C/2007 K1 (Lemmon)}
%\DeclareComet{C2007K10}{C/2007 K10}{C/2007 K10 (SOHO)}
%\DeclareComet{C2007K11}{C/2007 K11}{C/2007 K11 (SOHO)}
%\DeclareComet{C2007K12}{C/2007 K12}{C/2007 K12 (SOHO)}
%\DeclareComet{C2007K13}{C/2007 K13}{C/2007 K13 (SOHO)}
%\DeclareComet{C2007K14}{C/2007 K14}{C/2007 K14 (SOHO)}
%\DeclareComet{C2007K15}{C/2007 K15}{C/2007 K15 (SOHO)}
%\DeclareComet{C2007K16}{C/2007 K16}{C/2007 K16 (SOHO)}
%\DeclareComet{C2007K17}{C/2007 K17}{C/2007 K17 (SOHO)}
%\DeclareComet{C2007K18}{C/2007 K18}{C/2007 K18 (SOHO)}
%\DeclareComet{C2007K19}{C/2007 K19}{C/2007 K19 (SOHO)}
%\DeclareComet{C2007K20}{C/2007 K20}{C/2007 K20 (SOHO)}
%\DeclareComet{C2007K21}{C/2007 K21}{C/2007 K21 (SOHO)}
%\DeclareComet{C2007K3}{C/2007 K3}{C/2007 K3 (SidingSpring)}
%\DeclareComet{C2007K4}{C/2007 K4}{C/2007 K4 (Gibbs)}
%\DeclareComet{C2007K5}{C/2007 K5}{C/2007 K5 (Lovejoy)}
%\DeclareComet{C2007K6}{C/2007 K6}{C/2007 K6 (McNaught)}
%\DeclareComet{C2007K7}{C/2007 K7}{C/2007 K7 (SOHO)}
%\DeclareComet{C2007K8}{C/2007 K8}{C/2007 K8 (SOHO)}
%\DeclareComet{C2007K9}{C/2007 K9}{C/2007 K9 (SOHO)}
%\DeclareComet{C2007L1}{C/2007 L1}{C/2007 L1 (SOHO)}
%\DeclareComet{C2007L10}{C/2007 L10}{C/2007 L10 (SOHO)}
%\DeclareComet{C2007L11}{C/2007 L11}{C/2007 L11 (SOHO)}
%\DeclareComet{C2007L12}{C/2007 L12}{C/2007 L12 (SOHO)}
%\DeclareComet{C2007L13}{C/2007 L13}{C/2007 L13 (SOHO)}
%\DeclareComet{C2007L2}{C/2007 L2}{C/2007 L2 (SOHO)}
%\DeclareComet{C2007L3}{C/2007 L3}{C/2007 L3 (SOHO)}
%\DeclareComet{C2007L4}{C/2007 L4}{C/2007 L4 (SOHO)}
%\DeclareComet{C2007L5}{C/2007 L5}{C/2007 L5 (SOHO)}
%\DeclareComet{C2007L6}{C/2007 L6}{C/2007 L6 (SOHO)}
%\DeclareComet{C2007L7}{C/2007 L7}{C/2007 L7 (SOHO)}
%\DeclareComet{C2007L8}{C/2007 L8}{C/2007 L8 (SOHO)}
%\DeclareComet{C2007L9}{C/2007 L9}{C/2007 L9 (SOHO)}
%\DeclareComet{C2007M1}{C/2007 M1}{C/2007 M1 (McNaught)}
%\DeclareComet{C2007M10}{C/2007 M10}{C/2007 M10 (SOHO)}
%\DeclareComet{C2007M2}{C/2007 M2}{C/2007 M2 (Catalina)}
%\DeclareComet{C2007M3}{C/2007 M3}{C/2007 M3 (LINEAR)}
%\DeclareComet{C2007M4}{C/2007 M4}{C/2007 M4 (SOHO)}
%\DeclareComet{C2007M5}{C/2007 M5}{C/2007 M5 (SOHO)}
%\DeclareComet{C2007M6}{C/2007 M6}{C/2007 M6 (SOHO)}
%\DeclareComet{C2007M7}{C/2007 M7}{C/2007 M7 (SOHO)}
%\DeclareComet{C2007M8}{C/2007 M8}{C/2007 M8 (SOHO)}
%\DeclareComet{C2007M9}{C/2007 M9}{C/2007 M9 (SOHO)}
%\DeclareComet{C2007N3}{C/2007 N3}{C/2007 N3 (Lulin)}
%\DeclareComet{C2007N4}{C/2007 N4}{C/2007 N4 (SOHO)}
%\DeclareComet{C2007N5}{C/2007 N5}{C/2007 N5 (SOHO)}
%\DeclareComet{C2007N6}{C/2007 N6}{C/2007 N6 (SOHO)}
%\DeclareComet{C2007N7}{C/2007 N7}{C/2007 N7 (SOHO)}
%\DeclareComet{C2007N8}{C/2007 N8}{C/2007 N8 (SOHO)}
%\DeclareComet{C2007O1}{C/2007 O1}{C/2007 O1 (LINEAR)}
%\DeclareComet{C2007O3}{C/2007 O3}{C/2007 O3 (SOHO)}
%\DeclareComet{C2007O4}{C/2007 O4}{C/2007 O4 (SOHO)}
%\DeclareComet{C2007P1}{C/2007 P1}{C/2007 P1 (McNaught)}
%\DeclareComet{C2007Q1}{C/2007 Q1}{C/2007 Q1 (Garradd)}
%\DeclareComet{C2007Q3}{C/2007 Q3}{C/2007 Q3 (SidingSpring)}
%\DeclareComet{C2007Q4}{C/2007 Q4}{C/2007 Q4 (SOHO)}
%\DeclareComet{C2007Q5}{C/2007 Q5}{C/2007 Q5 (SOHO)}
%\DeclareComet{C2007Q6}{C/2007 Q6}{C/2007 Q6 (SOHO)}
%\DeclareComet{C2007Q7}{C/2007 Q7}{C/2007 Q7 (SOHO)}
%\DeclareComet{C2007Q8}{C/2007 Q8}{C/2007 Q8 (SOHO)}
%\DeclareComet{C2007Q9}{C/2007 Q9}{C/2007 Q9 (SOHO)}
%\DeclareComet{C2007R10}{C/2007 R10}{C/2007 R10 (SOHO)}
%\DeclareComet{C2007R6}{C/2007 R6}{C/2007 R6 (SOHO)}
%\DeclareComet{C2007R7}{C/2007 R7}{C/2007 R7 (SOHO)}
%\DeclareComet{C2007R8}{C/2007 R8}{C/2007 R8 (SOHO)}
%\DeclareComet{C2007R9}{C/2007 R9}{C/2007 R9 (SOHO)}
%\DeclareComet{C2007S10}{C/2007 S10}{C/2007 S10 (SOHO)}
%\DeclareComet{C2007S11}{C/2007 S11}{C/2007 S11 (SOHO)}
%\DeclareComet{C2007S2}{C/2007 S2}{C/2007 S2 (Lemmon)}
%\DeclareComet{C2007S3}{C/2007 S3}{C/2007 S3 (SOHO)}
%\DeclareComet{C2007S4}{C/2007 S4}{C/2007 S4 (SOHO)}
%\DeclareComet{C2007S5}{C/2007 S5}{C/2007 S5 (SOHO)}
%\DeclareComet{C2007S6}{C/2007 S6}{C/2007 S6 (SOHO)}
%\DeclareComet{C2007S7}{C/2007 S7}{C/2007 S7 (SOHO)}
%\DeclareComet{C2007S8}{C/2007 S8}{C/2007 S8 (SOHO)}
%\DeclareComet{C2007S9}{C/2007 S9}{C/2007 S9 (SOHO)}
%\DeclareComet{C2007T1}{C/2007 T1}{C/2007 T1 (McNaught)}
%\DeclareComet{C2007T10}{C/2007 T10}{C/2007 T10 (SOHO)}
%\DeclareComet{C2007T11}{C/2007 T11}{C/2007 T11 (SOHO)}
%\DeclareComet{C2007T12}{C/2007 T12}{C/2007 T12 (SOHO)}
%\DeclareComet{C2007T13}{C/2007 T13}{C/2007 T13 (SOHO)}
%\DeclareComet{C2007T14}{C/2007 T14}{C/2007 T14 (SOHO)}
%\DeclareComet{C2007T5}{C/2007 T5}{C/2007 T5 (Gibbs)}
%\DeclareComet{C2007T7}{C/2007 T7}{C/2007 T7 (SOHO)}
%\DeclareComet{C2007T8}{C/2007 T8}{C/2007 T8 (SOHO)}
%\DeclareComet{C2007T9}{C/2007 T9}{C/2007 T9 (SOHO)}
%\DeclareComet{C2007U1}{C/2007 U1}{C/2007 U1 (LINEAR)}
%\DeclareComet{C2007U10}{C/2007 U10}{C/2007 U10 (SOHO)}
%\DeclareComet{C2007U11}{C/2007 U11}{C/2007 U11 (SOHO)}
%\DeclareComet{C2007U12}{C/2007 U12}{C/2007 U12 (SOHO)}
%\DeclareComet{C2007U13}{C/2007 U13}{C/2007 U13 (SOHO)}
%\DeclareComet{C2007U3}{C/2007 U3}{C/2007 U3 (SOHO)}
%\DeclareComet{C2007U4}{C/2007 U4}{C/2007 U4 (SOHO)}
%\DeclareComet{C2007U5}{C/2007 U5}{C/2007 U5 (SOHO)}
%\DeclareComet{C2007U6}{C/2007 U6}{C/2007 U6 (SOHO)}
%\DeclareComet{C2007U7}{C/2007 U7}{C/2007 U7 (SOHO)}
%\DeclareComet{C2007U8}{C/2007 U8}{C/2007 U8 (SOHO)}
%\DeclareComet{C2007U9}{C/2007 U9}{C/2007 U9 (SOHO)}
%\DeclareComet{C2007V10}{C/2007 V10}{C/2007 V10 (SOHO)}
%\DeclareComet{C2007V11}{C/2007 V11}{C/2007 V11 (SOHO)}
%\DeclareComet{C2007V12}{C/2007 V12}{C/2007 V12 (SOHO)}
%\DeclareComet{C2007V13}{C/2007 V13}{C/2007 V13 (SOHO)}
%\DeclareComet{C2007V14}{C/2007 V14}{C/2007 V14 (SOHO)}
%\DeclareComet{C2007V3}{C/2007 V3}{C/2007 V3 (SOHO)}
%\DeclareComet{C2007V4}{C/2007 V4}{C/2007 V4 (SOHO)}
%\DeclareComet{C2007V5}{C/2007 V5}{C/2007 V5 (SOHO)}
%\DeclareComet{C2007V6}{C/2007 V6}{C/2007 V6 (SOHO)}
%\DeclareComet{C2007V7}{C/2007 V7}{C/2007 V7 (SOHO)}
%\DeclareComet{C2007V8}{C/2007 V8}{C/2007 V8 (SOHO)}
%\DeclareComet{C2007V9}{C/2007 V9}{C/2007 V9 (SOHO)}
%\DeclareComet{C2007VO53}{C/2007 VO53}{C/2007 VO53 (Spacewatch)}
%\DeclareComet{C2007W1}{C/2007 W1}{C/2007 W1 (Boattini)}
%\DeclareComet{C2007W10}{C/2007 W10}{C/2007 W10 (SOHO)}
%\DeclareComet{C2007W11}{C/2007 W11}{C/2007 W11 (SOHO)}
%\DeclareComet{C2007W12}{C/2007 W12}{C/2007 W12 (SOHO)}
%\DeclareComet{C2007W3}{C/2007 W3}{C/2007 W3 (LINEAR)}
%\DeclareComet{C2007W4}{C/2007 W4}{C/2007 W4 (SOHO)}
%\DeclareComet{C2007W5}{C/2007 W5}{C/2007 W5 (SOHO)}
%\DeclareComet{C2007W6}{C/2007 W6}{C/2007 W6 (SOHO)}
%\DeclareComet{C2007W7}{C/2007 W7}{C/2007 W7 (SOHO)}
%\DeclareComet{C2007W8}{C/2007 W8}{C/2007 W8 (SOHO)}
%\DeclareComet{C2007W9}{C/2007 W9}{C/2007 W9 (SOHO)}
%\DeclareComet{C2007X1}{C/2007 X1}{C/2007 X1 (SOHO)}
%\DeclareComet{C2007X10}{C/2007 X10}{C/2007 X10 (SOHO)}
%\DeclareComet{C2007X11}{C/2007 X11}{C/2007 X11 (SOHO)}
%\DeclareComet{C2007X12}{C/2007 X12}{C/2007 X12 (SOHO)}
%\DeclareComet{C2007X13}{C/2007 X13}{C/2007 X13 (SOHO)}
%\DeclareComet{C2007X14}{C/2007 X14}{C/2007 X14 (SOHO)}
%\DeclareComet{C2007X15}{C/2007 X15}{C/2007 X15 (SOHO)}
%\DeclareComet{C2007X2}{C/2007 X2}{C/2007 X2 (SOHO)}
%\DeclareComet{C2007X3}{C/2007 X3}{C/2007 X3 (SOHO)}
%\DeclareComet{C2007X4}{C/2007 X4}{C/2007 X4 (SOHO)}
%\DeclareComet{C2007X5}{C/2007 X5}{C/2007 X5 (SOHO)}
%\DeclareComet{C2007X6}{C/2007 X6}{C/2007 X6 (SOHO)}
%\DeclareComet{C2007X7}{C/2007 X7}{C/2007 X7 (SOHO)}
%\DeclareComet{C2007X8}{C/2007 X8}{C/2007 X8 (SOHO)}
%\DeclareComet{C2007X9}{C/2007 X9}{C/2007 X9 (SOHO)}
%\DeclareComet{C2007Y1}{C/2007 Y1}{C/2007 Y1 (LINEAR)}
%\DeclareComet{C2007Y10}{C/2007 Y10}{C/2007 Y10 (SOHO)}
%\DeclareComet{C2007Y2}{C/2007 Y2}{C/2007 Y2 (McNaught)}
%\DeclareComet{C2007Y3}{C/2007 Y3}{C/2007 Y3 (SOHO)}
%\DeclareComet{C2007Y4}{C/2007 Y4}{C/2007 Y4 (SOHO)}
%\DeclareComet{C2007Y5}{C/2007 Y5}{C/2007 Y5 (SOHO)}
%\DeclareComet{C2007Y6}{C/2007 Y6}{C/2007 Y6 (SOHO)}
%\DeclareComet{C2007Y7}{C/2007 Y7}{C/2007 Y7 (SOHO)}
%\DeclareComet{C2007Y8}{C/2007 Y8}{C/2007 Y8 (SOHO)}
%\DeclareComet{C2007Y9}{C/2007 Y9}{C/2007 Y9 (SOHO)}
%\DeclareComet{C2008A1}{C/2008 A1}{C/2008 A1 (McNaught)}
%\DeclareComet{C2008A3}{C/2008 A3}{C/2008 A3 (SOHO)}
%\DeclareComet{C2008B1}{C/2008 B1}{C/2008 B1 (SOHO)}
%\DeclareComet{C2008B2}{C/2008 B2}{C/2008 B2 (SOHO)}
%\DeclareComet{C2008B3}{C/2008 B3}{C/2008 B3 (SOHO)}
%\DeclareComet{C2008B4}{C/2008 B4}{C/2008 B4 (SOHO)}
%\DeclareComet{C2008C1}{C/2008 C1}{C/2008 C1 (Chen-Gao)}
%\DeclareComet{C2008C3}{C/2008 C3}{C/2008 C3 (SOHO)}
%\DeclareComet{C2008C4}{C/2008 C4}{C/2008 C4 (SOHO)}
%\DeclareComet{C2008C5}{C/2008 C5}{C/2008 C5 (SOHO)}
%\DeclareComet{C2008C6}{C/2008 C6}{C/2008 C6 (SOHO)}
%\DeclareComet{C2008C7}{C/2008 C7}{C/2008 C7 (SOHO)}
%\DeclareComet{C2008C8}{C/2008 C8}{C/2008 C8 (SOHO)}
%\DeclareComet{C2008C9}{C/2008 C9}{C/2008 C9 (SOHO)}
%\DeclareComet{C2008D1}{C/2008 D1}{C/2008 D1 (STEREO)}
%\DeclareComet{C2008D2}{C/2008 D2}{C/2008 D2 (STEREO)}
%\DeclareComet{C2008D3}{C/2008 D3}{C/2008 D3 (STEREO)}
%\DeclareComet{C2008D4}{C/2008 D4}{C/2008 D4 (STEREO)}
%\DeclareComet{C2008D5}{C/2008 D5}{C/2008 D5 (SOHO)}
%\DeclareComet{C2008D6}{C/2008 D6}{C/2008 D6 (SOHO)}
%\DeclareComet{C2008D7}{C/2008 D7}{C/2008 D7 (SOHO)}
%\DeclareComet{C2008D8}{C/2008 D8}{C/2008 D8 (SOHO)}
%\DeclareComet{C2008D9}{C/2008 D9}{C/2008 D9 (SOHO)}
%\DeclareComet{C2008E1}{C/2008 E1}{C/2008 E1 (Catalina)}
%\DeclareComet{C2008E10}{C/2008 E10}{C/2008 E10 (STEREO)}
%\DeclareComet{C2008E3}{C/2008 E3}{C/2008 E3 (Garradd)}
%\DeclareComet{C2008E4}{C/2008 E4}{C/2008 E4 (SOHO)}
%\DeclareComet{C2008E5}{C/2008 E5}{C/2008 E5 (STEREO)}
%\DeclareComet{C2008E6}{C/2008 E6}{C/2008 E6 (STEREO)}
%\DeclareComet{C2008E7}{C/2008 E7}{C/2008 E7 (SOHO)}
%\DeclareComet{C2008E8}{C/2008 E8}{C/2008 E8 (SOHO)}
%\DeclareComet{C2008E9}{C/2008 E9}{C/2008 E9 (SOHO)}
%\DeclareComet{C2008F1}{C/2008 F1}{C/2008 F1 (SOHO)}
%\DeclareComet{C2008FK75}{C/2008 FK75}{C/2008 FK75 (Lemmon-SidingSpring)}
%\DeclareComet{C2008G1}{C/2008 G1}{C/2008 G1 (Gibbs)}
%\DeclareComet{C2008G3}{C/2008 G3}{C/2008 G3 (SOHO)}
%\DeclareComet{C2008G4}{C/2008 G4}{C/2008 G4 (SOHO)}
%\DeclareComet{C2008G5}{C/2008 G5}{C/2008 G5 (SOHO)}
%\DeclareComet{C2008G6}{C/2008 G6}{C/2008 G6 (SOHO)}
%\DeclareComet{C2008H1}{C/2008 H1}{C/2008 H1 (LINEAR)}
%\DeclareComet{C2008H2}{C/2008 H2}{C/2008 H2 (SOHO)}
%\DeclareComet{C2008H3}{C/2008 H3}{C/2008 H3 (SOHO)}
%\DeclareComet{C2008H4}{C/2008 H4}{C/2008 H4 (SOHO)}
%\DeclareComet{C2008H5}{C/2008 H5}{C/2008 H5 (SOHO)}
%\DeclareComet{C2008H6}{C/2008 H6}{C/2008 H6 (SOHO)}
%\DeclareComet{C2008H7}{C/2008 H7}{C/2008 H7 (SOHO)}
%\DeclareComet{C2008H8}{C/2008 H8}{C/2008 H8 (SOHO)}
%\DeclareComet{C2008H9}{C/2008 H9}{C/2008 H9 (SOHO)}
%\DeclareComet{C2008J1}{C/2008 J1}{C/2008 J1 (Boattini)}
%\DeclareComet{C2008J10}{C/2008 J10}{C/2008 J10 (SOHO)}
%\DeclareComet{C2008J11}{C/2008 J11}{C/2008 J11 (SOHO)}
%\DeclareComet{C2008J12}{C/2008 J12}{C/2008 J12 (SOHO)}
%\DeclareComet{C2008J13}{C/2008 J13}{C/2008 J13 (SOHO)}
%\DeclareComet{C2008J14}{C/2008 J14}{C/2008 J14 (SOHO)}
%\DeclareComet{C2008J15}{C/2008 J15}{C/2008 J15 (SOHO)}
%\DeclareComet{C2008J16}{C/2008 J16}{C/2008 J16 (SOHO)}
%\DeclareComet{C2008J4}{C/2008 J4}{C/2008 J4 (McNaught)}
%\DeclareComet{C2008J5}{C/2008 J5}{C/2008 J5 (Garradd)}
%\DeclareComet{C2008J6}{C/2008 J6}{C/2008 J6 (Hill)}
%\DeclareComet{C2008J7}{C/2008 J7}{C/2008 J7 (SOHO)}
%\DeclareComet{C2008J8}{C/2008 J8}{C/2008 J8 (SOHO)}
%\DeclareComet{C2008J9}{C/2008 J9}{C/2008 J9 (SOHO)}
%\DeclareComet{C2008K1}{C/2008 K1}{C/2008 K1 (SOHO)}
%\DeclareComet{C2008K11}{C/2008 K11}{C/2008 K11 (SOHO)}
%\DeclareComet{C2008K2}{C/2008 K2}{C/2008 K2 (SOHO)}
%\DeclareComet{C2008K3}{C/2008 K3}{C/2008 K3 (SOHO)}
%\DeclareComet{C2008K4}{C/2008 K4}{C/2008 K4 (SOHO)}
%\DeclareComet{C2008K5}{C/2008 K5}{C/2008 K5 (SOHO)}
%\DeclareComet{C2008K6}{C/2008 K6}{C/2008 K6 (SOHO)}
%\DeclareComet{C2008K7}{C/2008 K7}{C/2008 K7 (SOHO)}
%\DeclareComet{C2008K8}{C/2008 K8}{C/2008 K8 (SOHO)}
%\DeclareComet{C2008K9}{C/2008 K9}{C/2008 K9 (SOHO)}
%\DeclareComet{C2008L10}{C/2008 L10}{C/2008 L10 (SOHO)}
%\DeclareComet{C2008L11}{C/2008 L11}{C/2008 L11 (SOHO)}
%\DeclareComet{C2008L12}{C/2008 L12}{C/2008 L12 (SOHO)}
%\DeclareComet{C2008L13}{C/2008 L13}{C/2008 L13 (SOHO)}
%\DeclareComet{C2008L14}{C/2008 L14}{C/2008 L14 (SOHO)}
%\DeclareComet{C2008L15}{C/2008 L15}{C/2008 L15 (SOHO)}
%\DeclareComet{C2008L3}{C/2008 L3}{C/2008 L3 (Hill)}
%\DeclareComet{C2008L4}{C/2008 L4}{C/2008 L4 (SOHO)}
%\DeclareComet{C2008L5}{C/2008 L5}{C/2008 L5 (SOHO)}
%\DeclareComet{C2008L6}{C/2008 L6}{C/2008 L6 (SOHO)}
%\DeclareComet{C2008L7}{C/2008 L7}{C/2008 L7 (SOHO)}
%\DeclareComet{C2008L8}{C/2008 L8}{C/2008 L8 (SOHO)}
%\DeclareComet{C2008L9}{C/2008 L9}{C/2008 L9 (SOHO)}
%\DeclareComet{C2008M1}{C/2008 M1}{C/2008 M1 (SOHO)}
%\DeclareComet{C2008M2}{C/2008 M2}{C/2008 M2 (SOHO)}
%\DeclareComet{C2008M3}{C/2008 M3}{C/2008 M3 (SOHO)}
%\DeclareComet{C2008M4}{C/2008 M4}{C/2008 M4 (SOHO)}
%\DeclareComet{C2008M5}{C/2008 M5}{C/2008 M5 (SOHO)}
%\DeclareComet{C2008M6}{C/2008 M6}{C/2008 M6 (SOHO)}
%\DeclareComet{C2008M7}{C/2008 M7}{C/2008 M7 (SOHO)}
%\DeclareComet{C2008N1}{C/2008 N1}{C/2008 N1 (Holmes)}
%\DeclareComet{C2008N10}{C/2008 N10}{C/2008 N10 (SOHO)}
%\DeclareComet{C2008N11}{C/2008 N11}{C/2008 N11 (SOHO)}
%\DeclareComet{C2008N2}{C/2008 N2}{C/2008 N2 (SOHO)}
%\DeclareComet{C2008N3}{C/2008 N3}{C/2008 N3 (SOHO)}
%\DeclareComet{C2008N4}{C/2008 N4}{C/2008 N4 (SOHO)}
%\DeclareComet{C2008N5}{C/2008 N5}{C/2008 N5 (SOHO)}
%\DeclareComet{C2008N6}{C/2008 N6}{C/2008 N6 (SOHO)}
%\DeclareComet{C2008N7}{C/2008 N7}{C/2008 N7 (SOHO)}
%\DeclareComet{C2008N8}{C/2008 N8}{C/2008 N8 (SOHO)}
%\DeclareComet{C2008N9}{C/2008 N9}{C/2008 N9 (SOHO)}
%\DeclareComet{C2008O1}{C/2008 O1}{C/2008 O1 (SOHO)}
%\DeclareComet{C2008O4}{C/2008 O4}{C/2008 O4 (SOHO)}
%\DeclareComet{C2008O5}{C/2008 O5}{C/2008 O5 (SOHO)}
%\DeclareComet{C2008O6}{C/2008 O6}{C/2008 O6 (SOHO)}
%\DeclareComet{C2008O7}{C/2008 O7}{C/2008 O7 (SOHO)}
%\DeclareComet{C2008P1}{C/2008 P1}{C/2008 P1 (Garradd)}
%\DeclareComet{C2008P2}{C/2008 P2}{C/2008 P2 (SOHO)}
%\DeclareComet{C2008P3}{C/2008 P3}{C/2008 P3 (SOHO)}
%\DeclareComet{C2008P4}{C/2008 P4}{C/2008 P4 (SOHO)}
%\DeclareComet{C2008P5}{C/2008 P5}{C/2008 P5 (SOHO)}
%\DeclareComet{C2008P6}{C/2008 P6}{C/2008 P6 (SOHO)}
%\DeclareComet{C2008P7}{C/2008 P7}{C/2008 P7 (SOHO)}
%\DeclareComet{C2008Q1}{C/2008 Q1}{C/2008 Q1 (Maticic)}
%\DeclareComet{C2008Q3}{C/2008 Q3}{C/2008 Q3 (Garradd)}
%\DeclareComet{C2008Q5}{C/2008 Q5}{C/2008 Q5 (SOHO)}
%\DeclareComet{C2008R10}{C/2008 R10}{C/2008 R10 (SOHO)}
%\DeclareComet{C2008R11}{C/2008 R11}{C/2008 R11 (SOHO)}
%\DeclareComet{C2008R12}{C/2008 R12}{C/2008 R12 (SOHO)}
%\DeclareComet{C2008R13}{C/2008 R13}{C/2008 R13 (SOHO)}
%\DeclareComet{C2008R3}{C/2008 R3}{C/2008 R3 (LINEAR)}
%\DeclareComet{C2008R7}{C/2008 R7}{C/2008 R7 (SOHO)}
%\DeclareComet{C2008R8}{C/2008 R8}{C/2008 R8 (SOHO)}
%\DeclareComet{C2008R9}{C/2008 R9}{C/2008 R9 (SOHO)}
%\DeclareComet{C2008S3}{C/2008 S3}{C/2008 S3 (Boattini)}
%\DeclareComet{C2008S4}{C/2008 S4}{C/2008 S4 (SOHO)}
%\DeclareComet{C2008S5}{C/2008 S5}{C/2008 S5 (SOHO)}
%\DeclareComet{C2008S6}{C/2008 S6}{C/2008 S6 (SOHO)}
%\DeclareComet{C2008S7}{C/2008 S7}{C/2008 S7 (SOHO)}
%\DeclareComet{C2008S8}{C/2008 S8}{C/2008 S8 (SOHO)}
%\DeclareComet{C2008T10}{C/2008 T10}{C/2008 T10 (SOHO)}
%\DeclareComet{C2008T11}{C/2008 T11}{C/2008 T11 (SOHO)}
%\DeclareComet{C2008T12}{C/2008 T12}{C/2008 T12 (SOHO)}
%\DeclareComet{C2008T2}{C/2008 T2}{C/2008 T2 (Cardinal)}
%\DeclareComet{C2008T6}{C/2008 T6}{C/2008 T6 (SOHO)}
%\DeclareComet{C2008T7}{C/2008 T7}{C/2008 T7 (SOHO)}
%\DeclareComet{C2008T8}{C/2008 T8}{C/2008 T8 (SOHO)}
%\DeclareComet{C2008T9}{C/2008 T9}{C/2008 T9 (SOHO)}
%\DeclareComet{C2008U10}{C/2008 U10}{C/2008 U10 (SOHO)}
%\DeclareComet{C2008U11}{C/2008 U11}{C/2008 U11 (SOHO)}
%\DeclareComet{C2008U12}{C/2008 U12}{C/2008 U12 (SOHO)}
%\DeclareComet{C2008U13}{C/2008 U13}{C/2008 U13 (SOHO)}
%\DeclareComet{C2008U14}{C/2008 U14}{C/2008 U14 (SOHO)}
%\DeclareComet{C2008U15}{C/2008 U15}{C/2008 U15 (SOHO)}
%\DeclareComet{C2008U16}{C/2008 U16}{C/2008 U16 (SOHO)}
%\DeclareComet{C2008U2}{C/2008 U2}{C/2008 U2 (SOHO)}
%\DeclareComet{C2008U3}{C/2008 U3}{C/2008 U3 (SOHO)}
%\DeclareComet{C2008U4}{C/2008 U4}{C/2008 U4 (SOHO)}
%\DeclareComet{C2008U5}{C/2008 U5}{C/2008 U5 (SOHO)}
%\DeclareComet{C2008U6}{C/2008 U6}{C/2008 U6 (SOHO)}
%\DeclareComet{C2008U7}{C/2008 U7}{C/2008 U7 (SOHO)}
%\DeclareComet{C2008U8}{C/2008 U8}{C/2008 U8 (SOHO)}
%\DeclareComet{C2008U9}{C/2008 U9}{C/2008 U9 (SOHO)}
%\DeclareComet{C2008V1}{C/2008 V1}{C/2008 V1 (SOHO)}
%\DeclareComet{C2008V2}{C/2008 V2}{C/2008 V2 (SOHO)}
%\DeclareComet{C2008V3}{C/2008 V3}{C/2008 V3 (SOHO)}
%\DeclareComet{C2008V4}{C/2008 V4}{C/2008 V4 (SOHO)}
%\DeclareComet{C2008V5}{C/2008 V5}{C/2008 V5 (SOHO)}
%\DeclareComet{C2008V6}{C/2008 V6}{C/2008 V6 (SOHO)}
%\DeclareComet{C2008W1}{C/2008 W1}{C/2008 W1 (STEREO)}
%\DeclareComet{C2008W10}{C/2008 W10}{C/2008 W10 (SOHO)}
%\DeclareComet{C2008W11}{C/2008 W11}{C/2008 W11 (SOHO)}
%\DeclareComet{C2008W12}{C/2008 W12}{C/2008 W12 (SOHO)}
%\DeclareComet{C2008W2}{C/2008 W2}{C/2008 W2 (SOHO)}
%\DeclareComet{C2008W3}{C/2008 W3}{C/2008 W3 (SOHO)}
%\DeclareComet{C2008W4}{C/2008 W4}{C/2008 W4 (SOHO)}
%\DeclareComet{C2008W5}{C/2008 W5}{C/2008 W5 (SOHO)}
%\DeclareComet{C2008W6}{C/2008 W6}{C/2008 W6 (SOHO)}
%\DeclareComet{C2008W7}{C/2008 W7}{C/2008 W7 (SOHO)}
%\DeclareComet{C2008W8}{C/2008 W8}{C/2008 W8 (SOHO)}
%\DeclareComet{C2008W9}{C/2008 W9}{C/2008 W9 (SOHO)}
%\DeclareComet{C2008X10}{C/2008 X10}{C/2008 X10 (SOHO)}
%\DeclareComet{C2008X11}{C/2008 X11}{C/2008 X11 (SOHO)}
%\DeclareComet{C2008X12}{C/2008 X12}{C/2008 X12 (SOHO)}
%\DeclareComet{C2008X13}{C/2008 X13}{C/2008 X13 (SOHO)}
%\DeclareComet{C2008X14}{C/2008 X14}{C/2008 X14 (SOHO)}
%\DeclareComet{C2008X3}{C/2008 X3}{C/2008 X3 (LINEAR)}
%\DeclareComet{C2008X5}{C/2008 X5}{C/2008 X5 (SOHO)}
%\DeclareComet{C2008X6}{C/2008 X6}{C/2008 X6 (SOHO)}
%\DeclareComet{C2008X7}{C/2008 X7}{C/2008 X7 (SOHO)}
%\DeclareComet{C2008X8}{C/2008 X8}{C/2008 X8 (SOHO)}
%\DeclareComet{C2008X9}{C/2008 X9}{C/2008 X9 (SOHO)}
%\DeclareComet{C2008Y10}{C/2008 Y10}{C/2008 Y10 (SOHO)}
%\DeclareComet{C2008Y11}{C/2008 Y11}{C/2008 Y11 (SOHO)}
%\DeclareComet{C2008Y13}{C/2008 Y13}{C/2008 Y13 (SOHO)}
%\DeclareComet{C2008Y14}{C/2008 Y14}{C/2008 Y14 (SOHO)}
%\DeclareComet{C2008Y15}{C/2008 Y15}{C/2008 Y15 (SOHO)}
%\DeclareComet{C2008Y16}{C/2008 Y16}{C/2008 Y16 (STEREO)}
%\DeclareComet{C2008Y17}{C/2008 Y17}{C/2008 Y17 (STEREO)}
%\DeclareComet{C2008Y18}{C/2008 Y18}{C/2008 Y18 (SOHO)}
%\DeclareComet{C2008Y4}{C/2008 Y4}{C/2008 Y4 (SOHO)}
%\DeclareComet{C2008Y5}{C/2008 Y5}{C/2008 Y5 (SOHO)}
%\DeclareComet{C2008Y6}{C/2008 Y6}{C/2008 Y6 (SOHO)}
%\DeclareComet{C2008Y7}{C/2008 Y7}{C/2008 Y7 (SOHO)}
%\DeclareComet{C2008Y8}{C/2008 Y8}{C/2008 Y8 (SOHO)}
%\DeclareComet{C2008Y9}{C/2008 Y9}{C/2008 Y9 (SOHO)}
%\DeclareComet{C2009A1}{C/2009 A1}{C/2009 A1 (STEREO)}
%\DeclareComet{C2009A10}{C/2009 A10}{C/2009 A10 (STEREO)}
%\DeclareComet{C2009A2}{C/2009 A2}{C/2009 A2 (SOHO)}
%\DeclareComet{C2009A3}{C/2009 A3}{C/2009 A3 (SOHO)}
%\DeclareComet{C2009A4}{C/2009 A4}{C/2009 A4 (SOHO)}
%\DeclareComet{C2009A5}{C/2009 A5}{C/2009 A5 (SOHO)}
%\DeclareComet{C2009A6}{C/2009 A6}{C/2009 A6 (STEREO)}
%\DeclareComet{C2009A7}{C/2009 A7}{C/2009 A7 (SOHO)}
%\DeclareComet{C2009A8}{C/2009 A8}{C/2009 A8 (STEREO)}
%\DeclareComet{C2009A9}{C/2009 A9}{C/2009 A9 (STEREO)}
%\DeclareComet{C2009B10}{C/2009 B10}{C/2009 B10 (SOHO)}
%\DeclareComet{C2009B11}{C/2009 B11}{C/2009 B11 (SOHO)}
%\DeclareComet{C2009B2}{C/2009 B2}{C/2009 B2 (LINEAR)}
%\DeclareComet{C2009B6}{C/2009 B6}{C/2009 B6 (STEREO)}
%\DeclareComet{C2009B7}{C/2009 B7}{C/2009 B7 (STEREO)}
%\DeclareComet{C2009B8}{C/2009 B8}{C/2009 B8 (SOHO)}
%\DeclareComet{C2009B9}{C/2009 B9}{C/2009 B9 (SOHO)}
%\DeclareComet{C2009C1}{C/2009 C1}{C/2009 C1 (STEREO)}
%\DeclareComet{C2009C2}{C/2009 C2}{C/2009 C2 (STEREO)}
%\DeclareComet{C2009C3}{C/2009 C3}{C/2009 C3 (SOHO)}
%\DeclareComet{C2009C4}{C/2009 C4}{C/2009 C4 (SOHO)}
%\DeclareComet{C2009C5}{C/2009 C5}{C/2009 C5 (SOHO)}
%\DeclareComet{C2009D2}{C/2009 D2}{C/2009 D2 (SOHO)}
%\DeclareComet{C2009D3}{C/2009 D3}{C/2009 D3 (SOHO)}
%\DeclareComet{C2009D4}{C/2009 D4}{C/2009 D4 (SOHO)}
%\DeclareComet{C2009D5}{C/2009 D5}{C/2009 D5 (SOHO)}
%\DeclareComet{C2009D6}{C/2009 D6}{C/2009 D6 (SOHO)}
%\DeclareComet{C2009D7}{C/2009 D7}{C/2009 D7 (SOHO)}
%\DeclareComet{C2009D8}{C/2009 D8}{C/2009 D8 (SOHO)}
%\DeclareComet{C2009E1}{C/2009 E1}{C/2009 E1 (Itagaki)}
%\DeclareComet{C2009E2}{C/2009 E2}{C/2009 E2 (SOHO)}
%\DeclareComet{C2009E3}{C/2009 E3}{C/2009 E3 (SOHO)}
%\DeclareComet{C2009E4}{C/2009 E4}{C/2009 E4 (SOHO)}
%\DeclareComet{C2009E5}{C/2009 E5}{C/2009 E5 (SOHO)}
%\DeclareComet{C2009F1}{C/2009 F1}{C/2009 F1 (Larson)}
%\DeclareComet{C2009F10}{C/2009 F10}{C/2009 F10 (SOHO)}
%\DeclareComet{C2009F2}{C/2009 F2}{C/2009 F2 (McNaught)}
%\DeclareComet{C2009F4}{C/2009 F4}{C/2009 F4 (McNaught)}
%\DeclareComet{C2009F5}{C/2009 F5}{C/2009 F5 (McNaught)}
%\DeclareComet{C2009F6}{C/2009 F6}{C/2009 F6 (Yi-SWAN)}
%\DeclareComet{C2009F8}{C/2009 F8}{C/2009 F8 (SOHO)}
%\DeclareComet{C2009F9}{C/2009 F9}{C/2009 F9 (SOHO)}
%\DeclareComet{C2009G1}{C/2009 G1}{C/2009 G1 (STEREO)}
%\DeclareComet{C2009G2}{C/2009 G2}{C/2009 G2 (SOHO)}
%\DeclareComet{C2009G3}{C/2009 G3}{C/2009 G3 (SOHO)}
%\DeclareComet{C2009G4}{C/2009 G4}{C/2009 G4 (SOHO)}
%\DeclareComet{C2009G5}{C/2009 G5}{C/2009 G5 (SOHO)}
%\DeclareComet{C2009G6}{C/2009 G6}{C/2009 G6 (SOHO)}
%\DeclareComet{C2009G7}{C/2009 G7}{C/2009 G7 (SOHO)}
%\DeclareComet{C2009G8}{C/2009 G8}{C/2009 G8 (SOHO)}
%\DeclareComet{C2009H3}{C/2009 H3}{C/2009 H3 (SOHO)}
%\DeclareComet{C2009H4}{C/2009 H4}{C/2009 H4 (SOHO)}
%\DeclareComet{C2009H5}{C/2009 H5}{C/2009 H5 (SOHO)}
%\DeclareComet{C2009H6}{C/2009 H6}{C/2009 H6 (SOHO)}
%\DeclareComet{C2009H7}{C/2009 H7}{C/2009 H7 (SOHO)}
%\DeclareComet{C2009H8}{C/2009 H8}{C/2009 H8 (SOHO)}
%\DeclareComet{C2009J1}{C/2009 J1}{C/2009 J1 (SOHO)}
%\DeclareComet{C2009J10}{C/2009 J10}{C/2009 J10 (SOHO)}
%\DeclareComet{C2009J11}{C/2009 J11}{C/2009 J11 (SOHO)}
%\DeclareComet{C2009J12}{C/2009 J12}{C/2009 J12 (SOHO)}
%\DeclareComet{C2009J2}{C/2009 J2}{C/2009 J2 (SOHO)}
%\DeclareComet{C2009J3}{C/2009 J3}{C/2009 J3 (SOHO)}
%\DeclareComet{C2009J4}{C/2009 J4}{C/2009 J4 (SOHO)}
%\DeclareComet{C2009J5}{C/2009 J5}{C/2009 J5 (SOHO)}
%\DeclareComet{C2009J6}{C/2009 J6}{C/2009 J6 (SOHO)}
%\DeclareComet{C2009J7}{C/2009 J7}{C/2009 J7 (SOHO)}
%\DeclareComet{C2009J8}{C/2009 J8}{C/2009 J8 (SOHO)}
%\DeclareComet{C2009J9}{C/2009 J9}{C/2009 J9 (SOHO)}
%\DeclareComet{C2009K10}{C/2009 K10}{C/2009 K10 (SOHO)}
%\DeclareComet{C2009K11}{C/2009 K11}{C/2009 K11 (SOHO)}
%\DeclareComet{C2009K12}{C/2009 K12}{C/2009 K12 (SOHO)}
%\DeclareComet{C2009K13}{C/2009 K13}{C/2009 K13 (SOHO)}
%\DeclareComet{C2009K14}{C/2009 K14}{C/2009 K14 (SOHO)}
%\DeclareComet{C2009K2}{C/2009 K2}{C/2009 K2 (Catalina)}
%\DeclareComet{C2009K3}{C/2009 K3}{C/2009 K3 (Beshore)}
%\DeclareComet{C2009K4}{C/2009 K4}{C/2009 K4 (Gibbs)}
%\DeclareComet{C2009K5}{C/2009 K5}{C/2009 K5 (McNaught)}
%\DeclareComet{C2009K6}{C/2009 K6}{C/2009 K6 (SOHO)}
%\DeclareComet{C2009K7}{C/2009 K7}{C/2009 K7 (SOHO)}
%\DeclareComet{C2009K8}{C/2009 K8}{C/2009 K8 (SOHO)}
%\DeclareComet{C2009K9}{C/2009 K9}{C/2009 K9 (SOHO)}
%\DeclareComet{C2009L10}{C/2009 L10}{C/2009 L10 (SOHO)}
%\DeclareComet{C2009L11}{C/2009 L11}{C/2009 L11 (SOHO)}
%\DeclareComet{C2009L12}{C/2009 L12}{C/2009 L12 (SOHO)}
%\DeclareComet{C2009L13}{C/2009 L13}{C/2009 L13 (SOHO)}
%\DeclareComet{C2009L14}{C/2009 L14}{C/2009 L14 (SOHO)}
%\DeclareComet{C2009L15}{C/2009 L15}{C/2009 L15 (SOHO)}
%\DeclareComet{C2009L16}{C/2009 L16}{C/2009 L16 (SOHO)}
%\DeclareComet{C2009L17}{C/2009 L17}{C/2009 L17 (SOHO)}
%\DeclareComet{C2009L3}{C/2009 L3}{C/2009 L3 (SOHO)}
%\DeclareComet{C2009L4}{C/2009 L4}{C/2009 L4 (SOHO)}
%\DeclareComet{C2009L5}{C/2009 L5}{C/2009 L5 (SOHO)}
%\DeclareComet{C2009L6}{C/2009 L6}{C/2009 L6 (SOHO)}
%\DeclareComet{C2009L7}{C/2009 L7}{C/2009 L7 (SOHO)}
%\DeclareComet{C2009L8}{C/2009 L8}{C/2009 L8 (SOHO)}
%\DeclareComet{C2009L9}{C/2009 L9}{C/2009 L9 (SOHO)}
%\DeclareComet{C2009M1}{C/2009 M1}{C/2009 M1 (SOHO)}
%\DeclareComet{C2009M2}{C/2009 M2}{C/2009 M2 (SOHO)}
%\DeclareComet{C2009M3}{C/2009 M3}{C/2009 M3 (SOHO)}
%\DeclareComet{C2009M4}{C/2009 M4}{C/2009 M4 (SOHO)}
%\DeclareComet{C2009M5}{C/2009 M5}{C/2009 M5 (SOHO)}
%\DeclareComet{C2009M6}{C/2009 M6}{C/2009 M6 (SOHO)}
%\DeclareComet{C2009M7}{C/2009 M7}{C/2009 M7 (SOHO)}
%\DeclareComet{C2009M8}{C/2009 M8}{C/2009 M8 (SOHO)}
%\DeclareComet{C2009N1}{C/2009 N1}{C/2009 N1 (SOHO)}
%\DeclareComet{C2009N2}{C/2009 N2}{C/2009 N2 (SOHO)}
%\DeclareComet{C2009N3}{C/2009 N3}{C/2009 N3 (SOHO)}
%\DeclareComet{C2009O1}{C/2009 O1}{C/2009 O1 (STEREO)}
%\DeclareComet{C2009O2}{C/2009 O2}{C/2009 O2 (Catalina)}
%\DeclareComet{C2009O4}{C/2009 O4}{C/2009 O4 (Hill)}
%\DeclareComet{C2009O5}{C/2009 O5}{C/2009 O5 (SOHO)}
%\DeclareComet{C2009P1}{C/2009 P1}{C/2009 P1 (Garradd)}
%\DeclareComet{C2009P2}{C/2009 P2}{C/2009 P2 (Boattini)}
%\DeclareComet{C2009P3}{C/2009 P3}{C/2009 P3 (SOHO)}
%\DeclareComet{C2009P4}{C/2009 P4}{C/2009 P4 (SOHO)}
%\DeclareComet{C2009P5}{C/2009 P5}{C/2009 P5 (SOHO)}
%\DeclareComet{C2009Q6}{C/2009 Q6}{C/2009 Q6 (SOHO)}
%\DeclareComet{C2009Q7}{C/2009 Q7}{C/2009 Q7 (SOHO)}
%\DeclareComet{C2009Q8}{C/2009 Q8}{C/2009 Q8 (SOHO)}
%\DeclareComet{C2009R1}{C/2009 R1}{C/2009 R1 (McNaught)}
%\DeclareComet{C2009R3}{C/2009 R3}{C/2009 R3 (SOHO)}
%\DeclareComet{C2009R4}{C/2009 R4}{C/2009 R4 (SOHO)}
%\DeclareComet{C2009R5}{C/2009 R5}{C/2009 R5 (SOHO)}
%\DeclareComet{C2009S10}{C/2009 S10}{C/2009 S10 (SOHO)}
%\DeclareComet{C2009S11}{C/2009 S11}{C/2009 S11 (SOHO)}
%\DeclareComet{C2009S12}{C/2009 S12}{C/2009 S12 (SOHO)}
%\DeclareComet{C2009S3}{C/2009 S3}{C/2009 S3 (Lemmon)}
%\DeclareComet{C2009S5}{C/2009 S5}{C/2009 S5 (SOHO)}
%\DeclareComet{C2009S6}{C/2009 S6}{C/2009 S6 (SOHO)}
%\DeclareComet{C2009S7}{C/2009 S7}{C/2009 S7 (SOHO)}
%\DeclareComet{C2009S8}{C/2009 S8}{C/2009 S8 (SOHO)}
%\DeclareComet{C2009S9}{C/2009 S9}{C/2009 S9 (SOHO)}
%\DeclareComet{C2009T1}{C/2009 T1}{C/2009 T1 (McNaught)}
%\DeclareComet{C2009T10}{C/2009 T10}{C/2009 T10 (SOHO)}
%\DeclareComet{C2009T11}{C/2009 T11}{C/2009 T11 (SOHO)}
%\DeclareComet{C2009T12}{C/2009 T12}{C/2009 T12 (SOHO)}
%\DeclareComet{C2009T13}{C/2009 T13}{C/2009 T13 (SOHO)}
%\DeclareComet{C2009T3}{C/2009 T3}{C/2009 T3 (LINEAR)}
%\DeclareComet{C2009T4}{C/2009 T4}{C/2009 T4 (SOHO)}
%\DeclareComet{C2009T5}{C/2009 T5}{C/2009 T5 (SOHO)}
%\DeclareComet{C2009T6}{C/2009 T6}{C/2009 T6 (SOHO)}
%\DeclareComet{C2009T7}{C/2009 T7}{C/2009 T7 (SOHO)}
%\DeclareComet{C2009T8}{C/2009 T8}{C/2009 T8 (SOHO)}
%\DeclareComet{C2009T9}{C/2009 T9}{C/2009 T9 (SOHO)}
%\DeclareComet{C2009U1}{C/2009 U1}{C/2009 U1 (Garradd)}
%\DeclareComet{C2009U10}{C/2009 U10}{C/2009 U10 (SOHO)}
%\DeclareComet{C2009U11}{C/2009 U11}{C/2009 U11 (SOHO)}
%\DeclareComet{C2009U12}{C/2009 U12}{C/2009 U12 (SOHO)}
%\DeclareComet{C2009U13}{C/2009 U13}{C/2009 U13 (SOHO)}
%\DeclareComet{C2009U14}{C/2009 U14}{C/2009 U14 (SOHO)}
%\DeclareComet{C2009U3}{C/2009 U3}{C/2009 U3 (Hill)}
%\DeclareComet{C2009U5}{C/2009 U5}{C/2009 U5 (Grauer)}
%\DeclareComet{C2009U7}{C/2009 U7}{C/2009 U7 (SOHO)}
%\DeclareComet{C2009U8}{C/2009 U8}{C/2009 U8 (SOHO)}
%\DeclareComet{C2009U9}{C/2009 U9}{C/2009 U9 (SOHO)}
%\DeclareComet{C2009UG89}{C/2009 UG89}{C/2009 UG89 (Lemmon)}
%\DeclareComet{C2009V1}{C/2009 V1}{C/2009 V1 (SOHO)}
%\DeclareComet{C2009V2}{C/2009 V2}{C/2009 V2 (SOHO)}
%\DeclareComet{C2009V3}{C/2009 V3}{C/2009 V3 (SOHO)}
%\DeclareComet{C2009V4}{C/2009 V4}{C/2009 V4 (SOHO)}
%\DeclareComet{C2009V5}{C/2009 V5}{C/2009 V5 (SOHO)}
%\DeclareComet{C2009V6}{C/2009 V6}{C/2009 V6 (SOHO)}
%\DeclareComet{C2009V7}{C/2009 V7}{C/2009 V7 (SOHO)}
%\DeclareComet{C2009W10}{C/2009 W10}{C/2009 W10 (SOHO)}
%\DeclareComet{C2009W11}{C/2009 W11}{C/2009 W11 (SOHO)}
%\DeclareComet{C2009W12}{C/2009 W12}{C/2009 W12 (SOHO)}
%\DeclareComet{C2009W13}{C/2009 W13}{C/2009 W13 (SOHO)}
%\DeclareComet{C2009W14}{C/2009 W14}{C/2009 W14 (SOHO)}
%\DeclareComet{C2009W15}{C/2009 W15}{C/2009 W15 (SOHO)}
%\DeclareComet{C2009W16}{C/2009 W16}{C/2009 W16 (SOHO)}
%\DeclareComet{C2009W2}{C/2009 W2}{C/2009 W2 (Boattini)}
%\DeclareComet{C2009W3}{C/2009 W3}{C/2009 W3 (SOHO)}
%\DeclareComet{C2009W4}{C/2009 W4}{C/2009 W4 (SOHO)}
%\DeclareComet{C2009W5}{C/2009 W5}{C/2009 W5 (SOHO)}
%\DeclareComet{C2009W6}{C/2009 W6}{C/2009 W6 (SOHO)}
%\DeclareComet{C2009W7}{C/2009 W7}{C/2009 W7 (SOHO)}
%\DeclareComet{C2009W8}{C/2009 W8}{C/2009 W8 (SOHO)}
%\DeclareComet{C2009W9}{C/2009 W9}{C/2009 W9 (SOHO)}
%\DeclareComet{C2009X10}{C/2009 X10}{C/2009 X10 (SOHO)}
%\DeclareComet{C2009X11}{C/2009 X11}{C/2009 X11 (SOHO)}
%\DeclareComet{C2009X12}{C/2009 X12}{C/2009 X12 (SOHO)}
%\DeclareComet{C2009X13}{C/2009 X13}{C/2009 X13 (SOHO)}
%\DeclareComet{C2009X14}{C/2009 X14}{C/2009 X14 (SOHO)}
%\DeclareComet{C2009X15}{C/2009 X15}{C/2009 X15 (SOHO)}
%\DeclareComet{C2009X16}{C/2009 X16}{C/2009 X16 (SOHO)}
%\DeclareComet{C2009X17}{C/2009 X17}{C/2009 X17 (SOHO)}
%\DeclareComet{C2009X2}{C/2009 X2}{C/2009 X2 (SOHO)}
%\DeclareComet{C2009X3}{C/2009 X3}{C/2009 X3 (SOHO)}
%\DeclareComet{C2009X4}{C/2009 X4}{C/2009 X4 (SOHO)}
%\DeclareComet{C2009X5}{C/2009 X5}{C/2009 X5 (SOHO)}
%\DeclareComet{C2009X6}{C/2009 X6}{C/2009 X6 (SOHO)}
%\DeclareComet{C2009X7}{C/2009 X7}{C/2009 X7 (SOHO)}
%\DeclareComet{C2009X8}{C/2009 X8}{C/2009 X8 (SOHO)}
%\DeclareComet{C2009X9}{C/2009 X9}{C/2009 X9 (SOHO)}
%\DeclareComet{C2009Y1}{C/2009 Y1}{C/2009 Y1 (Catalina)}
%\DeclareComet{C2009Y10}{C/2009 Y10}{C/2009 Y10 (SOHO)}
%\DeclareComet{C2009Y11}{C/2009 Y11}{C/2009 Y11 (SOHO)}
%\DeclareComet{C2009Y12}{C/2009 Y12}{C/2009 Y12 (SOHO)}
%\DeclareComet{C2009Y13}{C/2009 Y13}{C/2009 Y13 (SOHO)}
%\DeclareComet{C2009Y14}{C/2009 Y14}{C/2009 Y14 (SOHO)}
%\DeclareComet{C2009Y15}{C/2009 Y15}{C/2009 Y15 (STEREO)}
%\DeclareComet{C2009Y16}{C/2009 Y16}{C/2009 Y16 (STEREO)}
%\DeclareComet{C2009Y17}{C/2009 Y17}{C/2009 Y17 (STEREO)}
%\DeclareComet{C2009Y18}{C/2009 Y18}{C/2009 Y18 (SOHO)}
%\DeclareComet{C2009Y19}{C/2009 Y19}{C/2009 Y19 (SOHO)}
%\DeclareComet{C2009Y3}{C/2009 Y3}{C/2009 Y3 (STEREO)}
%\DeclareComet{C2009Y4}{C/2009 Y4}{C/2009 Y4 (STEREO)}
%\DeclareComet{C2009Y5}{C/2009 Y5}{C/2009 Y5 (SOHO)}
%\DeclareComet{C2009Y6}{C/2009 Y6}{C/2009 Y6 (SOHO)}
%\DeclareComet{C2009Y7}{C/2009 Y7}{C/2009 Y7 (SOHO)}
%\DeclareComet{C2009Y8}{C/2009 Y8}{C/2009 Y8 (SOHO)}
%\DeclareComet{C2009Y9}{C/2009 Y9}{C/2009 Y9 (SOHO)}
%\DeclareComet{C2010A10}{C/2010 A10}{C/2010 A10 (SOHO)}
%\DeclareComet{C2010A11}{C/2010 A11}{C/2010 A11 (SOHO)}
%\DeclareComet{C2010A12}{C/2010 A12}{C/2010 A12 (SOHO)}
%\DeclareComet{C2010A13}{C/2010 A13}{C/2010 A13 (STEREO)}
%\DeclareComet{C2010A14}{C/2010 A14}{C/2010 A14 (SOHO)}
%\DeclareComet{C2010A15}{C/2010 A15}{C/2010 A15 (SOHO)}
%\DeclareComet{C2010A16}{C/2010 A16}{C/2010 A16 (SOHO)}
%\DeclareComet{C2010A17}{C/2010 A17}{C/2010 A17 (SOHO)}
%\DeclareComet{C2010A18}{C/2010 A18}{C/2010 A18 (STEREO)}
%\DeclareComet{C2010A19}{C/2010 A19}{C/2010 A19 (STEREO)}
%\DeclareComet{C2010A20}{C/2010 A20}{C/2010 A20 (STEREO)}
%\DeclareComet{C2010A21}{C/2010 A21}{C/2010 A21 (STEREO)}
%\DeclareComet{C2010A22}{C/2010 A22}{C/2010 A22 (STEREO)}
%\DeclareComet{C2010A23}{C/2010 A23}{C/2010 A23 (STEREO)}
%\DeclareComet{C2010A4}{C/2010 A4}{C/2010 A4 (SidingSpring)}
%\DeclareComet{C2010A6}{C/2010 A6}{C/2010 A6 (SOHO)}
%\DeclareComet{C2010A7}{C/2010 A7}{C/2010 A7 (SOHO)}
%\DeclareComet{C2010A8}{C/2010 A8}{C/2010 A8 (SOHO)}
%\DeclareComet{C2010A9}{C/2010 A9}{C/2010 A9 (SOHO)}
%\DeclareComet{C2010B1}{C/2010 B1}{C/2010 B1 (Cardinal)}
%\DeclareComet{C2010B10}{C/2010 B10}{C/2010 B10 (SOHO)}
%\DeclareComet{C2010B11}{C/2010 B11}{C/2010 B11 (SOHO)}
%\DeclareComet{C2010B12}{C/2010 B12}{C/2010 B12 (SOHO)}
%\DeclareComet{C2010B13}{C/2010 B13}{C/2010 B13 (SOHO)}
%\DeclareComet{C2010B3}{C/2010 B3}{C/2010 B3 (STEREO)}
%\DeclareComet{C2010B4}{C/2010 B4}{C/2010 B4 (STEREO)}
%\DeclareComet{C2010B5}{C/2010 B5}{C/2010 B5 (STEREO)}
%\DeclareComet{C2010B6}{C/2010 B6}{C/2010 B6 (SOHO)}
%\DeclareComet{C2010B7}{C/2010 B7}{C/2010 B7 (SOHO)}
%\DeclareComet{C2010B8}{C/2010 B8}{C/2010 B8 (SOHO)}
%\DeclareComet{C2010B9}{C/2010 B9}{C/2010 B9 (SOHO)}
%\DeclareComet{C2010C3}{C/2010 C3}{C/2010 C3 (SOHO)}
%\DeclareComet{C2010C4}{C/2010 C4}{C/2010 C4 (SOHO)}
%\DeclareComet{C2010C5}{C/2010 C5}{C/2010 C5 (SOHO)}
%\DeclareComet{C2010C6}{C/2010 C6}{C/2010 C6 (SOHO)}
%\DeclareComet{C2010C7}{C/2010 C7}{C/2010 C7 (SOHO)}
%\DeclareComet{C2010C8}{C/2010 C8}{C/2010 C8 (SOHO)}
%\DeclareComet{C2010D3}{C/2010 D3}{C/2010 D3 (WISE)}
%\DeclareComet{C2010D4}{C/2010 D4}{C/2010 D4 (WISE)}
%\DeclareComet{C2010D5}{C/2010 D5}{C/2010 D5 (SOHO)}
%\DeclareComet{C2010D6}{C/2010 D6}{C/2010 D6 (SOHO)}
%\DeclareComet{C2010D7}{C/2010 D7}{C/2010 D7 (SOHO)}
%\DeclareComet{C2010D8}{C/2010 D8}{C/2010 D8 (SOHO)}
%\DeclareComet{C2010DG56}{C/2010 DG56}{C/2010 DG56 (WISE)}
%\DeclareComet{C2010E1}{C/2010 E1}{C/2010 E1 (Garradd)}
%\DeclareComet{C2010E10}{C/2010 E10}{C/2010 E10 (SOHO)}
%\DeclareComet{C2010E11}{C/2010 E11}{C/2010 E11 (SOHO)}
%\DeclareComet{C2010E12}{C/2010 E12}{C/2010 E12 (SOHO)}
%\DeclareComet{C2010E13}{C/2010 E13}{C/2010 E13 (SOHO)}
%\DeclareComet{C2010E3}{C/2010 E3}{C/2010 E3 (WISE)}
%\DeclareComet{C2010E5}{C/2010 E5}{C/2010 E5 (Scotti)}
%\DeclareComet{C2010E6}{C/2010 E6}{C/2010 E6 (STEREO)}
%\DeclareComet{C2010E7}{C/2010 E7}{C/2010 E7 (SOHO)}
%\DeclareComet{C2010E8}{C/2010 E8}{C/2010 E8 (SOHO)}
%\DeclareComet{C2010E9}{C/2010 E9}{C/2010 E9 (SOHO)}
%\DeclareComet{C2010F1}{C/2010 F1}{C/2010 F1 (Boattini)}
%\DeclareComet{C2010F10}{C/2010 F10}{C/2010 F10 (SOHO)}
%\DeclareComet{C2010F11}{C/2010 F11}{C/2010 F11 (SOHO)}
%\DeclareComet{C2010F3}{C/2010 F3}{C/2010 F3 (Scotti)}
%\DeclareComet{C2010F4}{C/2010 F4}{C/2010 F4 (Machholz)}
%\DeclareComet{C2010F5}{C/2010 F5}{C/2010 F5 (SOHO)}
%\DeclareComet{C2010F6}{C/2010 F6}{C/2010 F6 (SOHO)}
%\DeclareComet{C2010F7}{C/2010 F7}{C/2010 F7 (SOHO)}
%\DeclareComet{C2010F8}{C/2010 F8}{C/2010 F8 (SOHO)}
%\DeclareComet{C2010F9}{C/2010 F9}{C/2010 F9 (SOHO)}
%\DeclareComet{C2010FB87}{C/2010 FB87}{C/2010 FB87 (WISE-Garradd)}
%\DeclareComet{C2010G1}{C/2010 G1}{C/2010 G1 (Boattini)}
%\DeclareComet{C2010G2}{C/2010 G2}{C/2010 G2 (Hill)}
%\DeclareComet{C2010G3}{C/2010 G3}{C/2010 G3 (WISE)}
%\DeclareComet{C2010G4}{C/2010 G4}{C/2010 G4 (SOHO)}
%\DeclareComet{C2010G5}{C/2010 G5}{C/2010 G5 (SOHO)}
%\DeclareComet{C2010G6}{C/2010 G6}{C/2010 G6 (SOHO)}
%\DeclareComet{C2010H1}{C/2010 H1}{C/2010 H1 (Garradd)}
%\DeclareComet{C2010H10}{C/2010 H10}{C/2010 H10 (SOHO)}
%\DeclareComet{C2010H11}{C/2010 H11}{C/2010 H11 (SOHO)}
%\DeclareComet{C2010H12}{C/2010 H12}{C/2010 H12 (SOHO)}
%\DeclareComet{C2010H6}{C/2010 H6}{C/2010 H6 (SOHO)}
%\DeclareComet{C2010H7}{C/2010 H7}{C/2010 H7 (SOHO)}
%\DeclareComet{C2010H8}{C/2010 H8}{C/2010 H8 (SOHO)}
%\DeclareComet{C2010H9}{C/2010 H9}{C/2010 H9 (SOHO)}
%\DeclareComet{C2010J1}{C/2010 J1}{C/2010 J1 (Boattini)}
%\DeclareComet{C2010J10}{C/2010 J10}{C/2010 J10 (SOHO)}
%\DeclareComet{C2010J11}{C/2010 J11}{C/2010 J11 (SOHO)}
%\DeclareComet{C2010J12}{C/2010 J12}{C/2010 J12 (SOHO)}
%\DeclareComet{C2010J13}{C/2010 J13}{C/2010 J13 (SOHO)}
%\DeclareComet{C2010J14}{C/2010 J14}{C/2010 J14 (SOHO)}
%\DeclareComet{C2010J15}{C/2010 J15}{C/2010 J15 (SOHO)}
%\DeclareComet{C2010J16}{C/2010 J16}{C/2010 J16 (SOHO)}
%\DeclareComet{C2010J2}{C/2010 J2}{C/2010 J2 (McNaught)}
%\DeclareComet{C2010J4}{C/2010 J4}{C/2010 J4 (WISE)}
%\DeclareComet{C2010J6}{C/2010 J6}{C/2010 J6 (SOHO)}
%\DeclareComet{C2010J7}{C/2010 J7}{C/2010 J7 (SOHO)}
%\DeclareComet{C2010J8}{C/2010 J8}{C/2010 J8 (SOHO)}
%\DeclareComet{C2010J9}{C/2010 J9}{C/2010 J9 (SOHO)}
%\DeclareComet{C2010K10}{C/2010 K10}{C/2010 K10 (SOHO)}
%\DeclareComet{C2010K11}{C/2010 K11}{C/2010 K11 (SOHO)}
%\DeclareComet{C2010K12}{C/2010 K12}{C/2010 K12 (SOHO)}
%\DeclareComet{C2010K3}{C/2010 K3}{C/2010 K3 (SOHO)}
%\DeclareComet{C2010K4}{C/2010 K4}{C/2010 K4 (SOHO)}
%\DeclareComet{C2010K5}{C/2010 K5}{C/2010 K5 (SOHO)}
%\DeclareComet{C2010K6}{C/2010 K6}{C/2010 K6 (SOHO)}
%\DeclareComet{C2010K7}{C/2010 K7}{C/2010 K7 (SOHO)}
%\DeclareComet{C2010K8}{C/2010 K8}{C/2010 K8 (SOHO)}
%\DeclareComet{C2010K9}{C/2010 K9}{C/2010 K9 (SOHO)}
%\DeclareComet{C2010KW7}{C/2010 KW7}{C/2010 KW7 (WISE)}
%\DeclareComet{C2010L10}{C/2010 L10}{C/2010 L10 (SOHO)}
%\DeclareComet{C2010L11}{C/2010 L11}{C/2010 L11 (SOHO)}
%\DeclareComet{C2010L12}{C/2010 L12}{C/2010 L12 (SOHO)}
%\DeclareComet{C2010L13}{C/2010 L13}{C/2010 L13 (SOHO)}
%\DeclareComet{C2010L14}{C/2010 L14}{C/2010 L14 (SOHO)}
%\DeclareComet{C2010L15}{C/2010 L15}{C/2010 L15 (SOHO)}
%\DeclareComet{C2010L16}{C/2010 L16}{C/2010 L16 (SOHO)}
%\DeclareComet{C2010L17}{C/2010 L17}{C/2010 L17 (SOHO)}
%\DeclareComet{C2010L18}{C/2010 L18}{C/2010 L18 (SOHO)}
%\DeclareComet{C2010L19}{C/2010 L19}{C/2010 L19 (SOHO)}
%\DeclareComet{C2010L3}{C/2010 L3}{C/2010 L3 (Catalina)}
%\DeclareComet{C2010L4}{C/2010 L4}{C/2010 L4 (WISE)}
%\DeclareComet{C2010L5}{C/2010 L5}{C/2010 L5 (WISE)}
%\DeclareComet{C2010L6}{C/2010 L6}{C/2010 L6 (SOHO)}
%\DeclareComet{C2010L7}{C/2010 L7}{C/2010 L7 (SOHO)}
%\DeclareComet{C2010L8}{C/2010 L8}{C/2010 L8 (SOHO)}
%\DeclareComet{C2010L9}{C/2010 L9}{C/2010 L9 (SOHO)}
%\DeclareComet{C2010M1}{C/2010 M1}{C/2010 M1 (Gibbs)}
%\DeclareComet{C2010M2}{C/2010 M2}{C/2010 M2 (SOHO)}
%\DeclareComet{C2010M3}{C/2010 M3}{C/2010 M3 (SOHO)}
%\DeclareComet{C2010M4}{C/2010 M4}{C/2010 M4 (SOHO)}
%\DeclareComet{C2010M5}{C/2010 M5}{C/2010 M5 (SOHO)}
%\DeclareComet{C2010M6}{C/2010 M6}{C/2010 M6 (SOHO)}
%\DeclareComet{C2010M7}{C/2010 M7}{C/2010 M7 (SOHO)}
%\DeclareComet{C2010M8}{C/2010 M8}{C/2010 M8 (SOHO)}
%\DeclareComet{C2010N3}{C/2010 N3}{C/2010 N3 (SOHO)}
%\DeclareComet{C2010N4}{C/2010 N4}{C/2010 N4 (SOHO)}
%\DeclareComet{C2010N5}{C/2010 N5}{C/2010 N5 (SOHO)}
%\DeclareComet{C2010O1}{C/2010 O1}{C/2010 O1 (SOHO)}
%\DeclareComet{C2010O2}{C/2010 O2}{C/2010 O2 (SOHO)}
%\DeclareComet{C2010O3}{C/2010 O3}{C/2010 O3 (SOHO)}
%\DeclareComet{C2010O4}{C/2010 O4}{C/2010 O4 (SOHO)}
%\DeclareComet{C2010O5}{C/2010 O5}{C/2010 O5 (SOHO)}
%\DeclareComet{C2010O6}{C/2010 O6}{C/2010 O6 (SOHO)}
%\DeclareComet{C2010O7}{C/2010 O7}{C/2010 O7 (SOHO)}
%\DeclareComet{C2010P6}{C/2010 P6}{C/2010 P6 (SOHO)}
%\DeclareComet{C2010P7}{C/2010 P7}{C/2010 P7 (SOHO)}
%\DeclareComet{C2010P8}{C/2010 P8}{C/2010 P8 (SOHO)}
%\DeclareComet{C2010P9}{C/2010 P9}{C/2010 P9 (SOHO)}
%\DeclareComet{C2010Q2}{C/2010 Q2}{C/2010 Q2 (SOHO)}
%\DeclareComet{C2010Q3}{C/2010 Q3}{C/2010 Q3 (SOHO)}
%\DeclareComet{C2010R1}{C/2010 R1}{C/2010 R1 (LINEAR)}
%\DeclareComet{C2010R3}{C/2010 R3}{C/2010 R3 (SOHO)}
%\DeclareComet{C2010R4}{C/2010 R4}{C/2010 R4 (SOHO)}
%\DeclareComet{C2010R5}{C/2010 R5}{C/2010 R5 (SOHO)}
%\DeclareComet{C2010R6}{C/2010 R6}{C/2010 R6 (SOHO)}
%\DeclareComet{C2010S1}{C/2010 S1}{C/2010 S1 (LINEAR)}
%\DeclareComet{C2010S2}{C/2010 S2}{C/2010 S2 (SOHO)}
%\DeclareComet{C2010S3}{C/2010 S3}{C/2010 S3 (SOHO)}
%\DeclareComet{C2010S4}{C/2010 S4}{C/2010 S4 (SOHO)}
%\DeclareComet{C2010S5}{C/2010 S5}{C/2010 S5 (SOHO)}
%\DeclareComet{C2010S6}{C/2010 S6}{C/2010 S6 (SOHO)}
%\DeclareComet{C2010S7}{C/2010 S7}{C/2010 S7 (SOHO)}
%\DeclareComet{C2010S8}{C/2010 S8}{C/2010 S8 (SOHO)}
%\DeclareComet{C2010S9}{C/2010 S9}{C/2010 S9 (SOHO)}
%\DeclareComet{C2010T3}{C/2010 T3}{C/2010 T3 (SOHO)}
%\DeclareComet{C2010T4}{C/2010 T4}{C/2010 T4 (SOHO)}
%\DeclareComet{C2010T5}{C/2010 T5}{C/2010 T5 (SOHO)}
%\DeclareComet{C2010T6}{C/2010 T6}{C/2010 T6 (SOHO)}
%\DeclareComet{C2010T7}{C/2010 T7}{C/2010 T7 (SOHO)}
%\DeclareComet{C2010U10}{C/2010 U10}{C/2010 U10 (SOHO)}
%\DeclareComet{C2010U11}{C/2010 U11}{C/2010 U11 (SOHO)}
%\DeclareComet{C2010U12}{C/2010 U12}{C/2010 U12 (SOHO)}
%\DeclareComet{C2010U3}{C/2010 U3}{C/2010 U3 (Boattini)}
%\DeclareComet{C2010U4}{C/2010 U4}{C/2010 U4 (SOHO)}
%\DeclareComet{C2010U5}{C/2010 U5}{C/2010 U5 (SOHO)}
%\DeclareComet{C2010U6}{C/2010 U6}{C/2010 U6 (SOHO)}
%\DeclareComet{C2010U7}{C/2010 U7}{C/2010 U7 (SOHO)}
%\DeclareComet{C2010U8}{C/2010 U8}{C/2010 U8 (SOHO)}
%\DeclareComet{C2010U9}{C/2010 U9}{C/2010 U9 (SOHO)}
%\DeclareComet{C2010V10}{C/2010 V10}{C/2010 V10 (SOHO)}
%\DeclareComet{C2010V11}{C/2010 V11}{C/2010 V11 (SOHO)}
%\DeclareComet{C2010V4}{C/2010 V4}{C/2010 V4 (SOHO)}
%\DeclareComet{C2010V5}{C/2010 V5}{C/2010 V5 (SOHO)}
%\DeclareComet{C2010V6}{C/2010 V6}{C/2010 V6 (SOHO)}
%\DeclareComet{C2010V7}{C/2010 V7}{C/2010 V7 (SOHO)}
%\DeclareComet{C2010V8}{C/2010 V8}{C/2010 V8 (SOHO)}
%\DeclareComet{C2010V9}{C/2010 V9}{C/2010 V9 (SOHO)}
%\DeclareComet{C2010W2}{C/2010 W2}{C/2010 W2 (SOHO)}
%\DeclareComet{C2010W3}{C/2010 W3}{C/2010 W3 (SOHO)}
%\DeclareComet{C2010W4}{C/2010 W4}{C/2010 W4 (SOHO)}
%\DeclareComet{C2010W5}{C/2010 W5}{C/2010 W5 (SOHO)}
%\DeclareComet{C2010W6}{C/2010 W6}{C/2010 W6 (SOHO)}
%\DeclareComet{C2010W7}{C/2010 W7}{C/2010 W7 (SOHO)}
%\DeclareComet{C2010W8}{C/2010 W8}{C/2010 W8 (SOHO)}
%\DeclareComet{C2010W9}{C/2010 W9}{C/2010 W9 (SOHO)}
%\DeclareComet{C2010X1}{C/2010 X1}{C/2010 X1 (Elenin)}
%\DeclareComet{C2010X10}{C/2010 X10}{C/2010 X10 (SOHO)}
%\DeclareComet{C2010X11}{C/2010 X11}{C/2010 X11 (SOHO)}
%\DeclareComet{C2010X12}{C/2010 X12}{C/2010 X12 (SOHO)}
%\DeclareComet{C2010X13}{C/2010 X13}{C/2010 X13 (SOHO)}
%\DeclareComet{C2010X14}{C/2010 X14}{C/2010 X14 (SOHO)}
%\DeclareComet{C2010X15}{C/2010 X15}{C/2010 X15 (SOHO)}
%\DeclareComet{C2010X16}{C/2010 X16}{C/2010 X16 (SOHO)}
%\DeclareComet{C2010X17}{C/2010 X17}{C/2010 X17 (SOHO)}
%\DeclareComet{C2010X2}{C/2010 X2}{C/2010 X2 (SOHO)}
%\DeclareComet{C2010X3}{C/2010 X3}{C/2010 X3 (SOHO)}
%\DeclareComet{C2010X4}{C/2010 X4}{C/2010 X4 (SOHO)}
%\DeclareComet{C2010X5}{C/2010 X5}{C/2010 X5 (SOHO)}
%\DeclareComet{C2010X6}{C/2010 X6}{C/2010 X6 (SOHO)}
%\DeclareComet{C2010X7}{C/2010 X7}{C/2010 X7 (SOHO)}
%\DeclareComet{C2010X8}{C/2010 X8}{C/2010 X8 (SOHO)}
%\DeclareComet{C2010X9}{C/2010 X9}{C/2010 X9 (SOHO)}
%\DeclareComet{C2010Y1}{C/2010 Y1}{C/2010 Y1 (SOHO)}
%\DeclareComet{C2010Y10}{C/2010 Y10}{C/2010 Y10 (SOHO)}
%\DeclareComet{C2010Y11}{C/2010 Y11}{C/2010 Y11 (SOHO)}
%\DeclareComet{C2010Y12}{C/2010 Y12}{C/2010 Y12 (SOHO)}
%\DeclareComet{C2010Y13}{C/2010 Y13}{C/2010 Y13 (SOHO)}
%\DeclareComet{C2010Y14}{C/2010 Y14}{C/2010 Y14 (SOHO)}
%\DeclareComet{C2010Y15}{C/2010 Y15}{C/2010 Y15 (SOHO)}
%\DeclareComet{C2010Y16}{C/2010 Y16}{C/2010 Y16 (SOHO)}
%\DeclareComet{C2010Y17}{C/2010 Y17}{C/2010 Y17 (SOHO)}
%\DeclareComet{C2010Y18}{C/2010 Y18}{C/2010 Y18 (SOHO)}
%\DeclareComet{C2010Y19}{C/2010 Y19}{C/2010 Y19 (SOHO)}
%\DeclareComet{C2010Y2}{C/2010 Y2}{C/2010 Y2 (SOHO)}
%\DeclareComet{C2010Y20}{C/2010 Y20}{C/2010 Y20 (SOHO)}
%\DeclareComet{C2010Y3}{C/2010 Y3}{C/2010 Y3 (SOHO)}
%\DeclareComet{C2010Y4}{C/2010 Y4}{C/2010 Y4 (SOHO)}
%\DeclareComet{C2010Y5}{C/2010 Y5}{C/2010 Y5 (SOHO)}
%\DeclareComet{C2010Y6}{C/2010 Y6}{C/2010 Y6 (SOHO)}
%\DeclareComet{C2010Y7}{C/2010 Y7}{C/2010 Y7 (SOHO)}
%\DeclareComet{C2010Y8}{C/2010 Y8}{C/2010 Y8 (SOHO)}
%\DeclareComet{C2010Y9}{C/2010 Y9}{C/2010 Y9 (SOHO)}
%\DeclareComet{C2011A3}{C/2011 A3}{C/2011 A3 (Gibbs)}
%\DeclareComet{C2011B1}{C/2011 B1}{C/2011 B1 (SOHO)}
%\DeclareComet{C2011C1}{C/2011 C1}{C/2011 C1 (McNaught)}
%\DeclareComet{C2011C3}{C/2011 C3}{C/2011 C3 (Gibbs)}
%\DeclareComet{C2011F1}{C/2011 F1}{C/2011 F1 (LINEAR)}
%\DeclareComet{C2011G1}{C/2011 G1}{C/2011 G1 (McNaught)}
%\DeclareComet{C2011J2}{C/2011 J2}{C/2011 J2 (LINEAR)}
%\DeclareComet{C2011J2-B}{C/2011 J2-B}{C/2011 J2-B}
%\DeclareComet{C2011J2-C}{C/2011 J2-C}{C/2011 J2-C}
%\DeclareComet{C2011J3}{C/2011 J3}{C/2011 J3 (LINEAR)}
%\DeclareComet{C2011K1}{C/2011 K1}{C/2011 K1 (Schwartz-Holvorcem)}
%\DeclareComet{C2011KP36}{C/2011 KP36}{C/2011 KP36 (Spacewatch)}
%\DeclareComet{C2011L1}{C/2011 L1}{C/2011 L1 (McNaught)}
%\DeclareComet{C2011L2}{C/2011 L2}{C/2011 L2 (McNaught)}
%\DeclareComet{C2011L3}{C/2011 L3}{C/2011 L3 (McNaught)}
%\DeclareComet{C2011L4}{C/2011 L4}{C/2011 L4 (PANSTARRS)}
%\DeclareComet{C2011L6}{C/2011 L6}{C/2011 L6 (Boattini)}
%\DeclareComet{C2011M1}{C/2011 M1}{C/2011 M1 (LINEAR)}
%\DeclareComet{C2011N2}{C/2011 N2}{C/2011 N2 (McNaught)}
%\DeclareComet{C2011N3}{C/2011 N3}{C/2011 N3 (SOHO)}
%\DeclareComet{C2011O1}{C/2011 O1}{C/2011 O1 (LINEAR)}
%\DeclareComet{C2011P2}{C/2011 P2}{C/2011 P2 (PANSTARRS)}
%\DeclareComet{C2011Q1}{C/2011 Q1}{C/2011 Q1 (PANSTARRS)}
%\DeclareComet{C2011Q2}{C/2011 Q2}{C/2011 Q2 (McNaught)}
%\DeclareComet{C2011Q4}{C/2011 Q4}{C/2011 Q4 (SWAN)}
%\DeclareComet{C2011R1}{C/2011 R1}{C/2011 R1 (McNaught)}
%\DeclareComet{C2011S2}{C/2011 S2}{C/2011 S2 (Kowalski)}
%\DeclareComet{C2011U3}{C/2011 U3}{C/2011 U3 (PANSTARRS)}
%\DeclareComet{C2011UF305}{C/2011 UF305}{C/2011 UF305 (LINEAR)}
%\DeclareComet{C2011W3}{C/2011 W3}{C/2011 W3 (Lovejoy)}
%\DeclareComet{C2011Y3}{C/2011 Y3}{C/2011 Y3 (Boattini)}
%\DeclareComet{C2012A1}{C/2012 A1}{C/2012 A1 (PANSTARRS)}
%\DeclareComet{C2012A2}{C/2012 A2}{C/2012 A2 (LINEAR)}
%\DeclareComet{C2012B3}{C/2012 B3}{C/2012 B3 (LaSagra)}
%\DeclareComet{C2012BJ98}{C/2012 BJ98}{C/2012 BJ98 (Lemmon)}
%\DeclareComet{C2012C1}{C/2012 C1}{C/2012 C1 (McNaught)}
%\DeclareComet{C2012C2}{C/2012 C2}{C/2012 C2 (Bruenjes)}
%\DeclareComet{C2012CH17}{C/2012 CH17}{C/2012 CH17 (MOSS)}
%\DeclareComet{C2012E1}{C/2012 E1}{C/2012 E1 (Hill)}
%\DeclareComet{C2012E2}{C/2012 E2}{C/2012 E2 (SWAN)}
%\DeclareComet{C2012E3}{C/2012 E3}{C/2012 E3 (PANSTARRS)}
%\DeclareComet{C2012F1}{C/2012 F1}{C/2012 F1 (Gibbs)}
%\DeclareComet{C2012F3}{C/2012 F3}{C/2012 F3 (PANSTARRS)}
%\DeclareComet{C2012F6}{C/2012 F6}{C/2012 F6 (Lemmon)}
%\DeclareComet{C2012H2}{C/2012 H2}{C/2012 H2 (McNaught)}
%\DeclareComet{C2012J1}{C/2012 J1}{C/2012 J1 (Catalina)}
%\DeclareComet{C2012K1}{C/2012 K1}{C/2012 K1 (PANSTARRS)}
%\DeclareComet{C2012K5}{C/2012 K5}{C/2012 K5 (LINEAR)}
%\DeclareComet{C2012K6}{C/2012 K6}{C/2012 K6 (McNaught)}
%\DeclareComet{C2012K8}{C/2012 K8}{C/2012 K8 (Lemmon)}
%\DeclareComet{C2012KA51}{C/2012 KA51}{C/2012 KA51 (Palomar)}
%\DeclareComet{C2012L1}{C/2012 L1}{C/2012 L1 (LINEAR)}
%\DeclareComet{C2012L2}{C/2012 L2}{C/2012 L2 (LINEAR)}
%\DeclareComet{C2012L3}{C/2012 L3}{C/2012 L3 (LINEAR)}
%\DeclareComet{C2012LP26}{C/2012 LP26}{C/2012 LP26 (Palomar)}
%\DeclareComet{C2012OP}{C/2012 OP}{C/2012 OP (SidingSpring)}
%\DeclareComet{C2012Q1}{C/2012 Q1}{C/2012 Q1 (Kowalski)}
%\DeclareComet{C2012S1}{C/2012 S1}{C/2012 S1 (ISON)}
%\DeclareComet{C2012S3}{C/2012 S3}{C/2012 S3 (PANSTARRS)}
%\DeclareComet{C2012S4}{C/2012 S4}{C/2012 S4 (PANSTARRS)}
%\DeclareComet{C2012T4}{C/2012 T4}{C/2012 T4 (McNaught)}
%\DeclareComet{C2012T5}{C/2012 T5}{C/2012 T5 (Bressi)}
%\DeclareComet{C2012T6}{C/2012 T6}{C/2012 T6 (Kowalski)}
%\DeclareComet{C2012U1}{C/2012 U1}{C/2012 U1 (PANSTARRS)}
%\DeclareComet{C2012U3}{C/2012 U3}{C/2012 U3 (STEREO)}
%\DeclareComet{C2012V1}{C/2012 V1}{C/2012 V1 (PANSTARRS)}
%\DeclareComet{C2012V2}{C/2012 V2}{C/2012 V2 (LINEAR)}
%\DeclareComet{C2012X1}{C/2012 X1}{C/2012 X1 (LINEAR)}
%\DeclareComet{C2012X2}{C/2012 X2}{C/2012 X2 (PANSTARRS)}
%\DeclareComet{C2012Y1}{C/2012 Y1}{C/2012 Y1 (LINEAR)}
%\DeclareComet{C2012Y3}{C/2012 Y3}{C/2012 Y3 (McNaught)}
%\DeclareComet{C2013A1}{C/2013 A1}{C/2013 A1 (SidingSpring)}
%\DeclareComet{C2013B2}{C/2013 B2}{C/2013 B2 (Catalina)}
%\DeclareComet{C2013C2}{C/2013 C2}{C/2013 C2 (Tenagra)}
%\DeclareComet{C2013D1}{C/2013 D1}{C/2013 D1 (Holvorcem)}
%\DeclareComet{C2013E1}{C/2013 E1}{C/2013 E1 (McNaught)}
%\DeclareComet{C2013E2}{C/2013 E2}{C/2013 E2 (Iwamoto)}
%\DeclareComet{C2013E3}{C/2013 E3}{C/2013 E3 (STEREO)}
%\DeclareComet{C2013F1}{C/2013 F1}{C/2013 F1 (Boattini)}
%\DeclareComet{C2013F2}{C/2013 F2}{C/2013 F2 (Catalina)}
%\DeclareComet{C2013F3}{C/2013 F3}{C/2013 F3 (McNaught)}
%\DeclareComet{C2013F4}{C/2013 F4}{C/2013 F4 (STEREO)}
%\DeclareComet{C2013F5}{C/2013 F5}{C/2013 F5 (STEREO)}
%\DeclareComet{C2013G2}{C/2013 G2}{C/2013 G2 (McNaught)}
%\DeclareComet{C2013G3}{C/2013 G3}{C/2013 G3 (PANSTARRS)}
%\DeclareComet{C2013G5}{C/2013 G5}{C/2013 G5 (Catalina)}
%\DeclareComet{C2013G6}{C/2013 G6}{C/2013 G6 (Lemmon)}
%\DeclareComet{C2013G7}{C/2013 G7}{C/2013 G7 (McNaught)}
%\DeclareComet{C2013G8}{C/2013 G8}{C/2013 G8 (PANSTARRS)}
%\DeclareComet{C2013G9}{C/2013 G9}{C/2013 G9 (Tenagra)}
%\DeclareComet{C2013H1}{C/2013 H1}{C/2013 H1 (LaSagra)}
%\DeclareComet{C2013H2}{C/2013 H2}{C/2013 H2 (Boattini)}
%\DeclareComet{C2013J3}{C/2013 J3}{C/2013 J3 (McNaught)}
%\DeclareComet{C2013J5}{C/2013 J5}{C/2013 J5 (Boattini)}
%\DeclareComet{C2013J6}{C/2013 J6}{C/2013 J6 (Catalina)}
%\DeclareComet{C2013K1}{C/2013 K1}{C/2013 K1 (Christensen)}
%\DeclareComet{C2013L2}{C/2013 L2}{C/2013 L2 (Catalina)}
%\DeclareComet{C2013N4}{C/2013 N4}{C/2013 N4 (Borisov)}
%\DeclareComet{C2013O3}{C/2013 O3}{C/2013 O3 (McNaught)}
%\DeclareComet{C2013P2}{C/2013 P2}{C/2013 P2 (PANSTARRS)}
%\DeclareComet{C2013P3}{C/2013 P3}{C/2013 P3 (Palomar)}
%\DeclareComet{C2013P4}{C/2013 P4}{C/2013 P4 (PANSTARRS)}
%\DeclareComet{C2013PE67}{C/2013 PE67}{C/2013 PE67 (Catalina-Spacewatch)}
%\DeclareComet{C2013R1}{C/2013 R1}{C/2013 R1 (Lovejoy)}
%\DeclareComet{C2013S1}{C/2013 S1}{C/2013 S1 (Catalina)}
%\DeclareComet{C2013TW5}{C/2013 TW5}{C/2013 TW5 (Spacewatch)}
%\DeclareComet{C2013U1}{C/2013 U1}{C/2013 U1 (Catalina)}
%\DeclareComet{C2013U2}{C/2013 U2}{C/2013 U2 (Holvorcem)}
%\DeclareComet{C2013UQ4}{C/2013 UQ4}{C/2013 UQ4 (Catalina)}
%\DeclareComet{C2013US10}{C/2013 US10}{C/2013 US10 (Catalina)}
%\DeclareComet{C2013V1}{C/2013 V1}{C/2013 V1 (Boattini)}
%\DeclareComet{C2013V2}{C/2013 V2}{C/2013 V2 (Borisov)}
%\DeclareComet{C2013V3}{C/2013 V3}{C/2013 V3 (Nevski)}
%\DeclareComet{C2013V4}{C/2013 V4}{C/2013 V4 (Catalina)}
%\DeclareComet{C2013V5}{C/2013 V5}{C/2013 V5 (Oukaimeden)}
%\DeclareComet{C2013W2}{C/2013 W2}{C/2013 W2 (PANSTARRS)}
%\DeclareComet{C2013X1}{C/2013 X1}{C/2013 X1 (PANSTARRS)}
%\DeclareComet{C2013Y2}{C/2013 Y2}{C/2013 Y2 (PANSTARRS)}
%\DeclareComet{C2014A4}{C/2014 A4}{C/2014 A4 (SONEAR)}
%\DeclareComet{C2014A5}{C/2014 A5}{C/2014 A5 (PANSTARRS)}
%\DeclareComet{C2014AA52}{C/2014 AA52}{C/2014 AA52 (Catalina)}
%\DeclareComet{C2014B1}{C/2014 B1}{C/2014 B1 (Schwartz)}
%\DeclareComet{C2014C2}{C/2014 C2}{C/2014 C2 (STEREO)}
%\DeclareComet{C2014C3}{C/2014 C3}{C/2014 C3 (NEOWISE)}
%\DeclareComet{C2014E2}{C/2014 E2}{C/2014 E2 (Jacques)}
%\DeclareComet{C2014F1}{C/2014 F1}{C/2014 F1 (Hill)}
%\DeclareComet{C2014F2}{C/2014 F2}{C/2014 F2 (Tenagra)}
%\DeclareComet{C2014F3}{C/2014 F3}{C/2014 F3 (Sheppard-Trujillo)}
%\DeclareComet{C2014G1}{C/2014 G1}{C/2014 G1 (PANSTARRS)}
%\DeclareComet{C2014G3}{C/2014 G3}{C/2014 G3 (PANSTARRS)}
%\DeclareComet{C2014H1}{C/2014 H1}{C/2014 H1 (Christensen)}
%\DeclareComet{C2014HU195}{C/2014 HU195}{C/2014 HU195 (Valdes-TOTAS)}
%\DeclareComet{C2014J1}{C/2014 J1}{C/2014 J1 (Catalina)}
%\DeclareComet{C2014L5}{C/2014 L5}{C/2014 L5 (Lemmon)}
%\DeclareComet{C2014M1}{C/2014 M1}{C/2014 M1 (PANSTARRS)}
%\DeclareComet{C2014M2}{C/2014 M2}{C/2014 M2 (Christensen)}
%\DeclareComet{C2014M3}{C/2014 M3}{C/2014 M3 (Catalina)}
%\DeclareComet{C2014N2}{C/2014 N2}{C/2014 N2 (PANSTARRS)}
%\DeclareComet{C2014N3}{C/2014 N3}{C/2014 N3 (NEOWISE)}
%\DeclareComet{C2014OE4}{C/2014 OE4}{C/2014 OE4 (PANSTARRS)}
%\DeclareComet{C2014OG392}{C/2014 OG392}{C/2014 OG392 (PANSTARRS)}
%\DeclareComet{C2014Q1}{C/2014 Q1}{C/2014 Q1 (PANSTARRS)}
%\DeclareComet{C2014Q2}{C/2014 Q2}{C/2014 Q2 (Lovejoy)}
%\DeclareComet{C2014Q3}{C/2014 Q3}{C/2014 Q3 (Borisov)}
%\DeclareComet{C2014Q6}{C/2014 Q6}{C/2014 Q6 (PANSTARRS)}
%\DeclareComet{C2014QU2}{C/2014 QU2}{C/2014 QU2 (PANSTARRS)}
%\DeclareComet{C2014R1}{C/2014 R1}{C/2014 R1 (Borisov)}
%\DeclareComet{C2014R3}{C/2014 R3}{C/2014 R3 (PANSTARRS)}
%\DeclareComet{C2014R4}{C/2014 R4}{C/2014 R4 (Gibbs)}
%\DeclareComet{C2014S1}{C/2014 S1}{C/2014 S1 (PANSTARRS)}
%\DeclareComet{C2014S2}{C/2014 S2}{C/2014 S2 (PANSTARRS)}
%\DeclareComet{C2014S3}{C/2014 S3}{C/2014 S3 (PANSTARRS)}
%\DeclareComet{C2014TG64}{C/2014 TG64}{C/2014 TG64 (Catalina)}
%\DeclareComet{C2014U3}{C/2014 U3}{C/2014 U3 (Kowalski)}
%\DeclareComet{C2014UN271}{C/2014 UN271}{C/2014 UN271 (Bernardinelli-Bernstein)}
%\DeclareComet{C2014W10}{C/2014 W10}{C/2014 W10 (PANSTARRS)}
%\DeclareComet{C2014W11}{C/2014 W11}{C/2014 W11 (PANSTARRS)}
%\DeclareComet{C2014W2}{C/2014 W2}{C/2014 W2 (PANSTARRS)}
%\DeclareComet{C2014W3}{C/2014 W3}{C/2014 W3 (PANSTARRS)}
%\DeclareComet{C2014W5}{C/2014 W5}{C/2014 W5 (Lemmon-PANSTARRS)}
%\DeclareComet{C2014W6}{C/2014 W6}{C/2014 W6 (Catalina)}
%\DeclareComet{C2014W7}{C/2014 W7}{C/2014 W7 (Christensen)}
%\DeclareComet{C2014W8}{C/2014 W8}{C/2014 W8 (PANSTARRS)}
%\DeclareComet{C2014W9}{C/2014 W9}{C/2014 W9 (PANSTARRS)}
%\DeclareComet{C2014XB8}{C/2014 XB8}{C/2014 XB8 (PANSTARRS)}
%\DeclareComet{C2014Y1}{C/2014 Y1}{C/2014 Y1 (PANSTARRS)}
%\DeclareComet{C2015A1}{C/2015 A1}{C/2015 A1 (PANSTARRS)}
%\DeclareComet{C2015A2}{C/2015 A2}{C/2015 A2 (PANSTARRS)}
%\DeclareComet{C2015B2}{C/2015 B2}{C/2015 B2 (PANSTARRS)}
%\DeclareComet{C2015C2}{C/2015 C2}{C/2015 C2 (SWAN)}
%\DeclareComet{C2015D1}{C/2015 D1}{C/2015 D1 (SOHO)}
%\DeclareComet{C2015D2}{C/2015 D2}{C/2015 D2 (PANSTARRS)}
%\DeclareComet{C2015D3}{C/2015 D3}{C/2015 D3 (PANSTARRS)}
%\DeclareComet{C2015D4}{C/2015 D4}{C/2015 D4 (Borisov)}
%\DeclareComet{C2015E61-B}{C/2015 E61-B}{C/2015 E61-B (PANSTARRS)}
%\DeclareComet{C2015ER61}{C/2015 ER61}{C/2015 ER61 (PANSTARRS)}
%\DeclareComet{C2015F2}{C/2015 F2}{C/2015 F2 (Polonia)}
%\DeclareComet{C2015F3}{C/2015 F3}{C/2015 F3 (SWAN)}
%\DeclareComet{C2015F4}{C/2015 F4}{C/2015 F4 (Jacques)}
%\DeclareComet{C2015F5}{C/2015 F5}{C/2015 F5 (SWAN-Xingming)}
%\DeclareComet{C2015G2}{C/2015 G2}{C/2015 G2 (MASTER)}
%\DeclareComet{C2015GX}{C/2015 GX}{C/2015 GX (PANSTARRS)}
%\DeclareComet{C2015H1}{C/2015 H1}{C/2015 H1 (Bressi)}
%\DeclareComet{C2015H2}{C/2015 H2}{C/2015 H2 (PANSTARRS)}
%\DeclareComet{C2015J1}{C/2015 J1}{C/2015 J1 (PANSTARRS)}
%\DeclareComet{C2015J2}{C/2015 J2}{C/2015 J2 (PANSTARRS)}
%\DeclareComet{C2015K1}{C/2015 K1}{C/2015 K1 (MASTER)}
%\DeclareComet{C2015K2}{C/2015 K2}{C/2015 K2 (PANSTARRS)}
%\DeclareComet{C2015K4}{C/2015 K4}{C/2015 K4 (PANSTARRS)}
%\DeclareComet{C2015K7}{C/2015 K7}{C/2015 K7 (COIAS)}
%\DeclareComet{C2015LC2}{C/2015 LC2}{C/2015 LC2 (PANSTARRS)}
%\DeclareComet{C2015M1}{C/2015 M1}{C/2015 M1 (PANSTARRS)}
%\DeclareComet{C2015M3}{C/2015 M3}{C/2015 M3 (PANSTARRS)}
%\DeclareComet{C2015O1}{C/2015 O1}{C/2015 O1 (PANSTARRS)}
%\DeclareComet{C2015P3}{C/2015 P3}{C/2015 P3 (SWAN)}
%\DeclareComet{C2015R3}{C/2015 R3}{C/2015 R3 (PANSTARRS)}
%\DeclareComet{C2015T2}{C/2015 T2}{C/2015 T2 (PANSTARRS)}
%\DeclareComet{C2015T4}{C/2015 T4}{C/2015 T4 (PANSTARRS)}
%\DeclareComet{C2015T5}{C/2015 T5}{C/2015 T5 (Sheppard-Tholen)}
%\DeclareComet{C2015TQ209}{C/2015 TQ209}{C/2015 TQ209 (LINEAR)}
%\DeclareComet{C2015V1}{C/2015 V1}{C/2015 V1 (PANSTARRS)}
%\DeclareComet{C2015V2}{C/2015 V2}{C/2015 V2 (Johnson)}
%\DeclareComet{C2015V3}{C/2015 V3}{C/2015 V3 (PANSTARRS)}
%\DeclareComet{C2015V4}{C/2015 V4}{C/2015 V4 (PANSTARRS)}
%\DeclareComet{C2015VL62}{C/2015 VL62}{C/2015 VL62 (Lemmon-Yeung-PANSTARRS)}
%\DeclareComet{C2015W1}{C/2015 W1}{C/2015 W1 (Gibbs)}
%\DeclareComet{C2015WZ}{C/2015 WZ}{C/2015 WZ (PANSTARRS)}
%\DeclareComet{C2015X2}{C/2015 X2}{C/2015 X2 (Catalina)}
%\DeclareComet{C2015X4}{C/2015 X4}{C/2015 X4 (Elenin)}
%\DeclareComet{C2015X5}{C/2015 X5}{C/2015 X5 (PANSTARRS)}
%\DeclareComet{C2015X7}{C/2015 X7}{C/2015 X7 (ATLAS)}
%\DeclareComet{C2015X8}{C/2015 X8}{C/2015 X8 (NEOWISE)}
%\DeclareComet{C2015XY1}{C/2015 XY1}{C/2015 XY1 (Lemmon)}
%\DeclareComet{C2015Y1}{C/2015 Y1}{C/2015 Y1 (LINEAR)}
%\DeclareComet{C2015YG1}{C/2015 YG1}{C/2015 YG1 (NEOWISE)}
%\DeclareComet{C2016A1}{C/2016 A1}{C/2016 A1 (PANSTARRS)}
%\DeclareComet{C2016A5}{C/2016 A5}{C/2016 A5 (PANSTARRS)}
%\DeclareComet{C2016A6}{C/2016 A6}{C/2016 A6 (PANSTARRS)}
%\DeclareComet{C2016A8}{C/2016 A8}{C/2016 A8 (LINEAR)}
%\DeclareComet{C2016B1}{C/2016 B1}{C/2016 B1 (NEOWISE)}
%\DeclareComet{C2016C1}{C/2016 C1}{C/2016 C1 (PANSTARRS)}
%\DeclareComet{C2016C2}{C/2016 C2}{C/2016 C2 (NEOWISE)}
%\DeclareComet{C2016E1}{C/2016 E1}{C/2016 E1 (PANSTARRS)}
%\DeclareComet{C2016E2}{C/2016 E2}{C/2016 E2 (Kowalski)}
%\DeclareComet{C2016J2}{C/2016 J2}{C/2016 J2 (Denneau)}
%\DeclareComet{C2016K1}{C/2016 K1}{C/2016 K1 (LINEAR)}
%\DeclareComet{C2016KA}{C/2016 KA}{C/2016 KA (Catalina)}
%\DeclareComet{C2016M1}{C/2016 M1}{C/2016 M1 (PANSTARRS)}
%\DeclareComet{C2016N4}{C/2016 N4}{C/2016 N4 (MASTER)}
%\DeclareComet{C2016N6}{C/2016 N6}{C/2016 N6 (PANSTARRS)}
%\DeclareComet{C2016P4}{C/2016 P4}{C/2016 P4 (PANSTARRS)}
%\DeclareComet{C2016Q2}{C/2016 Q2}{C/2016 Q2 (PANSTARRS)}
%\DeclareComet{C2016Q4}{C/2016 Q4}{C/2016 Q4 (Kowalski)}
%\DeclareComet{C2016R2}{C/2016 R2}{C/2016 R2 (PANSTARRS)}
%\DeclareComet{C2016R3}{C/2016 R3}{C/2016 R3 (Borisov)}
%\DeclareComet{C2016T1}{C/2016 T1}{C/2016 T1 (Matheny)}
%\DeclareComet{C2016T2}{C/2016 T2}{C/2016 T2 (Matheny)}
%\DeclareComet{C2016T3}{C/2016 T3}{C/2016 T3 (PANSTARRS)}
%\DeclareComet{C2016U1}{C/2016 U1}{C/2016 U1 (NEOWISE)}
%\DeclareComet{C2016VZ18}{C/2016 VZ18}{C/2016 VZ18 (PANSTARRS)}
%\DeclareComet{C2016X1}{C/2016 X1}{C/2016 X1 (Lemmon)}
%\DeclareComet{C2017A1}{C/2017 A1}{C/2017 A1 (PANSTARRS)}
%\DeclareComet{C2017A3}{C/2017 A3}{C/2017 A3 (Elenin)}
%\DeclareComet{C2017AB5}{C/2017 AB5}{C/2017 AB5 (PANSTARRS)}
%\DeclareComet{C2017B3}{C/2017 B3}{C/2017 B3 (LINEAR)}
%\DeclareComet{C2017C1}{C/2017 C1}{C/2017 C1 (NEOWISE)}
%\DeclareComet{C2017C2}{C/2017 C2}{C/2017 C2 (PANSTARRS)}
%\DeclareComet{C2017D2}{C/2017 D2}{C/2017 D2 (Barros)}
%\DeclareComet{C2017D3}{C/2017 D3}{C/2017 D3 (ATLAS)}
%\DeclareComet{C2017D5}{C/2017 D5}{C/2017 D5 (PANSTARRS)}
%\DeclareComet{C2017E1}{C/2017 E1}{C/2017 E1 (Borisov)}
%\DeclareComet{C2017E2}{C/2017 E2}{C/2017 E2 (Tsuchinshan)}
%\DeclareComet{C2017E3}{C/2017 E3}{C/2017 E3 (PANSTARRS)}
%\DeclareComet{C2017E4}{C/2017 E4}{C/2017 E4 (Lovejoy)}
%\DeclareComet{C2017E5}{C/2017 E5}{C/2017 E5 (Lemmon)}
%\DeclareComet{C2017F1}{C/2017 F1}{C/2017 F1 (Lemmon)}
%\DeclareComet{C2017F2}{C/2017 F2}{C/2017 F2 (PANSTARRS)}
%\DeclareComet{C2017G3}{C/2017 G3}{C/2017 G3 (PANSTARRS)}
%\DeclareComet{C2017K1}{C/2017 K1}{C/2017 K1 (PANSTARRS)}
%\DeclareComet{C2017K2}{C/2017 K2}{C/2017 K2 (PANSTARRS)}
%\DeclareComet{C2017K4}{C/2017 K4}{C/2017 K4 (ATLAS)}
%\DeclareComet{C2017K5}{C/2017 K5}{C/2017 K5 (PANSTARRS)}
%\DeclareComet{C2017K6}{C/2017 K6}{C/2017 K6 (Jacques)}
%\DeclareComet{C2017M3}{C/2017 M3}{C/2017 M3 (PANSTARRS)}
%\DeclareComet{C2017M4}{C/2017 M4}{C/2017 M4 (ATLAS)}
%\DeclareComet{C2017M5}{C/2017 M5}{C/2017 M5 (TOTAS)}
%\DeclareComet{C2017O1}{C/2017 O1}{C/2017 O1 (ASASSN)}
%\DeclareComet{C2017P2}{C/2017 P2}{C/2017 P2 (PANSTARRS)}
%\DeclareComet{C2017S2}{C/2017 S2}{C/2017 S2 (PANSTARRS)}
%\DeclareComet{C2017S3}{C/2017 S3}{C/2017 S3 (PANSTARRS)}
%\DeclareComet{C2017S6}{C/2017 S6}{C/2017 S6 (Catalina)}
%\DeclareComet{C2017S7}{C/2017 S7}{C/2017 S7 (Lemmon)}
%\DeclareComet{C2017T1}{C/2017 T1}{C/2017 T1 (Heinze)}
%\DeclareComet{C2017T2}{C/2017 T2}{C/2017 T2 (PANSTARRS)}
%\DeclareComet{C2017T3}{C/2017 T3}{C/2017 T3 (ATLAS)}
%\DeclareComet{C2017U2}{C/2017 U2}{C/2017 U2 (Fuls)}
%\DeclareComet{C2017U4}{C/2017 U4}{C/2017 U4 (PANSTARRS)}
%\DeclareComet{C2017U5}{C/2017 U5}{C/2017 U5 (PANSTARRS)}
%\DeclareComet{C2017U7}{C/2017 U7}{C/2017 U7 (PANSTARRS)}
%\DeclareComet{C2017W2}{C/2017 W2}{C/2017 W2 (Leonard)}
%\DeclareComet{C2017X1}{C/2017 X1}{C/2017 X1 (PANSTARRS)}
%\DeclareComet{C2017Y1}{C/2017 Y1}{C/2017 Y1 (PANSTARRS)}
%\DeclareComet{C2017Y2}{C/2017 Y2}{C/2017 Y2 (PANSTARRS)}
%\DeclareComet{C2018A1}{C/2018 A1}{C/2018 A1 (PANSTARRS)}
%\DeclareComet{C2018A3}{C/2018 A3}{C/2018 A3 (ATLAS)}
%\DeclareComet{C2018A4}{C/2018 A4}{C/2018 A4 (PANSTARRS)}
%\DeclareComet{C2018A6}{C/2018 A6}{C/2018 A6 (Gibbs)}
%\DeclareComet{C2018B1}{C/2018 B1}{C/2018 B1 (Lemmon)}
%\DeclareComet{C2018C2}{C/2018 C2}{C/2018 C2 (Lemmon)}
%\DeclareComet{C2018DO4}{C/2018 DO4}{C/2018 DO4 (Lemmon)}
%\DeclareComet{C2018E1}{C/2018 E1}{C/2018 E1 (ATLAS)}
%\DeclareComet{C2018E2}{C/2018 E2}{C/2018 E2 (Barros)}
%\DeclareComet{C2018EF9}{C/2018 EF9}{C/2018 EF9 (Lemmon)}
%\DeclareComet{C2018EN4}{C/2018 EN4}{C/2018 EN4 (NEOWISE)}
%\DeclareComet{C2018F1}{C/2018 F1}{C/2018 F1 (Grauer)}
%\DeclareComet{C2018F3}{C/2018 F3}{C/2018 F3 (Johnson)}
%\DeclareComet{C2018F4}{C/2018 F4}{C/2018 F4 (PANSTARRS)}
%\DeclareComet{C2018F4-A}{C/2018 F4-A}{C/2018 F4-A (PANSTARRS)}
%\DeclareComet{C2018F4-B}{C/2018 F4-B}{C/2018 F4-B (PANSTARRS)}
%\DeclareComet{C2018K1}{C/2018 K1}{C/2018 K1 (Weiland)}
%\DeclareComet{C2018KJ3}{C/2018 KJ3}{C/2018 KJ3 (Lemmon)}
%\DeclareComet{C2018L2}{C/2018 L2}{C/2018 L2 (ATLAS)}
%\DeclareComet{C2018M1}{C/2018 M1}{C/2018 M1 (Catalina)}
%\DeclareComet{C2018N1}{C/2018 N1}{C/2018 N1 (NEOWISE)}
%\DeclareComet{C2018N2}{C/2018 N2}{C/2018 N2 (ASASSN)}
%\DeclareComet{C2018O1}{C/2018 O1}{C/2018 O1 (ATLAS)}
%\DeclareComet{C2018P5}{C/2018 P5}{C/2018 P5 (PANSTARRS)}
%\DeclareComet{C2018R3}{C/2018 R3}{C/2018 R3 (Lemmon)}
%\DeclareComet{C2018R4}{C/2018 R4}{C/2018 R4 (Fuls)}
%\DeclareComet{C2018R5}{C/2018 R5}{C/2018 R5 (Lemmon)}
%\DeclareComet{C2018S2}{C/2018 S2}{C/2018 S2 (TESS)}
%\DeclareComet{C2018S3}{C/2018 S3}{C/2018 S3 (TESS)}
%\DeclareComet{C2018U1}{C/2018 U1}{C/2018 U1 (Lemmon)}
%\DeclareComet{C2018V1}{C/2018 V1}{C/2018 V1 (Machholz-Fujikawa-Iwamoto)}
%\DeclareComet{C2018V2}{C/2018 V2}{C/2018 V2 (ATLAS)}
%\DeclareComet{C2018V4}{C/2018 V4}{C/2018 V4 (Africano)}
%\DeclareComet{C2018W1}{C/2018 W1}{C/2018 W1 (Catalina)}
%\DeclareComet{C2018W2}{C/2018 W2}{C/2018 W2 (Africano)}
%\DeclareComet{C2018X2}{C/2018 X2}{C/2018 X2 (Fitzsimmons)}
%\DeclareComet{C2018X3}{C/2018 X3}{C/2018 X3 (PANSTARRS)}
%\DeclareComet{C2018Y1}{C/2018 Y1}{C/2018 Y1 (Iwamoto)}
%\DeclareComet{C2019A5}{C/2019 A5}{C/2019 A5 (PANSTARRS)}
%\DeclareComet{C2019A9}{C/2019 A9}{C/2019 A9 (PANSTARRS)}
%\DeclareComet{C2019B1}{C/2019 B1}{C/2019 B1 (Africano)}
%\DeclareComet{C2019B3}{C/2019 B3}{C/2019 B3 (PANSTARRS)}
%\DeclareComet{C2019C1}{C/2019 C1}{C/2019 C1 (ATLAS)}
%\DeclareComet{C2019D1}{C/2019 D1}{C/2019 D1 (Flewelling)}
%\DeclareComet{C2019E3}{C/2019 E3}{C/2019 E3 (ATLAS)}
%\DeclareComet{C2019F1}{C/2019 F1}{C/2019 F1 (ATLAS-Africano)}
%\DeclareComet{C2019F2}{C/2019 F2}{C/2019 F2 (ATLAS)}
%\DeclareComet{C2019G2}{C/2019 G2}{C/2019 G2 (PANSTARRS)}
%\DeclareComet{C2019G4}{C/2019 G4}{C/2019 G4 (PANSTARRS)}
%\DeclareComet{C2019H1}{C/2019 H1}{C/2019 H1 (NEOWISE)}
%\DeclareComet{C2019J1}{C/2019 J1}{C/2019 J1 (Lemmon)}
%\DeclareComet{C2019J2}{C/2019 J2}{C/2019 J2 (Palomar)}
%\DeclareComet{C2019J3}{C/2019 J3}{C/2019 J3 (ATLAS)}
%\DeclareComet{C2019JU6}{C/2019 JU6}{C/2019 JU6 (ATLAS)}
%\DeclareComet{C2019K1}{C/2019 K1}{C/2019 K1 (ATLAS)}
%\DeclareComet{C2019K4}{C/2019 K4}{C/2019 K4 (Ye)}
%\DeclareComet{C2019K5}{C/2019 K5}{C/2019 K5 (Young)}
%\DeclareComet{C2019K6}{C/2019 K6}{C/2019 K6 (PANSTARRS)}
%\DeclareComet{C2019K7}{C/2019 K7}{C/2019 K7 (Smith)}
%\DeclareComet{C2019K8}{C/2019 K8}{C/2019 K8 (ATLAS)}
%\DeclareComet{C2019L1}{C/2019 L1}{C/2019 L1 (PANSTARRS)}
%\DeclareComet{C2019L2}{C/2019 L2}{C/2019 L2 (NEOWISE)}
%\DeclareComet{C2019L3}{C/2019 L3}{C/2019 L3 (ATLAS)}
%\DeclareComet{C2019LB7}{C/2019 LB7}{C/2019 LB7 (Kleyna)}
%\DeclareComet{C2019M3}{C/2019 M3}{C/2019 M3 (ATLAS)}
%\DeclareComet{C2019M4}{C/2019 M4}{C/2019 M4 (TESS)}
%\DeclareComet{C2019N1}{C/2019 N1}{C/2019 N1 (ATLAS)}
%\DeclareComet{C2019NJ3}{C/2019 NJ3}{C/2019 NJ3 (Lemmon)}
%\DeclareComet{C2019O2}{C/2019 O2}{C/2019 O2 (PANSTARRS)}
%\DeclareComet{C2019O3}{C/2019 O3}{C/2019 O3 (Palomar)}
%\DeclareComet{C2019Q1}{C/2019 Q1}{C/2019 Q1 (Lemmon)}
%\DeclareComet{C2019Q3}{C/2019 Q3}{C/2019 Q3 (PANSTARRS)}
%\DeclareComet{C2019S4}{C/2019 S4}{C/2019 S4 (Lemmon)}
%\DeclareComet{C2019T2}{C/2019 T2}{C/2019 T2 (Lemmon)}
%\DeclareComet{C2019T3}{C/2019 T3}{C/2019 T3 (ATLAS)}
%\DeclareComet{C2019T4}{C/2019 T4}{C/2019 T4 (ATLAS)}
%\DeclareComet{C2019U5}{C/2019 U5}{C/2019 U5 (PANSTARRS)}
%\DeclareComet{C2019U6}{C/2019 U6}{C/2019 U6 (Lemmon)}
%\DeclareComet{C2019V1}{C/2019 V1}{C/2019 V1 (Borisov)}
%\DeclareComet{C2019Y1}{C/2019 Y1}{C/2019 Y1 (ATLAS)}
%\DeclareComet{C2019Y4}{C/2019 Y4}{C/2019 Y4 (ATLAS)}
%\DeclareComet{C2019Y4-A}{C/2019 Y4-A}{C/2019 Y4-A (ATLAS)}
%\DeclareComet{C2019Y4-B}{C/2019 Y4-B}{C/2019 Y4-B (ATLAS)}
%\DeclareComet{C2019Y4-C}{C/2019 Y4-C}{C/2019 Y4-C (ATLAS)}
%\DeclareComet{C2019Y4-D}{C/2019 Y4-D}{C/2019 Y4-D (ATLAS)}
%\DeclareComet{C2019Y5}{C/2019 Y5}{C/2019 Y5 (PANSTARRS)}
%\DeclareComet{C2020A2}{C/2020 A2}{C/2020 A2 (Iwamoto)}
%\DeclareComet{C2020A3}{C/2020 A3}{C/2020 A3 (ATLAS)}
%\DeclareComet{C2020B2}{C/2020 B2}{C/2020 B2 (Lemmon)}
%\DeclareComet{C2020B3}{C/2020 B3}{C/2020 B3 (Rankin)}
%\DeclareComet{C2020F2}{C/2020 F2}{C/2020 F2 (ATLAS)}
%\DeclareComet{C2020F3}{C/2020 F3}{C/2020 F3 (NEOWISE)}
%\DeclareComet{C2020F5}{C/2020 F5}{C/2020 F5 (MASTER)}
%\DeclareComet{C2020F6}{C/2020 F6}{C/2020 F6 (PANSTARRS)}
%\DeclareComet{C2020F7}{C/2020 F7}{C/2020 F7 (Lemmon)}
%\DeclareComet{C2020F8}{C/2020 F8}{C/2020 F8 (SWAN)}
%\DeclareComet{C2020H11}{C/2020 H11}{C/2020 H11 (PANSTARRS-Lemmon)}
%\DeclareComet{C2020H2}{C/2020 H2}{C/2020 H2 (Pruyne)}
%\DeclareComet{C2020H3}{C/2020 H3}{C/2020 H3 (Wierzchos)}
%\DeclareComet{C2020H4}{C/2020 H4}{C/2020 H4 (Leonard)}
%\DeclareComet{C2020H5}{C/2020 H5}{C/2020 H5 (Robinson)}
%\DeclareComet{C2020H6}{C/2020 H6}{C/2020 H6 (ATLAS)}
%\DeclareComet{C2020H7}{C/2020 H7}{C/2020 H7 (Lemmon)}
%\DeclareComet{C2020H8}{C/2020 H8}{C/2020 H8 (PANSTARRS)}
%\DeclareComet{C2020J1}{C/2020 J1}{C/2020 J1 (SONEAR)}
%\DeclareComet{C2020K1}{C/2020 K1}{C/2020 K1 (PANSTARRS)}
%\DeclareComet{C2020K2}{C/2020 K2}{C/2020 K2 (PANSTARRS)}
%\DeclareComet{C2020K3}{C/2020 K3}{C/2020 K3 (Leonard)}
%\DeclareComet{C2020K4}{C/2020 K4}{C/2020 K4 (PANSTARRS)}
%\DeclareComet{C2020K5}{C/2020 K5}{C/2020 K5 (PANSTARRS)}
%\DeclareComet{C2020K6}{C/2020 K6}{C/2020 K6 (Rankin)}
%\DeclareComet{C2020K7}{C/2020 K7}{C/2020 K7 (PANSTARRS)}
%\DeclareComet{C2020K8}{C/2020 K8}{C/2020 K8 (Catalina-ATLAS)}
%\DeclareComet{C2020M3}{C/2020 M3}{C/2020 M3 (ATLAS)}
%\DeclareComet{C2020M5}{C/2020 M5}{C/2020 M5 (ATLAS)}
%\DeclareComet{C2020N1}{C/2020 N1}{C/2020 N1 (PANSTARRS)}
%\DeclareComet{C2020N2}{C/2020 N2}{C/2020 N2 (ATLAS)}
%\DeclareComet{C2020O2}{C/2020 O2}{C/2020 O2 (Amaral)}
%\DeclareComet{C2020P1}{C/2020 P1}{C/2020 P1 (NEOWISE)}
%\DeclareComet{C2020P3}{C/2020 P3}{C/2020 P3 (ATLAS)}
%\DeclareComet{C2020P4-A}{C/2020 P4-A}{C/2020 P4-A (SOHO)}
%\DeclareComet{C2020P4-B}{C/2020 P4-B}{C/2020 P4-B (SOHO)}
%\DeclareComet{C2020P4-C}{C/2020 P4-C}{C/2020 P4-C (SOHO)}
%\DeclareComet{C2020PV6}{C/2020 PV6}{C/2020 PV6 (PANSTARRS)}
%\DeclareComet{C2020Q1}{C/2020 Q1}{C/2020 Q1 (Borisov)}
%\DeclareComet{C2020Q2}{C/2020 Q2}{C/2020 Q2 (PANSTARRS)}
%\DeclareComet{C2020R2}{C/2020 R2}{C/2020 R2 (PANSTARRS)}
%\DeclareComet{C2020R4}{C/2020 R4}{C/2020 R4 (ATLAS)}
%\DeclareComet{C2020R6}{C/2020 R6}{C/2020 R6 (Rankin)}
%\DeclareComet{C2020R7}{C/2020 R7}{C/2020 R7 (ATLAS)}
%\DeclareComet{C2020S2}{C/2020 S2}{C/2020 S2 (PANSTARRS)}
%\DeclareComet{C2020S3}{C/2020 S3}{C/2020 S3 (Erasmus)}
%\DeclareComet{C2020S4}{C/2020 S4}{C/2020 S4 (PANSTARRS)}
%\DeclareComet{C2020S8}{C/2020 S8}{C/2020 S8 (Lemmon)}
%\DeclareComet{C2020T2}{C/2020 T2}{C/2020 T2 (Palomar)}
%\DeclareComet{C2020T4}{C/2020 T4}{C/2020 T4 (PANSTARRS)}
%\DeclareComet{C2020T5}{C/2020 T5}{C/2020 T5 (Lemmon)}
%\DeclareComet{C2020U3}{C/2020 U3}{C/2020 U3 (Rankin)}
%\DeclareComet{C2020U4}{C/2020 U4}{C/2020 U4 (PANSTARRS)}
%\DeclareComet{C2020U5}{C/2020 U5}{C/2020 U5 (PANSTARRS)}
%\DeclareComet{C2020V2}{C/2020 V2}{C/2020 V2 (ZTF)}
%\DeclareComet{C2020W5}{C/2020 W5}{C/2020 W5 (Lemmon)}
%\DeclareComet{C2020X2}{C/2020 X2}{C/2020 X2 (ATLAS)}
%\DeclareComet{C2020X3}{C/2020 X3}{C/2020 X3 (SOHO)}
%\DeclareComet{C2020X4}{C/2020 X4}{C/2020 X4 (Leonard)}
%\DeclareComet{C2020Y2}{C/2020 Y2}{C/2020 Y2 (ATLAS)}
%\DeclareComet{C2020Y3}{C/2020 Y3}{C/2020 Y3 (ATLAS)}
%\DeclareComet{C2021A1}{C/2021 A1}{C/2021 A1 (Leonard)}
%\DeclareComet{C2021A10}{C/2021 A10}{C/2021 A10 (NEOWISE)}
%\DeclareComet{C2021A2}{C/2021 A2}{C/2021 A2 (NEOWISE)}
%\DeclareComet{C2021A4}{C/2021 A4}{C/2021 A4 (NEOWISE)}
%\DeclareComet{C2021A6}{C/2021 A6}{C/2021 A6 (PANSTARRS)}
%\DeclareComet{C2021A7}{C/2021 A7}{C/2021 A7 (NEOWISE)}
%\DeclareComet{C2021A9}{C/2021 A9}{C/2021 A9 (PANSTARRS)}
%\DeclareComet{C2021B2}{C/2021 B2}{C/2021 B2 (PANSTARRS)}
%\DeclareComet{C2021B3}{C/2021 B3}{C/2021 B3 (NEOWISE)}
%\DeclareComet{C2021C1}{C/2021 C1}{C/2021 C1 (Rankin)}
%\DeclareComet{C2021C3}{C/2021 C3}{C/2021 C3 (Catalina)}
%\DeclareComet{C2021C4}{C/2021 C4}{C/2021 C4 (ATLAS)}
%\DeclareComet{C2021C5}{C/2021 C5}{C/2021 C5 (PANSTARRS)}
%\DeclareComet{C2021C6}{C/2021 C6}{C/2021 C6 (Lemmon)}
%\DeclareComet{C2021D1}{C/2021 D1}{C/2021 D1 (SWAN)}
%\DeclareComet{C2021D2}{C/2021 D2}{C/2021 D2 (ZTF)}
%\DeclareComet{C2021E3}{C/2021 E3}{C/2021 E3 (ZTF)}
%\DeclareComet{C2021F1}{C/2021 F1}{C/2021 F1 (Lemmon-PANSTARRS)}
%\DeclareComet{C2021G1}{C/2021 G1}{C/2021 G1 (Leonard)}
%\DeclareComet{C2021G2}{C/2021 G2}{C/2021 G2 (ATLAS)}
%\DeclareComet{C2021G3}{C/2021 G3}{C/2021 G3 (PANSTARRS)}
%\DeclareComet{C2021J1}{C/2021 J1}{C/2021 J1 (Maury-Attard)}
%\DeclareComet{C2021J2}{C/2021 J2}{C/2021 J2 (PANSTARRS)}
%\DeclareComet{C2021K1}{C/2021 K1}{C/2021 K1 (ATLAS)}
%\DeclareComet{C2021K2}{C/2021 K2}{C/2021 K2 (MASTER)}
%\DeclareComet{C2021K3}{C/2021 K3}{C/2021 K3 (Catalina)}
%\DeclareComet{C2021L3}{C/2021 L3}{C/2021 L3 (Borisov)}
%\DeclareComet{C2021N3}{C/2021 N3}{C/2021 N3 (PANSTARRS)}
%\DeclareComet{C2021O1}{C/2021 O1}{C/2021 O1 (Nishimura)}
%\DeclareComet{C2021O3}{C/2021 O3}{C/2021 O3 (PANSTARRS)}
%\DeclareComet{C2021P1}{C/2021 P1}{C/2021 P1 (PANSTARRS)}
%\DeclareComet{C2021P2}{C/2021 P2}{C/2021 P2 (PANSTARRS)}
%\DeclareComet{C2021P4}{C/2021 P4}{C/2021 P4 (ATLAS)}
%\DeclareComet{C2021Q3}{C/2021 Q3}{C/2021 Q3 (ATLAS)}
%\DeclareComet{C2021Q4}{C/2021 Q4}{C/2021 Q4 (Fuls)}
\DeclareComet{C2021Q6}{C/2021 Q6}{C/2021 Q6 (PANSTARRS)}
%\DeclareComet{C2021QM45}{C/2021 QM45}{C/2021 QM45 (PANSTARRS)}
%\DeclareComet{C2021R2}{C/2021 R2}{C/2021 R2 (PANSTARRS)}
%\DeclareComet{C2021R7}{C/2021 R7}{C/2021 R7 (PANSTARRS)}
%\DeclareComet{C2021S1}{C/2021 S1}{C/2021 S1 (ATLAS)}
%\DeclareComet{C2021S3}{C/2021 S3}{C/2021 S3 (PANSTARRS)}
%\DeclareComet{C2021S4}{C/2021 S4}{C/2021 S4 (Tsuchinshan)}
%\DeclareComet{C2021T1}{C/2021 T1}{C/2021 T1 (Lemmon)}
%\DeclareComet{C2021T2}{C/2021 T2}{C/2021 T2 (Fuls)}
%\DeclareComet{C2021T4}{C/2021 T4}{C/2021 T4 (Lemmon)}
%\DeclareComet{C2021U4}{C/2021 U4}{C/2021 U4 (Leonard)}
%\DeclareComet{C2021U5}{C/2021 U5}{C/2021 U5 (Catalina)}
%\DeclareComet{C2021V1}{C/2021 V1}{C/2021 V1 (Rankin)}
%\DeclareComet{C2021X1}{C/2021 X1}{C/2021 X1 (Maury-Attard)}
%\DeclareComet{C2021X2}{C/2021 X2}{C/2021 X2 (Bok)}
%\DeclareComet{C2021Y1}{C/2021 Y1}{C/2021 Y1 (ATLAS)}
%\DeclareComet{C2022A1}{C/2022 A1}{C/2022 A1 (Sarneczky)}
%\DeclareComet{C2022A2}{C/2022 A2}{C/2022 A2 (PANSTARRS)}
%\DeclareComet{C2022A3}{C/2022 A3}{C/2022 A3 (Lemmon-ATLAS)}
%\DeclareComet{C2022B4}{C/2022 B4}{C/2022 B4 (Bok)}
%\DeclareComet{C2022D2}{C/2022 D2}{C/2022 D2 (Kowalski)}
%\DeclareComet{C2022E2}{C/2022 E2}{C/2022 E2 (ATLAS)}
%\DeclareComet{C2022E3}{C/2022 E3}{C/2022 E3 (ZTF)}
%\DeclareComet{C2022F1}{C/2022 F1}{C/2022 F1 (ATLAS)}
%\DeclareComet{C2022F2}{C/2022 F2}{C/2022 F2 (NEOWISE)}
%\DeclareComet{C2022H1}{C/2022 H1}{C/2022 H1 (PANSTARRS)}
%\DeclareComet{C2022J1}{C/2022 J1}{C/2022 J1 (Maury-Attard)}
%\DeclareComet{C2022J2}{C/2022 J2}{C/2022 J2 (Bok)}
%\DeclareComet{C2022JK5}{C/2022 JK5}{C/2022 JK5 (PANSTARRS)}
%\DeclareComet{C2022K1}{C/2022 K1}{C/2022 K1 (Leonard)}
%\DeclareComet{C2022L1}{C/2022 L1}{C/2022 L1 (Catalina)}
%\DeclareComet{C2022L2}{C/2022 L2}{C/2022 L2 (ATLAS)}
%\DeclareComet{C2022L4}{C/2022 L4}{C/2022 L4 (PANSTARRS)}
%\DeclareComet{C2022N1}{C/2022 N1}{C/2022 N1 (Attard-Maury)}
%\DeclareComet{C2022N2}{C/2022 N2}{C/2022 N2 (PANSTARRS)}
%\DeclareComet{C2022O1}{C/2022 O1}{C/2022 O1 (ATLAS)}
%\DeclareComet{C2022P1}{C/2022 P1}{C/2022 P1 (NEOWISE)}
%\DeclareComet{C2022P3}{C/2022 P3}{C/2022 P3 (ZTF)}
%\DeclareComet{C2022Q2}{C/2022 Q2}{C/2022 Q2 (ATLAS)}
%\DeclareComet{C2022QE78}{C/2022 QE78}{C/2022 QE78 (ATLAS)}
%\DeclareComet{C2022R2}{C/2022 R2}{C/2022 R2 (ATLAS)}
%\DeclareComet{C2022R3}{C/2022 R3}{C/2022 R3 (Leonard)}
%\DeclareComet{C2022R6}{C/2022 R6}{C/2022 R6 (PANSTARRS)}
%\DeclareComet{C2022S3}{C/2022 S3}{C/2022 S3 (PANSTARRS)}
%\DeclareComet{C2022S4}{C/2022 S4}{C/2022 S4 (Lemmon)}
%\DeclareComet{C2022S5}{C/2022 S5}{C/2022 S5 (PANSTARRS)}
%\DeclareComet{C2022T1}{C/2022 T1}{C/2022 T1 (Lemmon)}
%\DeclareComet{C2022U1}{C/2022 U1}{C/2022 U1 (Leonard)}
%\DeclareComet{C2022U2}{C/2022 U2}{C/2022 U2 (ATLAS)}
%\DeclareComet{C2022U3}{C/2022 U3}{C/2022 U3 (Bok)}
%\DeclareComet{C2022U4}{C/2022 U4}{C/2022 U4 (Bok)}
%\DeclareComet{C2022V2}{C/2022 V2}{C/2022 V2 (Lemmon)}
%\DeclareComet{C2022W2}{C/2022 W2}{C/2022 W2 (ATLAS)}
%\DeclareComet{C2022W3}{C/2022 W3}{C/2022 W3 (Leonard)}
%\DeclareComet{C2022Y1}{C/2022 Y1}{C/2022 Y1 (Hogan)}
%\DeclareComet{C2022Y2}{C/2022 Y2}{C/2022 Y2 (Lemmon)}
%\DeclareComet{C2023A1}{C/2023 A1}{C/2023 A1 (Leonard)}
%\DeclareComet{C2023A2}{C/2023 A2}{C/2023 A2 (SWAN)}
%\DeclareComet{C2023A3}{C/2023 A3}{C/2023 A3 (Tsuchinshan--ATLAS)}
%\DeclareComet{C2023B2}{C/2023 B2}{C/2023 B2 (ATLAS)}
%\DeclareComet{C2023C2}{C/2023 C2}{C/2023 C2 (ATLAS)}
%\DeclareComet{C2023E1}{C/2023 E1}{C/2023 E1 (ATLAS)}
%\DeclareComet{C2023F1}{C/2023 F1}{C/2023 F1 (PANSTARRS)}
%\DeclareComet{C2023F2}{C/2023 F2}{C/2023 F2 (SOHO)}
%\DeclareComet{C2023F3}{C/2023 F3}{C/2023 F3 (ATLAS)}
%\DeclareComet{C2023H1}{C/2023 H1}{C/2023 H1 (PANSTARRS)}
%\DeclareComet{C2023H2}{C/2023 H2}{C/2023 H2 (Lemmon)}
%\DeclareComet{C2023H3}{C/2023 H3}{C/2023 H3 (PANSTARRS)}
%\DeclareComet{C2023H5}{C/2023 H5}{C/2023 H5 (Lemmon)}
%\DeclareComet{C2023K1}{C/2023 K1}{C/2023 K1 (ATLAS)}
%\DeclareComet{C2023P1}{C/2023 P1}{C/2023 P1 (Nishimura)}
%\DeclareComet{C2023Q1}{C/2023 Q1}{C/2023 Q1 (PANSTARRS)}
%\DeclareComet{C2023Q2}{C/2023 Q2}{C/2023 Q2 (PANSTARRS)}
%\DeclareComet{C2023R1}{C/2023 R1}{C/2023 R1 (PANSTARRS)}
%\DeclareComet{C2023R1-B}{C/2023 R1-B}{C/2023 R1-B}
%\DeclareComet{C2023R2}{C/2023 R2}{C/2023 R2 (PANSTARRS)}
%\DeclareComet{C2023RN3}{C/2023 RN3}{C/2023 RN3 (ATLAS)}
%\DeclareComet{C2023RS61}{C/2023 RS61}{C/2023 RS61 (PANSTARRS)}
%\DeclareComet{C2023S2}{C/2023 S2}{C/2023 S2 (ATLAS)}
%\DeclareComet{C2023S3}{C/2023 S3}{C/2023 S3 (Lemmon)}
%\DeclareComet{C2023T2}{C/2023 T2}{C/2023 T2 (Borisov)}
%\DeclareComet{C2023T3}{C/2023 T3}{C/2023 T3 (Fuls)}
%\DeclareComet{C2023TD22}{C/2023 TD22}{C/2023 TD22 (Lemmon)}
%\DeclareComet{C2023U1}{C/2023 U1}{C/2023 U1 (Fuls)}
%\DeclareComet{C2023V1}{C/2023 V1}{C/2023 V1 (Lemmon)}
%\DeclareComet{C2023V3}{C/2023 V3}{C/2023 V3 (PANSTARRS)}
%\DeclareComet{C2023V4}{C/2023 V4}{C/2023 V4 (Camarasa-Duszanowicz)}
%\DeclareComet{C2023V5}{C/2023 V5}{C/2023 V5 (Leonard)}
%\DeclareComet{C2023X1}{C/2023 X1}{C/2023 X1 (Leonard)}
%\DeclareComet{C2023X2}{C/2023 X2}{C/2023 X2 (Lemmon)}
%\DeclareComet{C2023X4}{C/2023 X4}{C/2023 X4 (Hogan)}
%\DeclareComet{C2023X7}{C/2023 X7}{C/2023 X7 (PANSTARRS)}
%\DeclareComet{C2024A1}{C/2024 A1}{C/2024 A1 (ATLAS)}
%\DeclareComet{C2024A2}{C/2024 A2}{C/2024 A2 (ATLAS)}
%\DeclareComet{C2024B1}{C/2024 B1}{C/2024 B1 (Lemmon)}
%\DeclareComet{C2024B2}{C/2024 B2}{C/2024 B2 (Lemmon)}
%\DeclareComet{C2024C1}{C/2024 C1}{C/2024 C1 (PANSTARRS)}
%\DeclareComet{C2024C2}{C/2024 C2}{C/2024 C2 (PANSTARRS)}
%\DeclareComet{C2024C3}{C/2024 C3}{C/2024 C3 (PANSTARRS)}
%\DeclareComet{C2024C4}{C/2024 C4}{C/2024 C4 (ATLAS)}
%\DeclareComet{C2024D1}{C/2024 D1}{C/2024 D1 (Lemmon)}
%\DeclareComet{C2024E1}{C/2024 E1}{C/2024 E1 (Wierzchos)}
%\DeclareComet{C2024E2}{C/2024 E2}{C/2024 E2 (Bok)}
%\DeclareComet{C2024F2}{C/2024 F2}{C/2024 F2 (PANSTARRS)}
%\DeclareComet{C2024G1}{C/2024 G1}{C/2024 G1 (Wierzchos)}
%\DeclareComet{C2024G2}{C/2024 G2}{C/2024 G2 (ATLAS)}
%\DeclareComet{C2024G3}{C/2024 G3}{C/2024 G3 (ATLAS)}
%\DeclareComet{C2024G4}{C/2024 G4}{C/2024 G4 (PANSTARRS)}
%\DeclareComet{C2024G5}{C/2024 G5}{C/2024 G5 (Leonard)}
%\DeclareComet{C2024G6}{C/2024 G6}{C/2024 G6 (ATLAS)}
%\DeclareComet{C2024G7}{C/2024 G7}{C/2024 G7 (ATLAS)}
%\DeclareComet{C2024J2}{C/2024 J2}{C/2024 J2 (Wierzchos)}
%\DeclareComet{C2024J3}{C/2024 J3}{C/2024 J3 (ATLAS)}
%\DeclareComet{C2024J4}{C/2024 J4}{C/2024 J4 (Lemmon)}
%\DeclareComet{C2024L1}{C/2024 L1}{C/2024 L1 (PANSTARRS)}
%\DeclareComet{C2024L2}{C/2024 L2}{C/2024 L2 (PANSTARRS)}
%\DeclareComet{C2024L3}{C/2024 L3}{C/2024 L3 (PANSTARRS)}
%\DeclareComet{C2024L5}{C/2024 L5}{C/2024 L5 (ATLAS)}
%\DeclareComet{C2024M1}{C/2024 M1}{C/2024 M1 (ATLAS)}
%\DeclareComet{C2024N1}{C/2024 N1}{C/2024 N1 (PANSTARRS)}
%\DeclareComet{C2024N3}{C/2024 N3}{C/2024 N3 (Sarneczky)}
%\DeclareComet{C2024N4}{C/2024 N4}{C/2024 N4 (Sarneczky)}
%\DeclareComet{C2024O1}{C/2024 O1}{C/2024 O1 (PANSTARRS)}
%\DeclareComet{C2024PN7}{C/2024 PN7}{C/2024 PN7 (PANSTARRS)}
%\DeclareComet{C2024Q3}{C/2024 Q3}{C/2024 Q3 (PANSTARRS)}
%\DeclareComet{C2024Q4}{C/2024 Q4}{C/2024 Q4 (PANSTARRS)}
%\DeclareComet{C2024R4}{C/2024 R4}{C/2024 R4 (PANSTARRS)}
%\DeclareComet{C2024S1}{C/2024 S1}{C/2024 S1 (ATLAS)}
%\DeclareComet{C2024T3}{C/2024 T3}{C/2024 T3 (PANSTARRS)}
%\DeclareComet{C2024T5}{C/2024 T5}{C/2024 T5 (ATLAS)}
%\DeclareComet{C2024U1}{C/2024 U1}{C/2024 U1 (PANSTARRS)}
%\DeclareComet{C2024V1}{C/2024 V1}{C/2024 V1 (Borisov)}
%\DeclareComet{C2024V2}{C/2024 V2}{C/2024 V2 (Sarneczky)}
%\DeclareComet{C2024W1}{C/2024 W1}{C/2024 W1 (PANSTARRS)}
%\DeclareComet{C2024X1}{C/2024 X1}{C/2024 X1 (Fazekas)}
%\DeclareComet{C2024X2}{C/2024 X2}{C/2024 X2 (ATLAS)}
%\DeclareComet{C2024X4}{C/2024 X4}{C/2024 X4 (PANSTARRS)}
%\DeclareComet{C2024XK14}{C/2024 XK14}{C/2024 XK14 (Bok)}
%\DeclareComet{C2024Y1}{C/2024 Y1}{C/2024 Y1 (Masek)}
%\DeclareComet{C2025A1}{C/2025 A1}{C/2025 A1 (Lemmon)}
%\DeclareComet{C2025A3}{C/2025 A3}{C/2025 A3 (Tsuchinshan)}
%\DeclareComet{C2025A4}{C/2025 A4}{C/2025 A4 (PANSTARRS)}
%\DeclareComet{C2025A6}{C/2025 A6}{C/2025 A6 (Lemmon)}
%\DeclareComet{C2025B1}{C/2025 B1}{C/2025 B1 (PANSTARRS)}
%\DeclareComet{C2025B2}{C/2025 B2}{C/2025 B2 (Borisov)}
%\DeclareComet{C2025D1}{C/2025 D1}{C/2025 D1 (Groeller)}
%\DeclareComet{C2025D5}{C/2025 D5}{C/2025 D5 (PANSTARRS)}
%\DeclareComet{C2025D6}{C/2025 D6}{C/2025 D6 (ATLAS)}
%\DeclareComet{C2025E1}{C/2025 E1}{C/2025 E1 (PANSTARRS)}
%\DeclareComet{C2025F1}{C/2025 F1}{C/2025 F1 (ATLAS)}
%\DeclareComet{C2025F2}{C/2025 F2}{C/2025 F2 (SWAN)}
%\DeclareComet{C2025J1}{C/2025 J1}{C/2025 J1 (Borisov)}
%\DeclareComet{C2025K1}{C/2025 K1}{C/2025 K1 (ATLAS)}
%\DeclareComet{C2025K1-B}{C/2025 K1-B}{C/2025 K1-B (ATLAS)}
%\DeclareComet{C2025K1-C}{C/2025 K1-C}{C/2025 K1-C (ATLAS)}
%\DeclareComet{C2025K1-D}{C/2025 K1-D}{C/2025 K1-D (ATLAS)}
%\DeclareComet{C2025K2}{C/2025 K2}{C/2025 K2 (PANSTARRS)}
%\DeclareComet{C2025K3}{C/2025 K3}{C/2025 K3 (PANSTARRS)}
%\DeclareComet{C2025K4}{C/2025 K4}{C/2025 K4 (Siverd)}
%\DeclareComet{C2025L1}{C/2025 L1}{C/2025 L1 (ATLAS)}
%\DeclareComet{C2025L2}{C/2025 L2}{C/2025 L2 (MAPS)}
%\DeclareComet{C2025M1}{C/2025 M1}{C/2025 M1 (PANSTARRS)}
%\DeclareComet{C2025M2}{C/2025 M2}{C/2025 M2 (PANSTARRS)}
%\DeclareComet{C2025M3}{C/2025 M3}{C/2025 M3 (PANSTARRS)}
%\DeclareComet{C2025N2}{C/2025 N2}{C/2025 N2 (ATLAS)}
%\DeclareComet{C2025O2}{C/2025 O2}{C/2025 O2 (MAPS)}
%\DeclareComet{C2025Q1}{C/2025 Q1}{C/2025 Q1 (ATLAS)}
%\DeclareComet{C2025Q3}{C/2025 Q3}{C/2025 Q3 (ATLAS)}
%\DeclareComet{C2025R1}{C/2025 R1}{C/2025 R1 (ATLAS)}
%\DeclareComet{C2025R2}{C/2025 R2}{C/2025 R2 (SWAN)}
%\DeclareComet{C2025R3}{C/2025 R3}{C/2025 R3 (PANSTARRS)}
%\DeclareComet{C2025T1}{C/2025 T1}{C/2025 T1 (ATLAS)}
%\DeclareComet{C2025V1}{C/2025 V1}{C/2025 V1 (Borisov)}
%\DeclareComet{C2025V2}{C/2025 V2}{C/2025 V2 (Rankin)}
%\DeclareComet{C2025W1}{C/2025 W1}{C/2025 W1 (Sankovich)}
%\DeclareComet{C2025W2}{C/2025 W2}{C/2025 W2 (ATLAS)}
%\DeclareComet{C2025X1}{C/2025 X1}{C/2025 X1 (PANSTARRS)}
%\DeclareComet{C2025Y1}{C/2025 Y1}{C/2025 Y1 (ATLAS)}
%\DeclareComet{C2025Y3}{C/2025 Y3}{C/2025 Y3 (PANSTARRS)}
%\DeclareComet{C2026A1}{C/2026 A1}{C/2026 A1 (MAPS)}
%\DeclareComet{C2026A2}{C/2026 A2}{C/2026 A2 (Bok)}
%\DeclareComet{C2026A3}{C/2026 A3}{C/2026 A3 (PANSTARRS)}
%\DeclareComet{C2026AZ17}{C/2026 AZ17}{C/2026 AZ17 (Bok)}
%\DeclareComet{C2026B2}{C/2026 B2}{C/2026 B2 (Sun-Gao)}
%\DeclareComet{C2026B3}{C/2026 B3}{C/2026 B3 (PANSTARRS)}
%\DeclareComet{C2026C1}{C/2026 C1}{C/2026 C1 (Tsuchinshan)}
%\DeclareComet{C2026H1}{C/2026 H1}{C/2026 H1 (PANSTARRS)}
%\DeclareComet{C2026H2}{C/2026 H2}{C/2026 H2 (Leonard)}
%\DeclareComet{C2026H3}{C/2026 H3}{C/2026 H3 (Bok)}
%\DeclareComet{C2026J1}{C/2026 J1}{C/2026 J1 (PANSTARRS)}
%\DeclareComet{C2026L1}{C/2026 L1}{C/2026 L1 (PANSTARRS)}
%\DeclareComet{C2026L2}{C/2026 L2}{C/2026 L2 (PANSTARRS)}
%\DeclareComet{C2026M3}{C/2026 M3}{C/2026 M3 (MASTER)}
%\DeclareComet{C2026M5}{C/2026 M5}{C/2026 M5 (PANSTARRS)}
%\DeclareComet{C2026N1}{C/2026 N1}{C/2026 N1 (PANSTARRS)}
%\DeclareComet{C2026O1}{C/2026 O1}{C/2026 O1 (PANSTARRS)}
%\DeclareComet{C2026P2}{C/2026 P2}{C/2026 P2 (PANSTARRS)}
%\DeclareComet{C240V1}{C/ 240 V1}{C/ 240 V1}
%\DeclareComet{C390Q1}{C/ 390 Q1}{C/ 390 Q1}
%\DeclareComet{C400F1}{C/ 400 F1}{C/ 400 F1}
%\DeclareComet{C418M1}{C/ 418 M1}{C/ 418 M1}
%\DeclareComet{C442V1}{C/ 442 V1}{C/ 442 V1}
%\DeclareComet{C539W1}{C/ 539 W1}{C/ 539 W1}
%\DeclareComet{C565O1}{C/ 565 O1}{C/ 565 O1}
%\DeclareComet{C568O1}{C/ 568 O1}{C/ 568 O1}
%\DeclareComet{C574G1}{C/ 574 G1}{C/ 574 G1}
%\DeclareComet{C770K1}{C/ 770 K1}{C/ 770 K1}
%\DeclareComet{C817C1}{C/ 817 C1}{C/ 817 C1}
%\DeclareComet{C868B1}{C/ 868 B1}{C/ 868 B1}
%\DeclareComet{C905K1}{C/ 905 K1}{C/ 905 K1}
%\DeclareComet{C962B1}{C/ 962 B1}{C/ 962 B1}
%\DeclareComet{D1766G1}{D/1766 G1}{D/1766 G1 (Helfenzrieder)}
%\DeclareComet{D1770L1}{D/1770 L1}{D/1770 L1 (Lexell)}
%\DeclareComet{D1884O1}{D/1884 O1}{D/1884 O1 (Barnard)}
%\DeclareComet{D1886K1}{D/1886 K1}{D/1886 K1 (Brooks)}
%\DeclareComet{D1895Q1}{D/1895 Q1}{D/1895 Q1 (Swift)}
%\DeclareComet{D1918W1}{D/1918 W1}{D/1918 W1 (Schorr)}
%\DeclareComet{D1952B1}{D/1952 B1}{D/1952 B1 (Harrington-Wilson)}
%\DeclareComet{D1977C1}{D/1977 C1}{D/1977 C1 (Skiff-Kosai)}
%\DeclareComet{D1978R1}{D/1978 R1}{D/1978 R1 (Haneda-Campos)}
%\DeclareComet{D1993F2-A}{D/1993 F2-A}{D/1993 F2-A (Shoemaker-Levy)}
%\DeclareComet{D1993F2-B}{D/1993 F2-B}{D/1993 F2-B (Shoemaker-Levy)}
%\DeclareComet{D1993F2-C}{D/1993 F2-C}{D/1993 F2-C (Shoemaker-Levy)}
%\DeclareComet{D1993F2-D}{D/1993 F2-D}{D/1993 F2-D (Shoemaker-Levy)}
%\DeclareComet{D1993F2-E}{D/1993 F2-E}{D/1993 F2-E (Shoemaker-Levy)}
%\DeclareComet{D1993F2-F}{D/1993 F2-F}{D/1993 F2-F (Shoemaker-Levy)}
%\DeclareComet{D1993F2-G}{D/1993 F2-G}{D/1993 F2-G (Shoemaker-Levy)}
%\DeclareComet{D1993F2-H}{D/1993 F2-H}{D/1993 F2-H (Shoemaker-Levy)}
%\DeclareComet{D1993F2-K}{D/1993 F2-K}{D/1993 F2-K (Shoemaker-Levy)}
%\DeclareComet{D1993F2-L}{D/1993 F2-L}{D/1993 F2-L (Shoemaker-Levy)}
%\DeclareComet{D1993F2-N}{D/1993 F2-N}{D/1993 F2-N (Shoemaker-Levy)}
%\DeclareComet{D1993F2-P}{D/1993 F2-P}{D/1993 F2-P (Shoemaker-Levy)}
%\DeclareComet{D1993F2-Q}{D/1993 F2-Q}{D/1993 F2-Q (Shoemaker-Levy)}
%\DeclareComet{D1993F2-R}{D/1993 F2-R}{D/1993 F2-R (Shoemaker-Levy)}
%\DeclareComet{D1993F2-S}{D/1993 F2-S}{D/1993 F2-S (Shoemaker-Levy)}
%\DeclareComet{D1993F2-T}{D/1993 F2-T}{D/1993 F2-T (Shoemaker-Levy)}
%\DeclareComet{D1993F2-U}{D/1993 F2-U}{D/1993 F2-U (Shoemaker-Levy)}
%\DeclareComet{D1993F2-V}{D/1993 F2-V}{D/1993 F2-V (Shoemaker-Levy)}
%\DeclareComet{D1993F2-W}{D/1993 F2-W}{D/1993 F2-W (Shoemaker-Levy)}
%\DeclareComet{P1996R2}{P/1996 R2}{P/1996 R2 (Lagerkvist)}
%\DeclareComet{P1998VS24}{P/1998 VS24}{P/1998 VS24 (LINEAR)}
%\DeclareComet{P1999J6}{P/1999 J6}{P/1999 J6 (SOHO)}
%\DeclareComet{P1999RO28}{P/1999 RO28}{P/1999 RO28 (LONEOS)}
%\DeclareComet{P1999XN120}{P/1999 XN120}{P/1999 XN120 (Catalina)}
%\DeclareComet{P2000O3}{P/2000 O3}{P/2000 O3 (SOHO)}
%\DeclareComet{P2000R2}{P/2000 R2}{P/2000 R2 (LINEAR)}
%\DeclareComet{P2001H5}{P/2001 H5}{P/2001 H5 (NEAT)}
%\DeclareComet{P2002EJ57}{P/2002 EJ57}{P/2002 EJ57 (LINEAR)}
%\DeclareComet{P2003F2}{P/2003 F2}{P/2003 F2 (NEAT)}
%\DeclareComet{P2003L1}{P/2003 L1}{P/2003 L1 (Scotti)}
%\DeclareComet{P2003R5}{P/2003 R5}{P/2003 R5 (SOHO)}
%\DeclareComet{P2003T12}{P/2003 T12}{P/2003 T12 (SOHO)}
%\DeclareComet{P2004FY140}{P/2004 FY140}{P/2004 FY140 (LINEAR)}
%\DeclareComet{P2004R3}{P/2004 R3}{P/2004 R3 (LINEAR-NEAT)}
%\DeclareComet{P2004V5}{P/2004 V5}{P/2004 V5 (LINEAR-Hill)}
%\DeclareComet{P2004V5-A}{P/2004 V5-A}{P/2004 V5-A (LINEAR-Hill)}
%\DeclareComet{P2004V5-B}{P/2004 V5-B}{P/2004 V5-B (LINEAR-Hill)}
%\DeclareComet{P2004V9}{P/2004 V9}{P/2004 V9 (SOHO)}
%\DeclareComet{P2005E1}{P/2005 E1}{P/2005 E1 (Tubbiolo)}
%\DeclareComet{P2005L1}{P/2005 L1}{P/2005 L1 (McNaught)}
%\DeclareComet{P2005S2}{P/2005 S2}{P/2005 S2 (Skiff)}
%\DeclareComet{P2005T3}{P/2005 T3}{P/2005 T3 (Read)}
%\DeclareComet{P2005T4}{P/2005 T4}{P/2005 T4 (SWAN)}
%\DeclareComet{P2005W4}{P/2005 W4}{P/2005 W4 (SOHO)}
%\DeclareComet{P2006HR30}{P/2006 HR30}{P/2006 HR30 (Siding Spring)}
%\DeclareComet{P2007K2}{P/2007 K2}{P/2007 K2 (Gibbs)}
%\DeclareComet{P2007Q2}{P/2007 Q2}{P/2007 Q2 (Gilmore)}
%\DeclareComet{P2007S1}{P/2007 S1}{P/2007 S1 (Zhao)}
%\DeclareComet{P2007T2}{P/2007 T2}{P/2007 T2 (Kowalski)}
%\DeclareComet{P2008O3}{P/2008 O3}{P/2008 O3 (Boattini)}
%\DeclareComet{P2008Y12}{P/2008 Y12}{P/2008 Y12 (SOHO)}
%\DeclareComet{P2008Y3}{P/2008 Y3}{P/2008 Y3 (McNaught)}
%\DeclareComet{P2009B1}{P/2009 B1}{P/2009 B1 (Boattini)}
%\DeclareComet{P2009O3}{P/2009 O3}{P/2009 O3 (Hill)}
%\DeclareComet{P2009Q5}{P/2009 Q5}{P/2009 Q5 (McNaught)}
%\DeclareComet{P2009T2}{P/2009 T2}{P/2009 T2 (LaSagra)}
%\DeclareComet{P2009WX51}{P/2009 WX51}{P/2009 WX51 (Catalina)}
%\DeclareComet{P2009Y2}{P/2009 Y2}{P/2009 Y2 (Kowalski)}
%\DeclareComet{P2010C1}{P/2010 C1}{P/2010 C1 (Scotti)}
%\DeclareComet{P2010D2}{P/2010 D2}{P/2010 D2 (WISE)}
%\DeclareComet{P2010E2}{P/2010 E2}{P/2010 E2 (Jarnac)}
%\DeclareComet{P2010H2}{P/2010 H2}{P/2010 H2 (Vales)}
%\DeclareComet{P2010H3}{P/2010 H3}{P/2010 H3 (SOHO)}
%\DeclareComet{P2010H4}{P/2010 H4}{P/2010 H4 (Scotti)}
%\DeclareComet{P2010H5}{P/2010 H5}{P/2010 H5 (Scotti)}
%\DeclareComet{P2010J3}{P/2010 J3}{P/2010 J3 (McMillan)}
%\DeclareComet{P2010JC81}{P/2010 JC81}{P/2010 JC81 (WISE)}
%\DeclareComet{P2010T2}{P/2010 T2}{P/2010 T2 (PANSTARRS)}
%\DeclareComet{P2010UH55}{P/2010 UH55}{P/2010 UH55 (Spacewatch)}
%\DeclareComet{P2011C2}{P/2011 C2}{P/2011 C2 (Gibbs)}
%\DeclareComet{P2011E1}{P/2011 E1}{P/2011 E1 (SOHO)}
%\DeclareComet{P2011FR143}{P/2011 FR143}{P/2011 FR143 (Lemmon)}
%\DeclareComet{P2011JB15}{P/2011 JB15}{P/2011 JB15 (Spacewatch-Boattini)}
%\DeclareComet{P2011N1}{P/2011 N1}{P/2011 N1 (ASH)}
%\DeclareComet{P2011P1}{P/2011 P1}{P/2011 P1 (McNaught)}
%\DeclareComet{P2011S1}{P/2011 S1}{P/2011 S1 (Gibbs)}
%\DeclareComet{P2011V1}{P/2011 V1}{P/2011 V1 (Boattini)}
%\DeclareComet{P2011W1}{P/2011 W1}{P/2011 W1 (PANSTARRS)}
%\DeclareComet{P2011Y2}{P/2011 Y2}{P/2011 Y2 (Boattini)}
%\DeclareComet{P2012A3}{P/2012 A3}{P/2012 A3 (SOHO)}
%\DeclareComet{P2012B1}{P/2012 B1}{P/2012 B1 (PANSTARRS)}
%\DeclareComet{P2012C3}{P/2012 C3}{P/2012 C3 (PANSTARRS)}
%\DeclareComet{P2012F2}{P/2012 F2}{P/2012 F2 (PANSTARRS)}
%\DeclareComet{P2012G1}{P/2012 G1}{P/2012 G1 (PANSTARRS)}
%\DeclareComet{P2012K3}{P/2012 K3}{P/2012 K3 (Gibbs)}
%\DeclareComet{P2012NJ}{P/2012 NJ}{P/2012 NJ (LaSagra)}
%\DeclareComet{P2012O1}{P/2012 O1}{P/2012 O1 (McNaught)}
%\DeclareComet{P2012O2}{P/2012 O2}{P/2012 O2 (McNaught)}
%\DeclareComet{P2012T3}{P/2012 T3}{P/2012 T3 (PANSTARRS)}
%\DeclareComet{P2012U2}{P/2012 U2}{P/2012 U2 (PANSTARRS)}
%\DeclareComet{P2013AL76}{P/2013 AL76}{P/2013 AL76 (Catalina)}
%\DeclareComet{P2013CU129}{P/2013 CU129}{P/2013 CU129 (PANSTARRS)}
%\DeclareComet{P2013G1}{P/2013 G1}{P/2013 G1 (Kowalski)}
%\DeclareComet{P2013G4}{P/2013 G4}{P/2013 G4 (PANSTARRS)}
%\DeclareComet{P2013J2}{P/2013 J2}{P/2013 J2 (McNaught)}
%\DeclareComet{P2013N3}{P/2013 N3}{P/2013 N3 (PANSTARRS)}
%\DeclareComet{P2013N5}{P/2013 N5}{P/2013 N5 (PANSTARRS)}
%\DeclareComet{P2013P1}{P/2013 P1}{P/2013 P1 (PANSTARRS)}
%\DeclareComet{P2013R3}{P/2013 R3}{P/2013 R3 (Catalina-PANSTARRS)}
%\DeclareComet{P2013R3-A}{P/2013 R3-A}{P/2013 R3-A (Catalina-PANSTARRS)}
%\DeclareComet{P2013R3-B}{P/2013 R3-B}{P/2013 R3-B (Catalina-PANSTARRS)}
%\DeclareComet{P2013T1}{P/2013 T1}{P/2013 T1 (PANSTARRS)}
%\DeclareComet{P2013T2}{P/2013 T2}{P/2013 T2 (Schwartz)}
%\DeclareComet{P2013W1}{P/2013 W1}{P/2013 W1 (PANSTARRS)}
%\DeclareComet{P2013YG46}{P/2013 YG46}{P/2013 YG46 (Spacewatch)}
%\DeclareComet{P2014A2}{P/2014 A2}{P/2014 A2 (Hill)}
%\DeclareComet{P2014C1}{P/2014 C1}{P/2014 C1 (TOTAS)}
%\DeclareComet{P2014L2}{P/2014 L2}{P/2014 L2 (NEOWISE)}
%\DeclareComet{P2014L3}{P/2014 L3}{P/2014 L3 (Hill)}
%\DeclareComet{P2014M4}{P/2014 M4}{P/2014 M4 (PANSTARRS)}
%\DeclareComet{P2014O3}{P/2014 O3}{P/2014 O3 (PANSTARRS)}
%\DeclareComet{P2014U4}{P/2014 U4}{P/2014 U4 (PANSTARRS)}
%\DeclareComet{P2014V1}{P/2014 V1}{P/2014 V1 (PANSTARRS)}
%\DeclareComet{P2014W4}{P/2014 W4}{P/2014 W4 (PANSTARRS)}
%\DeclareComet{P2014X1}{P/2014 X1}{P/2014 X1 (Elenin)}
%\DeclareComet{P2015A3}{P/2015 A3}{P/2015 A3 (PANSTARRS)}
%\DeclareComet{P2015B1}{P/2015 B1}{P/2015 B1 (PANSTARRS)}
%\DeclareComet{P2015B4}{P/2015 B4}{P/2015 B4 (Lemmon-PANSTARRS)}
%\DeclareComet{P2015C1}{P/2015 C1}{P/2015 C1 (TOTAS-Gibbs)}
%\DeclareComet{P2015D5}{P/2015 D5}{P/2015 D5 (Kowalski)}
%\DeclareComet{P2015D6}{P/2015 D6}{P/2015 D6 (Lemmon-PANSTARRS)}
%\DeclareComet{P2015K5}{P/2015 K5}{P/2015 K5 (PANSTARRS)}
%\DeclareComet{P2015M2}{P/2015 M2}{P/2015 M2 (PANSTARRS)}
%\DeclareComet{P2015P4}{P/2015 P4}{P/2015 P4 (PANSTARRS)}
%\DeclareComet{P2015PD229}{P/2015 PD229}{P/2015 PD229 (Cameron-ISON)}
%\DeclareComet{P2015Q2}{P/2015 Q2}{P/2015 Q2 (Pimentel)}
%\DeclareComet{P2015R1}{P/2015 R1}{P/2015 R1 (PANSTARRS)}
%\DeclareComet{P2015R2}{P/2015 R2}{P/2015 R2 (PANSTARRS)}
%\DeclareComet{P2015TP200}{P/2015 TP200}{P/2015 TP200 (LINEAR)}
%\DeclareComet{P2015W2}{P/2015 W2}{P/2015 W2 (Catalina)}
%\DeclareComet{P2015X3}{P/2015 X3}{P/2015 X3 (PANSTARRS)}
%\DeclareComet{P2015X6}{P/2015 X6}{P/2015 X6 (PANSTARRS)}
%\DeclareComet{P2016A3}{P/2016 A3}{P/2016 A3 (PANSTARRS)}
%\DeclareComet{P2016A7}{P/2016 A7}{P/2016 A7 (PANSTARRS)}
%\DeclareComet{P2016G1}{P/2016 G1}{P/2016 G1 (PANSTARRS)}
%\DeclareComet{P2016P1}{P/2016 P1}{P/2016 P1 (PANSTARRS)}
%\DeclareComet{P2016P5}{P/2016 P5}{P/2016 P5 (COIAS)}
%\DeclareComet{P2016R4}{P/2016 R4}{P/2016 R4 (Gibbs)}
%\DeclareComet{P2016S1}{P/2016 S1}{P/2016 S1 (PANSTARRS)}
%\DeclareComet{P2016WM48}{P/2016 WM48}{P/2016 WM48 (Lemmon)}
%\DeclareComet{P2017D1}{P/2017 D1}{P/2017 D1 (Fuls)}
%\DeclareComet{P2017D4}{P/2017 D4}{P/2017 D4 (PANSTARRS)}
%\DeclareComet{P2017FL36}{P/2017 FL36}{P/2017 FL36 (PANSTARRS)}
%\DeclareComet{P2017G1}{P/2017 G1}{P/2017 G1 (PANSTARRS)}
%\DeclareComet{P2017G2}{P/2017 G2}{P/2017 G2 (PANSTARRS)}
%\DeclareComet{P2017K3}{P/2017 K3}{P/2017 K3 (Gasparovic)}
%\DeclareComet{P2017P1}{P/2017 P1}{P/2017 P1 (PANSTARRS)}
%\DeclareComet{P2017S8}{P/2017 S8}{P/2017 S8 (PANSTARRS)}
%\DeclareComet{P2017TW13}{P/2017 TW13}{P/2017 TW13 (Lemmon)}
%\DeclareComet{P2017U3}{P/2017 U3}{P/2017 U3 (PANSTARRS)}
%\DeclareComet{P2017W3}{P/2017 W3}{P/2017 W3 (Gibbs)}
%\DeclareComet{P2017Y3}{P/2017 Y3}{P/2017 Y3 (Leonard)}
%\DeclareComet{P2018A5}{P/2018 A5}{P/2018 A5 (PANSTARRS)}
%\DeclareComet{P2018C1}{P/2018 C1}{P/2018 C1 (Lemmon-Read)}
%\DeclareComet{P2018H2}{P/2018 H2}{P/2018 H2 (PANSTARRS)}
%\DeclareComet{P2018L4}{P/2018 L4}{P/2018 L4 (PANSTARRS)}
%\DeclareComet{P2018P4}{P/2018 P4}{P/2018 P4 (PANSTARRS)}
%\DeclareComet{P2018V5}{P/2018 V5}{P/2018 V5 (Trujillo-Sheppard)}
%\DeclareComet{P2018VN2}{P/2018 VN2}{P/2018 VN2 (Leonard)}
%\DeclareComet{P2018Y2}{P/2018 Y2}{P/2018 Y2 (Africano)}
%\DeclareComet{P2019A1}{P/2019 A1}{P/2019 A1 (PANSTARRS)}
%\DeclareComet{P2019A2}{P/2019 A2}{P/2019 A2 (ATLAS)}
%\DeclareComet{P2019A3}{P/2019 A3}{P/2019 A3 (PANSTARRS)}
%\DeclareComet{P2019A4}{P/2019 A4}{P/2019 A4 (PANSTARRS)}
%\DeclareComet{P2019A6}{P/2019 A6}{P/2019 A6 (Lemmon-PANSTARRS)}
%\DeclareComet{P2019B2}{P/2019 B2}{P/2019 B2 (Groeller)}
%\DeclareComet{P2019GG21}{P/2019 GG21}{P/2019 GG21 (PANSTARRS)}
%\DeclareComet{P2019LD2}{P/2019 LD2}{P/2019 LD2 (ATLAS)}
%\DeclareComet{P2019LM4}{P/2019 LM4}{P/2019 LM4 (Palomar)}
%\DeclareComet{P2019S2}{P/2019 S2}{P/2019 S2 (PANSTARRS)}
%\DeclareComet{P2019S3}{P/2019 S3}{P/2019 S3 (PANSTARRS)}
%\DeclareComet{P2019T5}{P/2019 T5}{P/2019 T5 (ATLAS)}
%\DeclareComet{P2019T6}{P/2019 T6}{P/2019 T6 (PANSTARRS)}
%\DeclareComet{P2019U4}{P/2019 U4}{P/2019 U4 (PANSTARRS)}
%\DeclareComet{P2019V2}{P/2019 V2}{P/2019 V2 (Groeller)}
%\DeclareComet{P2019W1}{P/2019 W1}{P/2019 W1 (PANSTARRS)}
%\DeclareComet{P2019X1}{P/2019 X1}{P/2019 X1 (Pruyne)}
%\DeclareComet{P2019X2}{P/2019 X2}{P/2019 X2 (Pan-STARRS)}
%\DeclareComet{P2020A4}{P/2020 A4}{P/2020 A4 (PANSTARRS-Lemmon)}
%\DeclareComet{P2020B4}{P/2020 B4}{P/2020 B4 (Sheppard)}
%\DeclareComet{P2020G1}{P/2020 G1}{P/2020 G1 (Pimentel)}
%\DeclareComet{P2020K9}{P/2020 K9}{P/2020 K9 (Lemmon-PANSTARRS)}
%\DeclareComet{P2020M1}{P/2020 M1}{P/2020 M1 (PANSTARRS)}
%\DeclareComet{P2020MK4}{P/2020 MK4}{P/2020 MK4 (PANSTARRS)}
%\DeclareComet{P2020O3}{P/2020 O3}{P/2020 O3 (PANSTARRS)}
%\DeclareComet{P2020R5}{P/2020 R5}{P/2020 R5 (PANSTARRS)}
%\DeclareComet{P2020S1}{P/2020 S1}{P/2020 S1 (PANSTARRS)}
%\DeclareComet{P2020S5}{P/2020 S5}{P/2020 S5 (PANSTARRS)}
%\DeclareComet{P2020S7}{P/2020 S7}{P/2020 S7 (PANSTARRS)}
%\DeclareComet{P2020T3}{P/2020 T3}{P/2020 T3 (PANSTARRS)}
%\DeclareComet{P2020U2}{P/2020 U2}{P/2020 U2 (PANSTARRS)}
%\DeclareComet{P2020V3}{P/2020 V3}{P/2020 V3 (PANSTARRS)}
%\DeclareComet{P2020V4}{P/2020 V4}{P/2020 V4 (Rankin)}
%\DeclareComet{P2020W1}{P/2020 W1}{P/2020 W1 (Rankin)}
%\DeclareComet{P2020WJ5}{P/2020 WJ5}{P/2020 WJ5 (Lemmon)}
%\DeclareComet{P2020X1}{P/2020 X1}{P/2020 X1 (ATLAS)}
%\DeclareComet{P2021A5}{P/2021 A5}{P/2021 A5 (PANSTARRS)}
%\DeclareComet{P2021C2}{P/2021 C2}{P/2021 C2 (PANSTARRS)}
%\DeclareComet{P2021HS}{P/2021 HS}{P/2021 HS (PANSTARRS)}
%\DeclareComet{P2021J3}{P/2021 J3}{P/2021 J3 (ATLAS)}
%\DeclareComet{P2021L2}{P/2021 L2}{P/2021 L2 (Leonard)}
%\DeclareComet{P2021N1}{P/2021 N1}{P/2021 N1 (ZTF)}
%\DeclareComet{P2021N2}{P/2021 N2}{P/2021 N2 (Fuls)}
%\DeclareComet{P2021P3}{P/2021 P3}{P/2021 P3 (PANSTARRS)}
%\DeclareComet{P2021PE20}{P/2021 PE20}{P/2021 PE20 (ATLAS)}
%\DeclareComet{P2021Q5}{P/2021 Q5}{P/2021 Q5 (ATLAS)}
%\DeclareComet{P2021R1}{P/2021 R1}{P/2021 R1 (PANSTARRS)}
%\DeclareComet{P2021R3}{P/2021 R3}{P/2021 R3 (PANSTARRS)}
%\DeclareComet{P2021R4}{P/2021 R4}{P/2021 R4 (Wierzchos)}
%\DeclareComet{P2021R5}{P/2021 R5}{P/2021 R5 (Rankin)}
%\DeclareComet{P2021R6}{P/2021 R6}{P/2021 R6 (Groeller)}
%\DeclareComet{P2021R8}{P/2021 R8}{P/2021 R8 (Sheppard)}
%\DeclareComet{P2021TR81}{P/2021 TR81}{P/2021 TR81 (Lemmon)}
%\DeclareComet{P2021U1}{P/2021 U1}{P/2021 U1 (Wierzchos)}
%\DeclareComet{P2021U3}{P/2021 U3}{P/2021 U3 (Attard-Maury)}
%\DeclareComet{P2021V2}{P/2021 V2}{P/2021 V2 (Fuls)}
%\DeclareComet{P2022B1}{P/2022 B1}{P/2022 B1 (Wierzchos)}
%\DeclareComet{P2022BV9}{P/2022 BV9}{P/2022 BV9 (Lemmon)}
%\DeclareComet{P2022C1}{P/2022 C1}{P/2022 C1 (PANSTARRS)}
%\DeclareComet{P2022C2}{P/2022 C2}{P/2022 C2 (PANSTARRS)}
%\DeclareComet{P2022C3}{P/2022 C3}{P/2022 C3 (PANSTARRS)}
%\DeclareComet{P2022D1}{P/2022 D1}{P/2022 D1 (PANSTARRS)}
%\DeclareComet{P2022E1}{P/2022 E1}{P/2022 E1 (Christensen)}
%\DeclareComet{P2022L3}{P/2022 L3}{P/2022 L3 (ATLAS)}
%\DeclareComet{P2022O2}{P/2022 O2}{P/2022 O2 (PANSTARRS)}
%\DeclareComet{P2022P2}{P/2022 P2}{P/2022 P2 (ZTF)}
%\DeclareComet{P2022R1}{P/2022 R1}{P/2022 R1 (PANSTARRS)}
%\DeclareComet{P2022R4}{P/2022 R4}{P/2022 R4 (PANSTARRS)}
%\DeclareComet{P2022R5}{P/2022 R5}{P/2022 R5 (PANSTARRS)}
%\DeclareComet{P2022S1}{P/2022 S1}{P/2022 S1 (PANSTARRS)}
%\DeclareComet{P2022W1}{P/2022 W1}{P/2022 W1 (Rankin)}
%\DeclareComet{P2023B1}{P/2023 B1}{P/2023 B1 (PANSTARRS)}
%\DeclareComet{P2023B3}{P/2023 B3}{P/2023 B3 (PANSTARRS)}
%\DeclareComet{P2023JN16}{P/2023 JN16}{P/2023 JN16 (Lemmon)}
%\DeclareComet{P2023M1}{P/2023 M1}{P/2023 M1 (PANSTARRS)}
%\DeclareComet{P2023M2}{P/2023 M2}{P/2023 M2 (PANSTARRS)}
%\DeclareComet{P2023M4}{P/2023 M4}{P/2023 M4 (ATLAS)}
%\DeclareComet{P2023S1}{P/2023 S1}{P/2023 S1 (PANSTARRS)}
%\DeclareComet{P2023T1}{P/2023 T1}{P/2023 T1 (PANSTARRS)}
%\DeclareComet{P2023V2}{P/2023 V2}{P/2023 V2 (PANSTARRS)}
%\DeclareComet{P2023V6}{P/2023 V6}{P/2023 V6 (PANSTARRS)}
%\DeclareComet{P2023X3}{P/2023 X3}{P/2023 X3 (PANSTARRS)}
%\DeclareComet{P2023Y1}{P/2023 Y1}{P/2023 Y1 (Gibbs)}
%\DeclareComet{P2023Y2}{P/2023 Y2}{P/2023 Y2 (Gibbs)}
%\DeclareComet{P2024F1}{P/2024 F1}{P/2024 F1 (PANSTARRS)}
%\DeclareComet{P2024FG9}{P/2024 FG9}{P/2024 FG9 (Nanshan-Hahn)}
%\DeclareComet{P2024J1}{P/2024 J1}{P/2024 J1 (PANSTARRS)}
%\DeclareComet{P2024K1}{P/2024 K1}{P/2024 K1 (PANSTARRS)}
%\DeclareComet{P2024O2}{P/2024 O2}{P/2024 O2 (PANSTARRS)}
%\DeclareComet{P2024OC2}{P/2024 OC2}{P/2024 OC2 (PANSTARRS)}
%\DeclareComet{P2024Q1}{P/2024 Q1}{P/2024 Q1 (PANSTARRS)}
%\DeclareComet{P2024R1}{P/2024 R1}{P/2024 R1 (PANSTARRS)}
%\DeclareComet{P2024R2}{P/2024 R2}{P/2024 R2 (PANSTARRS)}
%\DeclareComet{P2024R3}{P/2024 R3}{P/2024 R3 (PANSTARRS)}
%\DeclareComet{P2024S2}{P/2024 S2}{P/2024 S2 (Rankin)}
%\DeclareComet{P2024T1}{P/2024 T1}{P/2024 T1 (Rankin)}
%\DeclareComet{P2024T2}{P/2024 T2}{P/2024 T2 (Rankin)}
%\DeclareComet{P2024X3}{P/2024 X3}{P/2024 X3 (PANSTARRS)}
%\DeclareComet{P2025A2}{P/2025 A2}{P/2025 A2 (PANSTARRS)}
%\DeclareComet{P2025C1}{P/2025 C1}{P/2025 C1 (ATLAS)}
%\DeclareComet{P2025D2}{P/2025 D2}{P/2025 D2 (PANSTARRS)}
%\DeclareComet{P2025D3}{P/2025 D3}{P/2025 D3 (PANSTARRS)}
%\DeclareComet{P2025D4}{P/2025 D4}{P/2025 D4 (ATLAS)}
%\DeclareComet{P2025U1}{P/2025 U1}{P/2025 U1 (Hogan)}
%\DeclareComet{P2025UX109}{P/2025 UX109}{P/2025 UX109 (Ye)}
%\DeclareComet{P2025W3}{P/2025 W3}{P/2025 W3 (Kresken)}
%\DeclareComet{P2025W4}{P/2025 W4}{P/2025 W4 (PANSTARRS)}
%\DeclareComet{P2025Y2}{P/2025 Y2}{P/2025 Y2 (PANSTARRS)}
%\DeclareComet{P2026C2}{P/2026 C2}{P/2026 C2 (PANSTARRS)}
%\DeclareComet{P2026N2}{P/2026 N2}{P/2026 N2}
%\DeclareComet{P2026P1}{P/2026 P1}{P/2026 P1 (PANSTARRS)}

